High-Speed Stereo Visual SLAM for Low-Powered Computing Devices

We present an accurate and GPU-accelerated Stereo Visual SLAM design called Jetson-SLAM. It exhibits frame-processing rates above 60FPS on NVIDIA's low-powered 10W Jetson-NX embedded computer and above 200FPS on desktop-grade 200W GPUs, even in stereo configuration and in the multiscale setting. Our contributions are threefold: (i) a Bounded Rectification technique to prevent tagging many non-corner points as a corner in FAST detection, improving SLAM accuracy. (ii) A novel Pyramidal Culling and Aggregation (PyCA) technique that yields robust features while suppressing redundant ones at high speeds by harnessing a GPU device. PyCA uses our new Multi-Location Per Thread culling strategy (MLPT) and Thread-Efficient Warp-Allocation (TEWA) scheme for GPU to enable Jetson-SLAM achieving high accuracy and speed on embedded devices. (iii) Jetson-SLAM library achieves resource efficiency by having a data-sharing mechanism. Our experiments on three challenging datasets: KITTI, EuRoC, and KAIST-VIO, and two highly accurate SLAM backends: Full-BA and ICE-BA show that Jetson-SLAM is the fastest available accurate and GPU-accelerated SLAM system (Fig. 1).

==> plots/euroc_traj_coords/mh01_full_ba_jetson_slam.tex <==
\addplot[
    fill=none,draw = clr6,
    very thick,
    line width= \linew ex
    ]
    coordinates {
    (4.67, -1.77)
(4.67, -1.78)
(4.68, -1.79)
(4.68, -1.79)
(4.65, -1.78)
(4.66, -1.78)
(4.67, -1.78)
(4.69, -1.79)
(4.67, -1.79)
(4.66, -1.78)
(4.66, -1.77)
(4.67, -1.76)
(4.69, -1.77)
(4.68, -1.78)
(4.65, -1.76)
(4.65, -1.76)
(4.64, -1.75)
(4.67, -1.76)
(4.70, -1.77)
(4.73, -1.79)
(4.75, -1.78)
(4.74, -1.76)
(4.74, -1.70)
(4.76, -1.58)
(4.79, -1.48)
(4.80, -1.46)
(4.79, -1.54)
(4.75, -1.68)
(4.71, -1.85)
(4.68, -1.99)
(4.66, -2.06)
(4.70, -1.99)
(4.74, -1.84)
(4.78, -1.69)
(4.78, -1.62)
(4.76, -1.58)
(4.70, -1.52)
(4.58, -1.52)
(4.50, -1.67)
(4.57, -1.89)
(4.72, -1.94)
(4.84, -1.81)
(4.83, -1.59)
(4.69, -1.49)
(4.56, -1.68)
(4.59, -1.86)
(4.73, -1.78)
(4.87, -1.70)
(4.95, -1.84)
(4.94, -1.89)
(4.78, -1.77)
(4.59, -1.70)
(4.61, -1.78)
(4.74, -1.83)
(4.71, -1.78)
(4.62, -1.72)
(4.57, -1.70)
(4.55, -1.69)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.55, -1.68)
(4.57, -1.67)
(4.61, -1.64)
(4.66, -1.62)
(4.65, -1.62)
(4.60, -1.63)
(4.55, -1.63)
(4.54, -1.61)
(4.56, -1.58)
(4.59, -1.55)
(4.62, -1.52)
(4.64, -1.48)
(4.61, -1.43)
(4.60, -1.36)
(4.59, -1.26)
(4.57, -1.14)
(4.53, -1.00)
(4.49, -0.82)
(4.42, -0.63)
(4.31, -0.46)
(4.25, -0.29)
(4.16, -0.11)
(4.07, 0.04)
(3.97, 0.17)
(3.87, 0.28)
(3.75, 0.38)
(3.60, 0.51)
(3.43, 0.63)
(3.24, 0.77)
(3.04, 0.95)
(2.83, 1.14)
(2.64, 1.31)
(2.44, 1.46)
(2.23, 1.62)
(2.00, 1.80)
(1.77, 2.02)
(1.59, 2.20)
(1.44, 2.30)
(1.30, 2.36)
(1.14, 2.43)
(0.99, 2.48)
(0.85, 2.54)
(0.66, 2.64)
(0.46, 2.78)
(0.25, 2.97)
(0.04, 3.14)
(-0.13, 3.29)
(-0.27, 3.43)
(-0.39, 3.54)
(-0.51, 3.64)
(-0.60, 3.73)
(-0.68, 3.81)
(-0.73, 3.88)
(-0.75, 3.94)
(-0.78, 4.01)
(-0.83, 4.08)
(-0.88, 4.17)
(-1.01, 4.28)
(-1.18, 4.41)
(-1.32, 4.60)
(-1.42, 4.79)
(-1.62, 5.00)
(-1.84, 5.22)
(-2.12, 5.47)
(-2.35, 5.72)
(-2.53, 5.98)
(-2.65, 6.21)
(-2.75, 6.41)
(-2.79, 6.63)
(-2.78, 6.84)
(-2.73, 7.02)
(-2.67, 7.16)
(-2.62, 7.35)
(-2.57, 7.49)
(-2.48, 7.60)
(-2.35, 7.68)
(-2.23, 7.72)
(-2.09, 7.74)
(-2.02, 7.71)
(-1.90, 7.65)
(-1.70, 7.59)
(-1.55, 7.51)
(-1.36, 7.44)
(-1.18, 7.45)
(-1.00, 7.47)
(-0.85, 7.45)
(-0.72, 7.40)
(-0.61, 7.32)
(-0.50, 7.23)
(-0.42, 7.13)
(-0.35, 6.98)
(-0.28, 6.79)
(-0.16, 6.62)
(-0.02, 6.46)
(0.09, 6.29)
(0.20, 6.08)
(0.29, 5.84)
(0.46, 5.58)
(0.65, 5.33)
(0.86, 5.13)
(1.02, 4.99)
(1.13, 4.84)
(1.20, 4.71)
(1.25, 4.62)
(1.30, 4.57)
(1.36, 4.62)
(1.35, 4.69)
(1.28, 4.76)
(1.19, 4.81)
(1.08, 4.81)
(0.95, 4.81)
(0.85, 4.81)
(0.84, 4.80)
(0.86, 4.86)
(0.89, 5.04)
(0.85, 5.32)
(0.76, 5.59)
(0.64, 5.84)
(0.55, 6.08)
(0.39, 6.33)
(0.25, 6.57)
(0.11, 6.76)
(-0.04, 6.90)
(-0.11, 7.06)
(-0.20, 7.21)
(-0.26, 7.35)
(-0.32, 7.52)
(-0.36, 7.68)
(-0.41, 7.91)
(-0.53, 8.13)
(-0.69, 8.34)
(-0.92, 8.48)
(-1.09, 8.47)
(-1.15, 8.27)
(-1.03, 7.89)
(-0.71, 7.34)
(-0.33, 6.79)
(0.04, 6.39)
(0.31, 6.26)
(0.45, 6.19)
(0.54, 6.14)
(0.55, 6.19)
(0.50, 6.32)
(0.38, 6.47)
(0.23, 6.57)
(0.12, 6.73)
(0.04, 6.94)
(-0.10, 7.23)
(-0.29, 7.49)
(-0.50, 7.73)
(-0.75, 7.93)
(-1.01, 8.11)
(-1.25, 8.28)
(-1.48, 8.38)
(-1.65, 8.44)
(-1.78, 8.52)
(-1.90, 8.60)
(-2.00, 8.62)
(-2.10, 8.58)
(-2.15, 8.55)
(-2.15, 8.51)
(-2.09, 8.41)
(-1.97, 8.20)
(-1.86, 7.97)
(-1.78, 7.74)
(-1.69, 7.51)
(-1.58, 7.24)
(-1.47, 7.01)
(-1.36, 6.77)
(-1.20, 6.52)
(-1.03, 6.28)
(-0.86, 6.03)
(-0.72, 5.81)
(-0.54, 5.62)
(-0.34, 5.44)
(-0.14, 5.28)
(0.06, 5.10)
(0.27, 4.90)
(0.46, 4.71)
(0.62, 4.53)
(0.75, 4.37)
(0.88, 4.23)
(1.02, 4.11)
(1.15, 4.01)
(1.30, 3.90)
(1.45, 3.77)
(1.58, 3.61)
(1.68, 3.45)
(1.72, 3.31)
(1.67, 3.22)
(1.55, 3.15)
(1.39, 3.16)
(1.27, 3.34)
(1.25, 3.60)
(1.24, 3.85)
(1.26, 4.09)
(1.30, 4.31)
(1.35, 4.46)
(1.38, 4.55)
(1.33, 4.61)
(1.24, 4.64)
(1.15, 4.68)
(1.08, 4.70)
(1.00, 4.76)
(0.92, 4.82)
(0.87, 4.85)
(0.82, 4.87)
(0.78, 4.87)
(0.78, 4.88)
(0.82, 4.85)
(0.89, 4.74)
(0.96, 4.61)
(1.02, 4.46)
(1.07, 4.30)
(1.12, 4.13)
(1.14, 3.99)
(1.18, 3.91)
(1.23, 3.88)
(1.30, 3.90)
(1.38, 3.93)
(1.48, 4.01)
(1.55, 4.05)
(1.61, 4.14)
(1.69, 4.22)
(1.76, 4.33)
(1.79, 4.44)
(1.78, 4.56)
(1.80, 4.71)
(1.84, 4.85)
(1.86, 4.98)
(1.88, 5.15)
(1.86, 5.34)
(1.77, 5.60)
(1.63, 5.86)
(1.48, 6.15)
(1.37, 6.43)
(1.23, 6.69)
(1.07, 6.94)
(0.89, 7.20)
(0.65, 7.46)
(0.41, 7.75)
(0.22, 8.05)
(0.07, 8.34)
(-0.07, 8.57)
(-0.24, 8.73)
(-0.44, 8.86)
(-0.69, 8.93)
(-0.94, 9.01)
(-1.15, 9.06)
(-1.34, 9.09)
(-1.53, 9.06)
(-1.67, 8.94)
(-1.77, 8.79)
(-1.84, 8.58)
(-1.85, 8.35)
(-1.82, 8.08)
(-1.76, 7.81)
(-1.65, 7.57)
(-1.53, 7.36)
(-1.40, 7.18)
(-1.31, 7.04)
(-1.27, 6.93)
(-1.21, 6.86)
(-1.11, 6.79)
(-0.96, 6.72)
(-0.82, 6.63)
(-0.67, 6.54)
(-0.52, 6.43)
(-0.39, 6.28)
(-0.26, 6.06)
(-0.15, 5.84)
(-0.05, 5.66)
(0.05, 5.49)
(0.19, 5.33)
(0.32, 5.20)
(0.45, 5.09)
(0.56, 5.01)
(0.65, 4.96)
(0.74, 4.94)
(0.86, 4.92)
(0.99, 4.90)
(1.11, 4.86)
(1.23, 4.81)
(1.34, 4.75)
(1.45, 4.69)
(1.59, 4.59)
(1.71, 4.52)
(1.81, 4.44)
(1.89, 4.36)
(1.95, 4.29)
(2.02, 4.24)
(2.07, 4.20)
(2.10, 4.17)
(2.15, 4.13)
(2.23, 4.13)
(2.33, 4.10)
(2.40, 4.04)
(2.48, 3.94)
(2.56, 3.82)
(2.64, 3.69)
(2.74, 3.57)
(2.85, 3.40)
(2.99, 3.24)
(3.11, 3.08)
(3.22, 2.92)
(3.27, 2.79)
(3.30, 2.71)
(3.33, 2.67)
(3.38, 2.66)
(3.43, 2.65)
(3.50, 2.62)
(3.61, 2.52)
(3.73, 2.38)
(3.88, 2.22)
(4.00, 2.06)
(4.12, 1.89)
(4.25, 1.73)
(4.33, 1.57)
(4.40, 1.44)
(4.43, 1.34)
(4.46, 1.24)
(4.46, 1.15)
(4.49, 1.04)
(4.53, 0.90)
(4.56, 0.76)
(4.59, 0.65)
(4.58, 0.59)
(4.57, 0.57)
(4.55, 0.57)
(4.55, 0.65)
(4.58, 0.73)
(4.61, 0.81)
(4.63, 0.87)
(4.66, 0.92)
(4.70, 0.96)
(4.74, 0.98)
(4.78, 1.00)
(4.79, 1.03)
(4.79, 1.07)
(4.76, 1.12)
(4.75, 1.16)
(4.70, 1.25)
(4.63, 1.40)
(4.54, 1.54)
(4.47, 1.66)
(4.44, 1.77)
(4.45, 1.86)
(4.44, 1.96)
(4.43, 2.03)
(4.39, 2.04)
(4.35, 1.97)
(4.28, 1.93)
(4.22, 1.93)
(4.12, 1.93)
(4.00, 1.93)
(3.93, 1.95)
(3.85, 1.98)
(3.80, 2.02)
(3.80, 2.08)
(3.81, 2.12)
(3.81, 2.11)
(3.83, 2.04)
(3.85, 1.97)
(3.86, 1.87)
(3.85, 1.79)
(3.86, 1.75)
(3.85, 1.77)
(3.85, 1.79)
(3.85, 1.79)
(3.86, 1.76)
(3.82, 1.68)
(3.80, 1.60)
(3.80, 1.49)
(3.84, 1.33)
(3.90, 1.14)
(3.97, 0.93)
(4.02, 0.70)
(4.06, 0.47)
(4.11, 0.22)
(4.19, -0.03)
(4.29, -0.28)
(4.40, -0.54)
(4.50, -0.81)
(4.51, -1.06)
(4.53, -1.31)
(4.51, -1.48)
(4.49, -1.61)
(4.51, -1.65)
(4.56, -1.67)
(4.59, -1.69)
(4.63, -1.70)
(4.67, -1.73)
(4.67, -1.78)
(4.63, -1.83)
(4.62, -1.86)
(4.61, -1.90)
(4.55, -1.94)
};
 %   


==> plots/euroc_traj_coords/mh01_gt.tex <==
\addplot[
    fill=none,draw = clr1,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(4.69, -1.79)
(4.68, -1.78)
(4.69, -1.78)
(4.70, -1.78)
(4.71, -1.79)
(4.69, -1.79)
(4.69, -1.77)
(4.70, -1.77)
(4.70, -1.76)
(4.72, -1.77)
(4.70, -1.77)
(4.68, -1.76)
(4.68, -1.76)
(4.69, -1.75)
(4.72, -1.76)
(4.74, -1.78)
(4.77, -1.79)
(4.78, -1.76)
(4.76, -1.73)
(4.78, -1.63)
(4.81, -1.50)
(4.83, -1.45)
(4.82, -1.50)
(4.79, -1.63)
(4.75, -1.80)
(4.71, -1.96)
(4.68, -2.05)
(4.71, -2.00)
(4.76, -1.86)
(4.80, -1.70)
(4.81, -1.62)
(4.79, -1.58)
(4.74, -1.52)
(4.62, -1.52)
(4.52, -1.67)
(4.57, -1.89)
(4.74, -1.92)
(4.88, -1.78)
(4.86, -1.56)
(4.70, -1.50)
(4.57, -1.73)
(4.63, -1.86)
(4.79, -1.73)
(4.92, -1.72)
(4.99, -1.88)
(4.93, -1.86)
(4.73, -1.72)
(4.58, -1.71)
(4.67, -1.80)
(4.76, -1.81)
(4.67, -1.74)
(4.60, -1.70)
(4.56, -1.68)
(4.56, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.68)
(4.57, -1.67)
(4.57, -1.68)
(4.57, -1.67)
(4.57, -1.67)
(4.60, -1.65)
(4.66, -1.62)
(4.67, -1.61)
(4.64, -1.62)
(4.58, -1.63)
(4.55, -1.61)
(4.56, -1.58)
(4.60, -1.55)
(4.63, -1.53)
(4.67, -1.49)
(4.64, -1.44)
(4.62, -1.37)
(4.62, -1.27)
(4.60, -1.15)
(4.58, -1.01)
(4.53, -0.82)
(4.45, -0.62)
(4.37, -0.44)
(4.27, -0.26)
(4.17, -0.08)
(4.08, 0.08)
(3.97, 0.21)
(3.86, 0.32)
(3.71, 0.44)
(3.56, 0.56)
(3.39, 0.69)
(3.19, 0.84)
(2.97, 1.04)
(2.76, 1.23)
(2.56, 1.39)
(2.34, 1.54)
(2.11, 1.72)
(1.89, 1.93)
(1.67, 2.15)
(1.50, 2.29)
(1.36, 2.37)
(1.21, 2.43)
(1.04, 2.49)
(0.89, 2.55)
(0.72, 2.64)
(0.51, 2.76)
(0.29, 2.94)
(0.08, 3.13)
(-0.11, 3.29)
(-0.27, 3.44)
(-0.40, 3.56)
(-0.52, 3.66)
(-0.61, 3.76)
(-0.69, 3.84)
(-0.74, 3.92)
(-0.76, 3.98)
(-0.80, 4.05)
(-0.84, 4.12)
(-0.91, 4.22)
(-1.03, 4.33)
(-1.21, 4.48)
(-1.34, 4.68)
(-1.45, 4.87)
(-1.66, 5.09)
(-1.92, 5.33)
(-2.19, 5.57)
(-2.40, 5.84)
(-2.56, 6.09)
(-2.69, 6.32)
(-2.77, 6.53)
(-2.78, 6.75)
(-2.75, 6.95)
(-2.68, 7.12)
(-2.62, 7.30)
(-2.57, 7.46)
(-2.49, 7.60)
(-2.38, 7.69)
(-2.25, 7.73)
(-2.13, 7.76)
(-2.01, 7.75)
(-1.90, 7.72)
(-1.75, 7.65)
(-1.56, 7.53)
(-1.37, 7.45)
(-1.17, 7.45)
(-0.99, 7.46)
(-0.83, 7.45)
(-0.70, 7.40)
(-0.58, 7.31)
(-0.47, 7.21)
(-0.38, 7.11)
(-0.31, 6.94)
(-0.23, 6.76)
(-0.12, 6.57)
(0.02, 6.41)
(0.15, 6.24)
(0.24, 6.01)
(0.36, 5.77)
(0.53, 5.50)
(0.74, 5.25)
(0.93, 5.05)
(1.08, 4.90)
(1.18, 4.75)
(1.24, 4.63)
(1.29, 4.54)
(1.35, 4.54)
(1.38, 4.60)
(1.35, 4.67)
(1.27, 4.74)
(1.16, 4.76)
(1.04, 4.76)
(0.91, 4.76)
(0.86, 4.76)
(0.87, 4.78)
(0.91, 4.92)
(0.90, 5.18)
(0.82, 5.46)
(0.70, 5.72)
(0.57, 5.98)
(0.45, 6.23)
(0.30, 6.48)
(0.15, 6.69)
(0.01, 6.84)
(-0.09, 7.00)
(-0.17, 7.16)
(-0.25, 7.31)
(-0.30, 7.47)
(-0.34, 7.66)
(-0.40, 7.88)
(-0.52, 8.11)
(-0.70, 8.31)
(-0.93, 8.43)
(-1.09, 8.40)
(-1.11, 8.18)
(-0.94, 7.76)
(-0.57, 7.19)
(-0.18, 6.66)
(0.17, 6.34)
(0.40, 6.23)
(0.53, 6.17)
(0.59, 6.16)
(0.57, 6.25)
(0.49, 6.40)
(0.34, 6.55)
(0.20, 6.70)
(0.10, 6.87)
(-0.01, 7.16)
(-0.21, 7.43)
(-0.41, 7.67)
(-0.64, 7.89)
(-0.91, 8.09)
(-1.17, 8.28)
(-1.42, 8.41)
(-1.62, 8.47)
(-1.76, 8.56)
(-1.89, 8.65)
(-2.02, 8.68)
(-2.12, 8.64)
(-2.18, 8.60)
(-2.20, 8.57)
(-2.13, 8.46)
(-2.01, 8.25)
(-1.90, 8.01)
(-1.82, 7.77)
(-1.72, 7.52)
(-1.60, 7.26)
(-1.49, 7.01)
(-1.36, 6.76)
(-1.20, 6.49)
(-1.02, 6.23)
(-0.86, 5.98)
(-0.69, 5.75)
(-0.52, 5.55)
(-0.32, 5.38)
(-0.11, 5.20)
(0.10, 5.00)
(0.31, 4.79)
(0.49, 4.60)
(0.65, 4.42)
(0.78, 4.26)
(0.92, 4.12)
(1.06, 4.01)
(1.20, 3.89)
(1.36, 3.76)
(1.50, 3.60)
(1.61, 3.42)
(1.67, 3.27)
(1.64, 3.16)
(1.53, 3.09)
(1.37, 3.07)
(1.24, 3.23)
(1.20, 3.49)
(1.19, 3.75)
(1.22, 4.01)
(1.26, 4.25)
(1.31, 4.42)
(1.34, 4.52)
(1.29, 4.57)
(1.19, 4.61)
(1.11, 4.65)
(1.03, 4.68)
(0.95, 4.73)
(0.87, 4.79)
(0.82, 4.83)
(0.76, 4.85)
(0.73, 4.85)
(0.75, 4.85)
(0.80, 4.79)
(0.88, 4.67)
(0.95, 4.53)
(1.02, 4.37)
(1.07, 4.21)
(1.11, 4.04)
(1.14, 3.93)
(1.18, 3.88)
(1.24, 3.87)
(1.32, 3.90)
(1.43, 3.94)
(1.52, 4.00)
(1.58, 4.09)
(1.66, 4.18)
(1.73, 4.27)
(1.78, 4.37)
(1.78, 4.51)
(1.80, 4.67)
(1.83, 4.81)
(1.86, 4.95)
(1.88, 5.11)
(1.86, 5.31)
(1.78, 5.57)
(1.65, 5.85)
(1.49, 6.14)
(1.37, 6.42)
(1.24, 6.70)
(1.07, 6.97)
(0.87, 7.24)
(0.63, 7.52)
(0.40, 7.82)
(0.20, 8.12)
(0.06, 8.41)
(-0.09, 8.63)
(-0.27, 8.78)
(-0.49, 8.90)
(-0.76, 8.99)
(-1.00, 9.05)
(-1.21, 9.11)
(-1.41, 9.11)
(-1.58, 9.04)
(-1.71, 8.90)
(-1.79, 8.73)
(-1.84, 8.51)
(-1.82, 8.25)
(-1.78, 7.96)
(-1.69, 7.70)
(-1.57, 7.47)
(-1.44, 7.27)
(-1.34, 7.11)
(-1.28, 6.99)
(-1.24, 6.92)
(-1.14, 6.85)
(-1.00, 6.76)
(-0.86, 6.68)
(-0.71, 6.59)
(-0.56, 6.48)
(-0.42, 6.32)
(-0.30, 6.10)
(-0.18, 5.86)
(-0.08, 5.67)
(0.02, 5.49)
(0.16, 5.32)
(0.30, 5.19)
(0.43, 5.07)
(0.54, 4.99)
(0.64, 4.94)
(0.75, 4.92)
(0.88, 4.91)
(1.00, 4.88)
(1.12, 4.83)
(1.25, 4.78)
(1.37, 4.71)
(1.49, 4.64)
(1.63, 4.55)
(1.75, 4.48)
(1.84, 4.40)
(1.91, 4.32)
(1.98, 4.26)
(2.04, 4.21)
(2.09, 4.17)
(2.13, 4.13)
(2.20, 4.12)
(2.29, 4.10)
(2.37, 4.05)
(2.45, 3.96)
(2.52, 3.83)
(2.61, 3.70)
(2.71, 3.57)
(2.82, 3.41)
(2.95, 3.25)
(3.08, 3.08)
(3.19, 2.92)
(3.24, 2.78)
(3.26, 2.70)
(3.30, 2.65)
(3.34, 2.63)
(3.40, 2.63)
(3.48, 2.60)
(3.59, 2.49)
(3.73, 2.34)
(3.87, 2.18)
(3.99, 2.01)
(4.11, 1.84)
(4.22, 1.67)
(4.30, 1.52)
(4.36, 1.40)
(4.39, 1.30)
(4.41, 1.21)
(4.44, 1.12)
(4.46, 0.99)
(4.50, 0.85)
(4.53, 0.71)
(4.54, 0.63)
(4.54, 0.58)
(4.53, 0.58)
(4.53, 0.63)
(4.56, 0.71)
(4.58, 0.78)
(4.61, 0.85)
(4.63, 0.91)
(4.67, 0.95)
(4.71, 0.97)
(4.75, 0.98)
(4.77, 1.02)
(4.76, 1.05)
(4.73, 1.10)
(4.72, 1.14)
(4.68, 1.24)
(4.60, 1.38)
(4.52, 1.52)
(4.45, 1.64)
(4.43, 1.74)
(4.43, 1.84)
(4.42, 1.94)
(4.41, 2.00)
(4.37, 1.99)
(4.32, 1.92)
(4.26, 1.89)
(4.18, 1.90)
(4.08, 1.90)
(3.98, 1.90)
(3.90, 1.93)
(3.82, 1.96)
(3.80, 2.01)
(3.80, 2.06)
(3.80, 2.08)
(3.81, 2.04)
(3.84, 1.97)
(3.86, 1.89)
(3.85, 1.80)
(3.85, 1.74)
(3.85, 1.75)
(3.84, 1.77)
(3.84, 1.78)
(3.83, 1.76)
(3.80, 1.71)
(3.78, 1.63)
(3.78, 1.53)
(3.81, 1.38)
(3.86, 1.18)
(3.94, 0.97)
(4.00, 0.74)
(4.04, 0.49)
(4.09, 0.25)
(4.17, -0.01)
(4.27, -0.27)
(4.39, -0.54)
(4.48, -0.82)
(4.51, -1.09)
(4.54, -1.34)
(4.52, -1.51)
(4.51, -1.62)
(4.53, -1.66)
(4.57, -1.68)
(4.61, -1.69)
(4.65, -1.71)
(4.68, -1.75)
(4.66, -1.80)
(4.63, -1.85)
(4.62, -1.87)
(4.59, -1.93)
    };
%


==> plots/euroc_traj_coords/mh01_ice_ba.tex <==
\addplot[
    fill=none,draw = clr2,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(4.73, -1.76)
(4.74, -1.77)
(4.76, -1.79)
(4.75, -1.78)
(4.70, -1.77)
(4.70, -1.75)
(4.73, -1.76)
(4.76, -1.78)
(4.74, -1.77)
(4.71, -1.75)
(4.70, -1.74)
(4.73, -1.75)
(4.76, -1.76)
(4.75, -1.76)
(4.71, -1.74)
(4.69, -1.73)
(4.70, -1.73)
(4.74, -1.74)
(4.77, -1.75)
(4.79, -1.77)
(4.81, -1.76)
(4.80, -1.74)
(4.80, -1.68)
(4.82, -1.56)
(4.86, -1.45)
(4.86, -1.43)
(4.85, -1.51)
(4.81, -1.66)
(4.77, -1.82)
(4.73, -1.97)
(4.71, -2.04)
(4.75, -1.97)
(4.80, -1.82)
(4.83, -1.67)
(4.84, -1.59)
(4.82, -1.56)
(4.77, -1.50)
(4.65, -1.51)
(4.55, -1.65)
(4.60, -1.86)
(4.76, -1.91)
(4.91, -1.78)
(4.91, -1.58)
(4.77, -1.48)
(4.62, -1.67)
(4.63, -1.85)
(4.78, -1.76)
(4.94, -1.68)
(5.02, -1.83)
(5.01, -1.88)
(4.84, -1.76)
(4.65, -1.68)
(4.65, -1.76)
(4.78, -1.82)
(4.76, -1.77)
(4.66, -1.71)
(4.62, -1.68)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.60, -1.67)
(4.62, -1.66)
(4.66, -1.63)
(4.71, -1.61)
(4.70, -1.60)
(4.65, -1.61)
(4.60, -1.62)
(4.58, -1.59)
(4.61, -1.56)
(4.64, -1.54)
(4.68, -1.51)
(4.70, -1.47)
(4.67, -1.42)
(4.65, -1.35)
(4.66, -1.25)
(4.64, -1.14)
(4.62, -1.00)
(4.57, -0.82)
(4.49, -0.63)
(4.42, -0.46)
(4.32, -0.28)
(4.22, -0.11)
(4.12, 0.05)
(4.01, 0.18)
(3.91, 0.29)
(3.78, 0.40)
(3.63, 0.53)
(3.47, 0.65)
(3.28, 0.80)
(3.07, 0.99)
(2.86, 1.18)
(2.66, 1.34)
(2.46, 1.49)
(2.23, 1.65)
(2.00, 1.84)
(1.77, 2.05)
(1.57, 2.23)
(1.43, 2.33)
(1.28, 2.40)
(1.13, 2.46)
(0.97, 2.52)
(0.83, 2.58)
(0.66, 2.68)
(0.46, 2.82)
(0.25, 3.01)
(0.05, 3.19)
(-0.13, 3.35)
(-0.28, 3.49)
(-0.41, 3.61)
(-0.51, 3.70)
(-0.60, 3.79)
(-0.68, 3.88)
(-0.73, 3.97)
(-0.75, 4.02)
(-0.78, 4.08)
(-0.83, 4.16)
(-0.89, 4.25)
(-0.99, 4.37)
(-1.16, 4.51)
(-1.30, 4.70)
(-1.41, 4.88)
(-1.60, 5.08)
(-1.85, 5.29)
(-2.12, 5.54)
(-2.35, 5.80)
(-2.51, 6.05)
(-2.63, 6.28)
(-2.74, 6.49)
(-2.77, 6.65)
(-2.76, 6.84)
(-2.71, 7.00)
(-2.64, 7.15)
(-2.59, 7.32)
(-2.54, 7.46)
(-2.44, 7.60)
(-2.32, 7.67)
(-2.20, 7.69)
(-2.09, 7.71)
(-1.98, 7.70)
(-1.87, 7.66)
(-1.70, 7.61)
(-1.51, 7.49)
(-1.30, 7.43)
(-1.11, 7.44)
(-0.94, 7.45)
(-0.78, 7.45)
(-0.64, 7.40)
(-0.52, 7.30)
(-0.43, 7.21)
(-0.34, 7.11)
(-0.28, 6.95)
(-0.20, 6.76)
(-0.12, 6.59)
(0.01, 6.43)
(0.14, 6.27)
(0.22, 6.08)
(0.33, 5.85)
(0.45, 5.58)
(0.65, 5.34)
(0.83, 5.14)
(1.00, 4.99)
(1.10, 4.84)
(1.17, 4.72)
(1.21, 4.62)
(1.26, 4.58)
(1.33, 4.60)
(1.31, 4.67)
(1.25, 4.73)
(1.16, 4.78)
(1.06, 4.78)
(0.94, 4.77)
(0.84, 4.77)
(0.82, 4.76)
(0.85, 4.81)
(0.88, 5.00)
(0.85, 5.26)
(0.76, 5.53)
(0.63, 5.78)
(0.51, 6.02)
(0.39, 6.27)
(0.25, 6.51)
(0.10, 6.70)
(-0.03, 6.86)
(-0.11, 7.01)
(-0.20, 7.17)
(-0.28, 7.33)
(-0.33, 7.49)
(-0.36, 7.68)
(-0.42, 7.89)
(-0.54, 8.11)
(-0.70, 8.33)
(-0.92, 8.47)
(-1.09, 8.47)
(-1.14, 8.28)
(-1.02, 7.90)
(-0.70, 7.36)
(-0.33, 6.81)
(0.03, 6.44)
(0.30, 6.29)
(0.45, 6.22)
(0.53, 6.18)
(0.54, 6.22)
(0.50, 6.36)
(0.38, 6.50)
(0.22, 6.64)
(0.11, 6.78)
(0.02, 7.00)
(-0.12, 7.29)
(-0.30, 7.55)
(-0.48, 7.78)
(-0.72, 7.98)
(-0.97, 8.16)
(-1.22, 8.34)
(-1.45, 8.45)
(-1.63, 8.52)
(-1.76, 8.61)
(-1.87, 8.70)
(-1.99, 8.72)
(-2.10, 8.68)
(-2.16, 8.65)
(-2.16, 8.62)
(-2.09, 8.51)
(-1.98, 8.29)
(-1.88, 8.07)
(-1.79, 7.84)
(-1.69, 7.58)
(-1.57, 7.32)
(-1.46, 7.08)
(-1.34, 6.83)
(-1.19, 6.57)
(-1.03, 6.32)
(-0.87, 6.07)
(-0.71, 5.84)
(-0.54, 5.62)
(-0.35, 5.45)
(-0.14, 5.28)
(0.06, 5.09)
(0.25, 4.90)
(0.44, 4.70)
(0.60, 4.51)
(0.74, 4.35)
(0.87, 4.20)
(1.00, 4.08)
(1.13, 3.97)
(1.27, 3.85)
(1.42, 3.71)
(1.55, 3.55)
(1.64, 3.39)
(1.67, 3.24)
(1.62, 3.16)
(1.51, 3.09)
(1.35, 3.10)
(1.24, 3.28)
(1.21, 3.55)
(1.21, 3.81)
(1.24, 4.06)
(1.29, 4.30)
(1.34, 4.46)
(1.37, 4.54)
(1.32, 4.60)
(1.22, 4.65)
(1.14, 4.68)
(1.06, 4.71)
(0.98, 4.76)
(0.90, 4.80)
(0.84, 4.84)
(0.79, 4.87)
(0.76, 4.87)
(0.76, 4.88)
(0.80, 4.83)
(0.87, 4.73)
(0.94, 4.60)
(1.01, 4.45)
(1.06, 4.29)
(1.11, 4.12)
(1.13, 3.99)
(1.17, 3.92)
(1.22, 3.89)
(1.28, 3.90)
(1.37, 3.94)
(1.47, 3.97)
(1.55, 4.05)
(1.62, 4.14)
(1.69, 4.24)
(1.75, 4.32)
(1.78, 4.43)
(1.78, 4.57)
(1.81, 4.72)
(1.83, 4.85)
(1.87, 4.98)
(1.88, 5.14)
(1.86, 5.33)
(1.77, 5.59)
(1.63, 5.86)
(1.48, 6.14)
(1.37, 6.42)
(1.24, 6.68)
(1.08, 6.95)
(0.88, 7.22)
(0.67, 7.47)
(0.44, 7.76)
(0.24, 8.05)
(0.10, 8.35)
(-0.04, 8.57)
(-0.21, 8.73)
(-0.41, 8.86)
(-0.66, 8.95)
(-0.93, 9.03)
(-1.13, 9.10)
(-1.33, 9.13)
(-1.51, 9.10)
(-1.66, 8.98)
(-1.76, 8.84)
(-1.84, 8.64)
(-1.84, 8.40)
(-1.82, 8.13)
(-1.76, 7.85)
(-1.66, 7.61)
(-1.54, 7.39)
(-1.37, 7.21)
(-1.29, 7.07)
(-1.25, 6.97)
(-1.19, 6.90)
(-1.09, 6.83)
(-0.96, 6.75)
(-0.82, 6.66)
(-0.68, 6.57)
(-0.53, 6.46)
(-0.40, 6.30)
(-0.28, 6.08)
(-0.17, 5.85)
(-0.09, 5.65)
(0.01, 5.49)
(0.14, 5.32)
(0.29, 5.17)
(0.42, 5.05)
(0.53, 4.96)
(0.63, 4.90)
(0.74, 4.89)
(0.85, 4.87)
(0.97, 4.85)
(1.09, 4.81)
(1.21, 4.76)
(1.33, 4.70)
(1.44, 4.63)
(1.57, 4.54)
(1.70, 4.46)
(1.80, 4.39)
(1.88, 4.31)
(1.95, 4.24)
(2.01, 4.20)
(2.06, 4.15)
(2.09, 4.12)
(2.13, 4.09)
(2.21, 4.09)
(2.30, 4.05)
(2.38, 4.00)
(2.46, 3.90)
(2.53, 3.78)
(2.62, 3.66)
(2.71, 3.52)
(2.82, 3.37)
(2.95, 3.21)
(3.07, 3.03)
(3.16, 2.88)
(3.21, 2.75)
(3.23, 2.67)
(3.26, 2.63)
(3.30, 2.61)
(3.36, 2.61)
(3.45, 2.58)
(3.54, 2.48)
(3.66, 2.34)
(3.79, 2.19)
(3.91, 2.03)
(4.03, 1.86)
(4.13, 1.70)
(4.22, 1.55)
(4.27, 1.42)
(4.31, 1.32)
(4.33, 1.23)
(4.35, 1.15)
(4.38, 1.05)
(4.41, 0.91)
(4.45, 0.77)
(4.48, 0.66)
(4.49, 0.60)
(4.48, 0.58)
(4.46, 0.59)
(4.48, 0.65)
(4.50, 0.72)
(4.52, 0.78)
(4.54, 0.84)
(4.57, 0.89)
(4.61, 0.93)
(4.65, 0.93)
(4.69, 0.95)
(4.71, 0.98)
(4.69, 1.01)
(4.66, 1.06)
(4.65, 1.10)
(4.61, 1.19)
(4.53, 1.33)
(4.45, 1.47)
(4.37, 1.58)
(4.36, 1.68)
(4.36, 1.77)
(4.35, 1.86)
(4.34, 1.92)
(4.31, 1.93)
(4.26, 1.87)
(4.19, 1.83)
(4.12, 1.84)
(4.03, 1.84)
(3.93, 1.84)
(3.85, 1.86)
(3.78, 1.89)
(3.73, 1.93)
(3.73, 1.98)
(3.74, 2.02)
(3.74, 2.01)
(3.76, 1.96)
(3.78, 1.88)
(3.80, 1.80)
(3.79, 1.72)
(3.79, 1.69)
(3.79, 1.71)
(3.78, 1.73)
(3.78, 1.73)
(3.76, 1.71)
(3.74, 1.65)
(3.72, 1.57)
(3.72, 1.47)
(3.75, 1.32)
(3.79, 1.13)
(3.87, 0.92)
(3.93, 0.70)
(3.96, 0.47)
(4.01, 0.22)
(4.08, -0.03)
(4.18, -0.28)
(4.29, -0.55)
(4.39, -0.83)
(4.44, -1.10)
(4.48, -1.36)
(4.47, -1.54)
(4.44, -1.67)
(4.45, -1.72)
(4.49, -1.73)
(4.52, -1.75)
(4.56, -1.76)
(4.60, -1.79)
(4.60, -1.84)
(4.57, -1.89)
(4.55, -1.92)
(4.53, -1.96)
(4.49, -2.00)
(4.53, -1.97)
(4.53, -1.97)
};
 %   


==> plots/euroc_traj_coords/mh01_ice_ba_fastergpu.tex <==
 \addplot[
    fill=none,draw = clr3,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.82, -1.71)
(4.84, -1.72)
(4.89, -1.75)
(4.86, -1.74)
(4.78, -1.72)
(4.76, -1.72)
(4.81, -1.73)
(4.88, -1.75)
(4.84, -1.75)
(4.77, -1.72)
(4.77, -1.71)
(4.82, -1.72)
(4.88, -1.73)
(4.86, -1.74)
(4.78, -1.71)
(4.75, -1.70)
(4.77, -1.70)
(4.83, -1.71)
(4.86, -1.73)
(4.88, -1.74)
(4.90, -1.72)
(4.89, -1.70)
(4.88, -1.65)
(4.90, -1.52)
(4.93, -1.42)
(4.94, -1.40)
(4.93, -1.48)
(4.90, -1.62)
(4.86, -1.79)
(4.82, -1.94)
(4.80, -2.00)
(4.83, -1.93)
(4.88, -1.78)
(4.91, -1.63)
(4.92, -1.56)
(4.91, -1.53)
(4.85, -1.46)
(4.73, -1.47)
(4.64, -1.62)
(4.69, -1.83)
(4.85, -1.87)
(5.00, -1.75)
(4.99, -1.54)
(4.86, -1.44)
(4.71, -1.63)
(4.72, -1.80)
(4.87, -1.72)
(5.03, -1.63)
(5.11, -1.78)
(5.10, -1.83)
(4.93, -1.71)
(4.73, -1.63)
(4.74, -1.71)
(4.87, -1.77)
(4.85, -1.72)
(4.76, -1.66)
(4.71, -1.63)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.61)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.71, -1.61)
(4.70, -1.62)
(4.70, -1.62)
(4.70, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.62)
(4.71, -1.61)
(4.70, -1.62)
(4.71, -1.61)
(4.71, -1.61)
(4.71, -1.61)
(4.71, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.71, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.71, -1.61)
(4.71, -1.61)
(4.71, -1.61)
(4.71, -1.61)
(4.71, -1.61)
(4.70, -1.61)
(4.71, -1.61)
(4.70, -1.61)
(4.71, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.71, -1.61)
(4.70, -1.61)
(4.70, -1.61)
(4.72, -1.60)
(4.76, -1.57)
(4.80, -1.56)
(4.80, -1.55)
(4.74, -1.56)
(4.69, -1.57)
(4.67, -1.55)
(4.70, -1.51)
(4.73, -1.49)
(4.76, -1.46)
(4.78, -1.42)
(4.75, -1.37)
(4.73, -1.30)
(4.74, -1.20)
(4.71, -1.09)
(4.70, -0.93)
(4.65, -0.75)
(4.59, -0.56)
(4.50, -0.37)
(4.40, -0.19)
(4.31, -0.02)
(4.20, 0.13)
(4.09, 0.26)
(3.99, 0.38)
(3.86, 0.49)
(3.70, 0.61)
(3.54, 0.74)
(3.34, 0.88)
(3.14, 1.04)
(2.93, 1.24)
(2.73, 1.40)
(2.52, 1.54)
(2.30, 1.70)
(2.07, 1.89)
(1.82, 2.10)
(1.63, 2.27)
(1.48, 2.37)
(1.34, 2.44)
(1.18, 2.50)
(1.03, 2.55)
(0.89, 2.61)
(0.72, 2.70)
(0.51, 2.83)
(0.31, 3.02)
(0.12, 3.19)
(-0.06, 3.35)
(-0.21, 3.48)
(-0.34, 3.61)
(-0.45, 3.70)
(-0.54, 3.80)
(-0.61, 3.88)
(-0.65, 3.95)
(-0.67, 4.01)
(-0.70, 4.08)
(-0.75, 4.16)
(-0.80, 4.25)
(-0.91, 4.36)
(-1.08, 4.51)
(-1.22, 4.71)
(-1.32, 4.89)
(-1.50, 5.10)
(-1.76, 5.29)
(-2.04, 5.52)
(-2.27, 5.78)
(-2.45, 6.02)
(-2.57, 6.23)
(-2.68, 6.44)
(-2.74, 6.63)
(-2.70, 6.79)
(-2.66, 6.96)
(-2.62, 7.11)
(-2.57, 7.28)
(-2.52, 7.41)
(-2.40, 7.56)
(-2.28, 7.63)
(-2.15, 7.66)
(-2.04, 7.68)
(-1.95, 7.70)
(-1.84, 7.66)
(-1.68, 7.58)
(-1.47, 7.48)
(-1.29, 7.42)
(-1.10, 7.43)
(-0.91, 7.46)
(-0.76, 7.45)
(-0.63, 7.40)
(-0.55, 7.30)
(-0.44, 7.21)
(-0.37, 7.11)
(-0.30, 6.95)
(-0.25, 6.77)
(-0.15, 6.60)
(-0.02, 6.45)
(0.12, 6.30)
(0.21, 6.09)
(0.33, 5.86)
(0.48, 5.61)
(0.67, 5.37)
(0.89, 5.15)
(1.05, 5.01)
(1.16, 4.87)
(1.24, 4.75)
(1.29, 4.66)
(1.34, 4.62)
(1.39, 4.66)
(1.38, 4.73)
(1.33, 4.80)
(1.23, 4.85)
(1.13, 4.85)
(1.00, 4.85)
(0.91, 4.85)
(0.89, 4.85)
(0.92, 4.90)
(0.95, 5.08)
(0.92, 5.35)
(0.82, 5.62)
(0.70, 5.87)
(0.59, 6.11)
(0.45, 6.36)
(0.32, 6.59)
(0.17, 6.78)
(0.04, 6.93)
(-0.06, 7.08)
(-0.14, 7.23)
(-0.21, 7.38)
(-0.25, 7.52)
(-0.30, 7.71)
(-0.36, 7.92)
(-0.48, 8.14)
(-0.65, 8.36)
(-0.87, 8.50)
(-1.05, 8.50)
(-1.09, 8.31)
(-0.98, 7.93)
(-0.65, 7.40)
(-0.26, 6.86)
(0.11, 6.48)
(0.38, 6.32)
(0.51, 6.26)
(0.59, 6.22)
(0.61, 6.26)
(0.56, 6.40)
(0.44, 6.55)
(0.30, 6.69)
(0.19, 6.84)
(0.10, 7.05)
(-0.04, 7.34)
(-0.25, 7.59)
(-0.44, 7.82)
(-0.67, 8.02)
(-0.94, 8.21)
(-1.19, 8.39)
(-1.44, 8.50)
(-1.62, 8.56)
(-1.76, 8.65)
(-1.88, 8.73)
(-2.01, 8.75)
(-2.11, 8.71)
(-2.17, 8.67)
(-2.19, 8.64)
(-2.13, 8.54)
(-2.00, 8.32)
(-1.88, 8.09)
(-1.80, 7.85)
(-1.69, 7.60)
(-1.57, 7.34)
(-1.45, 7.09)
(-1.33, 6.85)
(-1.18, 6.59)
(-1.01, 6.34)
(-0.85, 6.10)
(-0.70, 5.87)
(-0.53, 5.65)
(-0.34, 5.47)
(-0.14, 5.30)
(0.04, 5.13)
(0.25, 4.93)
(0.44, 4.74)
(0.62, 4.53)
(0.76, 4.34)
(0.89, 4.19)
(1.02, 4.07)
(1.16, 3.96)
(1.30, 3.84)
(1.45, 3.70)
(1.58, 3.53)
(1.67, 3.37)
(1.69, 3.24)
(1.64, 3.15)
(1.53, 3.08)
(1.37, 3.10)
(1.26, 3.28)
(1.23, 3.54)
(1.23, 3.80)
(1.25, 4.05)
(1.29, 4.26)
(1.33, 4.41)
(1.36, 4.50)
(1.32, 4.56)
(1.21, 4.59)
(1.13, 4.63)
(1.05, 4.65)
(0.97, 4.70)
(0.89, 4.75)
(0.84, 4.79)
(0.79, 4.82)
(0.75, 4.82)
(0.75, 4.82)
(0.79, 4.78)
(0.86, 4.67)
(0.93, 4.56)
(1.00, 4.41)
(1.06, 4.25)
(1.10, 4.09)
(1.13, 3.95)
(1.17, 3.88)
(1.22, 3.85)
(1.29, 3.86)
(1.38, 3.91)
(1.49, 3.94)
(1.56, 4.01)
(1.63, 4.10)
(1.70, 4.19)
(1.77, 4.28)
(1.81, 4.39)
(1.81, 4.53)
(1.84, 4.67)
(1.87, 4.81)
(1.90, 4.95)
(1.93, 5.11)
(1.91, 5.31)
(1.83, 5.58)
(1.70, 5.85)
(1.54, 6.14)
(1.43, 6.44)
(1.30, 6.72)
(1.11, 6.97)
(0.92, 7.25)
(0.69, 7.52)
(0.45, 7.82)
(0.25, 8.12)
(0.12, 8.40)
(-0.03, 8.63)
(-0.20, 8.79)
(-0.39, 8.91)
(-0.64, 9.01)
(-0.88, 9.09)
(-1.09, 9.16)
(-1.29, 9.19)
(-1.47, 9.17)
(-1.61, 9.05)
(-1.71, 8.90)
(-1.79, 8.71)
(-1.80, 8.47)
(-1.77, 8.17)
(-1.71, 7.90)
(-1.61, 7.65)
(-1.49, 7.43)
(-1.37, 7.25)
(-1.28, 7.10)
(-1.25, 6.99)
(-1.20, 6.92)
(-1.10, 6.84)
(-0.96, 6.76)
(-0.82, 6.67)
(-0.69, 6.58)
(-0.55, 6.46)
(-0.41, 6.30)
(-0.30, 6.08)
(-0.22, 5.86)
(-0.13, 5.68)
(-0.03, 5.50)
(0.09, 5.34)
(0.22, 5.21)
(0.32, 5.08)
(0.43, 4.99)
(0.53, 4.94)
(0.63, 4.91)
(0.74, 4.88)
(0.85, 4.85)
(0.97, 4.80)
(1.09, 4.75)
(1.20, 4.69)
(1.32, 4.63)
(1.44, 4.54)
(1.57, 4.45)
(1.67, 4.38)
(1.75, 4.29)
(1.81, 4.22)
(1.87, 4.17)
(1.92, 4.13)
(1.95, 4.09)
(1.99, 4.06)
(2.06, 4.05)
(2.13, 4.03)
(2.22, 3.96)
(2.29, 3.86)
(2.36, 3.74)
(2.45, 3.61)
(2.54, 3.48)
(2.66, 3.32)
(2.78, 3.15)
(2.89, 2.99)
(2.99, 2.83)
(3.04, 2.70)
(3.06, 2.60)
(3.11, 2.57)
(3.15, 2.53)
(3.21, 2.52)
(3.28, 2.48)
(3.39, 2.39)
(3.52, 2.25)
(3.63, 2.08)
(3.74, 1.91)
(3.84, 1.74)
(3.94, 1.57)
(4.03, 1.42)
(4.08, 1.28)
(4.12, 1.18)
(4.14, 1.09)
(4.14, 0.99)
(4.17, 0.89)
(4.19, 0.75)
(4.23, 0.61)
(4.25, 0.49)
(4.25, 0.42)
(4.23, 0.40)
(4.22, 0.41)
(4.24, 0.49)
(4.26, 0.56)
(4.29, 0.64)
(4.32, 0.72)
(4.36, 0.77)
(4.40, 0.82)
(4.45, 0.82)
(4.49, 0.84)
(4.50, 0.87)
(4.49, 0.90)
(4.47, 0.95)
(4.46, 1.00)
(4.42, 1.09)
(4.35, 1.23)
(4.27, 1.38)
(4.22, 1.50)
(4.22, 1.58)
(4.21, 1.70)
(4.21, 1.80)
(4.20, 1.85)
(4.17, 1.86)
(4.11, 1.80)
(4.05, 1.76)
(3.98, 1.77)
(3.89, 1.77)
(3.78, 1.76)
(3.70, 1.78)
(3.63, 1.81)
(3.58, 1.85)
(3.58, 1.90)
(3.58, 1.94)
(3.58, 1.92)
(3.59, 1.87)
(3.61, 1.79)
(3.61, 1.70)
(3.60, 1.62)
(3.60, 1.59)
(3.61, 1.60)
(3.60, 1.61)
(3.58, 1.61)
(3.57, 1.59)
(3.54, 1.53)
(3.52, 1.45)
(3.52, 1.35)
(3.54, 1.19)
(3.58, 1.01)
(3.65, 0.80)
(3.69, 0.58)
(3.72, 0.34)
(3.77, 0.10)
(3.85, -0.15)
(3.94, -0.41)
(4.05, -0.67)
(4.14, -0.95)
(4.17, -1.23)
(4.22, -1.49)
(4.21, -1.67)
(4.19, -1.80)
(4.22, -1.85)
(4.26, -1.87)
(4.30, -1.89)
(4.36, -1.91)
(4.39, -1.94)
(4.41, -1.98)
(4.37, -2.03)
(4.36, -2.06)
(4.34, -2.10)
(4.30, -2.14)
(4.34, -2.11)
(4.34, -2.10)
};


==> plots/euroc_traj_coords/mh01_ice_ba_jetson_slam.tex <==
\addplot[
    fill=none,draw = clr4,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.64, -1.76)
(4.65, -1.77)
(4.77, -1.82)
(4.71, -1.81)
(4.59, -1.76)
(4.57, -1.76)
(4.66, -1.79)
(4.74, -1.83)
(4.67, -1.81)
(4.57, -1.76)
(4.56, -1.75)
(4.66, -1.77)
(4.76, -1.80)
(4.73, -1.79)
(4.61, -1.74)
(4.56, -1.73)
(4.60, -1.74)
(4.68, -1.75)
(4.71, -1.76)
(4.73, -1.78)
(4.74, -1.78)
(4.73, -1.76)
(4.73, -1.70)
(4.75, -1.58)
(4.78, -1.47)
(4.79, -1.45)
(4.77, -1.53)
(4.74, -1.68)
(4.69, -1.84)
(4.65, -1.99)
(4.64, -2.06)
(4.67, -1.99)
(4.72, -1.84)
(4.76, -1.69)
(4.76, -1.62)
(4.75, -1.59)
(4.69, -1.52)
(4.57, -1.53)
(4.47, -1.68)
(4.52, -1.89)
(4.68, -1.94)
(4.82, -1.81)
(4.82, -1.60)
(4.68, -1.50)
(4.54, -1.69)
(4.55, -1.87)
(4.70, -1.78)
(4.86, -1.70)
(4.95, -1.84)
(4.94, -1.89)
(4.76, -1.77)
(4.57, -1.70)
(4.57, -1.78)
(4.71, -1.83)
(4.68, -1.78)
(4.59, -1.72)
(4.54, -1.70)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.69)
(4.53, -1.68)
(4.52, -1.68)
(4.52, -1.69)
(4.52, -1.69)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.53, -1.68)
(4.53, -1.68)
(4.53, -1.68)
(4.53, -1.68)
(4.53, -1.68)
(4.53, -1.68)
(4.53, -1.68)
(4.53, -1.68)
(4.53, -1.68)
(4.53, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.53, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.53, -1.68)
(4.52, -1.68)
(4.52, -1.68)
(4.54, -1.67)
(4.58, -1.64)
(4.63, -1.62)
(4.62, -1.62)
(4.57, -1.63)
(4.52, -1.63)
(4.50, -1.61)
(4.53, -1.58)
(4.56, -1.55)
(4.60, -1.52)
(4.61, -1.48)
(4.58, -1.44)
(4.57, -1.37)
(4.58, -1.27)
(4.55, -1.15)
(4.54, -1.01)
(4.49, -0.84)
(4.41, -0.64)
(4.32, -0.46)
(4.23, -0.29)
(4.13, -0.12)
(4.03, 0.05)
(3.92, 0.18)
(3.81, 0.28)
(3.69, 0.39)
(3.53, 0.52)
(3.36, 0.64)
(3.17, 0.79)
(2.97, 0.97)
(2.76, 1.16)
(2.57, 1.33)
(2.37, 1.47)
(2.16, 1.62)
(1.94, 1.80)
(1.70, 2.01)
(1.51, 2.19)
(1.36, 2.28)
(1.20, 2.35)
(1.05, 2.41)
(0.90, 2.47)
(0.77, 2.53)
(0.59, 2.63)
(0.37, 2.76)
(0.16, 2.95)
(-0.04, 3.13)
(-0.21, 3.29)
(-0.37, 3.43)
(-0.50, 3.54)
(-0.61, 3.64)
(-0.70, 3.73)
(-0.77, 3.81)
(-0.82, 3.89)
(-0.85, 3.95)
(-0.86, 4.01)
(-0.90, 4.08)
(-0.97, 4.17)
(-1.09, 4.29)
(-1.25, 4.42)
(-1.39, 4.61)
(-1.50, 4.78)
(-1.68, 4.99)
(-1.93, 5.21)
(-2.20, 5.43)
(-2.43, 5.70)
(-2.60, 5.95)
(-2.73, 6.17)
(-2.84, 6.38)
(-2.89, 6.59)
(-2.86, 6.75)
(-2.81, 6.92)
(-2.76, 7.07)
(-2.70, 7.24)
(-2.62, 7.38)
(-2.54, 7.50)
(-2.42, 7.56)
(-2.30, 7.58)
(-2.18, 7.63)
(-2.06, 7.61)
(-1.95, 7.58)
(-1.80, 7.50)
(-1.57, 7.41)
(-1.38, 7.35)
(-1.19, 7.36)
(-0.99, 7.40)
(-0.84, 7.39)
(-0.70, 7.34)
(-0.56, 7.26)
(-0.45, 7.16)
(-0.36, 7.06)
(-0.29, 6.90)
(-0.23, 6.73)
(-0.12, 6.56)
(0.03, 6.41)
(0.17, 6.25)
(0.27, 6.05)
(0.39, 5.82)
(0.54, 5.56)
(0.74, 5.33)
(0.94, 5.14)
(1.10, 5.01)
(1.22, 4.87)
(1.30, 4.75)
(1.34, 4.65)
(1.39, 4.61)
(1.43, 4.65)
(1.42, 4.71)
(1.35, 4.77)
(1.26, 4.82)
(1.15, 4.82)
(1.02, 4.82)
(0.92, 4.82)
(0.90, 4.81)
(0.92, 4.86)
(0.95, 5.04)
(0.91, 5.31)
(0.81, 5.57)
(0.68, 5.82)
(0.56, 6.06)
(0.45, 6.30)
(0.34, 6.51)
(0.14, 6.73)
(0.01, 6.87)
(-0.09, 7.02)
(-0.18, 7.16)
(-0.25, 7.31)
(-0.30, 7.46)
(-0.36, 7.65)
(-0.42, 7.85)
(-0.54, 8.07)
(-0.71, 8.26)
(-0.94, 8.41)
(-1.11, 8.41)
(-1.16, 8.22)
(-1.04, 7.85)
(-0.69, 7.34)
(-0.29, 6.82)
(0.07, 6.46)
(0.34, 6.31)
(0.49, 6.25)
(0.58, 6.21)
(0.61, 6.26)
(0.56, 6.39)
(0.43, 6.54)
(0.27, 6.67)
(0.15, 6.81)
(0.06, 7.02)
(-0.09, 7.31)
(-0.31, 7.56)
(-0.50, 7.78)
(-0.75, 7.99)
(-1.02, 8.17)
(-1.27, 8.33)
(-1.51, 8.43)
(-1.69, 8.49)
(-1.83, 8.58)
(-1.95, 8.66)
(-2.07, 8.68)
(-2.18, 8.63)
(-2.25, 8.60)
(-2.25, 8.57)
(-2.17, 8.47)
(-2.04, 8.26)
(-1.92, 8.03)
(-1.84, 7.79)
(-1.73, 7.54)
(-1.60, 7.28)
(-1.48, 7.03)
(-1.36, 6.78)
(-1.20, 6.52)
(-1.03, 6.28)
(-0.86, 6.04)
(-0.71, 5.82)
(-0.54, 5.61)
(-0.35, 5.45)
(-0.16, 5.28)
(0.06, 5.09)
(0.25, 4.90)
(0.45, 4.71)
(0.62, 4.53)
(0.76, 4.36)
(0.88, 4.22)
(1.02, 4.10)
(1.16, 3.99)
(1.31, 3.86)
(1.46, 3.72)
(1.61, 3.56)
(1.70, 3.40)
(1.74, 3.25)
(1.69, 3.17)
(1.59, 3.10)
(1.43, 3.11)
(1.32, 3.30)
(1.29, 3.56)
(1.28, 3.82)
(1.30, 4.07)
(1.34, 4.30)
(1.39, 4.46)
(1.42, 4.54)
(1.37, 4.60)
(1.26, 4.63)
(1.18, 4.67)
(1.10, 4.69)
(1.02, 4.74)
(0.94, 4.78)
(0.88, 4.81)
(0.84, 4.84)
(0.80, 4.84)
(0.80, 4.85)
(0.84, 4.81)
(0.91, 4.71)
(0.99, 4.59)
(1.06, 4.44)
(1.12, 4.28)
(1.16, 4.12)
(1.19, 3.98)
(1.24, 3.91)
(1.28, 3.88)
(1.35, 3.89)
(1.44, 3.93)
(1.53, 3.98)
(1.61, 4.05)
(1.67, 4.13)
(1.75, 4.22)
(1.81, 4.30)
(1.85, 4.41)
(1.84, 4.55)
(1.87, 4.70)
(1.89, 4.84)
(1.92, 4.97)
(1.93, 5.12)
(1.91, 5.32)
(1.81, 5.59)
(1.68, 5.86)
(1.51, 6.13)
(1.39, 6.41)
(1.26, 6.68)
(1.08, 6.96)
(0.88, 7.22)
(0.65, 7.50)
(0.41, 7.80)
(0.19, 8.10)
(0.05, 8.37)
(-0.10, 8.60)
(-0.27, 8.76)
(-0.45, 8.84)
(-0.70, 8.93)
(-0.96, 8.99)
(-1.17, 9.06)
(-1.36, 9.09)
(-1.55, 9.06)
(-1.69, 8.95)
(-1.78, 8.80)
(-1.82, 8.60)
(-1.83, 8.36)
(-1.80, 8.10)
(-1.71, 7.83)
(-1.60, 7.59)
(-1.47, 7.38)
(-1.35, 7.21)
(-1.25, 7.08)
(-1.23, 6.96)
(-1.18, 6.90)
(-1.07, 6.82)
(-0.93, 6.74)
(-0.79, 6.66)
(-0.67, 6.56)
(-0.53, 6.46)
(-0.39, 6.30)
(-0.26, 6.07)
(-0.16, 5.84)
(-0.06, 5.66)
(0.04, 5.49)
(0.17, 5.34)
(0.31, 5.20)
(0.44, 5.06)
(0.56, 4.98)
(0.66, 4.93)
(0.76, 4.91)
(0.88, 4.89)
(1.00, 4.86)
(1.12, 4.83)
(1.24, 4.78)
(1.36, 4.72)
(1.47, 4.66)
(1.60, 4.57)
(1.73, 4.49)
(1.84, 4.42)
(1.93, 4.35)
(2.00, 4.28)
(2.06, 4.24)
(2.11, 4.20)
(2.15, 4.16)
(2.19, 4.13)
(2.26, 4.12)
(2.35, 4.10)
(2.43, 4.04)
(2.51, 3.94)
(2.58, 3.82)
(2.68, 3.71)
(2.78, 3.58)
(2.89, 3.43)
(3.01, 3.27)
(3.14, 3.10)
(3.24, 2.95)
(3.29, 2.82)
(3.32, 2.74)
(3.34, 2.70)
(3.41, 2.68)
(3.47, 2.67)
(3.56, 2.64)
(3.66, 2.55)
(3.79, 2.41)
(3.93, 2.26)
(4.07, 2.13)
(4.16, 1.95)
(4.27, 1.79)
(4.36, 1.65)
(4.41, 1.50)
(4.45, 1.40)
(4.47, 1.31)
(4.51, 1.22)
(4.53, 1.11)
(4.57, 0.97)
(4.60, 0.82)
(4.63, 0.71)
(4.63, 0.65)
(4.60, 0.61)
(4.60, 0.63)
(4.62, 0.70)
(4.65, 0.78)
(4.66, 0.85)
(4.68, 0.91)
(4.70, 0.96)
(4.74, 1.01)
(4.78, 1.01)
(4.82, 1.02)
(4.84, 1.05)
(4.81, 1.09)
(4.78, 1.13)
(4.76, 1.17)
(4.72, 1.26)
(4.64, 1.40)
(4.54, 1.54)
(4.47, 1.65)
(4.45, 1.76)
(4.44, 1.85)
(4.43, 1.93)
(4.41, 2.00)
(4.38, 2.00)
(4.34, 1.95)
(4.28, 1.91)
(4.21, 1.92)
(4.13, 1.92)
(4.02, 1.92)
(3.95, 1.94)
(3.87, 1.96)
(3.82, 2.00)
(3.83, 2.06)
(3.83, 2.09)
(3.83, 2.08)
(3.85, 2.03)
(3.88, 1.96)
(3.89, 1.87)
(3.88, 1.80)
(3.89, 1.76)
(3.89, 1.78)
(3.88, 1.80)
(3.88, 1.81)
(3.86, 1.79)
(3.83, 1.73)
(3.82, 1.65)
(3.82, 1.54)
(3.86, 1.39)
(3.91, 1.20)
(3.98, 0.99)
(4.04, 0.76)
(4.09, 0.53)
(4.13, 0.29)
(4.21, 0.04)
(4.32, -0.21)
(4.45, -0.48)
(4.54, -0.75)
(4.57, -1.03)
(4.61, -1.28)
(4.62, -1.46)
(4.60, -1.59)
(4.61, -1.63)
(4.66, -1.66)
(4.69, -1.68)
(4.74, -1.69)
(4.77, -1.72)
(4.77, -1.77)
(4.74, -1.83)
(4.72, -1.85)
(4.70, -1.90)
(4.66, -1.94)
(4.69, -1.91)
(4.69, -1.91)
};
 %   


==> plots/euroc_traj_coords/mh01_orbslam2.tex <==
\addplot[
    fill=none,draw = clr5,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.68, -1.76)
(4.68, -1.77)
(4.69, -1.79)
(4.68, -1.78)
(4.66, -1.77)
(4.66, -1.77)
(4.68, -1.77)
(4.69, -1.78)
(4.68, -1.79)
(4.66, -1.76)
(4.67, -1.76)
(4.67, -1.75)
(4.69, -1.76)
(4.69, -1.77)
(4.66, -1.75)
(4.65, -1.75)
(4.65, -1.74)
(4.68, -1.75)
(4.71, -1.76)
(4.73, -1.78)
(4.76, -1.77)
(4.75, -1.75)
(4.75, -1.69)
(4.77, -1.57)
(4.80, -1.47)
(4.81, -1.45)
(4.79, -1.53)
(4.76, -1.67)
(4.72, -1.84)
(4.69, -1.99)
(4.67, -2.05)
(4.70, -1.98)
(4.75, -1.83)
(4.78, -1.69)
(4.79, -1.61)
(4.76, -1.57)
(4.71, -1.51)
(4.59, -1.51)
(4.51, -1.67)
(4.57, -1.88)
(4.73, -1.93)
(4.85, -1.80)
(4.84, -1.58)
(4.70, -1.48)
(4.57, -1.68)
(4.60, -1.85)
(4.74, -1.77)
(4.88, -1.69)
(4.96, -1.84)
(4.95, -1.89)
(4.78, -1.77)
(4.60, -1.69)
(4.61, -1.77)
(4.74, -1.82)
(4.72, -1.78)
(4.62, -1.71)
(4.57, -1.69)
(4.55, -1.68)
(4.56, -1.68)
(4.56, -1.68)
(4.56, -1.68)
(4.56, -1.68)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.68)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.68)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.68)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.68)
(4.56, -1.67)
(4.56, -1.68)
(4.56, -1.68)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.68)
(4.56, -1.68)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.56, -1.67)
(4.57, -1.66)
(4.62, -1.63)
(4.66, -1.61)
(4.66, -1.61)
(4.61, -1.62)
(4.56, -1.62)
(4.54, -1.60)
(4.57, -1.57)
(4.60, -1.54)
(4.63, -1.52)
(4.65, -1.47)
(4.62, -1.42)
(4.61, -1.35)
(4.61, -1.25)
(4.58, -1.14)
(4.56, -0.99)
(4.50, -0.81)
(4.44, -0.63)
(4.35, -0.44)
(4.27, -0.27)
(4.17, -0.10)
(4.08, 0.06)
(3.98, 0.19)
(3.87, 0.29)
(3.75, 0.40)
(3.61, 0.52)
(3.44, 0.64)
(3.25, 0.79)
(3.04, 0.96)
(2.83, 1.15)
(2.65, 1.32)
(2.44, 1.46)
(2.23, 1.62)
(2.00, 1.81)
(1.77, 2.03)
(1.59, 2.21)
(1.44, 2.31)
(1.30, 2.38)
(1.15, 2.44)
(0.99, 2.49)
(0.85, 2.55)
(0.66, 2.65)
(0.45, 2.79)
(0.25, 2.98)
(0.05, 3.15)
(-0.13, 3.30)
(-0.27, 3.44)
(-0.39, 3.55)
(-0.51, 3.65)
(-0.60, 3.74)
(-0.68, 3.82)
(-0.73, 3.90)
(-0.75, 3.96)
(-0.79, 4.02)
(-0.83, 4.09)
(-0.89, 4.18)
(-1.01, 4.29)
(-1.18, 4.43)
(-1.32, 4.61)
(-1.42, 4.80)
(-1.61, 5.01)
(-1.85, 5.22)
(-2.13, 5.46)
(-2.37, 5.74)
(-2.54, 5.99)
(-2.67, 6.21)
(-2.77, 6.43)
(-2.81, 6.64)
(-2.81, 6.85)
(-2.75, 7.04)
(-2.67, 7.19)
(-2.63, 7.37)
(-2.56, 7.51)
(-2.48, 7.63)
(-2.36, 7.71)
(-2.25, 7.75)
(-2.11, 7.77)
(-2.00, 7.76)
(-1.89, 7.72)
(-1.75, 7.64)
(-1.54, 7.54)
(-1.36, 7.49)
(-1.16, 7.50)
(-0.99, 7.51)
(-0.84, 7.50)
(-0.71, 7.45)
(-0.60, 7.36)
(-0.48, 7.27)
(-0.40, 7.17)
(-0.33, 7.01)
(-0.25, 6.83)
(-0.13, 6.65)
(0.01, 6.50)
(0.14, 6.33)
(0.23, 6.12)
(0.35, 5.88)
(0.51, 5.62)
(0.71, 5.37)
(0.91, 5.17)
(1.07, 5.02)
(1.17, 4.87)
(1.25, 4.74)
(1.30, 4.64)
(1.34, 4.61)
(1.40, 4.65)
(1.39, 4.72)
(1.33, 4.79)
(1.24, 4.84)
(1.13, 4.83)
(1.00, 4.84)
(0.90, 4.84)
(0.88, 4.83)
(0.91, 4.88)
(0.94, 5.07)
(0.90, 5.34)
(0.81, 5.61)
(0.68, 5.86)
(0.55, 6.11)
(0.43, 6.36)
(0.27, 6.59)
(0.13, 6.79)
(-0.02, 6.94)
(-0.10, 7.09)
(-0.19, 7.24)
(-0.26, 7.39)
(-0.31, 7.54)
(-0.35, 7.73)
(-0.41, 7.94)
(-0.53, 8.16)
(-0.70, 8.37)
(-0.93, 8.50)
(-1.10, 8.50)
(-1.15, 8.30)
(-1.03, 7.91)
(-0.70, 7.36)
(-0.30, 6.82)
(0.06, 6.44)
(0.32, 6.28)
(0.48, 6.22)
(0.56, 6.18)
(0.57, 6.22)
(0.53, 6.36)
(0.41, 6.50)
(0.25, 6.64)
(0.13, 6.78)
(0.04, 6.99)
(-0.10, 7.28)
(-0.31, 7.53)
(-0.51, 7.75)
(-0.75, 7.94)
(-1.02, 8.12)
(-1.27, 8.30)
(-1.50, 8.39)
(-1.67, 8.45)
(-1.79, 8.54)
(-1.91, 8.62)
(-2.02, 8.64)
(-2.11, 8.59)
(-2.16, 8.56)
(-2.17, 8.53)
(-2.10, 8.42)
(-1.98, 8.21)
(-1.87, 7.98)
(-1.80, 7.74)
(-1.71, 7.51)
(-1.58, 7.25)
(-1.47, 7.01)
(-1.35, 6.77)
(-1.20, 6.52)
(-1.03, 6.26)
(-0.86, 6.02)
(-0.71, 5.79)
(-0.54, 5.58)
(-0.35, 5.41)
(-0.14, 5.24)
(0.06, 5.05)
(0.27, 4.85)
(0.46, 4.66)
(0.62, 4.48)
(0.76, 4.31)
(0.88, 4.17)
(1.02, 4.04)
(1.16, 3.94)
(1.31, 3.82)
(1.46, 3.69)
(1.59, 3.51)
(1.69, 3.35)
(1.72, 3.21)
(1.67, 3.12)
(1.55, 3.05)
(1.39, 3.06)
(1.28, 3.25)
(1.25, 3.51)
(1.25, 3.77)
(1.27, 4.02)
(1.31, 4.25)
(1.36, 4.41)
(1.39, 4.50)
(1.35, 4.55)
(1.25, 4.59)
(1.16, 4.62)
(1.08, 4.65)
(1.01, 4.70)
(0.93, 4.76)
(0.87, 4.80)
(0.82, 4.83)
(0.78, 4.83)
(0.78, 4.83)
(0.82, 4.80)
(0.89, 4.69)
(0.96, 4.56)
(1.03, 4.41)
(1.07, 4.25)
(1.10, 4.08)
(1.12, 3.95)
(1.16, 3.87)
(1.20, 3.85)
(1.26, 3.87)
(1.35, 3.91)
(1.46, 3.95)
(1.53, 4.03)
(1.60, 4.11)
(1.67, 4.21)
(1.73, 4.30)
(1.76, 4.41)
(1.76, 4.55)
(1.79, 4.70)
(1.81, 4.83)
(1.84, 4.97)
(1.87, 5.13)
(1.84, 5.33)
(1.75, 5.59)
(1.61, 5.86)
(1.47, 6.14)
(1.35, 6.42)
(1.23, 6.68)
(1.07, 6.95)
(0.87, 7.21)
(0.64, 7.48)
(0.41, 7.78)
(0.20, 8.08)
(0.06, 8.37)
(-0.09, 8.59)
(-0.25, 8.75)
(-0.46, 8.87)
(-0.70, 8.97)
(-0.96, 9.03)
(-1.16, 9.08)
(-1.36, 9.11)
(-1.54, 9.07)
(-1.69, 8.95)
(-1.78, 8.80)
(-1.85, 8.60)
(-1.86, 8.36)
(-1.83, 8.09)
(-1.77, 7.82)
(-1.66, 7.58)
(-1.54, 7.36)
(-1.42, 7.18)
(-1.33, 7.03)
(-1.28, 6.93)
(-1.23, 6.86)
(-1.12, 6.79)
(-0.98, 6.71)
(-0.84, 6.63)
(-0.68, 6.54)
(-0.54, 6.43)
(-0.40, 6.27)
(-0.27, 6.05)
(-0.16, 5.82)
(-0.06, 5.64)
(0.04, 5.46)
(0.18, 5.30)
(0.32, 5.17)
(0.45, 5.05)
(0.56, 4.97)
(0.65, 4.92)
(0.75, 4.90)
(0.86, 4.88)
(0.98, 4.86)
(1.11, 4.82)
(1.23, 4.77)
(1.34, 4.71)
(1.45, 4.64)
(1.59, 4.56)
(1.71, 4.48)
(1.80, 4.41)
(1.88, 4.33)
(1.95, 4.26)
(2.02, 4.21)
(2.07, 4.17)
(2.11, 4.13)
(2.15, 4.10)
(2.23, 4.09)
(2.32, 4.07)
(2.40, 4.01)
(2.48, 3.91)
(2.55, 3.78)
(2.63, 3.66)
(2.74, 3.53)
(2.86, 3.38)
(2.98, 3.21)
(3.10, 3.05)
(3.21, 2.89)
(3.26, 2.76)
(3.28, 2.68)
(3.31, 2.64)
(3.36, 2.62)
(3.41, 2.62)
(3.49, 2.59)
(3.60, 2.50)
(3.73, 2.36)
(3.86, 2.20)
(3.98, 2.04)
(4.09, 1.87)
(4.21, 1.71)
(4.30, 1.56)
(4.37, 1.43)
(4.41, 1.33)
(4.42, 1.24)
(4.45, 1.15)
(4.47, 1.04)
(4.51, 0.90)
(4.54, 0.77)
(4.56, 0.65)
(4.56, 0.59)
(4.55, 0.57)
(4.53, 0.59)
(4.54, 0.66)
(4.56, 0.74)
(4.59, 0.81)
(4.61, 0.88)
(4.64, 0.92)
(4.67, 0.97)
(4.72, 0.98)
(4.76, 1.00)
(4.78, 1.03)
(4.76, 1.07)
(4.73, 1.11)
(4.72, 1.16)
(4.69, 1.25)
(4.61, 1.39)
(4.52, 1.54)
(4.45, 1.65)
(4.43, 1.75)
(4.43, 1.84)
(4.41, 1.94)
(4.40, 2.01)
(4.37, 2.02)
(4.33, 1.95)
(4.26, 1.90)
(4.19, 1.91)
(4.11, 1.91)
(4.00, 1.91)
(3.92, 1.94)
(3.84, 1.96)
(3.79, 2.00)
(3.79, 2.06)
(3.79, 2.09)
(3.79, 2.08)
(3.81, 2.02)
(3.84, 1.95)
(3.85, 1.86)
(3.84, 1.78)
(3.84, 1.75)
(3.84, 1.77)
(3.84, 1.78)
(3.84, 1.77)
(3.84, 1.75)
(3.81, 1.68)
(3.79, 1.60)
(3.79, 1.49)
(3.83, 1.34)
(3.89, 1.15)
(3.97, 0.93)
(4.02, 0.71)
(4.06, 0.48)
(4.12, 0.24)
(4.19, -0.01)
(4.28, -0.27)
(4.39, -0.52)
(4.48, -0.79)
(4.51, -1.05)
(4.54, -1.30)
(4.52, -1.48)
(4.50, -1.60)
(4.52, -1.64)
(4.56, -1.67)
(4.60, -1.68)
(4.64, -1.70)
(4.67, -1.73)
(4.68, -1.78)
(4.64, -1.83)
(4.62, -1.85)
(4.61, -1.90)
(4.56, -1.94)
(4.59, -1.91)
(4.59, -1.91)
};


==> plots/euroc_traj_coords/mh02_full_ba_jetson_slam.tex <==
%
\addplot[
    fill=none,draw = clr6,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.61, -1.87)
(4.61, -1.84)
(4.60, -1.82)
(4.60, -1.81)
(4.60, -1.81)
(4.62, -1.81)
(4.63, -1.81)
(4.62, -1.80)
(4.62, -1.79)
(4.62, -1.79)
(4.62, -1.81)
(4.63, -1.81)
(4.62, -1.80)
(4.61, -1.79)
(4.61, -1.79)
(4.62, -1.80)
(4.63, -1.80)
(4.63, -1.80)
(4.62, -1.79)
(4.61, -1.79)
(4.61, -1.80)
(4.61, -1.80)
(4.61, -1.81)
(4.60, -1.81)
(4.61, -1.80)
(4.60, -1.80)
(4.62, -1.80)
(4.65, -1.81)
(4.67, -1.82)
(4.70, -1.83)
(4.71, -1.83)
(4.72, -1.85)
(4.73, -1.87)
(4.74, -1.89)
(4.74, -1.89)
(4.73, -1.88)
(4.74, -1.80)
(4.75, -1.66)
(4.76, -1.51)
(4.77, -1.42)
(4.77, -1.41)
(4.77, -1.44)
(4.74, -1.56)
(4.70, -1.72)
(4.66, -1.88)
(4.64, -1.95)
(4.65, -1.91)
(4.68, -1.76)
(4.71, -1.59)
(4.75, -1.46)
(4.76, -1.44)
(4.74, -1.50)
(4.70, -1.65)
(4.65, -1.81)
(4.61, -1.88)
(4.65, -1.93)
(4.78, -1.92)
(4.89, -1.81)
(4.90, -1.64)
(4.80, -1.48)
(4.63, -1.48)
(4.50, -1.64)
(4.51, -1.83)
(4.62, -1.94)
(4.76, -1.92)
(4.85, -1.78)
(4.85, -1.59)
(4.77, -1.46)
(4.64, -1.46)
(4.57, -1.60)
(4.60, -1.75)
(4.74, -1.77)
(4.87, -1.80)
(4.90, -1.91)
(4.82, -1.99)
(4.70, -1.94)
(4.62, -1.78)
(4.62, -1.63)
(4.68, -1.62)
(4.65, -1.67)
(4.58, -1.70)
(4.53, -1.71)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.71)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.71)
(4.51, -1.72)
(4.51, -1.71)
(4.51, -1.71)
(4.53, -1.70)
(4.59, -1.67)
(4.61, -1.65)
(4.60, -1.63)
(4.57, -1.63)
(4.53, -1.63)
(4.46, -1.61)
(4.40, -1.56)
(4.36, -1.50)
(4.31, -1.42)
(4.29, -1.35)
(4.26, -1.28)
(4.22, -1.19)
(4.15, -1.06)
(4.10, -0.90)
(4.04, -0.75)
(4.00, -0.59)
(3.95, -0.44)
(3.90, -0.29)
(3.85, -0.16)
(3.82, -0.04)
(3.79, 0.08)
(3.72, 0.19)
(3.66, 0.33)
(3.60, 0.49)
(3.55, 0.66)
(3.50, 0.81)
(3.43, 0.93)
(3.35, 1.03)
(3.25, 1.12)
(3.13, 1.19)
(3.01, 1.27)
(2.90, 1.36)
(2.77, 1.44)
(2.61, 1.52)
(2.44, 1.64)
(2.26, 1.77)
(2.09, 1.90)
(1.92, 2.02)
(1.72, 2.15)
(1.50, 2.29)
(1.28, 2.44)
(1.07, 2.58)
(0.88, 2.67)
(0.70, 2.76)
(0.51, 2.84)
(0.35, 2.91)
(0.20, 2.99)
(0.04, 3.06)
(-0.10, 3.15)
(-0.25, 3.25)
(-0.42, 3.36)
(-0.56, 3.49)
(-0.69, 3.64)
(-0.79, 3.79)
(-0.88, 3.94)
(-0.98, 4.09)
(-1.06, 4.24)
(-1.13, 4.38)
(-1.20, 4.50)
(-1.28, 4.62)
(-1.38, 4.73)
(-1.47, 4.87)
(-1.55, 5.00)
(-1.62, 5.13)
(-1.69, 5.22)
(-1.76, 5.30)
(-1.83, 5.36)
(-1.86, 5.41)
(-1.89, 5.44)
(-1.92, 5.45)
(-1.99, 5.42)
(-2.08, 5.43)
(-2.12, 5.48)
(-2.12, 5.54)
(-2.09, 5.60)
(-2.04, 5.64)
(-1.96, 5.69)
(-1.87, 5.70)
(-1.79, 5.71)
(-1.72, 5.71)
(-1.64, 5.70)
(-1.56, 5.73)
(-1.50, 5.76)
(-1.47, 5.78)
(-1.46, 5.79)
(-1.41, 5.81)
(-1.35, 5.81)
(-1.33, 5.85)
(-1.36, 5.92)
(-1.45, 6.00)
(-1.55, 6.11)
(-1.60, 6.25)
(-1.59, 6.40)
(-1.63, 6.54)
(-1.74, 6.74)
(-1.89, 6.93)
(-1.98, 7.09)
(-2.04, 7.22)
(-2.07, 7.36)
(-2.06, 7.52)
(-2.06, 7.69)
(-2.11, 7.92)
(-2.18, 8.17)
(-2.24, 8.41)
(-2.30, 8.64)
(-2.38, 8.85)
(-2.40, 9.05)
(-2.40, 9.22)
(-2.41, 9.38)
(-2.39, 9.51)
(-2.37, 9.63)
(-2.31, 9.74)
(-2.20, 9.84)
(-2.09, 9.88)
(-2.00, 9.86)
(-1.94, 9.82)
(-1.83, 9.74)
(-1.76, 9.61)
(-1.70, 9.43)
(-1.65, 9.27)
(-1.63, 9.14)
(-1.59, 9.02)
(-1.58, 8.88)
(-1.51, 8.73)
(-1.43, 8.57)
(-1.38, 8.44)
(-1.30, 8.30)
(-1.22, 8.15)
(-1.10, 8.04)
(-1.00, 7.98)
(-0.88, 7.95)
(-0.77, 7.90)
(-0.67, 7.86)
(-0.60, 7.83)
(-0.51, 7.81)
(-0.48, 7.77)
(-0.48, 7.66)
(-0.39, 7.52)
(-0.28, 7.35)
(-0.17, 7.20)
(-0.05, 7.03)
(0.05, 6.83)
(0.16, 6.60)
(0.29, 6.35)
(0.42, 6.12)
(0.56, 5.92)
(0.70, 5.73)
(0.83, 5.53)
(0.95, 5.34)
(1.06, 5.15)
(1.22, 4.96)
(1.37, 4.77)
(1.52, 4.59)
(1.66, 4.41)
(1.77, 4.22)
(1.88, 4.05)
(2.00, 3.95)
(2.07, 3.87)
(2.12, 3.79)
(2.13, 3.69)
(2.13, 3.60)
(2.10, 3.54)
(2.07, 3.49)
(2.01, 3.45)
(1.96, 3.40)
(1.98, 3.33)
(2.03, 3.32)
(2.11, 3.36)
(2.17, 3.43)
(2.20, 3.55)
(2.17, 3.71)
(2.07, 3.89)
(1.97, 4.04)
(1.87, 4.16)
(1.80, 4.24)
(1.76, 4.35)
(1.72, 4.50)
(1.67, 4.64)
(1.60, 4.78)
(1.54, 4.90)
(1.50, 5.06)
(1.46, 5.26)
(1.39, 5.45)
(1.32, 5.61)
(1.23, 5.75)
(1.16, 5.89)
(1.13, 6.06)
(1.08, 6.22)
(1.03, 6.43)
(0.95, 6.63)
(0.82, 6.86)
(0.72, 7.08)
(0.61, 7.31)
(0.47, 7.53)
(0.32, 7.77)
(0.17, 7.97)
(0.06, 8.14)
(-0.07, 8.29)
(-0.17, 8.40)
(-0.26, 8.48)
(-0.34, 8.54)
(-0.41, 8.60)
(-0.47, 8.65)
(-0.50, 8.72)
(-0.55, 8.80)
(-0.58, 8.88)
(-0.64, 8.94)
(-0.71, 9.00)
(-0.79, 9.05)
(-0.86, 9.09)
(-1.01, 9.10)
(-1.12, 9.09)
(-1.24, 9.04)
(-1.35, 9.01)
(-1.46, 8.95)
(-1.54, 8.90)
(-1.62, 8.81)
(-1.68, 8.73)
(-1.74, 8.60)
(-1.77, 8.45)
(-1.78, 8.30)
(-1.77, 8.14)
(-1.75, 7.97)
(-1.70, 7.78)
(-1.64, 7.53)
(-1.55, 7.26)
(-1.46, 6.96)
(-1.46, 6.69)
(-1.42, 6.41)
(-1.37, 6.10)
(-1.28, 5.86)
(-1.18, 5.65)
(-1.05, 5.47)
(-0.89, 5.28)
(-0.69, 5.09)
(-0.47, 4.90)
(-0.23, 4.71)
(0.04, 4.51)
(0.32, 4.31)
(0.63, 4.11)
(0.87, 3.92)
(1.09, 3.73)
(1.29, 3.53)
(1.48, 3.34)
(1.62, 3.14)
(1.68, 2.95)
(1.71, 2.83)
(1.73, 2.76)
(1.76, 2.71)
(1.81, 2.69)
(1.85, 2.69)
(1.88, 2.70)
(1.90, 2.70)
(1.92, 2.70)
(1.94, 2.70)
(1.95, 2.70)
(1.96, 2.71)
(1.98, 2.71)
(1.98, 2.72)
(1.97, 2.75)
(1.98, 2.77)
(1.94, 2.80)
(1.93, 2.86)
(1.98, 2.90)
(2.00, 2.97)
(2.04, 3.04)
(2.07, 3.16)
(2.12, 3.27)
(2.20, 3.39)
(2.27, 3.50)
(2.32, 3.63)
(2.33, 3.80)
(2.33, 3.97)
(2.30, 4.15)
(2.22, 4.35)
(2.13, 4.55)
(2.01, 4.74)
(1.93, 4.91)
(1.83, 5.06)
(1.74, 5.20)
(1.66, 5.35)
(1.58, 5.49)
(1.45, 5.68)
(1.31, 5.90)
(1.19, 6.16)
(1.07, 6.41)
(0.96, 6.66)
(0.81, 6.90)
(0.65, 7.14)
(0.47, 7.39)
(0.26, 7.62)
(0.05, 7.84)
(-0.16, 8.04)
(-0.38, 8.22)
(-0.63, 8.37)
(-0.86, 8.43)
(-1.10, 8.44)
(-1.33, 8.45)
(-1.53, 8.46)
(-1.73, 8.45)
(-1.89, 8.41)
(-2.03, 8.33)
(-2.10, 8.24)
(-2.13, 8.14)
(-2.07, 8.03)
(-1.92, 7.87)
(-1.69, 7.68)
(-1.46, 7.49)
(-1.24, 7.29)
(-1.00, 7.08)
(-0.79, 6.85)
(-0.58, 6.63)
(-0.41, 6.41)
(-0.25, 6.20)
(-0.09, 6.01)
(0.07, 5.84)
(0.22, 5.69)
(0.35, 5.53)
(0.46, 5.37)
(0.54, 5.21)
(0.64, 5.04)
(0.73, 4.87)
(0.84, 4.69)
(0.97, 4.45)
(1.11, 4.21)
(1.30, 3.98)
(1.48, 3.74)
(1.68, 3.49)
(1.88, 3.28)
(2.08, 3.09)
(2.26, 2.89)
(2.40, 2.69)
(2.56, 2.54)
(2.68, 2.41)
(2.76, 2.29)
(2.81, 2.20)
(2.83, 2.12)
(2.85, 2.06)
(2.87, 1.99)
(2.90, 1.87)
(2.93, 1.74)
(2.98, 1.61)
(3.05, 1.45)
(3.10, 1.27)
(3.19, 1.08)
(3.27, 0.88)
(3.37, 0.67)
(3.48, 0.48)
(3.59, 0.28)
(3.68, 0.10)
(3.79, -0.08)
(3.86, -0.27)
(3.94, -0.45)
(4.02, -0.64)
(4.11, -0.81)
(4.18, -0.98)
(4.24, -1.14)
(4.30, -1.29)
(4.38, -1.39)
(4.45, -1.48)
(4.51, -1.56)
(4.54, -1.63)
(4.58, -1.69)
(4.59, -1.72)
(4.60, -1.73)
(4.61, -1.73)
(4.63, -1.75)
(4.65, -1.78)
(4.66, -1.81)
(4.66, -1.83)
(4.63, -1.86)
(4.61, -1.84)
(4.60, -1.80)
(4.62, -1.80)
(4.62, -1.79)
(4.62, -1.79)
(4.62, -1.79)
};
 %   


==> plots/euroc_traj_coords/mh02_gt.tex <==
\addplot[
    fill=none,draw = clr1,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.62, -1.84)
(4.61, -1.82)
(4.61, -1.82)
(4.62, -1.81)
(4.64, -1.82)
(4.64, -1.81)
(4.62, -1.80)
(4.63, -1.79)
(4.63, -1.80)
(4.64, -1.81)
(4.64, -1.81)
(4.62, -1.80)
(4.62, -1.79)
(4.62, -1.80)
(4.63, -1.81)
(4.64, -1.81)
(4.64, -1.80)
(4.63, -1.80)
(4.63, -1.80)
(4.63, -1.80)
(4.63, -1.81)
(4.62, -1.81)
(4.61, -1.81)
(4.62, -1.81)
(4.62, -1.81)
(4.63, -1.80)
(4.65, -1.81)
(4.68, -1.82)
(4.71, -1.83)
(4.71, -1.83)
(4.72, -1.84)
(4.73, -1.87)
(4.74, -1.89)
(4.74, -1.89)
(4.74, -1.89)
(4.75, -1.82)
(4.76, -1.68)
(4.77, -1.53)
(4.78, -1.43)
(4.79, -1.40)
(4.79, -1.42)
(4.76, -1.52)
(4.73, -1.67)
(4.68, -1.83)
(4.65, -1.94)
(4.65, -1.93)
(4.68, -1.82)
(4.71, -1.65)
(4.75, -1.49)
(4.77, -1.44)
(4.77, -1.46)
(4.73, -1.58)
(4.67, -1.75)
(4.63, -1.85)
(4.64, -1.92)
(4.74, -1.94)
(4.87, -1.89)
(4.95, -1.76)
(4.91, -1.58)
(4.76, -1.47)
(4.58, -1.53)
(4.48, -1.72)
(4.54, -1.89)
(4.67, -1.95)
(4.82, -1.88)
(4.89, -1.72)
(4.86, -1.54)
(4.76, -1.45)
(4.64, -1.49)
(4.57, -1.65)
(4.64, -1.77)
(4.79, -1.77)
(4.91, -1.83)
(4.91, -1.94)
(4.81, -2.00)
(4.69, -1.92)
(4.62, -1.76)
(4.64, -1.62)
(4.69, -1.63)
(4.65, -1.67)
(4.57, -1.69)
(4.52, -1.71)
(4.51, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.50, -1.71)
(4.54, -1.69)
(4.59, -1.66)
(4.59, -1.64)
(4.58, -1.63)
(4.55, -1.63)
(4.51, -1.63)
(4.44, -1.60)
(4.40, -1.56)
(4.35, -1.49)
(4.31, -1.41)
(4.29, -1.34)
(4.26, -1.27)
(4.21, -1.18)
(4.16, -1.05)
(4.10, -0.89)
(4.04, -0.74)
(3.99, -0.59)
(3.95, -0.43)
(3.90, -0.29)
(3.86, -0.16)
(3.82, -0.04)
(3.78, 0.07)
(3.72, 0.18)
(3.66, 0.32)
(3.60, 0.48)
(3.55, 0.64)
(3.50, 0.79)
(3.44, 0.92)
(3.36, 1.03)
(3.27, 1.11)
(3.14, 1.18)
(3.03, 1.26)
(2.91, 1.35)
(2.78, 1.43)
(2.64, 1.51)
(2.48, 1.61)
(2.29, 1.74)
(2.12, 1.87)
(1.95, 1.99)
(1.77, 2.11)
(1.56, 2.24)
(1.34, 2.38)
(1.12, 2.53)
(0.93, 2.65)
(0.75, 2.74)
(0.57, 2.82)
(0.39, 2.89)
(0.24, 2.98)
(0.09, 3.04)
(-0.06, 3.11)
(-0.21, 3.20)
(-0.36, 3.30)
(-0.51, 3.42)
(-0.64, 3.56)
(-0.76, 3.70)
(-0.86, 3.85)
(-0.95, 4.00)
(-1.04, 4.15)
(-1.12, 4.30)
(-1.19, 4.43)
(-1.25, 4.55)
(-1.34, 4.66)
(-1.44, 4.78)
(-1.53, 4.92)
(-1.60, 5.04)
(-1.67, 5.16)
(-1.74, 5.25)
(-1.80, 5.32)
(-1.85, 5.39)
(-1.89, 5.43)
(-1.92, 5.45)
(-1.95, 5.45)
(-2.02, 5.44)
(-2.10, 5.44)
(-2.13, 5.48)
(-2.14, 5.55)
(-2.12, 5.60)
(-2.07, 5.65)
(-1.98, 5.69)
(-1.89, 5.71)
(-1.81, 5.72)
(-1.74, 5.72)
(-1.66, 5.71)
(-1.59, 5.74)
(-1.53, 5.76)
(-1.48, 5.78)
(-1.47, 5.80)
(-1.42, 5.81)
(-1.36, 5.82)
(-1.33, 5.85)
(-1.36, 5.90)
(-1.43, 5.99)
(-1.52, 6.09)
(-1.58, 6.22)
(-1.59, 6.36)
(-1.62, 6.51)
(-1.70, 6.68)
(-1.84, 6.86)
(-1.96, 7.02)
(-2.02, 7.17)
(-2.05, 7.30)
(-2.05, 7.45)
(-2.04, 7.61)
(-2.07, 7.81)
(-2.13, 8.05)
(-2.19, 8.29)
(-2.25, 8.51)
(-2.32, 8.73)
(-2.36, 8.94)
(-2.38, 9.12)
(-2.38, 9.28)
(-2.38, 9.42)
(-2.36, 9.55)
(-2.33, 9.65)
(-2.25, 9.76)
(-2.14, 9.84)
(-2.03, 9.85)
(-1.94, 9.83)
(-1.85, 9.79)
(-1.78, 9.68)
(-1.72, 9.54)
(-1.67, 9.36)
(-1.63, 9.21)
(-1.60, 9.09)
(-1.58, 8.96)
(-1.53, 8.82)
(-1.47, 8.66)
(-1.41, 8.51)
(-1.34, 8.37)
(-1.28, 8.24)
(-1.20, 8.10)
(-1.10, 7.99)
(-0.99, 7.93)
(-0.87, 7.89)
(-0.76, 7.85)
(-0.66, 7.82)
(-0.57, 7.79)
(-0.50, 7.76)
(-0.47, 7.72)
(-0.46, 7.62)
(-0.39, 7.48)
(-0.28, 7.32)
(-0.17, 7.17)
(-0.06, 7.01)
(0.05, 6.82)
(0.16, 6.59)
(0.28, 6.35)
(0.41, 6.13)
(0.55, 5.92)
(0.69, 5.73)
(0.81, 5.54)
(0.93, 5.35)
(1.05, 5.16)
(1.18, 4.96)
(1.34, 4.78)
(1.49, 4.60)
(1.63, 4.42)
(1.75, 4.23)
(1.86, 4.06)
(1.97, 3.94)
(2.07, 3.86)
(2.12, 3.78)
(2.15, 3.69)
(2.15, 3.59)
(2.13, 3.51)
(2.11, 3.47)
(2.07, 3.43)
(2.00, 3.39)
(1.98, 3.33)
(2.02, 3.27)
(2.09, 3.28)
(2.16, 3.34)
(2.20, 3.43)
(2.22, 3.57)
(2.15, 3.74)
(2.06, 3.91)
(1.96, 4.05)
(1.87, 4.15)
(1.80, 4.24)
(1.76, 4.36)
(1.73, 4.50)
(1.67, 4.64)
(1.61, 4.77)
(1.56, 4.90)
(1.52, 5.07)
(1.47, 5.25)
(1.40, 5.44)
(1.33, 5.60)
(1.24, 5.73)
(1.18, 5.87)
(1.14, 6.02)
(1.09, 6.19)
(1.02, 6.38)
(0.94, 6.59)
(0.85, 6.82)
(0.74, 7.06)
(0.63, 7.28)
(0.49, 7.51)
(0.34, 7.73)
(0.19, 7.92)
(0.08, 8.09)
(-0.04, 8.25)
(-0.14, 8.36)
(-0.23, 8.45)
(-0.31, 8.53)
(-0.39, 8.59)
(-0.45, 8.66)
(-0.49, 8.72)
(-0.52, 8.79)
(-0.56, 8.86)
(-0.62, 8.94)
(-0.69, 8.99)
(-0.76, 9.04)
(-0.83, 9.09)
(-0.94, 9.11)
(-1.07, 9.10)
(-1.20, 9.07)
(-1.32, 9.04)
(-1.42, 9.00)
(-1.52, 8.95)
(-1.61, 8.89)
(-1.69, 8.81)
(-1.76, 8.69)
(-1.80, 8.54)
(-1.81, 8.40)
(-1.81, 8.24)
(-1.79, 8.08)
(-1.76, 7.90)
(-1.71, 7.69)
(-1.64, 7.43)
(-1.55, 7.14)
(-1.51, 6.84)
(-1.49, 6.56)
(-1.45, 6.28)
(-1.39, 6.02)
(-1.30, 5.80)
(-1.19, 5.61)
(-1.05, 5.42)
(-0.88, 5.24)
(-0.68, 5.05)
(-0.46, 4.87)
(-0.21, 4.69)
(0.06, 4.50)
(0.35, 4.30)
(0.63, 4.11)
(0.88, 3.91)
(1.09, 3.72)
(1.29, 3.53)
(1.47, 3.33)
(1.60, 3.13)
(1.65, 2.95)
(1.68, 2.84)
(1.70, 2.77)
(1.74, 2.73)
(1.78, 2.71)
(1.82, 2.71)
(1.85, 2.71)
(1.88, 2.72)
(1.89, 2.72)
(1.91, 2.72)
(1.94, 2.72)
(1.96, 2.73)
(1.98, 2.73)
(1.99, 2.74)
(1.99, 2.77)
(1.99, 2.79)
(1.96, 2.81)
(1.94, 2.85)
(1.96, 2.91)
(2.00, 2.98)
(2.03, 3.06)
(2.06, 3.16)
(2.11, 3.27)
(2.17, 3.38)
(2.25, 3.50)
(2.31, 3.62)
(2.33, 3.78)
(2.33, 3.94)
(2.31, 4.11)
(2.26, 4.30)
(2.17, 4.50)
(2.06, 4.70)
(1.96, 4.87)
(1.87, 5.03)
(1.78, 5.17)
(1.70, 5.31)
(1.63, 5.45)
(1.51, 5.60)
(1.38, 5.81)
(1.25, 6.05)
(1.13, 6.29)
(1.02, 6.54)
(0.90, 6.78)
(0.76, 7.00)
(0.59, 7.24)
(0.40, 7.48)
(0.19, 7.71)
(-0.01, 7.91)
(-0.22, 8.11)
(-0.44, 8.28)
(-0.68, 8.40)
(-0.91, 8.45)
(-1.15, 8.46)
(-1.37, 8.46)
(-1.56, 8.47)
(-1.74, 8.46)
(-1.90, 8.41)
(-2.02, 8.32)
(-2.10, 8.24)
(-2.11, 8.14)
(-2.04, 8.02)
(-1.88, 7.86)
(-1.66, 7.68)
(-1.43, 7.50)
(-1.21, 7.31)
(-0.99, 7.09)
(-0.78, 6.87)
(-0.59, 6.65)
(-0.41, 6.44)
(-0.26, 6.23)
(-0.11, 6.05)
(0.05, 5.88)
(0.20, 5.72)
(0.33, 5.56)
(0.44, 5.41)
(0.52, 5.25)
(0.61, 5.09)
(0.70, 4.93)
(0.80, 4.75)
(0.92, 4.53)
(1.07, 4.29)
(1.23, 4.06)
(1.42, 3.83)
(1.61, 3.59)
(1.81, 3.36)
(2.01, 3.16)
(2.19, 2.97)
(2.35, 2.78)
(2.50, 2.61)
(2.63, 2.47)
(2.73, 2.35)
(2.79, 2.25)
(2.82, 2.17)
(2.84, 2.11)
(2.86, 2.04)
(2.88, 1.94)
(2.91, 1.83)
(2.95, 1.70)
(3.01, 1.55)
(3.07, 1.38)
(3.14, 1.20)
(3.21, 1.01)
(3.31, 0.81)
(3.41, 0.61)
(3.52, 0.41)
(3.63, 0.23)
(3.73, 0.05)
(3.82, -0.14)
(3.90, -0.32)
(3.98, -0.50)
(4.06, -0.68)
(4.14, -0.86)
(4.21, -1.02)
(4.27, -1.17)
(4.34, -1.31)
(4.42, -1.41)
(4.48, -1.50)
(4.54, -1.58)
(4.57, -1.64)
(4.60, -1.70)
(4.61, -1.73)
(4.62, -1.74)
(4.62, -1.74)
(4.64, -1.75)
(4.66, -1.78)
(4.68, -1.81)
(4.67, -1.84)
(4.65, -1.86)
(4.63, -1.85)
(4.61, -1.81)
    };
%


==> plots/euroc_traj_coords/mh02_ice_ba.tex <==
\addplot[
    fill=none,draw = clr2,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.60, -1.91)
(4.60, -1.89)
(4.62, -1.85)
(4.61, -1.83)
(4.60, -1.82)
(4.60, -1.82)
(4.62, -1.81)
(4.64, -1.82)
(4.64, -1.81)
(4.62, -1.80)
(4.62, -1.79)
(4.62, -1.80)
(4.63, -1.82)
(4.63, -1.81)
(4.62, -1.80)
(4.61, -1.80)
(4.62, -1.80)
(4.64, -1.81)
(4.64, -1.81)
(4.63, -1.81)
(4.62, -1.81)
(4.62, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.62, -1.82)
(4.61, -1.82)
(4.61, -1.82)
(4.62, -1.81)
(4.64, -1.82)
(4.67, -1.83)
(4.69, -1.84)
(4.71, -1.84)
(4.72, -1.85)
(4.73, -1.87)
(4.75, -1.89)
(4.75, -1.90)
(4.74, -1.90)
(4.75, -1.86)
(4.76, -1.74)
(4.77, -1.59)
(4.78, -1.46)
(4.79, -1.41)
(4.79, -1.42)
(4.77, -1.50)
(4.74, -1.65)
(4.69, -1.82)
(4.66, -1.94)
(4.65, -1.95)
(4.67, -1.86)
(4.71, -1.68)
(4.75, -1.52)
(4.78, -1.45)
(4.77, -1.47)
(4.73, -1.58)
(4.68, -1.75)
(4.64, -1.87)
(4.64, -1.93)
(4.74, -1.95)
(4.88, -1.90)
(4.95, -1.76)
(4.90, -1.58)
(4.76, -1.48)
(4.58, -1.56)
(4.49, -1.76)
(4.56, -1.92)
(4.70, -1.97)
(4.84, -1.88)
(4.90, -1.70)
(4.85, -1.53)
(4.73, -1.46)
(4.62, -1.54)
(4.58, -1.71)
(4.68, -1.80)
(4.83, -1.80)
(4.93, -1.89)
(4.89, -1.99)
(4.77, -2.01)
(4.66, -1.89)
(4.61, -1.72)
(4.67, -1.63)
(4.69, -1.66)
(4.62, -1.70)
(4.55, -1.72)
(4.52, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.51, -1.73)
(4.52, -1.72)
(4.56, -1.70)
(4.61, -1.67)
(4.61, -1.65)
(4.59, -1.64)
(4.55, -1.64)
(4.49, -1.63)
(4.43, -1.60)
(4.38, -1.55)
(4.34, -1.48)
(4.30, -1.40)
(4.28, -1.33)
(4.24, -1.25)
(4.18, -1.15)
(4.12, -1.01)
(4.06, -0.85)
(4.00, -0.70)
(3.95, -0.55)
(3.90, -0.40)
(3.86, -0.26)
(3.82, -0.14)
(3.79, -0.01)
(3.74, 0.10)
(3.68, 0.23)
(3.63, 0.38)
(3.57, 0.54)
(3.52, 0.72)
(3.46, 0.86)
(3.39, 0.97)
(3.30, 1.06)
(3.18, 1.13)
(3.07, 1.22)
(2.95, 1.31)
(2.83, 1.39)
(2.69, 1.47)
(2.52, 1.57)
(2.34, 1.69)
(2.16, 1.82)
(1.99, 1.94)
(1.81, 2.07)
(1.59, 2.21)
(1.37, 2.35)
(1.15, 2.50)
(0.95, 2.61)
(0.76, 2.69)
(0.59, 2.78)
(0.41, 2.86)
(0.26, 2.94)
(0.11, 3.02)
(-0.04, 3.10)
(-0.20, 3.19)
(-0.35, 3.29)
(-0.50, 3.41)
(-0.63, 3.56)
(-0.73, 3.70)
(-0.83, 3.85)
(-0.93, 4.00)
(-1.00, 4.16)
(-1.08, 4.31)
(-1.15, 4.44)
(-1.21, 4.56)
(-1.31, 4.68)
(-1.41, 4.82)
(-1.49, 4.96)
(-1.58, 5.09)
(-1.66, 5.19)
(-1.72, 5.27)
(-1.78, 5.34)
(-1.83, 5.39)
(-1.87, 5.43)
(-1.90, 5.44)
(-1.94, 5.43)
(-2.03, 5.42)
(-2.10, 5.44)
(-2.10, 5.49)
(-2.09, 5.55)
(-2.07, 5.60)
(-2.00, 5.65)
(-1.90, 5.67)
(-1.81, 5.68)
(-1.74, 5.69)
(-1.66, 5.69)
(-1.58, 5.69)
(-1.52, 5.72)
(-1.47, 5.74)
(-1.45, 5.76)
(-1.42, 5.77)
(-1.37, 5.78)
(-1.32, 5.80)
(-1.33, 5.86)
(-1.39, 5.93)
(-1.49, 6.04)
(-1.56, 6.16)
(-1.58, 6.31)
(-1.59, 6.45)
(-1.67, 6.62)
(-1.81, 6.82)
(-1.94, 6.99)
(-2.01, 7.13)
(-2.03, 7.27)
(-2.03, 7.42)
(-2.01, 7.58)
(-2.04, 7.78)
(-2.11, 8.02)
(-2.18, 8.26)
(-2.24, 8.48)
(-2.31, 8.69)
(-2.36, 8.89)
(-2.37, 9.08)
(-2.38, 9.24)
(-2.38, 9.38)
(-2.36, 9.51)
(-2.33, 9.61)
(-2.24, 9.72)
(-2.12, 9.78)
(-2.02, 9.79)
(-1.93, 9.76)
(-1.85, 9.70)
(-1.78, 9.59)
(-1.72, 9.44)
(-1.67, 9.28)
(-1.63, 9.14)
(-1.60, 9.02)
(-1.57, 8.89)
(-1.52, 8.75)
(-1.45, 8.59)
(-1.38, 8.44)
(-1.31, 8.30)
(-1.24, 8.16)
(-1.15, 8.02)
(-1.04, 7.93)
(-0.93, 7.89)
(-0.78, 7.86)
(-0.67, 7.82)
(-0.57, 7.79)
(-0.49, 7.76)
(-0.43, 7.73)
(-0.42, 7.66)
(-0.38, 7.53)
(-0.28, 7.38)
(-0.14, 7.22)
(-0.02, 7.07)
(0.09, 6.90)
(0.21, 6.68)
(0.32, 6.44)
(0.46, 6.20)
(0.59, 5.98)
(0.72, 5.78)
(0.86, 5.59)
(0.98, 5.40)
(1.06, 5.22)
(1.18, 5.02)
(1.36, 4.83)
(1.52, 4.66)
(1.66, 4.48)
(1.79, 4.30)
(1.89, 4.11)
(2.01, 3.99)
(2.11, 3.90)
(2.17, 3.83)
(2.19, 3.74)
(2.19, 3.64)
(2.18, 3.56)
(2.16, 3.51)
(2.11, 3.47)
(2.05, 3.42)
(2.02, 3.36)
(2.06, 3.30)
(2.13, 3.32)
(2.20, 3.38)
(2.24, 3.48)
(2.25, 3.62)
(2.18, 3.79)
(2.08, 3.96)
(1.98, 4.09)
(1.89, 4.19)
(1.83, 4.29)
(1.80, 4.41)
(1.76, 4.55)
(1.69, 4.70)
(1.63, 4.82)
(1.58, 4.95)
(1.53, 5.13)
(1.48, 5.32)
(1.40, 5.50)
(1.32, 5.65)
(1.24, 5.79)
(1.18, 5.94)
(1.14, 6.10)
(1.08, 6.28)
(1.00, 6.49)
(0.92, 6.71)
(0.82, 6.96)
(0.71, 7.17)
(0.58, 7.33)
(0.42, 7.62)
(0.25, 7.85)
(0.12, 8.03)
(-0.01, 8.19)
(-0.12, 8.33)
(-0.21, 8.43)
(-0.30, 8.51)
(-0.38, 8.58)
(-0.45, 8.64)
(-0.49, 8.70)
(-0.52, 8.77)
(-0.57, 8.85)
(-0.62, 8.92)
(-0.69, 8.98)
(-0.76, 9.04)
(-0.84, 9.09)
(-0.94, 9.12)
(-1.06, 9.12)
(-1.20, 9.10)
(-1.34, 9.08)
(-1.44, 9.04)
(-1.54, 8.99)
(-1.63, 8.93)
(-1.70, 8.84)
(-1.77, 8.72)
(-1.81, 8.57)
(-1.82, 8.41)
(-1.82, 8.26)
(-1.81, 8.08)
(-1.79, 7.90)
(-1.75, 7.68)
(-1.68, 7.41)
(-1.60, 7.12)
(-1.57, 6.81)
(-1.55, 6.53)
(-1.52, 6.26)
(-1.46, 5.99)
(-1.37, 5.77)
(-1.25, 5.60)
(-1.10, 5.41)
(-0.92, 5.23)
(-0.71, 5.05)
(-0.48, 4.86)
(-0.22, 4.68)
(0.05, 4.49)
(0.38, 4.27)
(0.65, 4.08)
(0.89, 3.88)
(1.10, 3.69)
(1.31, 3.49)
(1.49, 3.28)
(1.58, 3.08)
(1.62, 2.92)
(1.65, 2.83)
(1.68, 2.77)
(1.73, 2.74)
(1.77, 2.73)
(1.80, 2.73)
(1.84, 2.74)
(1.87, 2.75)
(1.89, 2.75)
(1.92, 2.74)
(1.93, 2.74)
(1.95, 2.74)
(1.96, 2.74)
(1.96, 2.77)
(1.96, 2.79)
(1.94, 2.81)
(1.91, 2.84)
(1.91, 2.90)
(1.95, 2.98)
(1.98, 3.05)
(2.01, 3.15)
(2.05, 3.26)
(2.11, 3.37)
(2.20, 3.49)
(2.26, 3.62)
(2.30, 3.78)
(2.30, 3.95)
(2.28, 4.11)
(2.23, 4.30)
(2.14, 4.51)
(2.04, 4.71)
(1.93, 4.89)
(1.83, 5.05)
(1.73, 5.20)
(1.65, 5.34)
(1.57, 5.47)
(1.45, 5.64)
(1.32, 5.83)
(1.19, 6.07)
(1.08, 6.32)
(0.96, 6.58)
(0.83, 6.82)
(0.69, 7.05)
(0.51, 7.28)
(0.32, 7.52)
(0.11, 7.75)
(-0.10, 7.95)
(-0.31, 8.14)
(-0.53, 8.31)
(-0.75, 8.42)
(-0.97, 8.45)
(-1.20, 8.46)
(-1.42, 8.48)
(-1.60, 8.48)
(-1.76, 8.45)
(-1.91, 8.39)
(-2.02, 8.31)
(-2.06, 8.23)
(-2.05, 8.11)
(-1.95, 7.98)
(-1.76, 7.81)
(-1.54, 7.63)
(-1.33, 7.45)
(-1.11, 7.24)
(-0.89, 7.02)
(-0.69, 6.80)
(-0.50, 6.58)
(-0.33, 6.37)
(-0.19, 6.17)
(-0.03, 6.00)
(0.13, 5.82)
(0.26, 5.66)
(0.38, 5.50)
(0.47, 5.35)
(0.56, 5.19)
(0.65, 5.02)
(0.75, 4.85)
(0.86, 4.63)
(1.01, 4.39)
(1.18, 4.15)
(1.36, 3.91)
(1.56, 3.67)
(1.75, 3.44)
(1.95, 3.23)
(2.14, 3.03)
(2.32, 2.83)
(2.48, 2.66)
(2.60, 2.52)
(2.70, 2.40)
(2.78, 2.30)
(2.79, 2.23)
(2.80, 2.18)
(2.82, 2.11)
(2.84, 2.01)
(2.87, 1.89)
(2.91, 1.75)
(2.97, 1.59)
(3.03, 1.43)
(3.10, 1.24)
(3.18, 1.04)
(3.28, 0.83)
(3.39, 0.63)
(3.50, 0.43)
(3.61, 0.24)
(3.70, 0.05)
(3.80, -0.14)
(3.89, -0.32)
(3.97, -0.51)
(4.05, -0.70)
(4.14, -0.87)
(4.21, -1.04)
(4.28, -1.20)
(4.35, -1.33)
(4.43, -1.43)
(4.49, -1.49)
(4.53, -1.57)
(4.57, -1.63)
(4.59, -1.68)
(4.59, -1.69)
(4.59, -1.70)
(4.60, -1.70)
(4.63, -1.72)
(4.64, -1.76)
(4.65, -1.79)
(4.63, -1.81)
(4.61, -1.82)
(4.59, -1.79)
(4.58, -1.75)
(4.59, -1.75)
(4.59, -1.75)
(4.59, -1.75)
};


==> plots/euroc_traj_coords/mh02_ice_ba_fastergpu.tex <==
%
\addplot[
    fill=none,draw = clr3,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.60, -1.89)
(4.60, -1.87)
(4.61, -1.84)
(4.61, -1.83)
(4.60, -1.82)
(4.60, -1.82)
(4.61, -1.80)
(4.64, -1.80)
(4.64, -1.80)
(4.62, -1.80)
(4.61, -1.79)
(4.62, -1.79)
(4.64, -1.80)
(4.63, -1.79)
(4.61, -1.79)
(4.61, -1.79)
(4.62, -1.79)
(4.64, -1.78)
(4.65, -1.78)
(4.64, -1.77)
(4.63, -1.78)
(4.63, -1.77)
(4.63, -1.78)
(4.63, -1.78)
(4.63, -1.79)
(4.62, -1.79)
(4.63, -1.79)
(4.63, -1.78)
(4.65, -1.78)
(4.67, -1.80)
(4.70, -1.80)
(4.72, -1.81)
(4.72, -1.81)
(4.73, -1.84)
(4.75, -1.86)
(4.75, -1.87)
(4.74, -1.87)
(4.75, -1.83)
(4.76, -1.71)
(4.77, -1.56)
(4.79, -1.43)
(4.79, -1.38)
(4.79, -1.39)
(4.77, -1.47)
(4.74, -1.62)
(4.69, -1.78)
(4.65, -1.91)
(4.65, -1.92)
(4.67, -1.82)
(4.71, -1.65)
(4.75, -1.49)
(4.77, -1.42)
(4.77, -1.44)
(4.73, -1.55)
(4.68, -1.72)
(4.63, -1.83)
(4.63, -1.90)
(4.73, -1.92)
(4.87, -1.87)
(4.94, -1.74)
(4.90, -1.55)
(4.76, -1.46)
(4.58, -1.54)
(4.49, -1.73)
(4.55, -1.89)
(4.70, -1.94)
(4.84, -1.86)
(4.91, -1.68)
(4.87, -1.51)
(4.75, -1.44)
(4.63, -1.51)
(4.59, -1.68)
(4.69, -1.77)
(4.84, -1.77)
(4.94, -1.85)
(4.90, -1.96)
(4.79, -1.98)
(4.67, -1.86)
(4.63, -1.69)
(4.68, -1.59)
(4.70, -1.63)
(4.63, -1.67)
(4.56, -1.69)
(4.53, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.52, -1.70)
(4.53, -1.69)
(4.57, -1.67)
(4.61, -1.64)
(4.61, -1.62)
(4.59, -1.61)
(4.56, -1.61)
(4.50, -1.60)
(4.43, -1.57)
(4.39, -1.52)
(4.35, -1.45)
(4.31, -1.37)
(4.29, -1.29)
(4.25, -1.21)
(4.19, -1.10)
(4.13, -0.95)
(4.07, -0.79)
(4.01, -0.63)
(3.96, -0.48)
(3.91, -0.31)
(3.87, -0.17)
(3.83, -0.05)
(3.79, 0.07)
(3.74, 0.18)
(3.68, 0.31)
(3.62, 0.46)
(3.57, 0.63)
(3.51, 0.79)
(3.45, 0.94)
(3.38, 1.05)
(3.29, 1.15)
(3.17, 1.22)
(3.06, 1.27)
(2.95, 1.36)
(2.83, 1.45)
(2.68, 1.52)
(2.52, 1.62)
(2.33, 1.75)
(2.15, 1.88)
(1.98, 2.01)
(1.79, 2.13)
(1.58, 2.26)
(1.35, 2.41)
(1.13, 2.57)
(0.93, 2.69)
(0.74, 2.77)
(0.55, 2.86)
(0.37, 2.94)
(0.21, 3.01)
(0.06, 3.09)
(-0.10, 3.16)
(-0.26, 3.25)
(-0.42, 3.35)
(-0.54, 3.47)
(-0.68, 3.61)
(-0.80, 3.75)
(-0.89, 3.90)
(-0.98, 4.05)
(-1.07, 4.20)
(-1.15, 4.35)
(-1.22, 4.49)
(-1.30, 4.60)
(-1.39, 4.71)
(-1.49, 4.84)
(-1.57, 4.98)
(-1.64, 5.11)
(-1.71, 5.23)
(-1.78, 5.32)
(-1.84, 5.39)
(-1.89, 5.45)
(-1.93, 5.49)
(-1.96, 5.50)
(-2.00, 5.49)
(-2.09, 5.48)
(-2.16, 5.50)
(-2.18, 5.56)
(-2.11, 5.57)
(-2.07, 5.62)
(-2.00, 5.66)
(-1.91, 5.69)
(-1.82, 5.70)
(-1.75, 5.71)
(-1.67, 5.71)
(-1.59, 5.72)
(-1.53, 5.75)
(-1.47, 5.77)
(-1.45, 5.79)
(-1.42, 5.80)
(-1.35, 5.81)
(-1.30, 5.83)
(-1.31, 5.88)
(-1.38, 5.96)
(-1.48, 6.06)
(-1.55, 6.19)
(-1.57, 6.33)
(-1.59, 6.46)
(-1.67, 6.63)
(-1.81, 6.82)
(-1.94, 6.98)
(-2.01, 7.13)
(-2.05, 7.26)
(-2.04, 7.41)
(-2.03, 7.57)
(-2.06, 7.77)
(-2.13, 8.02)
(-2.20, 8.26)
(-2.27, 8.49)
(-2.34, 8.72)
(-2.39, 8.92)
(-2.40, 9.11)
(-2.41, 9.28)
(-2.40, 9.42)
(-2.38, 9.55)
(-2.34, 9.66)
(-2.26, 9.73)
(-2.14, 9.80)
(-2.04, 9.81)
(-1.96, 9.78)
(-1.88, 9.73)
(-1.80, 9.62)
(-1.75, 9.46)
(-1.70, 9.29)
(-1.65, 9.14)
(-1.63, 9.01)
(-1.60, 8.89)
(-1.55, 8.72)
(-1.48, 8.57)
(-1.40, 8.42)
(-1.33, 8.29)
(-1.26, 8.15)
(-1.16, 8.02)
(-1.05, 7.93)
(-0.93, 7.87)
(-0.81, 7.84)
(-0.72, 7.81)
(-0.62, 7.78)
(-0.53, 7.76)
(-0.49, 7.71)
(-0.48, 7.65)
(-0.43, 7.52)
(-0.33, 7.37)
(-0.22, 7.23)
(-0.07, 7.07)
(0.05, 6.89)
(0.16, 6.69)
(0.29, 6.47)
(0.43, 6.24)
(0.57, 6.03)
(0.72, 5.83)
(0.84, 5.64)
(0.96, 5.45)
(1.09, 5.26)
(1.23, 5.07)
(1.39, 4.89)
(1.55, 4.71)
(1.67, 4.55)
(1.80, 4.37)
(1.91, 4.19)
(2.03, 4.07)
(2.13, 3.99)
(2.19, 3.92)
(2.22, 3.83)
(2.22, 3.73)
(2.21, 3.64)
(2.18, 3.60)
(2.14, 3.55)
(2.08, 3.51)
(2.05, 3.45)
(2.10, 3.39)
(2.17, 3.41)
(2.24, 3.47)
(2.27, 3.57)
(2.28, 3.71)
(2.21, 3.89)
(2.11, 4.05)
(2.01, 4.18)
(1.93, 4.28)
(1.86, 4.37)
(1.82, 4.49)
(1.79, 4.63)
(1.72, 4.77)
(1.65, 4.89)
(1.60, 5.02)
(1.56, 5.19)
(1.49, 5.37)
(1.41, 5.55)
(1.33, 5.69)
(1.25, 5.84)
(1.19, 5.98)
(1.15, 6.14)
(1.09, 6.32)
(1.01, 6.50)
(0.91, 6.72)
(0.81, 6.96)
(0.70, 7.20)
(0.56, 7.43)
(0.41, 7.65)
(0.26, 7.84)
(0.13, 7.99)
(0.01, 8.11)
(-0.10, 8.29)
(-0.19, 8.39)
(-0.27, 8.46)
(-0.37, 8.57)
(-0.44, 8.63)
(-0.47, 8.70)
(-0.52, 8.77)
(-0.56, 8.84)
(-0.62, 8.92)
(-0.70, 8.98)
(-0.77, 9.03)
(-0.85, 9.08)
(-0.94, 9.10)
(-1.07, 9.10)
(-1.20, 9.08)
(-1.32, 9.05)
(-1.42, 9.01)
(-1.52, 8.96)
(-1.61, 8.90)
(-1.69, 8.81)
(-1.75, 8.70)
(-1.79, 8.55)
(-1.80, 8.40)
(-1.80, 8.25)
(-1.78, 8.07)
(-1.74, 7.88)
(-1.70, 7.66)
(-1.62, 7.39)
(-1.54, 7.10)
(-1.51, 6.80)
(-1.49, 6.52)
(-1.44, 6.24)
(-1.37, 5.98)
(-1.29, 5.77)
(-1.16, 5.58)
(-1.02, 5.39)
(-0.82, 5.22)
(-0.61, 5.03)
(-0.38, 4.84)
(-0.11, 4.66)
(0.17, 4.47)
(0.47, 4.28)
(0.74, 4.08)
(0.97, 3.89)
(1.18, 3.70)
(1.38, 3.51)
(1.55, 3.32)
(1.65, 3.07)
(1.69, 2.91)
(1.71, 2.79)
(1.74, 2.74)
(1.78, 2.70)
(1.82, 2.70)
(1.84, 2.70)
(1.87, 2.71)
(1.90, 2.71)
(1.92, 2.71)
(1.94, 2.71)
(1.96, 2.71)
(1.98, 2.71)
(2.01, 2.71)
(2.01, 2.74)
(2.00, 2.76)
(1.96, 2.77)
(1.93, 2.80)
(1.94, 2.86)
(1.98, 2.93)
(2.01, 3.00)
(2.04, 3.09)
(2.08, 3.20)
(2.14, 3.29)
(2.21, 3.43)
(2.28, 3.58)
(2.26, 3.68)
(2.34, 3.93)
(2.32, 4.10)
(2.27, 4.29)
(2.18, 4.50)
(2.07, 4.71)
(1.97, 4.90)
(1.86, 5.07)
(1.74, 5.23)
(1.66, 5.37)
(1.59, 5.47)
(1.47, 5.63)
(1.34, 5.79)
(1.21, 6.03)
(1.09, 6.26)
(0.98, 6.51)
(0.86, 6.74)
(0.70, 6.98)
(0.53, 7.22)
(0.34, 7.45)
(0.13, 7.67)
(-0.06, 7.87)
(-0.26, 8.06)
(-0.48, 8.22)
(-0.73, 8.35)
(-0.95, 8.39)
(-1.19, 8.41)
(-1.40, 8.41)
(-1.59, 8.41)
(-1.75, 8.39)
(-1.90, 8.34)
(-2.06, 8.28)
(-2.12, 8.19)
(-2.09, 8.08)
(-1.98, 7.94)
(-1.79, 7.77)
(-1.57, 7.58)
(-1.35, 7.38)
(-1.12, 7.17)
(-0.91, 6.95)
(-0.70, 6.72)
(-0.52, 6.51)
(-0.35, 6.29)
(-0.20, 6.09)
(-0.04, 5.91)
(0.12, 5.74)
(0.26, 5.58)
(0.38, 5.42)
(0.46, 5.27)
(0.55, 5.12)
(0.64, 4.96)
(0.74, 4.78)
(0.86, 4.57)
(1.00, 4.33)
(1.16, 4.09)
(1.34, 3.85)
(1.54, 3.59)
(1.74, 3.35)
(1.95, 3.14)
(2.14, 2.93)
(2.30, 2.75)
(2.46, 2.57)
(2.59, 2.42)
(2.70, 2.30)
(2.77, 2.19)
(2.80, 2.10)
(2.81, 2.05)
(2.82, 1.98)
(2.85, 1.88)
(2.86, 1.76)
(2.90, 1.62)
(2.97, 1.47)
(3.03, 1.29)
(3.09, 1.10)
(3.16, 0.90)
(3.26, 0.68)
(3.37, 0.47)
(3.46, 0.27)
(3.56, 0.08)
(3.65, -0.11)
(3.74, -0.31)
(3.82, -0.50)
(3.90, -0.70)
(4.01, -0.89)
(4.09, -1.08)
(4.16, -1.24)
(4.22, -1.37)
(4.29, -1.50)
(4.36, -1.60)
(4.43, -1.69)
(4.49, -1.77)
(4.52, -1.84)
(4.54, -1.88)
(4.54, -1.90)
(4.55, -1.90)
(4.55, -1.89)
(4.58, -1.92)
(4.59, -1.95)
(4.60, -1.98)
(4.58, -2.00)
(4.56, -2.01)
(4.54, -1.98)
(4.53, -1.94)
(4.54, -1.94)
(4.54, -1.94)
(4.54, -1.94)
};


==> plots/euroc_traj_coords/mh02_ice_ba_jetson_slam.tex <==
%
\addplot[
    fill=none,draw = clr4,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.57, -1.90)
(4.56, -1.89)
(4.57, -1.87)
(4.56, -1.86)
(4.54, -1.87)
(4.53, -1.88)
(4.57, -1.85)
(4.60, -1.81)
(4.60, -1.81)
(4.57, -1.81)
(4.57, -1.80)
(4.58, -1.80)
(4.60, -1.81)
(4.59, -1.81)
(4.56, -1.80)
(4.56, -1.80)
(4.58, -1.80)
(4.60, -1.80)
(4.61, -1.80)
(4.61, -1.78)
(4.60, -1.78)
(4.60, -1.78)
(4.60, -1.79)
(4.60, -1.79)
(4.59, -1.79)
(4.58, -1.79)
(4.59, -1.79)
(4.60, -1.78)
(4.62, -1.78)
(4.65, -1.80)
(4.67, -1.81)
(4.69, -1.81)
(4.69, -1.82)
(4.71, -1.84)
(4.72, -1.86)
(4.72, -1.87)
(4.72, -1.87)
(4.72, -1.83)
(4.73, -1.71)
(4.75, -1.57)
(4.76, -1.44)
(4.77, -1.39)
(4.77, -1.40)
(4.75, -1.48)
(4.72, -1.63)
(4.67, -1.79)
(4.64, -1.92)
(4.63, -1.93)
(4.65, -1.83)
(4.69, -1.66)
(4.73, -1.50)
(4.75, -1.43)
(4.74, -1.44)
(4.71, -1.55)
(4.66, -1.73)
(4.62, -1.84)
(4.62, -1.91)
(4.72, -1.93)
(4.86, -1.87)
(4.93, -1.74)
(4.89, -1.56)
(4.74, -1.47)
(4.56, -1.55)
(4.47, -1.74)
(4.54, -1.90)
(4.68, -1.95)
(4.82, -1.87)
(4.89, -1.69)
(4.85, -1.52)
(4.73, -1.45)
(4.62, -1.53)
(4.58, -1.70)
(4.68, -1.79)
(4.83, -1.79)
(4.93, -1.87)
(4.89, -1.97)
(4.77, -1.99)
(4.66, -1.87)
(4.61, -1.70)
(4.67, -1.61)
(4.69, -1.65)
(4.62, -1.68)
(4.55, -1.70)
(4.52, -1.71)
(4.51, -1.72)
(4.50, -1.71)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.50, -1.72)
(4.51, -1.71)
(4.55, -1.69)
(4.59, -1.66)
(4.60, -1.64)
(4.58, -1.63)
(4.54, -1.63)
(4.49, -1.62)
(4.42, -1.59)
(4.38, -1.54)
(4.31, -1.47)
(4.27, -1.40)
(4.24, -1.33)
(4.20, -1.24)
(4.15, -1.14)
(4.09, -0.99)
(4.03, -0.84)
(3.98, -0.68)
(3.93, -0.53)
(3.89, -0.38)
(3.85, -0.21)
(3.81, -0.08)
(3.77, 0.03)
(3.72, 0.14)
(3.67, 0.27)
(3.62, 0.43)
(3.56, 0.59)
(3.50, 0.76)
(3.45, 0.90)
(3.38, 1.02)
(3.29, 1.11)
(3.18, 1.19)
(3.06, 1.26)
(2.94, 1.34)
(2.82, 1.43)
(2.68, 1.51)
(2.51, 1.61)
(2.33, 1.73)
(2.15, 1.86)
(1.98, 1.99)
(1.79, 2.11)
(1.58, 2.24)
(1.35, 2.39)
(1.12, 2.55)
(0.92, 2.66)
(0.74, 2.75)
(0.56, 2.84)
(0.38, 2.91)
(0.23, 2.99)
(0.08, 3.07)
(-0.07, 3.14)
(-0.23, 3.23)
(-0.38, 3.34)
(-0.52, 3.46)
(-0.66, 3.61)
(-0.76, 3.74)
(-0.87, 3.89)
(-0.96, 4.05)
(-1.05, 4.20)
(-1.12, 4.35)
(-1.20, 4.52)
(-1.28, 4.64)
(-1.38, 4.75)
(-1.47, 4.88)
(-1.55, 5.03)
(-1.63, 5.17)
(-1.70, 5.28)
(-1.77, 5.37)
(-1.79, 5.37)
(-1.85, 5.42)
(-1.88, 5.45)
(-1.91, 5.47)
(-1.95, 5.46)
(-2.03, 5.45)
(-2.10, 5.47)
(-2.11, 5.53)
(-2.10, 5.60)
(-2.06, 5.64)
(-1.98, 5.69)
(-1.90, 5.71)
(-1.81, 5.73)
(-1.75, 5.73)
(-1.67, 5.73)
(-1.59, 5.74)
(-1.52, 5.77)
(-1.47, 5.79)
(-1.45, 5.81)
(-1.42, 5.81)
(-1.35, 5.82)
(-1.31, 5.84)
(-1.33, 5.89)
(-1.39, 5.97)
(-1.49, 6.08)
(-1.56, 6.20)
(-1.58, 6.34)
(-1.59, 6.48)
(-1.67, 6.65)
(-1.81, 6.84)
(-1.94, 7.02)
(-2.02, 7.16)
(-2.05, 7.31)
(-2.04, 7.45)
(-2.03, 7.61)
(-2.06, 7.81)
(-2.11, 8.05)
(-2.19, 8.29)
(-2.25, 8.51)
(-2.32, 8.74)
(-2.36, 8.94)
(-2.38, 9.13)
(-2.39, 9.29)
(-2.39, 9.44)
(-2.37, 9.57)
(-2.34, 9.68)
(-2.26, 9.78)
(-2.14, 9.85)
(-2.03, 9.86)
(-1.94, 9.83)
(-1.85, 9.78)
(-1.78, 9.67)
(-1.72, 9.52)
(-1.67, 9.34)
(-1.63, 9.19)
(-1.61, 9.07)
(-1.58, 8.93)
(-1.53, 8.78)
(-1.46, 8.61)
(-1.39, 8.47)
(-1.32, 8.34)
(-1.24, 8.19)
(-1.14, 8.05)
(-1.04, 7.95)
(-0.93, 7.91)
(-0.82, 7.88)
(-0.71, 7.84)
(-0.61, 7.81)
(-0.53, 7.77)
(-0.48, 7.74)
(-0.47, 7.66)
(-0.43, 7.53)
(-0.33, 7.38)
(-0.22, 7.22)
(-0.11, 7.07)
(-0.00, 6.89)
(0.11, 6.67)
(0.22, 6.43)
(0.35, 6.18)
(0.49, 5.97)
(0.63, 5.77)
(0.75, 5.58)
(0.87, 5.40)
(1.00, 5.21)
(1.13, 5.01)
(1.28, 4.82)
(1.45, 4.67)
(1.60, 4.49)
(1.73, 4.30)
(1.83, 4.12)
(1.94, 3.99)
(2.05, 3.90)
(2.11, 3.83)
(2.14, 3.73)
(2.14, 3.64)
(2.13, 3.55)
(2.10, 3.50)
(2.06, 3.46)
(2.00, 3.41)
(1.98, 3.35)
(2.02, 3.29)
(2.09, 3.31)
(2.15, 3.37)
(2.20, 3.47)
(2.20, 3.60)
(2.13, 3.79)
(2.03, 3.95)
(1.93, 4.08)
(1.85, 4.17)
(1.78, 4.27)
(1.75, 4.39)
(1.71, 4.54)
(1.65, 4.68)
(1.58, 4.80)
(1.54, 4.93)
(1.49, 5.11)
(1.43, 5.29)
(1.35, 5.47)
(1.27, 5.61)
(1.19, 5.74)
(1.13, 5.90)
(1.09, 6.05)
(1.03, 6.23)
(0.96, 6.44)
(0.87, 6.66)
(0.77, 6.89)
(0.66, 7.12)
(0.53, 7.35)
(0.37, 7.57)
(0.21, 7.78)
(0.09, 7.96)
(-0.03, 8.11)
(-0.14, 8.24)
(-0.23, 8.37)
(-0.32, 8.45)
(-0.40, 8.52)
(-0.46, 8.58)
(-0.49, 8.66)
(-0.52, 8.73)
(-0.56, 8.80)
(-0.62, 8.88)
(-0.68, 8.93)
(-0.74, 8.98)
(-0.82, 9.02)
(-0.91, 9.05)
(-1.04, 9.05)
(-1.18, 9.03)
(-1.31, 9.00)
(-1.41, 8.96)
(-1.51, 8.91)
(-1.60, 8.85)
(-1.67, 8.77)
(-1.73, 8.65)
(-1.77, 8.50)
(-1.79, 8.35)
(-1.78, 8.20)
(-1.76, 8.03)
(-1.73, 7.83)
(-1.68, 7.61)
(-1.61, 7.33)
(-1.52, 7.04)
(-1.50, 6.75)
(-1.48, 6.47)
(-1.43, 6.21)
(-1.38, 5.95)
(-1.29, 5.73)
(-1.18, 5.54)
(-1.01, 5.36)
(-0.83, 5.17)
(-0.61, 5.01)
(-0.37, 4.83)
(-0.11, 4.65)
(0.17, 4.46)
(0.47, 4.27)
(0.76, 4.06)
(1.00, 3.87)
(1.20, 3.68)
(1.40, 3.47)
(1.57, 3.28)
(1.68, 3.08)
(1.72, 2.92)
(1.75, 2.83)
(1.77, 2.77)
(1.82, 2.73)
(1.85, 2.73)
(1.89, 2.73)
(1.92, 2.73)
(1.94, 2.74)
(1.96, 2.74)
(1.99, 2.73)
(2.00, 2.74)
(2.03, 2.74)
(2.04, 2.74)
(2.04, 2.76)
(2.04, 2.79)
(2.02, 2.81)
(1.99, 2.85)
(2.01, 2.90)
(2.04, 2.96)
(2.07, 3.03)
(2.10, 3.13)
(2.14, 3.25)
(2.21, 3.38)
(2.29, 3.50)
(2.35, 3.63)
(2.37, 3.76)
(2.37, 3.91)
(2.35, 4.10)
(2.30, 4.31)
(2.21, 4.52)
(2.10, 4.71)
(2.00, 4.89)
(1.89, 5.06)
(1.78, 5.22)
(1.71, 5.33)
(1.64, 5.47)
(1.52, 5.64)
(1.37, 5.82)
(1.24, 6.07)
(1.11, 6.33)
(0.99, 6.59)
(0.86, 6.82)
(0.71, 7.07)
(0.53, 7.32)
(0.33, 7.56)
(0.11, 7.78)
(-0.10, 7.98)
(-0.31, 8.17)
(-0.54, 8.34)
(-0.77, 8.45)
(-1.00, 8.48)
(-1.23, 8.49)
(-1.45, 8.49)
(-1.63, 8.50)
(-1.80, 8.48)
(-1.99, 8.42)
(-2.10, 8.33)
(-2.15, 8.24)
(-2.12, 8.13)
(-2.03, 7.99)
(-1.84, 7.81)
(-1.60, 7.62)
(-1.37, 7.42)
(-1.15, 7.21)
(-0.92, 6.98)
(-0.72, 6.75)
(-0.53, 6.53)
(-0.35, 6.31)
(-0.20, 6.10)
(-0.04, 5.93)
(0.12, 5.77)
(0.27, 5.61)
(0.39, 5.45)
(0.48, 5.30)
(0.57, 5.14)
(0.67, 4.97)
(0.77, 4.80)
(0.89, 4.59)
(1.03, 4.34)
(1.20, 4.10)
(1.39, 3.86)
(1.59, 3.62)
(1.79, 3.38)
(2.00, 3.17)
(2.19, 2.97)
(2.35, 2.79)
(2.50, 2.61)
(2.64, 2.46)
(2.73, 2.35)
(2.80, 2.25)
(2.84, 2.16)
(2.86, 2.10)
(2.87, 2.05)
(2.90, 1.95)
(2.92, 1.83)
(2.97, 1.70)
(3.04, 1.54)
(3.10, 1.36)
(3.17, 1.18)
(3.26, 0.97)
(3.35, 0.77)
(3.46, 0.56)
(3.58, 0.35)
(3.67, 0.16)
(3.77, -0.03)
(3.85, -0.19)
(3.94, -0.38)
(4.01, -0.57)
(4.11, -0.76)
(4.20, -0.93)
(4.27, -1.10)
(4.34, -1.27)
(4.42, -1.40)
(4.49, -1.49)
(4.55, -1.58)
(4.60, -1.65)
(4.64, -1.72)
(4.67, -1.77)
(4.66, -1.78)
(4.67, -1.78)
(4.68, -1.78)
(4.71, -1.81)
(4.72, -1.84)
(4.73, -1.87)
(4.71, -1.89)
(4.69, -1.90)
(4.67, -1.87)
(4.66, -1.84)
(4.68, -1.83)
(4.68, -1.83)
(4.68, -1.83)
};


==> plots/euroc_traj_coords/mh02_orbslam2.tex <==
%
\addplot[
    fill=none,draw = clr5,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.59, -1.91)
(4.60, -1.89)
(4.61, -1.86)
(4.61, -1.84)
(4.59, -1.83)
(4.59, -1.82)
(4.61, -1.82)
(4.63, -1.82)
(4.63, -1.82)
(4.62, -1.80)
(4.61, -1.79)
(4.62, -1.80)
(4.63, -1.82)
(4.62, -1.82)
(4.61, -1.80)
(4.61, -1.79)
(4.61, -1.80)
(4.63, -1.81)
(4.63, -1.81)
(4.62, -1.80)
(4.61, -1.80)
(4.61, -1.80)
(4.61, -1.81)
(4.61, -1.81)
(4.61, -1.82)
(4.60, -1.81)
(4.60, -1.81)
(4.61, -1.81)
(4.63, -1.81)
(4.66, -1.82)
(4.68, -1.83)
(4.71, -1.84)
(4.71, -1.85)
(4.72, -1.87)
(4.74, -1.89)
(4.73, -1.90)
(4.73, -1.90)
(4.74, -1.86)
(4.74, -1.74)
(4.75, -1.59)
(4.77, -1.46)
(4.77, -1.41)
(4.77, -1.42)
(4.75, -1.50)
(4.72, -1.65)
(4.68, -1.82)
(4.65, -1.94)
(4.64, -1.95)
(4.66, -1.85)
(4.69, -1.68)
(4.73, -1.52)
(4.76, -1.45)
(4.75, -1.46)
(4.72, -1.58)
(4.67, -1.75)
(4.62, -1.86)
(4.61, -1.92)
(4.71, -1.94)
(4.84, -1.89)
(4.90, -1.74)
(4.86, -1.55)
(4.72, -1.46)
(4.55, -1.55)
(4.48, -1.75)
(4.55, -1.91)
(4.69, -1.96)
(4.81, -1.87)
(4.86, -1.69)
(4.82, -1.52)
(4.70, -1.45)
(4.59, -1.53)
(4.57, -1.70)
(4.66, -1.79)
(4.81, -1.78)
(4.90, -1.87)
(4.87, -1.97)
(4.76, -2.00)
(4.65, -1.88)
(4.60, -1.71)
(4.65, -1.61)
(4.68, -1.65)
(4.61, -1.69)
(4.55, -1.71)
(4.52, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.51, -1.72)
(4.52, -1.72)
(4.56, -1.69)
(4.60, -1.66)
(4.60, -1.64)
(4.59, -1.64)
(4.55, -1.63)
(4.50, -1.63)
(4.42, -1.59)
(4.38, -1.54)
(4.33, -1.47)
(4.30, -1.39)
(4.28, -1.32)
(4.24, -1.24)
(4.19, -1.13)
(4.13, -0.99)
(4.07, -0.83)
(4.02, -0.67)
(3.98, -0.52)
(3.93, -0.36)
(3.89, -0.22)
(3.85, -0.10)
(3.81, 0.01)
(3.76, 0.12)
(3.70, 0.26)
(3.64, 0.41)
(3.58, 0.58)
(3.52, 0.73)
(3.46, 0.88)
(3.40, 0.99)
(3.31, 1.08)
(3.20, 1.16)
(3.07, 1.23)
(2.96, 1.32)
(2.84, 1.40)
(2.70, 1.48)
(2.53, 1.58)
(2.35, 1.71)
(2.18, 1.84)
(2.00, 1.96)
(1.82, 2.08)
(1.61, 2.22)
(1.39, 2.36)
(1.16, 2.51)
(0.97, 2.63)
(0.78, 2.72)
(0.61, 2.80)
(0.43, 2.88)
(0.27, 2.96)
(0.12, 3.03)
(-0.03, 3.10)
(-0.18, 3.20)
(-0.34, 3.29)
(-0.49, 3.42)
(-0.62, 3.56)
(-0.73, 3.71)
(-0.84, 3.86)
(-0.93, 4.01)
(-1.01, 4.16)
(-1.10, 4.31)
(-1.17, 4.44)
(-1.24, 4.56)
(-1.34, 4.67)
(-1.43, 4.79)
(-1.51, 4.93)
(-1.59, 5.06)
(-1.66, 5.17)
(-1.73, 5.26)
(-1.79, 5.33)
(-1.84, 5.39)
(-1.88, 5.42)
(-1.90, 5.44)
(-1.95, 5.43)
(-2.04, 5.42)
(-2.10, 5.44)
(-2.13, 5.50)
(-2.12, 5.56)
(-2.08, 5.61)
(-2.01, 5.66)
(-1.91, 5.69)
(-1.83, 5.70)
(-1.76, 5.71)
(-1.68, 5.70)
(-1.60, 5.71)
(-1.54, 5.74)
(-1.48, 5.76)
(-1.46, 5.79)
(-1.44, 5.79)
(-1.38, 5.81)
(-1.32, 5.83)
(-1.34, 5.88)
(-1.40, 5.96)
(-1.50, 6.06)
(-1.57, 6.19)
(-1.59, 6.33)
(-1.61, 6.47)
(-1.68, 6.64)
(-1.82, 6.84)
(-1.94, 7.00)
(-2.01, 7.14)
(-2.05, 7.28)
(-2.06, 7.44)
(-2.04, 7.59)
(-2.07, 7.80)
(-2.13, 8.04)
(-2.20, 8.28)
(-2.26, 8.51)
(-2.33, 8.73)
(-2.38, 8.93)
(-2.39, 9.12)
(-2.40, 9.28)
(-2.40, 9.42)
(-2.37, 9.54)
(-2.33, 9.65)
(-2.25, 9.76)
(-2.13, 9.83)
(-2.03, 9.84)
(-1.94, 9.82)
(-1.86, 9.76)
(-1.78, 9.65)
(-1.73, 9.50)
(-1.67, 9.32)
(-1.64, 9.18)
(-1.61, 9.06)
(-1.58, 8.93)
(-1.53, 8.79)
(-1.47, 8.64)
(-1.40, 8.49)
(-1.33, 8.36)
(-1.26, 8.22)
(-1.17, 8.08)
(-1.07, 8.00)
(-0.94, 7.95)
(-0.83, 7.91)
(-0.73, 7.88)
(-0.63, 7.85)
(-0.55, 7.81)
(-0.50, 7.79)
(-0.49, 7.72)
(-0.45, 7.59)
(-0.35, 7.44)
(-0.23, 7.28)
(-0.12, 7.12)
(-0.01, 6.94)
(0.10, 6.72)
(0.20, 6.49)
(0.35, 6.25)
(0.49, 6.04)
(0.62, 5.84)
(0.75, 5.64)
(0.87, 5.45)
(0.99, 5.26)
(1.12, 5.06)
(1.28, 4.88)
(1.44, 4.70)
(1.59, 4.52)
(1.72, 4.34)
(1.82, 4.14)
(1.93, 4.01)
(2.04, 3.92)
(2.09, 3.85)
(2.12, 3.75)
(2.12, 3.65)
(2.11, 3.57)
(2.09, 3.53)
(2.05, 3.49)
(1.99, 3.45)
(1.96, 3.39)
(2.00, 3.33)
(2.07, 3.35)
(2.14, 3.40)
(2.18, 3.50)
(2.20, 3.65)
(2.12, 3.82)
(2.02, 3.99)
(1.91, 4.12)
(1.83, 4.22)
(1.77, 4.32)
(1.74, 4.45)
(1.70, 4.59)
(1.63, 4.73)
(1.57, 4.86)
(1.52, 5.00)
(1.48, 5.17)
(1.42, 5.37)
(1.35, 5.55)
(1.27, 5.70)
(1.19, 5.83)
(1.13, 5.98)
(1.10, 6.14)
(1.04, 6.31)
(0.96, 6.52)
(0.87, 6.74)
(0.77, 6.98)
(0.66, 7.21)
(0.53, 7.44)
(0.39, 7.67)
(0.23, 7.88)
(0.11, 8.06)
(-0.02, 8.23)
(-0.13, 8.35)
(-0.22, 8.44)
(-0.30, 8.51)
(-0.39, 8.57)
(-0.45, 8.62)
(-0.48, 8.68)
(-0.52, 8.76)
(-0.56, 8.83)
(-0.61, 8.90)
(-0.68, 8.96)
(-0.75, 9.01)
(-0.83, 9.06)
(-0.93, 9.09)
(-1.06, 9.08)
(-1.18, 9.05)
(-1.30, 9.01)
(-1.40, 8.97)
(-1.49, 8.91)
(-1.56, 8.85)
(-1.64, 8.77)
(-1.71, 8.65)
(-1.75, 8.50)
(-1.77, 8.36)
(-1.77, 8.21)
(-1.75, 8.04)
(-1.72, 7.86)
(-1.66, 7.64)
(-1.59, 7.37)
(-1.49, 7.08)
(-1.45, 6.78)
(-1.44, 6.50)
(-1.40, 6.23)
(-1.33, 5.95)
(-1.23, 5.75)
(-1.11, 5.55)
(-0.96, 5.36)
(-0.79, 5.17)
(-0.58, 4.99)
(-0.35, 4.80)
(-0.09, 4.62)
(0.19, 4.42)
(0.48, 4.22)
(0.76, 4.03)
(1.00, 3.83)
(1.20, 3.64)
(1.40, 3.44)
(1.57, 3.24)
(1.67, 3.05)
(1.71, 2.88)
(1.73, 2.79)
(1.76, 2.74)
(1.80, 2.70)
(1.84, 2.70)
(1.88, 2.70)
(1.91, 2.70)
(1.92, 2.71)
(1.93, 2.70)
(1.96, 2.70)
(1.96, 2.71)
(1.99, 2.72)
(2.00, 2.72)
(1.99, 2.75)
(1.99, 2.78)
(1.97, 2.80)
(1.94, 2.84)
(1.96, 2.90)
(1.98, 2.96)
(2.02, 3.04)
(2.05, 3.13)
(2.10, 3.25)
(2.15, 3.36)
(2.23, 3.48)
(2.30, 3.60)
(2.33, 3.75)
(2.33, 3.92)
(2.31, 4.08)
(2.26, 4.27)
(2.17, 4.48)
(2.06, 4.68)
(1.96, 4.86)
(1.87, 5.02)
(1.77, 5.16)
(1.70, 5.31)
(1.62, 5.44)
(1.50, 5.61)
(1.36, 5.82)
(1.23, 6.06)
(1.11, 6.31)
(1.00, 6.56)
(0.87, 6.79)
(0.72, 7.03)
(0.55, 7.27)
(0.35, 7.51)
(0.15, 7.73)
(-0.06, 7.94)
(-0.27, 8.13)
(-0.51, 8.30)
(-0.74, 8.41)
(-0.98, 8.44)
(-1.22, 8.44)
(-1.43, 8.45)
(-1.62, 8.46)
(-1.80, 8.43)
(-1.95, 8.37)
(-2.06, 8.27)
(-2.11, 8.19)
(-2.10, 8.08)
(-1.99, 7.95)
(-1.80, 7.77)
(-1.57, 7.59)
(-1.34, 7.40)
(-1.11, 7.19)
(-0.89, 6.97)
(-0.69, 6.75)
(-0.50, 6.53)
(-0.33, 6.32)
(-0.18, 6.12)
(-0.03, 5.95)
(0.14, 5.78)
(0.28, 5.62)
(0.40, 5.47)
(0.49, 5.31)
(0.58, 5.14)
(0.67, 4.98)
(0.77, 4.80)
(0.89, 4.60)
(1.03, 4.35)
(1.19, 4.11)
(1.38, 3.88)
(1.57, 3.64)
(1.76, 3.41)
(1.97, 3.20)
(2.17, 3.00)
(2.33, 2.80)
(2.50, 2.63)
(2.63, 2.48)
(2.73, 2.36)
(2.80, 2.25)
(2.83, 2.17)
(2.84, 2.11)
(2.86, 2.04)
(2.89, 1.94)
(2.92, 1.83)
(2.96, 1.69)
(3.02, 1.54)
(3.08, 1.37)
(3.15, 1.19)
(3.23, 0.99)
(3.32, 0.78)
(3.43, 0.58)
(3.53, 0.38)
(3.64, 0.20)
(3.74, 0.01)
(3.83, -0.18)
(3.91, -0.36)
(3.99, -0.55)
(4.07, -0.73)
(4.15, -0.90)
(4.21, -1.07)
(4.27, -1.22)
(4.34, -1.35)
(4.42, -1.44)
(4.48, -1.53)
(4.53, -1.60)
(4.56, -1.66)
(4.58, -1.71)
(4.59, -1.73)
(4.60, -1.74)
(4.62, -1.74)
(4.65, -1.77)
(4.66, -1.80)
(4.67, -1.83)
(4.64, -1.85)
(4.62, -1.87)
(4.60, -1.83)
(4.60, -1.80)
(4.61, -1.79)
(4.61, -1.79)
(4.61, -1.79)
};


==> plots/euroc_traj_coords/mh03_full_ba_jetson_slam.tex <==
%
\addplot[
    fill=none,draw = clr6,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(4.66, -1.79)
(4.66, -1.79)
(4.66, -1.79)
(4.66, -1.79)
(4.66, -1.79)
(4.66, -1.79)
(4.66, -1.79)
(4.66, -1.79)
(4.66, -1.79)
(4.66, -1.78)
(4.66, -1.79)
(4.66, -1.78)
(4.67, -1.78)
(4.67, -1.77)
(4.68, -1.77)
(4.67, -1.77)
(4.67, -1.77)
(4.67, -1.75)
(4.68, -1.75)
(4.68, -1.75)
(4.68, -1.75)
(4.67, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.67, -1.75)
(4.67, -1.75)
(4.67, -1.74)
(4.67, -1.73)
(4.66, -1.73)
(4.66, -1.74)
(4.68, -1.75)
(4.68, -1.73)
(4.67, -1.73)
(4.66, -1.72)
(4.65, -1.72)
(4.64, -1.73)
(4.63, -1.73)
(4.63, -1.73)
(4.63, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.64, -1.73)
(4.65, -1.73)
(4.66, -1.71)
(4.65, -1.66)
(4.61, -1.60)
(4.55, -1.53)
(4.50, -1.47)
(4.45, -1.42)
(4.42, -1.38)
(4.39, -1.33)
(4.37, -1.28)
(4.34, -1.23)
(4.31, -1.18)
(4.27, -1.11)
(4.23, -1.04)
(4.21, -0.97)
(4.17, -0.90)
(4.14, -0.84)
(4.10, -0.78)
(4.07, -0.73)
(4.04, -0.64)
(3.99, -0.54)
(3.92, -0.43)
(3.83, -0.32)
(3.73, -0.21)
(3.65, -0.10)
(3.59, 0.02)
(3.54, 0.15)
(3.52, 0.31)
(3.58, 0.46)
(3.64, 0.61)
(3.69, 0.78)
(3.76, 0.95)
(3.89, 1.18)
(4.04, 1.40)
(4.21, 1.62)
(4.39, 1.84)
(4.59, 2.03)
(4.84, 2.23)
(5.09, 2.41)
(5.35, 2.59)
(5.62, 2.77)
(5.90, 2.96)
(6.18, 3.17)
(6.49, 3.34)
(6.77, 3.51)
(7.01, 3.71)
(7.28, 3.90)
(7.57, 4.10)
(7.91, 4.27)
(8.24, 4.41)
(8.54, 4.48)
(8.82, 4.49)
(9.09, 4.45)
(9.40, 4.35)
(9.65, 4.19)
(9.86, 3.98)
(10.03, 3.72)
(10.21, 3.41)
(10.40, 3.05)
(10.61, 2.62)
(10.81, 2.19)
(11.03, 1.72)
(11.24, 1.26)
(11.44, 0.79)
(11.60, 0.35)
(11.76, -0.02)
(11.90, -0.34)
(12.00, -0.52)
(12.04, -0.68)
(12.00, -0.74)
(11.92, -0.73)
(11.76, -0.53)
(11.53, -0.27)
(11.32, 0.00)
(11.12, 0.29)
(10.96, 0.60)
(10.76, 0.92)
(10.57, 1.24)
(10.39, 1.57)
(10.16, 1.93)
(9.88, 2.32)
(9.58, 2.69)
(9.17, 3.07)
(8.78, 3.41)
(8.28, 3.70)
(7.82, 3.88)
(7.41, 3.95)
(7.00, 3.99)
(6.61, 3.91)
(6.22, 3.79)
(5.82, 3.57)
(5.42, 3.30)
(5.11, 3.00)
(4.89, 2.73)
(4.74, 2.53)
(4.66, 2.41)
(4.65, 2.33)
(4.76, 2.31)
(4.95, 2.33)
(5.17, 2.35)
(5.44, 2.33)
(5.71, 2.26)
(6.00, 2.16)
(6.28, 2.00)
(6.56, 1.77)
(6.86, 1.47)
(7.13, 1.14)
(7.42, 0.77)
(7.67, 0.37)
(7.92, -0.05)
(8.19, -0.46)
(8.50, -0.79)
(8.86, -1.05)
(9.22, -1.20)
(9.60, -1.28)
(9.89, -1.23)
(10.12, -1.04)
(10.30, -0.82)
(10.42, -0.56)
(10.50, -0.31)
(10.54, -0.05)
(10.54, 0.23)
(10.49, 0.56)
(10.39, 0.89)
(10.32, 1.23)
(10.23, 1.59)
(10.10, 2.00)
(9.92, 2.43)
(9.72, 2.84)
(9.50, 3.25)
(9.26, 3.66)
(8.99, 4.00)
(8.67, 4.30)
(8.32, 4.52)
(7.93, 4.67)
(7.52, 4.75)
(7.11, 4.70)
(6.70, 4.54)
(6.35, 4.26)
(6.02, 3.89)
(5.74, 3.51)
(5.53, 3.15)
(5.39, 2.82)
(5.34, 2.51)
(5.37, 2.25)
(5.42, 2.05)
(5.48, 1.84)
(5.54, 1.66)
(5.59, 1.49)
(5.65, 1.30)
(5.74, 1.07)
(5.86, 0.84)
(6.02, 0.59)
(6.22, 0.36)
(6.47, 0.16)
(6.74, 0.01)
(7.00, -0.15)
(7.24, -0.33)
(7.49, -0.54)
(7.74, -0.72)
(8.01, -0.96)
(8.25, -1.16)
(8.47, -1.35)
(8.69, -1.56)
(8.85, -1.73)
(9.01, -1.92)
(9.12, -2.09)
(9.23, -2.28)
(9.31, -2.45)
(9.36, -2.60)
(9.42, -2.67)
(9.49, -2.68)
(9.58, -2.65)
(9.69, -2.58)
(9.83, -2.49)
(10.01, -2.42)
(10.22, -2.33)
(10.42, -2.21)
(10.63, -2.09)
(10.82, -1.92)
(11.02, -1.73)
(11.23, -1.55)
(11.44, -1.33)
(11.63, -1.10)
(11.79, -0.88)
(11.92, -0.67)
(12.01, -0.40)
(12.01, -0.08)
(11.90, 0.31)
(11.69, 0.70)
(11.42, 1.11)
(11.07, 1.51)
(10.70, 1.89)
(10.29, 2.28)
(9.83, 2.63)
(9.36, 2.97)
(8.81, 3.31)
(8.26, 3.55)
(7.57, 3.76)
(6.91, 3.87)
(6.22, 3.91)
(5.59, 3.89)
(5.03, 3.77)
(4.56, 3.56)
(4.18, 3.31)
(3.86, 3.07)
(3.61, 2.80)
(3.42, 2.56)
(3.33, 2.35)
(3.35, 2.19)
(3.47, 2.07)
(3.64, 2.02)
(3.81, 2.02)
(3.99, 2.03)
(4.15, 2.04)
(4.28, 2.05)
(4.40, 2.05)
(4.49, 2.04)
(4.57, 2.04)
(4.62, 2.01)
(4.68, 1.98)
(4.72, 1.93)
(4.75, 1.90)
(4.76, 1.86)
(4.75, 1.81)
(4.73, 1.77)
(4.71, 1.72)
(4.70, 1.68)
(4.68, 1.63)
(4.67, 1.58)
(4.67, 1.50)
(4.68, 1.43)
(4.70, 1.36)
(4.71, 1.29)
(4.73, 1.23)
(4.77, 1.20)
(4.80, 1.14)
(4.82, 1.09)
(4.84, 1.02)
(4.83, 0.94)
(4.79, 0.90)
(4.70, 0.92)
(4.55, 1.00)
(4.34, 1.20)
(4.07, 1.47)
(3.77, 1.81)
(3.47, 2.20)
(3.20, 2.58)
(2.95, 2.97)
(2.71, 3.36)
(2.51, 3.77)
(2.31, 4.16)
(2.14, 4.55)
(1.96, 4.90)
(1.78, 5.27)
(1.59, 5.61)
(1.41, 5.97)
(1.18, 6.29)
(0.95, 6.60)
(0.69, 6.83)
(0.45, 7.01)
(0.17, 7.08)
(-0.12, 7.04)
(-0.39, 6.91)
(-0.60, 6.67)
(-0.76, 6.36)
(-0.86, 6.03)
(-0.95, 5.71)
(-0.96, 5.40)
(-0.90, 5.08)
(-0.74, 4.78)
(-0.52, 4.50)
(-0.23, 4.27)
(0.14, 4.03)
(0.57, 3.79)
(1.01, 3.52)
(1.49, 3.24)
(2.00, 2.97)
(2.50, 2.66)
(3.02, 2.32)
(3.51, 1.96)
(3.95, 1.59)
(4.31, 1.23)
(4.67, 0.87)
(4.95, 0.55)
(5.21, 0.28)
(5.46, 0.06)
(5.67, -0.15)
(5.83, -0.33)
(5.97, -0.47)
(6.05, -0.57)
(6.11, -0.65)
(6.16, -0.70)
(6.23, -0.74)
(6.26, -0.76)
(6.23, -0.75)
(6.24, -0.73)
(6.21, -0.72)
(6.20, -0.71)
(6.18, -0.72)
(6.17, -0.71)
(6.16, -0.74)
(6.16, -0.76)
(6.16, -0.79)
(6.18, -0.84)
(6.17, -0.90)
(6.19, -0.97)
(6.20, -1.06)
(6.18, -1.14)
(6.15, -1.23)
(6.09, -1.29)
(6.08, -1.32)
(6.03, -1.34)
(5.98, -1.33)
(5.95, -1.32)
(5.94, -1.33)
(5.95, -1.36)
(5.95, -1.41)
(5.96, -1.46)
(5.98, -1.52)
(6.00, -1.56)
(6.02, -1.55)
(6.03, -1.52)
(6.04, -1.54)
(6.03, -1.51)
(6.02, -1.51)
(6.05, -1.50)
(6.11, -1.44)
(6.21, -1.39)
(6.33, -1.32)
(6.48, -1.27)
(6.70, -1.22)
(6.94, -1.24)
(7.22, -1.29)
(7.59, -1.37)
(8.03, -1.43)
(8.54, -1.42)
(9.00, -1.31)
(9.40, -1.07)
(9.65, -0.66)
(9.81, -0.22)
(9.86, 0.29)
(9.84, 0.75)
(9.78, 1.15)
(9.69, 1.57)
(9.56, 2.00)
(9.33, 2.41)
(8.99, 2.86)
(8.59, 3.28)
(8.11, 3.63)
(7.61, 3.89)
(7.02, 3.96)
(6.45, 3.90)
(5.95, 3.70)
(5.53, 3.43)
(5.26, 3.09)
(5.11, 2.69)
(5.15, 2.28)
(5.45, 1.91)
(5.86, 1.62)
(6.37, 1.39)
(6.96, 1.11)
(7.58, 0.79)
(8.10, 0.51)
(8.66, 0.25)
(9.22, 0.07)
(9.74, -0.09)
(10.23, -0.20)
(10.67, -0.23)
(11.03, -0.19)
(11.27, -0.14)
(11.44, -0.04)
(11.48, 0.13)
(11.40, 0.33)
(11.24, 0.54)
(11.00, 0.77)
(10.73, 1.01)
(10.44, 1.24)
(10.19, 1.45)
(9.96, 1.63)
(9.77, 1.79)
(9.59, 1.98)
(9.48, 2.19)
(9.39, 2.43)
(9.35, 2.69)
(9.31, 2.95)
(9.26, 3.25)
(9.17, 3.49)
(9.07, 3.72)
(8.91, 3.88)
(8.72, 4.01)
(8.47, 4.12)
(8.26, 4.17)
(7.95, 4.14)
(7.65, 4.06)
(7.35, 3.96)
(7.05, 3.80)
(6.74, 3.64)
(6.43, 3.48)
(6.11, 3.30)
(5.76, 3.11)
(5.43, 2.88)
(5.11, 2.65)
(4.81, 2.44)
(4.57, 2.24)
(4.35, 2.08)
(4.17, 1.97)
(4.04, 1.88)
(3.94, 1.82)
(3.85, 1.77)
(3.78, 1.70)
(3.75, 1.60)
(3.76, 1.52)
(3.76, 1.46)
(3.79, 1.43)
(3.81, 1.38)
(3.86, 1.33)
(3.91, 1.27)
(3.95, 1.21)
(4.01, 1.10)
(4.05, 1.01)
(4.09, 0.91)
(4.14, 0.78)
(4.19, 0.65)
(4.26, 0.51)
(4.32, 0.37)
(4.37, 0.22)
(4.43, 0.05)
(4.49, -0.12)
(4.53, -0.29)
(4.59, -0.44)
(4.65, -0.60)
(4.68, -0.76)
(4.71, -0.92)
(4.69, -1.07)
(4.67, -1.22)
(4.64, -1.35)
(4.61, -1.47)
(4.59, -1.56)
(4.58, -1.63)
(4.59, -1.68)
(4.60, -1.69)
(4.62, -1.69)
(4.64, -1.69)
(4.65, -1.71)
(4.66, -1.73)
(4.67, -1.77)
(4.66, -1.81)
(4.64, -1.84)
(4.60, -1.87)
(4.57, -1.90)
(4.57, -1.91)
(4.58, -1.89)
(4.56, -1.89)
(4.58, -1.89)
(4.58, -1.89)
(4.57, -1.89)
(4.58, -1.89)
(4.57, -1.89)
(4.58, -1.89)
(4.57, -1.89)
(4.58, -1.89)
(4.56, -1.89)
};
 %   


==> plots/euroc_traj_coords/mh03_gt.tex <==
\addplot[
    fill=none,draw = clr1,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.63, -1.79)
(4.63, -1.79)
(4.64, -1.78)
(4.64, -1.78)
(4.65, -1.77)
(4.65, -1.77)
(4.65, -1.77)
(4.65, -1.76)
(4.65, -1.76)
(4.66, -1.76)
(4.65, -1.75)
(4.64, -1.74)
(4.64, -1.74)
(4.63, -1.74)
(4.64, -1.75)
(4.65, -1.75)
(4.64, -1.74)
(4.64, -1.74)
(4.64, -1.73)
(4.64, -1.75)
(4.65, -1.75)
(4.65, -1.73)
(4.65, -1.73)
(4.64, -1.72)
(4.62, -1.73)
(4.61, -1.73)
(4.61, -1.73)
(4.60, -1.73)
(4.61, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.62, -1.73)
(4.63, -1.71)
(4.62, -1.66)
(4.58, -1.60)
(4.52, -1.53)
(4.46, -1.46)
(4.42, -1.42)
(4.39, -1.37)
(4.36, -1.32)
(4.33, -1.27)
(4.30, -1.21)
(4.26, -1.15)
(4.22, -1.08)
(4.19, -1.01)
(4.16, -0.93)
(4.13, -0.87)
(4.10, -0.80)
(4.06, -0.75)
(4.02, -0.67)
(3.98, -0.57)
(3.92, -0.46)
(3.83, -0.35)
(3.73, -0.23)
(3.63, -0.12)
(3.57, -0.00)
(3.53, 0.14)
(3.54, 0.29)
(3.58, 0.45)
(3.65, 0.62)
(3.72, 0.80)
(3.82, 1.00)
(3.94, 1.22)
(4.10, 1.45)
(4.27, 1.68)
(4.47, 1.89)
(4.70, 2.09)
(4.95, 2.28)
(5.22, 2.46)
(5.50, 2.66)
(5.80, 2.85)
(6.09, 3.05)
(6.38, 3.24)
(6.68, 3.42)
(6.96, 3.61)
(7.24, 3.83)
(7.54, 4.04)
(7.88, 4.22)
(8.22, 4.38)
(8.54, 4.48)
(8.82, 4.50)
(9.09, 4.43)
(9.39, 4.32)
(9.65, 4.14)
(9.86, 3.91)
(10.04, 3.65)
(10.22, 3.32)
(10.43, 2.94)
(10.64, 2.51)
(10.86, 2.06)
(11.09, 1.58)
(11.29, 1.09)
(11.47, 0.63)
(11.64, 0.20)
(11.81, -0.15)
(11.97, -0.40)
(12.04, -0.58)
(12.05, -0.70)
(12.00, -0.71)
(11.84, -0.57)
(11.63, -0.32)
(11.41, -0.04)
(11.23, 0.25)
(10.99, 0.59)
(10.79, 0.90)
(10.59, 1.22)
(10.39, 1.56)
(10.16, 1.94)
(9.89, 2.33)
(9.57, 2.72)
(9.18, 3.10)
(8.72, 3.46)
(8.24, 3.74)
(7.75, 3.91)
(7.31, 3.99)
(6.89, 3.98)
(6.48, 3.89)
(6.08, 3.71)
(5.67, 3.46)
(5.31, 3.16)
(5.03, 2.85)
(4.83, 2.59)
(4.71, 2.43)
(4.67, 2.32)
(4.74, 2.26)
(4.92, 2.28)
(5.15, 2.31)
(5.41, 2.30)
(5.70, 2.23)
(6.00, 2.12)
(6.29, 1.97)
(6.59, 1.73)
(6.90, 1.45)
(7.21, 1.11)
(7.50, 0.73)
(7.76, 0.32)
(8.02, -0.11)
(8.29, -0.50)
(8.64, -0.83)
(9.02, -1.06)
(9.39, -1.20)
(9.72, -1.23)
(9.99, -1.12)
(10.18, -0.90)
(10.38, -0.65)
(10.48, -0.40)
(10.54, -0.14)
(10.57, 0.14)
(10.52, 0.46)
(10.44, 0.79)
(10.35, 1.14)
(10.26, 1.50)
(10.13, 1.92)
(9.95, 2.35)
(9.73, 2.77)
(9.50, 3.20)
(9.25, 3.61)
(8.97, 3.96)
(8.64, 4.26)
(8.26, 4.48)
(7.84, 4.62)
(7.44, 4.67)
(7.02, 4.61)
(6.63, 4.42)
(6.27, 4.09)
(5.95, 3.71)
(5.67, 3.32)
(5.48, 2.95)
(5.38, 2.61)
(5.36, 2.32)
(5.41, 2.08)
(5.48, 1.86)
(5.54, 1.67)
(5.60, 1.49)
(5.66, 1.31)
(5.75, 1.09)
(5.87, 0.83)
(6.03, 0.59)
(6.23, 0.36)
(6.50, 0.15)
(6.79, -0.02)
(7.05, -0.17)
(7.28, -0.35)
(7.52, -0.55)
(7.79, -0.75)
(8.06, -0.96)
(8.32, -1.17)
(8.55, -1.37)
(8.76, -1.58)
(8.93, -1.76)
(9.08, -1.94)
(9.21, -2.13)
(9.31, -2.31)
(9.38, -2.48)
(9.44, -2.59)
(9.50, -2.64)
(9.57, -2.62)
(9.68, -2.56)
(9.81, -2.47)
(9.98, -2.39)
(10.18, -2.31)
(10.39, -2.19)
(10.60, -2.06)
(10.80, -1.90)
(11.00, -1.71)
(11.21, -1.51)
(11.42, -1.28)
(11.61, -1.06)
(11.77, -0.83)
(11.91, -0.59)
(11.99, -0.32)
(11.97, 0.02)
(11.85, 0.40)
(11.62, 0.81)
(11.32, 1.24)
(10.97, 1.65)
(10.59, 2.05)
(10.17, 2.43)
(9.68, 2.79)
(9.13, 3.13)
(8.51, 3.42)
(7.87, 3.67)
(7.19, 3.84)
(6.48, 3.92)
(5.78, 3.93)
(5.16, 3.84)
(4.67, 3.64)
(4.26, 3.39)
(3.92, 3.12)
(3.64, 2.84)
(3.44, 2.57)
(3.34, 2.35)
(3.36, 2.18)
(3.48, 2.06)
(3.66, 2.01)
(3.84, 2.01)
(4.02, 2.03)
(4.18, 2.05)
(4.33, 2.06)
(4.44, 2.06)
(4.53, 2.06)
(4.60, 2.04)
(4.66, 2.00)
(4.71, 1.96)
(4.75, 1.92)
(4.77, 1.88)
(4.77, 1.84)
(4.76, 1.81)
(4.74, 1.76)
(4.71, 1.70)
(4.70, 1.65)
(4.69, 1.59)
(4.69, 1.53)
(4.69, 1.45)
(4.70, 1.37)
(4.73, 1.30)
(4.75, 1.24)
(4.78, 1.19)
(4.81, 1.14)
(4.84, 1.09)
(4.85, 1.02)
(4.83, 0.94)
(4.77, 0.91)
(4.67, 0.94)
(4.50, 1.06)
(4.26, 1.29)
(3.97, 1.60)
(3.66, 1.97)
(3.35, 2.36)
(3.08, 2.76)
(2.83, 3.15)
(2.60, 3.58)
(2.39, 3.99)
(2.20, 4.38)
(2.02, 4.76)
(1.83, 5.14)
(1.64, 5.52)
(1.45, 5.89)
(1.23, 6.23)
(0.98, 6.54)
(0.71, 6.80)
(0.44, 6.98)
(0.16, 7.05)
(-0.13, 7.01)
(-0.41, 6.86)
(-0.63, 6.60)
(-0.79, 6.28)
(-0.91, 5.95)
(-0.98, 5.62)
(-0.97, 5.29)
(-0.87, 4.96)
(-0.68, 4.64)
(-0.42, 4.38)
(-0.09, 4.15)
(0.31, 3.91)
(0.76, 3.66)
(1.25, 3.38)
(1.76, 3.08)
(2.28, 2.77)
(2.81, 2.43)
(3.33, 2.06)
(3.79, 1.69)
(4.20, 1.31)
(4.56, 0.95)
(4.87, 0.62)
(5.15, 0.33)
(5.41, 0.08)
(5.63, -0.14)
(5.81, -0.32)
(5.94, -0.47)
(6.04, -0.57)
(6.11, -0.64)
(6.18, -0.70)
(6.23, -0.74)
(6.25, -0.74)
(6.24, -0.73)
(6.22, -0.72)
(6.20, -0.71)
(6.19, -0.70)
(6.17, -0.70)
(6.16, -0.72)
(6.15, -0.73)
(6.15, -0.76)
(6.17, -0.81)
(6.18, -0.87)
(6.18, -0.94)
(6.19, -1.02)
(6.18, -1.11)
(6.15, -1.20)
(6.11, -1.27)
(6.06, -1.31)
(6.02, -1.33)
(5.98, -1.32)
(5.95, -1.32)
(5.93, -1.33)
(5.94, -1.36)
(5.95, -1.41)
(5.97, -1.47)
(5.99, -1.53)
(6.02, -1.56)
(6.04, -1.55)
(6.06, -1.54)
(6.05, -1.52)
(6.05, -1.52)
(6.07, -1.51)
(6.12, -1.47)
(6.20, -1.42)
(6.31, -1.34)
(6.48, -1.26)
(6.69, -1.21)
(6.93, -1.21)
(7.20, -1.26)
(7.56, -1.33)
(8.01, -1.39)
(8.54, -1.40)
(9.02, -1.29)
(9.41, -1.04)
(9.67, -0.64)
(9.82, -0.15)
(9.88, 0.35)
(9.86, 0.81)
(9.79, 1.24)
(9.69, 1.67)
(9.54, 2.11)
(9.27, 2.56)
(8.90, 3.01)
(8.44, 3.43)
(7.91, 3.76)
(7.33, 3.94)
(6.75, 3.94)
(6.20, 3.79)
(5.73, 3.53)
(5.37, 3.20)
(5.16, 2.80)
(5.13, 2.36)
(5.37, 1.97)
(5.80, 1.64)
(6.34, 1.36)
(6.93, 1.08)
(7.50, 0.79)
(8.06, 0.51)
(8.64, 0.27)
(9.22, 0.08)
(9.76, -0.08)
(10.28, -0.18)
(10.72, -0.20)
(11.06, -0.16)
(11.29, -0.10)
(11.44, 0.02)
(11.45, 0.21)
(11.36, 0.42)
(11.17, 0.65)
(10.90, 0.88)
(10.60, 1.13)
(10.31, 1.35)
(10.06, 1.54)
(9.86, 1.72)
(9.67, 1.90)
(9.51, 2.11)
(9.42, 2.33)
(9.37, 2.59)
(9.33, 2.87)
(9.29, 3.17)
(9.21, 3.45)
(9.10, 3.71)
(8.93, 3.89)
(8.72, 4.03)
(8.48, 4.14)
(8.23, 4.19)
(7.94, 4.17)
(7.64, 4.07)
(7.32, 3.95)
(7.00, 3.80)
(6.67, 3.62)
(6.33, 3.43)
(5.99, 3.24)
(5.65, 3.04)
(5.32, 2.82)
(4.99, 2.58)
(4.71, 2.35)
(4.46, 2.17)
(4.25, 2.01)
(4.09, 1.91)
(3.96, 1.83)
(3.86, 1.77)
(3.79, 1.70)
(3.75, 1.62)
(3.74, 1.53)
(3.74, 1.47)
(3.77, 1.42)
(3.80, 1.38)
(3.84, 1.33)
(3.89, 1.27)
(3.95, 1.19)
(4.00, 1.10)
(4.04, 1.00)
(4.08, 0.89)
(4.13, 0.77)
(4.18, 0.63)
(4.25, 0.49)
(4.31, 0.33)
(4.36, 0.17)
(4.42, -0.01)
(4.48, -0.19)
(4.53, -0.35)
(4.58, -0.52)
(4.63, -0.68)
(4.66, -0.85)
(4.66, -1.01)
(4.63, -1.17)
(4.60, -1.31)
(4.57, -1.44)
(4.54, -1.54)
(4.53, -1.62)
(4.53, -1.67)
(4.54, -1.69)
(4.56, -1.69)
(4.59, -1.69)
(4.60, -1.71)
(4.61, -1.74)
(4.61, -1.77)
(4.60, -1.82)
(4.58, -1.85)
(4.54, -1.88)
(4.52, -1.90)
(4.54, -1.89)
(4.54, -1.89)
(4.54, -1.89)
(4.54, -1.89)
(4.54, -1.89)
(4.54, -1.89)
(4.54, -1.89)
    };
%


==> plots/euroc_traj_coords/mh03_ice_ba.tex <==

\addplot[
    fill=none,draw = clr2,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.67, -1.67)
(4.68, -1.67)
(4.68, -1.66)
(4.69, -1.65)
(4.69, -1.65)
(4.69, -1.65)
(4.68, -1.63)
(4.69, -1.63)
(4.70, -1.64)
(4.69, -1.63)
(4.68, -1.63)
(4.68, -1.62)
(4.67, -1.62)
(4.68, -1.62)
(4.68, -1.62)
(4.68, -1.61)
(4.68, -1.60)
(4.68, -1.60)
(4.68, -1.61)
(4.69, -1.62)
(4.69, -1.60)
(4.69, -1.60)
(4.69, -1.59)
(4.67, -1.59)
(4.66, -1.60)
(4.65, -1.61)
(4.65, -1.61)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.67, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.66, -1.60)
(4.67, -1.60)
(4.67, -1.60)
(4.67, -1.60)
(4.67, -1.60)
(4.67, -1.60)
(4.68, -1.58)
(4.67, -1.54)
(4.63, -1.48)
(4.57, -1.41)
(4.52, -1.35)
(4.47, -1.30)
(4.43, -1.26)
(4.41, -1.21)
(4.38, -1.16)
(4.35, -1.11)
(4.32, -1.05)
(4.28, -0.99)
(4.25, -0.92)
(4.22, -0.85)
(4.19, -0.78)
(4.15, -0.72)
(4.11, -0.66)
(4.07, -0.61)
(4.03, -0.52)
(3.98, -0.42)
(3.91, -0.31)
(3.82, -0.19)
(3.72, -0.08)
(3.62, 0.03)
(3.55, 0.14)
(3.51, 0.28)
(3.53, 0.41)
(3.57, 0.55)
(3.63, 0.70)
(3.69, 0.87)
(3.76, 1.06)
(3.88, 1.27)
(4.02, 1.50)
(4.21, 1.73)
(4.39, 1.94)
(4.60, 2.13)
(4.83, 2.31)
(5.12, 2.49)
(5.38, 2.67)
(5.66, 2.85)
(5.95, 3.04)
(6.23, 3.22)
(6.52, 3.40)
(6.80, 3.57)
(7.06, 3.76)
(7.33, 3.97)
(7.62, 4.16)
(7.99, 4.36)
(8.32, 4.50)
(8.62, 4.58)
(8.90, 4.59)
(9.19, 4.54)
(9.47, 4.42)
(9.73, 4.23)
(9.93, 4.01)
(10.09, 3.75)
(10.26, 3.45)
(10.46, 3.08)
(10.65, 2.67)
(10.88, 2.23)
(11.11, 1.76)
(11.33, 1.30)
(11.53, 0.83)
(11.70, 0.40)
(11.87, 0.02)
(12.02, -0.28)
(12.15, -0.51)
(12.17, -0.66)
(12.16, -0.74)
(12.07, -0.69)
(11.90, -0.47)
(11.68, -0.22)
(11.47, 0.05)
(11.28, 0.34)
(11.10, 0.64)
(10.91, 0.94)
(10.72, 1.24)
(10.51, 1.57)
(10.29, 1.93)
(10.03, 2.30)
(9.71, 2.67)
(9.34, 3.03)
(8.91, 3.36)
(8.45, 3.63)
(7.97, 3.80)
(7.53, 3.90)
(7.13, 3.91)
(6.72, 3.88)
(6.33, 3.73)
(5.95, 3.50)
(5.49, 3.28)
(5.15, 3.01)
(4.93, 2.73)
(4.73, 2.53)
(4.63, 2.42)
(4.61, 2.32)
(4.70, 2.27)
(4.89, 2.30)
(5.12, 2.32)
(5.39, 2.29)
(5.68, 2.22)
(5.97, 2.11)
(6.26, 1.96)
(6.54, 1.72)
(6.84, 1.44)
(7.14, 1.12)
(7.41, 0.74)
(7.67, 0.35)
(7.92, -0.07)
(8.17, -0.46)
(8.49, -0.79)
(8.85, -1.04)
(9.22, -1.22)
(9.56, -1.29)
(9.86, -1.23)
(10.10, -1.05)
(10.27, -0.82)
(10.38, -0.58)
(10.46, -0.34)
(10.53, -0.09)
(10.54, 0.19)
(10.49, 0.52)
(10.41, 0.87)
(10.33, 1.21)
(10.24, 1.58)
(10.10, 2.00)
(9.93, 2.41)
(9.71, 2.83)
(9.49, 3.24)
(9.25, 3.62)
(8.96, 3.96)
(8.64, 4.25)
(8.27, 4.48)
(7.87, 4.63)
(7.47, 4.69)
(7.06, 4.64)
(6.65, 4.48)
(6.30, 4.19)
(5.97, 3.82)
(5.69, 3.42)
(5.47, 3.04)
(5.34, 2.70)
(5.28, 2.39)
(5.31, 2.13)
(5.36, 1.90)
(5.43, 1.69)
(5.49, 1.51)
(5.54, 1.33)
(5.60, 1.14)
(5.70, 0.92)
(5.82, 0.67)
(5.98, 0.44)
(6.17, 0.26)
(6.43, 0.10)
(6.69, -0.07)
(6.94, -0.20)
(7.19, -0.38)
(7.42, -0.56)
(7.68, -0.76)
(7.94, -0.97)
(8.18, -1.17)
(8.40, -1.36)
(8.63, -1.58)
(8.83, -1.78)
(8.98, -1.95)
(9.11, -2.13)
(9.23, -2.32)
(9.30, -2.49)
(9.36, -2.62)
(9.45, -2.73)
(9.52, -2.74)
(9.60, -2.70)
(9.72, -2.62)
(9.86, -2.53)
(10.05, -2.46)
(10.26, -2.37)
(10.46, -2.24)
(10.65, -2.09)
(10.84, -1.93)
(11.03, -1.74)
(11.23, -1.53)
(11.43, -1.32)
(11.62, -1.10)
(11.78, -0.87)
(11.91, -0.64)
(11.99, -0.38)
(11.98, -0.06)
(11.87, 0.30)
(11.68, 0.68)
(11.40, 1.09)
(11.07, 1.48)
(10.72, 1.85)
(10.32, 2.21)
(9.88, 2.56)
(9.39, 2.89)
(8.85, 3.20)
(8.23, 3.48)
(7.58, 3.67)
(6.90, 3.79)
(6.23, 3.87)
(5.57, 3.86)
(5.03, 3.73)
(4.59, 3.51)
(4.21, 3.26)
(3.88, 3.00)
(3.63, 2.73)
(3.43, 2.47)
(3.34, 2.25)
(3.33, 2.10)
(3.46, 1.98)
(3.63, 1.93)
(3.81, 1.93)
(3.99, 1.95)
(4.16, 1.97)
(4.30, 1.99)
(4.42, 1.99)
(4.51, 2.00)
(4.59, 1.98)
(4.65, 1.96)
(4.70, 1.92)
(4.74, 1.87)
(4.77, 1.83)
(4.78, 1.80)
(4.78, 1.76)
(4.76, 1.72)
(4.74, 1.68)
(4.72, 1.63)
(4.71, 1.58)
(4.70, 1.53)
(4.70, 1.46)
(4.70, 1.38)
(4.71, 1.30)
(4.74, 1.24)
(4.76, 1.18)
(4.78, 1.13)
(4.81, 1.08)
(4.85, 1.03)
(4.85, 0.96)
(4.84, 0.89)
(4.80, 0.85)
(4.71, 0.87)
(4.58, 0.94)
(4.37, 1.13)
(4.10, 1.39)
(3.79, 1.71)
(3.50, 2.09)
(3.23, 2.47)
(2.98, 2.84)
(2.73, 3.23)
(2.51, 3.64)
(2.31, 4.03)
(2.12, 4.41)
(1.95, 4.78)
(1.76, 5.16)
(1.57, 5.53)
(1.39, 5.89)
(1.18, 6.21)
(0.94, 6.52)
(0.68, 6.77)
(0.43, 6.94)
(0.15, 7.01)
(-0.14, 6.97)
(-0.41, 6.83)
(-0.63, 6.60)
(-0.79, 6.31)
(-0.90, 5.98)
(-0.97, 5.67)
(-1.00, 5.36)
(-0.95, 5.06)
(-0.79, 4.76)
(-0.56, 4.49)
(-0.28, 4.27)
(0.07, 4.04)
(0.45, 3.76)
(0.90, 3.49)
(1.38, 3.23)
(1.90, 2.94)
(2.43, 2.64)
(2.96, 2.30)
(3.45, 1.93)
(3.88, 1.58)
(4.27, 1.25)
(4.61, 0.91)
(4.92, 0.60)
(5.17, 0.31)
(5.41, 0.07)
(5.63, -0.16)
(5.80, -0.34)
(5.93, -0.49)
(6.04, -0.59)
(6.12, -0.66)
(6.19, -0.72)
(6.25, -0.76)
(6.28, -0.78)
(6.27, -0.77)
(6.26, -0.75)
(6.23, -0.73)
(6.21, -0.73)
(6.19, -0.73)
(6.18, -0.74)
(6.18, -0.75)
(6.17, -0.77)
(6.18, -0.80)
(6.16, -0.84)
(6.17, -0.90)
(6.17, -0.97)
(6.18, -1.06)
(6.17, -1.15)
(6.13, -1.23)
(6.09, -1.30)
(6.07, -1.32)
(6.04, -1.34)
(5.97, -1.34)
(5.94, -1.33)
(5.93, -1.34)
(5.93, -1.38)
(5.94, -1.42)
(5.95, -1.47)
(5.97, -1.54)
(5.99, -1.57)
(6.01, -1.57)
(6.02, -1.56)
(6.02, -1.54)
(6.02, -1.54)
(6.03, -1.54)
(6.07, -1.51)
(6.12, -1.46)
(6.22, -1.40)
(6.36, -1.33)
(6.55, -1.25)
(6.76, -1.22)
(6.99, -1.24)
(7.27, -1.29)
(7.64, -1.36)
(8.08, -1.41)
(8.58, -1.41)
(9.04, -1.29)
(9.41, -1.04)
(9.66, -0.65)
(9.81, -0.18)
(9.86, 0.30)
(9.86, 0.74)
(9.80, 1.13)
(9.72, 1.54)
(9.57, 1.95)
(9.33, 2.39)
(8.99, 2.83)
(8.57, 3.26)
(8.06, 3.64)
(7.51, 3.88)
(6.95, 3.96)
(6.39, 3.88)
(5.88, 3.66)
(5.46, 3.37)
(5.17, 3.00)
(5.08, 2.58)
(5.17, 2.15)
(5.48, 1.79)
(5.95, 1.49)
(6.50, 1.22)
(7.10, 0.96)
(7.66, 0.68)
(8.18, 0.42)
(8.74, 0.20)
(9.31, 0.02)
(9.82, -0.11)
(10.32, -0.21)
(10.76, -0.24)
(11.08, -0.19)
(11.32, -0.13)
(11.44, -0.01)
(11.47, 0.16)
(11.39, 0.36)
(11.23, 0.57)
(10.99, 0.79)
(10.72, 1.04)
(10.44, 1.26)
(10.19, 1.44)
(9.97, 1.62)
(9.77, 1.79)
(9.60, 1.98)
(9.47, 2.18)
(9.39, 2.39)
(9.33, 2.64)
(9.30, 2.92)
(9.24, 3.21)
(9.17, 3.47)
(9.05, 3.71)
(8.88, 3.89)
(8.67, 4.01)
(8.43, 4.14)
(8.20, 4.20)
(7.89, 4.19)
(7.60, 4.10)
(7.30, 3.98)
(7.00, 3.84)
(6.70, 3.67)
(6.39, 3.49)
(6.06, 3.31)
(5.72, 3.12)
(5.43, 2.89)
(5.12, 2.66)
(4.80, 2.42)
(4.54, 2.22)
(4.33, 2.05)
(4.16, 1.92)
(4.02, 1.83)
(3.87, 1.76)
(3.78, 1.71)
(3.71, 1.64)
(3.68, 1.55)
(3.68, 1.46)
(3.70, 1.42)
(3.72, 1.38)
(3.75, 1.34)
(3.80, 1.29)
(3.85, 1.24)
(3.90, 1.17)
(3.96, 1.08)
(4.00, 0.98)
(4.04, 0.88)
(4.08, 0.77)
(4.14, 0.64)
(4.17, 0.48)
(4.23, 0.33)
(4.29, 0.17)
(4.35, 0.01)
(4.41, -0.16)
(4.47, -0.33)
(4.54, -0.51)
(4.56, -0.64)
(4.61, -0.81)
(4.63, -0.97)
(4.60, -1.12)
(4.58, -1.26)
(4.54, -1.39)
(4.51, -1.51)
(4.49, -1.61)
(4.47, -1.68)
(4.47, -1.73)
(4.48, -1.74)
(4.50, -1.74)
(4.53, -1.74)
(4.55, -1.77)
(4.55, -1.80)
(4.57, -1.84)
(4.56, -1.88)
(4.54, -1.92)
(4.50, -1.95)
(4.47, -1.98)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
(4.49, -1.97)
};

==> plots/euroc_traj_coords/mh03_ice_ba_fastergpu.tex <==

%
\addplot[
    fill=none,draw = clr3,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.60)
(4.62, -1.63)
(4.62, -1.64)
(4.62, -1.65)
(4.61, -1.72)
(4.59, -1.83)
(4.66, -1.74)
(4.63, -1.57)
(4.64, -1.57)
(4.65, -1.57)
(4.65, -1.57)
(4.65, -1.57)
(4.64, -1.56)
(4.62, -1.56)
(4.63, -1.56)
(4.64, -1.56)
(4.65, -1.56)
(4.65, -1.55)
(4.64, -1.55)
(4.63, -1.56)
(4.64, -1.56)
(4.64, -1.56)
(4.64, -1.56)
(4.63, -1.55)
(4.61, -1.54)
(4.61, -1.55)
(4.60, -1.55)
(4.59, -1.55)
(4.60, -1.55)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.61, -1.54)
(4.62, -1.53)
(4.62, -1.48)
(4.57, -1.43)
(4.52, -1.36)
(4.45, -1.30)
(4.40, -1.25)
(4.35, -1.22)
(4.33, -1.17)
(4.30, -1.12)
(4.28, -1.07)
(4.24, -1.01)
(4.21, -0.94)
(4.18, -0.88)
(4.15, -0.81)
(4.13, -0.74)
(4.09, -0.67)
(4.05, -0.61)
(4.03, -0.56)
(3.99, -0.47)
(3.94, -0.37)
(3.87, -0.26)
(3.78, -0.15)
(3.68, -0.03)
(3.61, 0.07)
(3.56, 0.19)
(3.53, 0.32)
(3.55, 0.47)
(3.62, 0.62)
(3.69, 0.82)
(3.75, 0.98)
(3.82, 1.17)
(3.95, 1.38)
(4.09, 1.59)
(4.26, 1.82)
(4.47, 2.03)
(4.73, 2.23)
(4.92, 2.37)
(5.17, 2.55)
(5.42, 2.71)
(5.70, 2.90)
(5.99, 3.09)
(6.28, 3.28)
(6.56, 3.45)
(6.84, 3.62)
(7.11, 3.80)
(7.39, 4.02)
(7.70, 4.22)
(8.03, 4.39)
(8.36, 4.52)
(8.66, 4.60)
(8.93, 4.60)
(9.23, 4.55)
(9.52, 4.44)
(9.76, 4.24)
(9.96, 4.02)
(10.12, 3.76)
(10.29, 3.46)
(10.49, 3.09)
(10.69, 2.68)
(10.88, 2.24)
(11.11, 1.77)
(11.33, 1.30)
(11.51, 0.84)
(11.69, 0.39)
(11.86, 0.01)
(12.05, -0.25)
(12.15, -0.45)
(12.17, -0.61)
(12.16, -0.69)
(12.06, -0.63)
(11.86, -0.39)
(11.63, -0.13)
(11.42, 0.15)
(11.23, 0.44)
(11.05, 0.74)
(10.86, 1.05)
(10.68, 1.35)
(10.49, 1.68)
(10.27, 2.04)
(10.01, 2.42)
(9.71, 2.79)
(9.35, 3.15)
(8.92, 3.50)
(8.46, 3.78)
(8.00, 3.95)
(7.56, 4.04)
(7.16, 4.06)
(6.78, 4.00)
(6.39, 3.85)
(6.00, 3.64)
(5.57, 3.40)
(5.27, 3.11)
(5.05, 2.84)
(4.89, 2.63)
(4.80, 2.49)
(4.80, 2.41)
(4.87, 2.34)
(5.06, 2.38)
(5.28, 2.38)
(5.55, 2.36)
(5.84, 2.29)
(6.13, 2.19)
(6.41, 2.02)
(6.68, 1.79)
(6.98, 1.50)
(7.28, 1.18)
(7.55, 0.81)
(7.82, 0.42)
(8.06, 0.02)
(8.32, -0.37)
(8.63, -0.71)
(8.96, -0.95)
(9.32, -1.11)
(9.66, -1.19)
(9.96, -1.14)
(10.17, -0.92)
(10.34, -0.70)
(10.46, -0.47)
(10.56, -0.23)
(10.61, 0.03)
(10.61, 0.32)
(10.56, 0.66)
(10.47, 0.98)
(10.40, 1.32)
(10.30, 1.69)
(10.17, 2.08)
(9.99, 2.49)
(9.78, 2.91)
(9.56, 3.31)
(9.32, 3.69)
(9.05, 4.03)
(8.72, 4.31)
(8.36, 4.53)
(7.96, 4.68)
(7.55, 4.72)
(7.14, 4.67)
(6.74, 4.51)
(6.38, 4.21)
(6.08, 3.85)
(5.81, 3.46)
(5.62, 3.07)
(5.49, 2.73)
(5.45, 2.38)
(5.49, 2.12)
(5.55, 1.90)
(5.62, 1.71)
(5.68, 1.54)
(5.74, 1.38)
(5.81, 1.19)
(5.86, 1.03)
(5.98, 0.78)
(6.15, 0.55)
(6.36, 0.34)
(6.62, 0.16)
(6.88, 0.00)
(7.12, -0.14)
(7.36, -0.31)
(7.60, -0.49)
(7.85, -0.68)
(8.11, -0.89)
(8.38, -1.14)
(8.61, -1.34)
(8.82, -1.53)
(9.01, -1.71)
(9.16, -1.88)
(9.29, -2.06)
(9.39, -2.23)
(9.47, -2.40)
(9.53, -2.53)
(9.59, -2.61)
(9.66, -2.63)
(9.74, -2.59)
(9.86, -2.52)
(9.99, -2.42)
(10.19, -2.34)
(10.40, -2.25)
(10.61, -2.13)
(10.81, -1.98)
(11.00, -1.80)
(11.19, -1.61)
(11.39, -1.40)
(11.60, -1.18)
(11.78, -0.95)
(11.93, -0.72)
(12.07, -0.49)
(12.15, -0.22)
(12.15, 0.12)
(12.03, 0.49)
(11.82, 0.89)
(11.53, 1.31)
(11.19, 1.70)
(10.82, 2.07)
(10.42, 2.44)
(9.96, 2.78)
(9.46, 3.11)
(8.92, 3.41)
(8.31, 3.66)
(7.64, 3.82)
(6.95, 3.92)
(6.26, 3.96)
(5.59, 3.92)
(5.08, 3.78)
(4.64, 3.55)
(4.27, 3.29)
(3.94, 3.04)
(3.70, 2.78)
(3.52, 2.52)
(3.44, 2.31)
(3.37, 2.14)
(3.49, 2.02)
(3.67, 1.98)
(3.85, 1.98)
(4.03, 2.00)
(4.19, 2.02)
(4.33, 2.03)
(4.45, 2.05)
(4.54, 2.05)
(4.62, 2.03)
(4.67, 2.00)
(4.73, 1.97)
(4.77, 1.92)
(4.80, 1.89)
(4.81, 1.85)
(4.81, 1.82)
(4.80, 1.77)
(4.77, 1.73)
(4.76, 1.69)
(4.74, 1.63)
(4.73, 1.58)
(4.73, 1.51)
(4.74, 1.43)
(4.75, 1.35)
(4.78, 1.28)
(4.80, 1.23)
(4.82, 1.18)
(4.85, 1.13)
(4.89, 1.08)
(4.89, 1.01)
(4.88, 0.94)
(4.84, 0.90)
(4.75, 0.92)
(4.61, 0.99)
(4.40, 1.18)
(4.12, 1.46)
(3.80, 1.77)
(3.51, 2.13)
(3.23, 2.51)
(2.98, 2.86)
(2.75, 3.24)
(2.55, 3.61)
(2.36, 3.99)
(2.20, 4.33)
(2.02, 4.69)
(1.83, 5.04)
(1.65, 5.38)
(1.46, 5.74)
(1.26, 6.05)
(1.03, 6.33)
(0.78, 6.57)
(0.53, 6.77)
(0.27, 6.83)
(-0.00, 6.79)
(-0.29, 6.73)
(-0.54, 6.53)
(-0.70, 6.24)
(-0.83, 5.92)
(-0.90, 5.61)
(-0.92, 5.30)
(-0.85, 5.00)
(-0.69, 4.70)
(-0.47, 4.44)
(-0.21, 4.21)
(0.14, 3.97)
(0.52, 3.71)
(0.98, 3.46)
(1.46, 3.17)
(1.97, 2.88)
(2.49, 2.58)
(3.02, 2.19)
(3.51, 1.82)
(3.93, 1.45)
(4.31, 1.07)
(4.63, 0.77)
(4.91, 0.44)
(5.19, 0.16)
(5.44, -0.09)
(5.67, -0.32)
(5.84, -0.50)
(5.98, -0.65)
(6.08, -0.71)
(6.17, -0.79)
(6.24, -0.85)
(6.30, -0.89)
(6.26, -0.85)
(6.27, -0.84)
(6.25, -0.82)
(6.23, -0.81)
(6.20, -0.80)
(6.19, -0.80)
(6.18, -0.81)
(6.16, -0.80)
(6.17, -0.82)
(6.17, -0.86)
(6.18, -0.91)
(6.18, -0.97)
(6.18, -1.04)
(6.19, -1.12)
(6.18, -1.21)
(6.13, -1.29)
(6.09, -1.35)
(6.05, -1.38)
(6.01, -1.39)
(5.96, -1.39)
(5.93, -1.39)
(5.92, -1.40)
(5.93, -1.43)
(5.94, -1.47)
(5.95, -1.53)
(5.97, -1.59)
(6.00, -1.63)
(6.01, -1.63)
(6.01, -1.62)
(6.00, -1.60)
(6.00, -1.59)
(6.02, -1.59)
(6.02, -1.54)
(6.08, -1.50)
(6.17, -1.44)
(6.31, -1.36)
(6.49, -1.29)
(6.71, -1.26)
(6.94, -1.27)
(7.20, -1.34)
(7.56, -1.40)
(8.02, -1.44)
(8.53, -1.44)
(8.99, -1.33)
(9.34, -1.08)
(9.58, -0.70)
(9.73, -0.23)
(9.77, 0.24)
(9.76, 0.68)
(9.69, 1.09)
(9.60, 1.51)
(9.47, 1.93)
(9.25, 2.35)
(8.92, 2.79)
(8.51, 3.20)
(8.02, 3.57)
(7.47, 3.81)
(6.91, 3.88)
(6.36, 3.77)
(5.86, 3.56)
(5.44, 3.26)
(5.15, 2.89)
(5.01, 2.47)
(5.07, 2.05)
(5.41, 1.70)
(5.86, 1.40)
(6.40, 1.11)
(6.98, 0.84)
(7.53, 0.57)
(8.07, 0.29)
(8.56, 0.09)
(9.12, -0.08)
(9.64, -0.22)
(10.14, -0.33)
(10.56, -0.36)
(10.90, -0.32)
(11.15, -0.26)
(11.30, -0.17)
(11.28, 0.01)
(11.22, 0.21)
(11.05, 0.42)
(10.82, 0.63)
(10.54, 0.86)
(10.27, 1.08)
(10.02, 1.27)
(9.79, 1.44)
(9.61, 1.61)
(9.44, 1.80)
(9.33, 2.00)
(9.25, 2.22)
(9.21, 2.46)
(9.18, 2.74)
(9.13, 3.01)
(9.06, 3.28)
(8.95, 3.51)
(8.79, 3.68)
(8.58, 3.80)
(8.36, 3.93)
(8.12, 3.98)
(7.83, 3.99)
(7.54, 3.90)
(7.27, 3.79)
(6.96, 3.65)
(6.66, 3.49)
(6.35, 3.33)
(6.02, 3.15)
(5.69, 2.96)
(5.37, 2.76)
(5.03, 2.51)
(4.74, 2.29)
(4.45, 2.10)
(4.23, 1.93)
(4.05, 1.81)
(3.89, 1.71)
(3.77, 1.65)
(3.67, 1.59)
(3.60, 1.52)
(3.57, 1.43)
(3.57, 1.36)
(3.59, 1.31)
(3.61, 1.26)
(3.64, 1.22)
(3.69, 1.18)
(3.71, 1.11)
(3.76, 1.03)
(3.80, 0.94)
(3.84, 0.84)
(3.88, 0.74)
(3.92, 0.63)
(3.99, 0.51)
(4.05, 0.37)
(4.11, 0.23)
(4.17, 0.09)
(4.21, -0.08)
(4.26, -0.26)
(4.31, -0.42)
(4.36, -0.58)
(4.42, -0.73)
(4.46, -0.90)
(4.47, -1.06)
(4.45, -1.21)
(4.42, -1.36)
(4.38, -1.49)
(4.35, -1.61)
(4.31, -1.70)
(4.30, -1.78)
(4.31, -1.82)
(4.31, -1.84)
(4.33, -1.84)
(4.36, -1.84)
(4.38, -1.86)
(4.38, -1.90)
(4.39, -1.93)
(4.38, -1.97)
(4.36, -2.01)
(4.32, -2.04)
(4.29, -2.07)
(4.32, -2.06)
(4.32, -2.06)
(4.32, -2.06)
(4.32, -2.06)
(4.32, -2.06)
(4.32, -2.06)
(4.32, -2.06)
(4.32, -2.06)
(4.32, -2.06)
(4.32, -2.06)
(4.31, -2.06)
(4.31, -2.06)
};
 %   

==> plots/euroc_traj_coords/mh03_ice_ba_jetson_slam.tex <==
%
\addplot[
    fill=none,draw = clr4,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.67, -1.80)
(4.67, -1.80)
(4.67, -1.80)
(4.67, -1.80)
(4.67, -1.80)
(4.67, -1.80)
(4.67, -1.80)
(4.67, -1.80)
(4.67, -1.80)
(4.67, -1.80)
(4.67, -1.80)
(4.68, -1.80)
(4.68, -1.80)
(4.69, -1.79)
(4.69, -1.78)
(4.69, -1.78)
(4.68, -1.78)
(4.68, -1.76)
(4.68, -1.76)
(4.70, -1.77)
(4.69, -1.76)
(4.69, -1.76)
(4.68, -1.75)
(4.66, -1.75)
(4.67, -1.76)
(4.68, -1.77)
(4.68, -1.76)
(4.68, -1.75)
(4.67, -1.74)
(4.68, -1.76)
(4.69, -1.76)
(4.69, -1.75)
(4.69, -1.74)
(4.68, -1.73)
(4.66, -1.73)
(4.66, -1.74)
(4.65, -1.74)
(4.64, -1.75)
(4.65, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.66, -1.74)
(4.67, -1.72)
(4.67, -1.67)
(4.62, -1.61)
(4.57, -1.55)
(4.51, -1.49)
(4.47, -1.44)
(4.44, -1.40)
(4.41, -1.36)
(4.38, -1.31)
(4.35, -1.27)
(4.32, -1.20)
(4.28, -1.13)
(4.25, -1.07)
(4.23, -0.99)
(4.20, -0.93)
(4.17, -0.85)
(4.13, -0.79)
(4.09, -0.74)
(4.05, -0.66)
(4.01, -0.56)
(3.94, -0.45)
(3.85, -0.34)
(3.76, -0.23)
(3.67, -0.13)
(3.62, -0.03)
(3.61, 0.11)
(3.63, 0.27)
(3.70, 0.42)
(3.76, 0.58)
(3.82, 0.75)
(3.90, 0.96)
(4.01, 1.17)
(4.15, 1.40)
(4.32, 1.64)
(4.50, 1.86)
(4.71, 2.05)
(4.96, 2.24)
(5.21, 2.42)
(5.46, 2.58)
(5.75, 2.77)
(6.03, 2.97)
(6.30, 3.17)
(6.59, 3.34)
(6.86, 3.51)
(7.11, 3.70)
(7.37, 3.92)
(7.67, 4.11)
(8.00, 4.29)
(8.33, 4.43)
(8.62, 4.51)
(8.90, 4.51)
(9.19, 4.47)
(9.46, 4.40)
(9.73, 4.23)
(9.94, 4.01)
(10.11, 3.76)
(10.26, 3.42)
(10.47, 3.06)
(10.67, 2.65)
(10.91, 2.22)
(11.15, 1.76)
(11.38, 1.30)
(11.57, 0.84)
(11.74, 0.41)
(11.92, 0.04)
(12.05, -0.24)
(12.14, -0.46)
(12.17, -0.62)
(12.15, -0.69)
(12.05, -0.64)
(11.87, -0.45)
(11.65, -0.19)
(11.44, 0.08)
(11.24, 0.39)
(11.06, 0.69)
(10.87, 1.00)
(10.67, 1.30)
(10.47, 1.63)
(10.25, 1.99)
(9.99, 2.37)
(9.69, 2.74)
(9.32, 3.11)
(8.89, 3.45)
(8.42, 3.73)
(7.96, 3.90)
(7.52, 3.99)
(7.12, 4.01)
(6.72, 3.95)
(6.34, 3.81)
(5.95, 3.59)
(5.59, 3.32)
(5.24, 3.07)
(5.02, 2.80)
(4.84, 2.60)
(4.72, 2.49)
(4.71, 2.41)
(4.78, 2.32)
(4.96, 2.35)
(5.17, 2.36)
(5.43, 2.33)
(5.71, 2.26)
(6.00, 2.16)
(6.29, 2.00)
(6.58, 1.77)
(6.88, 1.49)
(7.17, 1.16)
(7.44, 0.79)
(7.69, 0.39)
(7.94, -0.02)
(8.19, -0.41)
(8.51, -0.75)
(8.86, -1.01)
(9.21, -1.19)
(9.56, -1.27)
(9.87, -1.20)
(10.10, -1.02)
(10.28, -0.79)
(10.40, -0.56)
(10.48, -0.31)
(10.53, -0.04)
(10.53, 0.24)
(10.49, 0.58)
(10.40, 0.90)
(10.33, 1.23)
(10.23, 1.60)
(10.09, 2.01)
(9.92, 2.43)
(9.71, 2.84)
(9.48, 3.24)
(9.24, 3.63)
(8.97, 3.97)
(8.65, 4.25)
(8.28, 4.47)
(7.89, 4.61)
(7.48, 4.67)
(7.05, 4.63)
(6.66, 4.47)
(6.31, 4.17)
(6.00, 3.81)
(5.72, 3.39)
(5.51, 3.01)
(5.37, 2.67)
(5.29, 2.35)
(5.32, 2.10)
(5.38, 1.87)
(5.44, 1.67)
(5.50, 1.49)
(5.56, 1.32)
(5.63, 1.13)
(5.72, 1.01)
(5.84, 0.77)
(6.01, 0.55)
(6.22, 0.33)
(6.46, 0.14)
(6.72, -0.02)
(6.97, -0.17)
(7.21, -0.35)
(7.45, -0.53)
(7.72, -0.74)
(7.98, -0.95)
(8.22, -1.14)
(8.46, -1.33)
(8.66, -1.52)
(8.83, -1.71)
(8.98, -1.88)
(9.10, -2.05)
(9.21, -2.23)
(9.28, -2.40)
(9.33, -2.53)
(9.38, -2.61)
(9.44, -2.61)
(9.52, -2.57)
(9.63, -2.50)
(9.78, -2.42)
(9.96, -2.35)
(10.17, -2.26)
(10.39, -2.14)
(10.59, -2.01)
(10.77, -1.85)
(10.96, -1.67)
(11.17, -1.47)
(11.38, -1.25)
(11.57, -1.03)
(11.74, -0.80)
(11.88, -0.57)
(11.97, -0.30)
(11.97, 0.01)
(11.86, 0.37)
(11.66, 0.76)
(11.38, 1.16)
(11.05, 1.55)
(10.68, 1.93)
(10.30, 2.31)
(9.87, 2.68)
(9.39, 3.01)
(8.84, 3.32)
(8.24, 3.60)
(7.56, 3.80)
(6.86, 3.91)
(6.16, 3.97)
(5.50, 3.95)
(4.96, 3.82)
(4.53, 3.60)
(4.15, 3.34)
(3.85, 3.08)
(3.62, 2.81)
(3.38, 2.56)
(3.29, 2.35)
(3.31, 2.19)
(3.43, 2.07)
(3.60, 2.01)
(3.79, 2.01)
(3.97, 2.03)
(4.13, 2.04)
(4.27, 2.06)
(4.38, 2.07)
(4.48, 2.07)
(4.56, 2.05)
(4.61, 2.02)
(4.66, 1.99)
(4.70, 1.95)
(4.73, 1.89)
(4.74, 1.85)
(4.73, 1.81)
(4.72, 1.77)
(4.69, 1.73)
(4.67, 1.68)
(4.66, 1.64)
(4.66, 1.59)
(4.66, 1.53)
(4.66, 1.45)
(4.67, 1.36)
(4.70, 1.30)
(4.72, 1.24)
(4.74, 1.19)
(4.77, 1.14)
(4.80, 1.09)
(4.81, 1.03)
(4.79, 0.95)
(4.75, 0.91)
(4.66, 0.92)
(4.53, 1.01)
(4.32, 1.18)
(4.06, 1.46)
(3.75, 1.80)
(3.46, 2.18)
(3.18, 2.56)
(2.92, 2.94)
(2.70, 3.33)
(2.49, 3.74)
(2.29, 4.12)
(2.12, 4.48)
(1.95, 4.84)
(1.77, 5.21)
(1.59, 5.56)
(1.42, 5.91)
(1.21, 6.24)
(0.98, 6.53)
(0.74, 6.78)
(0.48, 6.97)
(0.22, 7.04)
(-0.06, 7.01)
(-0.34, 6.87)
(-0.54, 6.65)
(-0.70, 6.36)
(-0.83, 6.06)
(-0.90, 5.75)
(-0.93, 5.45)
(-0.86, 5.14)
(-0.71, 4.84)
(-0.49, 4.57)
(-0.21, 4.34)
(0.14, 4.10)
(0.51, 3.83)
(0.96, 3.57)
(1.44, 3.29)
(1.95, 3.00)
(2.47, 2.67)
(2.97, 2.30)
(3.47, 1.93)
(3.90, 1.55)
(4.25, 1.19)
(4.60, 0.84)
(4.89, 0.55)
(5.18, 0.27)
(5.42, 0.02)
(5.66, -0.19)
(5.83, -0.38)
(5.97, -0.53)
(6.08, -0.63)
(6.15, -0.66)
(6.21, -0.72)
(6.26, -0.75)
(6.29, -0.76)
(6.29, -0.76)
(6.27, -0.74)
(6.22, -0.71)
(6.21, -0.70)
(6.19, -0.70)
(6.17, -0.71)
(6.17, -0.72)
(6.16, -0.74)
(6.17, -0.77)
(6.20, -0.82)
(6.18, -0.88)
(6.18, -0.94)
(6.19, -1.03)
(6.18, -1.12)
(6.13, -1.20)
(6.08, -1.26)
(6.05, -1.29)
(6.00, -1.31)
(5.96, -1.30)
(5.93, -1.30)
(5.91, -1.31)
(5.92, -1.34)
(5.93, -1.39)
(5.95, -1.44)
(5.97, -1.50)
(5.99, -1.54)
(6.02, -1.54)
(6.03, -1.53)
(6.02, -1.51)
(6.01, -1.51)
(6.02, -1.51)
(6.04, -1.48)
(6.10, -1.43)
(6.19, -1.37)
(6.34, -1.30)
(6.53, -1.23)
(6.74, -1.20)
(6.98, -1.22)
(7.26, -1.27)
(7.62, -1.34)
(8.09, -1.39)
(8.60, -1.39)
(9.08, -1.28)
(9.46, -1.04)
(9.69, -0.66)
(9.83, -0.20)
(9.88, 0.27)
(9.87, 0.71)
(9.80, 1.12)
(9.71, 1.54)
(9.58, 1.97)
(9.36, 2.41)
(9.02, 2.84)
(8.61, 3.27)
(8.12, 3.64)
(7.58, 3.88)
(7.02, 3.96)
(6.48, 3.88)
(5.98, 3.67)
(5.57, 3.38)
(5.26, 3.02)
(5.14, 2.62)
(5.20, 2.20)
(5.49, 1.84)
(5.94, 1.52)
(6.45, 1.24)
(7.02, 0.97)
(7.57, 0.68)
(8.10, 0.42)
(8.62, 0.20)
(9.18, 0.02)
(9.70, -0.12)
(10.20, -0.23)
(10.63, -0.27)
(10.97, -0.24)
(11.22, -0.17)
(11.32, -0.06)
(11.36, 0.11)
(11.29, 0.31)
(11.12, 0.52)
(10.88, 0.73)
(10.62, 0.98)
(10.34, 1.21)
(10.10, 1.41)
(9.88, 1.58)
(9.70, 1.75)
(9.53, 1.94)
(9.41, 2.14)
(9.34, 2.36)
(9.30, 2.60)
(9.27, 2.87)
(9.23, 3.16)
(9.16, 3.44)
(9.05, 3.66)
(8.89, 3.82)
(8.69, 3.95)
(8.46, 4.06)
(8.21, 4.12)
(7.93, 4.12)
(7.64, 4.05)
(7.36, 3.94)
(7.10, 3.81)
(6.74, 3.64)
(6.43, 3.47)
(6.11, 3.30)
(5.79, 3.11)
(5.42, 2.89)
(5.10, 2.68)
(4.81, 2.46)
(4.54, 2.25)
(4.33, 2.10)
(4.15, 1.97)
(3.98, 1.89)
(3.87, 1.82)
(3.78, 1.77)
(3.72, 1.70)
(3.68, 1.62)
(3.68, 1.54)
(3.72, 1.49)
(3.74, 1.44)
(3.77, 1.40)
(3.82, 1.36)
(3.87, 1.30)
(3.92, 1.22)
(3.96, 1.13)
(4.00, 1.03)
(4.04, 0.93)
(4.08, 0.82)
(4.13, 0.69)
(4.19, 0.55)
(4.24, 0.40)
(4.29, 0.25)
(4.35, 0.09)
(4.41, -0.08)
(4.45, -0.26)
(4.50, -0.42)
(4.55, -0.58)
(4.60, -0.73)
(4.61, -0.90)
(4.59, -1.05)
(4.56, -1.19)
(4.52, -1.33)
(4.49, -1.45)
(4.47, -1.54)
(4.46, -1.61)
(4.46, -1.66)
(4.47, -1.67)
(4.49, -1.67)
(4.51, -1.67)
(4.52, -1.70)
(4.53, -1.73)
(4.53, -1.77)
(4.52, -1.81)
(4.50, -1.84)
(4.46, -1.87)
(4.44, -1.91)
(4.46, -1.90)
(4.47, -1.90)
(4.47, -1.90)
(4.46, -1.90)
(4.46, -1.90)
(4.46, -1.90)
(4.46, -1.90)
(4.46, -1.90)
(4.46, -1.90)
(4.46, -1.90)
(4.46, -1.90)
(4.46, -1.90)
    };
 %   


==> plots/euroc_traj_coords/mh03_orbslam2.tex <==
%
\addplot[
    fill=none,draw = clr5,
    very thick,
    line width= \linew ex
    ]
    coordinates {
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.63, -1.81)
(4.64, -1.81)
(4.65, -1.80)
(4.65, -1.79)
(4.65, -1.79)
(4.64, -1.79)
(4.64, -1.78)
(4.64, -1.78)
(4.65, -1.78)
(4.65, -1.77)
(4.64, -1.76)
(4.63, -1.76)
(4.62, -1.76)
(4.63, -1.77)
(4.64, -1.77)
(4.64, -1.76)
(4.64, -1.76)
(4.63, -1.75)
(4.63, -1.76)
(4.65, -1.77)
(4.64, -1.76)
(4.64, -1.75)
(4.63, -1.75)
(4.62, -1.74)
(4.61, -1.75)
(4.60, -1.76)
(4.60, -1.76)
(4.60, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.61, -1.75)
(4.62, -1.75)
(4.63, -1.74)
(4.62, -1.69)
(4.58, -1.62)
(4.52, -1.56)
(4.47, -1.49)
(4.42, -1.44)
(4.39, -1.40)
(4.36, -1.35)
(4.34, -1.30)
(4.31, -1.25)
(4.28, -1.19)
(4.24, -1.13)
(4.21, -1.06)
(4.18, -0.99)
(4.16, -0.92)
(4.12, -0.86)
(4.08, -0.80)
(4.05, -0.74)
(4.01, -0.66)
(3.97, -0.56)
(3.90, -0.45)
(3.82, -0.34)
(3.71, -0.22)
(3.62, -0.11)
(3.56, 0.01)
(3.53, 0.15)
(3.52, 0.31)
(3.57, 0.47)
(3.63, 0.63)
(3.70, 0.80)
(3.78, 0.98)
(3.89, 1.19)
(4.04, 1.41)
(4.21, 1.63)
(4.39, 1.83)
(4.61, 2.04)
(4.85, 2.22)
(5.10, 2.40)
(5.36, 2.58)
(5.64, 2.76)
(5.92, 2.95)
(6.21, 3.16)
(6.51, 3.34)
(6.78, 3.52)
(7.05, 3.70)
(7.29, 3.89)
(7.58, 4.10)
(7.93, 4.26)
(8.26, 4.40)
(8.56, 4.48)
(8.83, 4.49)
(9.12, 4.44)
(9.40, 4.34)
(9.67, 4.18)
(9.88, 3.96)
(10.05, 3.70)
(10.22, 3.40)
(10.41, 3.04)
(10.61, 2.64)
(10.82, 2.20)
(11.04, 1.74)
(11.25, 1.27)
(11.43, 0.82)
(11.59, 0.38)
(11.75, -0.00)
(11.89, -0.30)
(11.99, -0.50)
(12.01, -0.66)
(11.99, -0.74)
(11.90, -0.69)
(11.72, -0.50)
(11.51, -0.23)
(11.30, 0.05)
(11.11, 0.34)
(10.94, 0.64)
(10.77, 0.95)
(10.57, 1.26)
(10.38, 1.59)
(10.16, 1.94)
(9.90, 2.32)
(9.59, 2.70)
(9.22, 3.06)
(8.80, 3.40)
(8.35, 3.67)
(7.84, 3.86)
(7.42, 3.95)
(7.01, 3.97)
(6.61, 3.90)
(6.23, 3.77)
(5.83, 3.55)
(5.44, 3.27)
(5.14, 2.99)
(4.91, 2.72)
(4.75, 2.52)
(4.66, 2.40)
(4.66, 2.33)
(4.77, 2.29)
(4.97, 2.33)
(5.18, 2.35)
(5.45, 2.32)
(5.74, 2.26)
(6.03, 2.15)
(6.32, 1.99)
(6.59, 1.77)
(6.89, 1.48)
(7.19, 1.15)
(7.46, 0.78)
(7.71, 0.38)
(7.95, -0.03)
(8.21, -0.42)
(8.52, -0.76)
(8.87, -1.00)
(9.25, -1.16)
(9.60, -1.23)
(9.90, -1.17)
(10.13, -0.99)
(10.30, -0.76)
(10.42, -0.53)
(10.50, -0.28)
(10.54, -0.02)
(10.55, 0.26)
(10.49, 0.58)
(10.41, 0.90)
(10.33, 1.24)
(10.24, 1.60)
(10.11, 2.01)
(9.93, 2.43)
(9.72, 2.85)
(9.50, 3.26)
(9.27, 3.66)
(9.00, 4.01)
(8.69, 4.29)
(8.33, 4.52)
(7.94, 4.67)
(7.54, 4.74)
(7.13, 4.69)
(6.73, 4.53)
(6.37, 4.25)
(6.06, 3.89)
(5.77, 3.52)
(5.56, 3.16)
(5.42, 2.82)
(5.37, 2.52)
(5.39, 2.27)
(5.45, 2.05)
(5.51, 1.85)
(5.57, 1.67)
(5.63, 1.50)
(5.69, 1.32)
(5.78, 1.08)
(5.90, 0.84)
(6.06, 0.60)
(6.27, 0.37)
(6.52, 0.19)
(6.78, 0.02)
(7.03, -0.13)
(7.27, -0.30)
(7.52, -0.50)
(7.77, -0.69)
(8.02, -0.89)
(8.27, -1.11)
(8.50, -1.30)
(8.70, -1.50)
(8.86, -1.68)
(9.01, -1.86)
(9.14, -2.04)
(9.24, -2.22)
(9.32, -2.39)
(9.37, -2.53)
(9.43, -2.61)
(9.49, -2.62)
(9.58, -2.58)
(9.69, -2.51)
(9.83, -2.42)
(10.01, -2.35)
(10.21, -2.27)
(10.42, -2.16)
(10.62, -2.02)
(10.80, -1.87)
(11.01, -1.69)
(11.21, -1.49)
(11.42, -1.28)
(11.61, -1.06)
(11.77, -0.83)
(11.90, -0.61)
(11.99, -0.36)
(11.99, -0.04)
(11.88, 0.33)
(11.69, 0.72)
(11.40, 1.14)
(11.07, 1.53)
(10.70, 1.90)
(10.31, 2.27)
(9.87, 2.63)
(9.38, 2.98)
(8.85, 3.29)
(8.27, 3.55)
(7.60, 3.76)
(6.92, 3.89)
(6.26, 3.94)
(5.60, 3.90)
(5.00, 3.78)
(4.57, 3.57)
(4.19, 3.31)
(3.88, 3.06)
(3.62, 2.80)
(3.43, 2.56)
(3.34, 2.35)
(3.36, 2.18)
(3.48, 2.07)
(3.65, 2.02)
(3.82, 2.02)
(4.00, 2.04)
(4.16, 2.05)
(4.30, 2.06)
(4.41, 2.06)
(4.51, 2.06)
(4.57, 2.04)
(4.63, 2.01)
(4.68, 1.98)
(4.72, 1.93)
(4.75, 1.89)
(4.76, 1.86)
(4.76, 1.82)
(4.74, 1.78)
(4.72, 1.73)
(4.70, 1.68)
(4.69, 1.63)
(4.68, 1.58)
(4.68, 1.51)
(4.68, 1.43)
(4.70, 1.35)
(4.72, 1.29)
(4.74, 1.24)
(4.77, 1.19)
(4.80, 1.14)
(4.82, 1.09)
(4.84, 1.02)
(4.82, 0.95)
(4.77, 0.90)
(4.69, 0.91)
(4.55, 1.01)
(4.34, 1.21)
(4.07, 1.48)
(3.77, 1.82)
(3.48, 2.20)
(3.21, 2.59)
(2.97, 2.96)
(2.74, 3.36)
(2.52, 3.77)
(2.33, 4.16)
(2.16, 4.53)
(1.99, 4.89)
(1.81, 5.26)
(1.63, 5.61)
(1.43, 5.96)
(1.23, 6.29)
(0.98, 6.59)
(0.74, 6.82)
(0.50, 7.00)
(0.23, 7.07)
(-0.05, 7.03)
(-0.33, 6.89)
(-0.53, 6.67)
(-0.71, 6.35)
(-0.81, 6.04)
(-0.90, 5.71)
(-0.91, 5.40)
(-0.85, 5.09)
(-0.70, 4.79)
(-0.48, 4.51)
(-0.18, 4.28)
(0.17, 4.04)
(0.60, 3.78)
(1.03, 3.52)
(1.52, 3.25)
(2.02, 2.97)
(2.52, 2.66)
(3.03, 2.31)
(3.52, 1.94)
(3.94, 1.58)
(4.32, 1.22)
(4.64, 0.86)
(4.94, 0.55)
(5.21, 0.28)
(5.44, 0.03)
(5.65, -0.18)
(5.82, -0.36)
(5.94, -0.50)
(6.03, -0.60)
(6.10, -0.66)
(6.16, -0.72)
(6.21, -0.76)
(6.24, -0.78)
(6.24, -0.77)
(6.22, -0.76)
(6.20, -0.74)
(6.19, -0.73)
(6.17, -0.74)
(6.15, -0.75)
(6.15, -0.76)
(6.15, -0.77)
(6.15, -0.81)
(6.17, -0.86)
(6.17, -0.92)
(6.17, -0.99)
(6.18, -1.08)
(6.17, -1.17)
(6.13, -1.25)
(6.09, -1.31)
(6.05, -1.34)
(6.01, -1.36)
(5.96, -1.35)
(5.93, -1.34)
(5.92, -1.35)
(5.93, -1.39)
(5.94, -1.43)
(5.95, -1.48)
(5.97, -1.55)
(5.99, -1.58)
(6.01, -1.57)
(6.02, -1.56)
(6.01, -1.53)
(6.00, -1.52)
(6.01, -1.52)
(6.03, -1.50)
(6.09, -1.43)
(6.18, -1.36)
(6.32, -1.28)
(6.50, -1.20)
(6.71, -1.16)
(6.95, -1.18)
(7.25, -1.24)
(7.61, -1.31)
(8.06, -1.37)
(8.55, -1.37)
(9.02, -1.27)
(9.40, -1.02)
(9.66, -0.63)
(9.81, -0.16)
(9.87, 0.31)
(9.85, 0.76)
(9.79, 1.17)
(9.70, 1.58)
(9.59, 2.00)
(9.35, 2.42)
(9.01, 2.86)
(8.61, 3.26)
(8.13, 3.63)
(7.58, 3.88)
(7.02, 3.96)
(6.47, 3.89)
(5.97, 3.70)
(5.55, 3.42)
(5.26, 3.09)
(5.12, 2.69)
(5.18, 2.28)
(5.47, 1.92)
(5.92, 1.62)
(6.44, 1.35)
(7.02, 1.10)
(7.59, 0.80)
(8.13, 0.53)
(8.68, 0.29)
(9.23, 0.11)
(9.75, -0.05)
(10.24, -0.16)
(10.67, -0.19)
(11.02, -0.16)
(11.27, -0.10)
(11.42, -0.01)
(11.46, 0.16)
(11.40, 0.36)
(11.23, 0.57)
(11.00, 0.79)
(10.73, 1.04)
(10.44, 1.27)
(10.19, 1.47)
(9.97, 1.64)
(9.78, 1.81)
(9.61, 2.00)
(9.48, 2.21)
(9.40, 2.44)
(9.37, 2.68)
(9.34, 2.97)
(9.28, 3.23)
(9.20, 3.49)
(9.07, 3.72)
(8.92, 3.88)
(8.72, 4.00)
(8.48, 4.11)
(8.25, 4.16)
(7.98, 4.14)
(7.67, 4.05)
(7.37, 3.94)
(7.06, 3.78)
(6.75, 3.63)
(6.44, 3.46)
(6.11, 3.28)
(5.77, 3.10)
(5.44, 2.88)
(5.12, 2.65)
(4.82, 2.43)
(4.57, 2.24)
(4.36, 2.08)
(4.18, 1.96)
(4.04, 1.88)
(3.93, 1.81)
(3.85, 1.75)
(3.79, 1.68)
(3.76, 1.60)
(3.75, 1.51)
(3.76, 1.46)
(3.78, 1.42)
(3.81, 1.37)
(3.85, 1.33)
(3.90, 1.27)
(3.96, 1.20)
(4.01, 1.10)
(4.05, 1.00)
(4.09, 0.90)
(4.13, 0.78)
(4.19, 0.65)
(4.25, 0.50)
(4.31, 0.35)
(4.37, 0.20)
(4.42, 0.04)
(4.47, -0.14)
(4.53, -0.30)
(4.57, -0.46)
(4.62, -0.62)
(4.66, -0.78)
(4.68, -0.94)
(4.67, -1.09)
(4.64, -1.24)
(4.61, -1.37)
(4.58, -1.49)
(4.56, -1.58)
(4.55, -1.66)
(4.55, -1.70)
(4.56, -1.71)
(4.58, -1.71)
(4.61, -1.71)
(4.62, -1.73)
(4.63, -1.76)
(4.63, -1.79)
(4.62, -1.83)
(4.60, -1.87)
(4.56, -1.90)
(4.53, -1.92)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
(4.54, -1.93)
};
 %   


==> plots/kaist_traj_coords/circle_gt.tex <==
\addplot3[
    fill=none,draw = clr1,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.02, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.07, 0.01, -0.00)
(-0.07, 0.01, 0.00)
(-0.07, 0.01, 0.00)
(-0.07, 0.01, 0.00)
(-0.07, 0.01, 0.01)
(-0.08, 0.01, 0.01)
(-0.08, 0.01, 0.01)
(-0.08, 0.01, 0.01)
(-0.08, 0.01, 0.01)
(-0.08, 0.01, 0.01)
(-0.08, 0.01, 0.01)
(-0.08, 0.00, 0.01)
(-0.08, 0.00, 0.01)
(-0.08, 0.01, 0.01)
(-0.08, 0.01, 0.00)
(-0.07, 0.01, 0.00)
(-0.07, 0.01, -0.00)
(-0.07, 0.01, 0.00)
(-0.07, 0.01, 0.02)
(-0.07, 0.01, 0.05)
(-0.07, 0.01, 0.07)
(-0.07, 0.01, 0.10)
(-0.07, 0.01, 0.09)
(-0.07, 0.02, 0.07)
(-0.07, 0.02, 0.05)
(-0.07, 0.01, 0.04)
(-0.06, 0.02, 0.05)
(-0.06, 0.02, 0.08)
(-0.07, 0.01, 0.11)
(-0.07, 0.02, 0.05)
(-0.06, 0.02, 0.02)
(-0.06, 0.02, 0.01)
(-0.06, 0.02, 0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.05, 0.02, -0.00)
(-0.05, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.05, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.05, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.05, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.05, 0.02, -0.00)
(-0.05, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, -0.00)
(-0.06, 0.02, 0.00)
(-0.08, 0.02, 0.02)
(-0.10, 0.02, 0.10)
(-0.14, 0.02, 0.26)
(-0.17, 0.02, 0.38)
(-0.20, 0.02, 0.45)
(-0.22, 0.03, 0.53)
(-0.23, 0.03, 0.57)
(-0.23, 0.04, 0.61)
(-0.22, 0.04, 0.63)
(-0.21, 0.04, 0.66)
(-0.20, 0.04, 0.68)
(-0.18, 0.05, 0.71)
(-0.17, 0.05, 0.73)
(-0.16, 0.05, 0.74)
(-0.16, 0.05, 0.75)
(-0.15, 0.05, 0.76)
(-0.15, 0.05, 0.76)
(-0.14, 0.05, 0.77)
(-0.14, 0.05, 0.77)
(-0.13, 0.06, 0.78)
(-0.12, 0.09, 0.78)
(-0.11, 0.17, 0.78)
(-0.10, 0.28, 0.79)
(-0.07, 0.39, 0.79)
(-0.04, 0.48, 0.80)
(0.00, 0.56, 0.81)
(0.06, 0.62, 0.81)
(0.11, 0.65, 0.82)
(0.18, 0.67, 0.82)
(0.26, 0.67, 0.82)
(0.35, 0.64, 0.81)
(0.45, 0.57, 0.81)
(0.50, 0.53, 0.82)
(0.55, 0.44, 0.82)
(0.60, 0.34, 0.83)
(0.66, 0.12, 0.85)
(0.68, -0.00, 0.85)
(0.68, -0.14, 0.87)
(0.65, -0.26, 0.87)
(0.63, -0.34, 0.88)
(0.60, -0.40, 0.88)
(0.55, -0.47, 0.88)
(0.50, -0.51, 0.89)
(0.45, -0.55, 0.89)
(0.38, -0.58, 0.90)
(0.30, -0.61, 0.90)
(0.23, -0.62, 0.90)
(0.17, -0.63, 0.91)
(0.10, -0.65, 0.92)
(0.04, -0.67, 0.92)
(-0.03, -0.69, 0.93)
(-0.10, -0.69, 0.93)
(-0.16, -0.68, 0.93)
(-0.22, -0.66, 0.93)
(-0.27, -0.64, 0.93)
(-0.33, -0.62, 0.93)
(-0.39, -0.59, 0.94)
(-0.46, -0.56, 0.94)
(-0.51, -0.53, 0.94)
(-0.55, -0.49, 0.95)
(-0.60, -0.44, 0.96)
(-0.64, -0.38, 0.96)
(-0.67, -0.33, 0.96)
(-0.70, -0.26, 0.97)
(-0.72, -0.19, 0.97)
(-0.73, -0.14, 0.97)
(-0.74, -0.07, 0.97)
(-0.75, -0.01, 0.98)
(-0.76, 0.09, 0.98)
(-0.75, 0.17, 0.99)
(-0.74, 0.23, 0.99)
(-0.72, 0.32, 0.99)
(-0.68, 0.38, 1.00)
(-0.64, 0.45, 1.01)
(-0.60, 0.49, 1.01)
(-0.53, 0.55, 1.01)
(-0.47, 0.59, 1.02)
(-0.41, 0.63, 1.02)
(-0.33, 0.66, 1.03)
(-0.25, 0.69, 1.03)
(-0.18, 0.70, 1.03)
(-0.12, 0.71, 1.03)
(-0.05, 0.72, 1.02)
(0.01, 0.71, 1.02)
(0.08, 0.70, 1.01)
(0.13, 0.69, 1.02)
(0.20, 0.66, 1.01)
(0.25, 0.63, 1.02)
(0.31, 0.60, 1.02)
(0.36, 0.57, 1.01)
(0.41, 0.53, 1.01)
(0.45, 0.49, 1.01)
(0.49, 0.43, 1.02)
(0.52, 0.37, 1.02)
(0.58, 0.24, 1.04)
(0.62, 0.11, 1.04)
(0.64, 0.02, 1.05)
(0.65, -0.06, 1.06)
(0.66, -0.15, 1.06)
(0.66, -0.23, 1.07)
(0.65, -0.30, 1.08)
(0.63, -0.37, 1.09)
(0.61, -0.43, 1.09)
(0.58, -0.50, 1.10)
(0.54, -0.54, 1.11)
(0.50, -0.57, 1.11)
(0.44, -0.60, 1.11)
(0.38, -0.62, 1.11)
(0.32, -0.62, 1.11)
(0.25, -0.63, 1.10)
(0.17, -0.63, 1.10)
(0.05, -0.64, 1.10)
(-0.06, -0.65, 1.10)
(-0.13, -0.65, 1.10)
(-0.19, -0.65, 1.11)
(-0.26, -0.65, 1.11)
(-0.32, -0.64, 1.11)
(-0.39, -0.62, 1.12)
(-0.44, -0.59, 1.12)
(-0.48, -0.56, 1.13)
(-0.53, -0.52, 1.13)
(-0.57, -0.48, 1.14)
(-0.61, -0.41, 1.15)
(-0.64, -0.35, 1.15)
(-0.67, -0.30, 1.15)
(-0.70, -0.24, 1.15)
(-0.72, -0.18, 1.15)
(-0.73, -0.11, 1.15)
(-0.74, -0.05, 1.15)
(-0.74, 0.01, 1.15)
(-0.73, 0.08, 1.15)
(-0.72, 0.15, 1.15)
(-0.69, 0.24, 1.16)
(-0.66, 0.31, 1.16)
(-0.63, 0.38, 1.17)
(-0.59, 0.44, 1.17)
(-0.54, 0.51, 1.17)
(-0.48, 0.56, 1.18)
(-0.41, 0.61, 1.18)
(-0.35, 0.64, 1.19)
(-0.29, 0.66, 1.19)
(-0.23, 0.68, 1.19)
(-0.17, 0.70, 1.20)
(-0.10, 0.71, 1.20)
(-0.04, 0.71, 1.21)
(0.03, 0.70, 1.21)
(0.08, 0.68, 1.21)
(0.14, 0.66, 1.21)
(0.20, 0.64, 1.22)
(0.23, 0.62, 1.22)
(0.29, 0.59, 1.23)
(0.33, 0.56, 1.24)
(0.38, 0.53, 1.25)
(0.43, 0.48, 1.25)
(0.47, 0.42, 1.24)
(0.52, 0.36, 1.24)
(0.55, 0.30, 1.24)
(0.58, 0.23, 1.24)
(0.61, 0.14, 1.24)
(0.63, 0.07, 1.24)
(0.64, -0.02, 1.24)
(0.64, -0.09, 1.25)
(0.63, -0.17, 1.25)
(0.62, -0.24, 1.26)
(0.60, -0.31, 1.27)
(0.58, -0.37, 1.28)
(0.55, -0.43, 1.28)
(0.51, -0.48, 1.28)
(0.47, -0.53, 1.28)
(0.43, -0.57, 1.28)
(0.39, -0.61, 1.28)
(0.34, -0.64, 1.28)
(0.27, -0.68, 1.28)
(0.20, -0.70, 1.28)
(0.12, -0.72, 1.28)
(0.05, -0.72, 1.28)
(-0.03, -0.72, 1.28)
(-0.11, -0.72, 1.29)
(-0.19, -0.71, 1.29)
(-0.27, -0.70, 1.30)
(-0.35, -0.68, 1.30)
(-0.42, -0.65, 1.30)
(-0.48, -0.61, 1.31)
(-0.55, -0.56, 1.31)
(-0.61, -0.50, 1.31)
(-0.64, -0.46, 1.32)
(-0.68, -0.39, 1.33)
(-0.71, -0.32, 1.33)
(-0.72, -0.25, 1.33)
(-0.73, -0.18, 1.33)
(-0.74, -0.11, 1.33)
(-0.73, -0.04, 1.33)
(-0.73, 0.02, 1.33)
(-0.72, 0.09, 1.33)
(-0.71, 0.15, 1.33)
(-0.70, 0.21, 1.34)
(-0.68, 0.27, 1.34)
(-0.64, 0.33, 1.35)
(-0.61, 0.39, 1.35)
(-0.57, 0.44, 1.35)
(-0.52, 0.49, 1.36)
(-0.47, 0.54, 1.37)
(-0.42, 0.57, 1.38)
(-0.35, 0.61, 1.39)
(-0.27, 0.64, 1.40)
(-0.19, 0.66, 1.41)
(-0.12, 0.67, 1.41)
(-0.05, 0.68, 1.41)
(0.02, 0.68, 1.40)
(0.09, 0.67, 1.40)
(0.16, 0.65, 1.39)
(0.21, 0.63, 1.38)
(0.27, 0.60, 1.39)
(0.31, 0.56, 1.39)
(0.38, 0.50, 1.39)
(0.42, 0.46, 1.39)
(0.46, 0.41, 1.39)
(0.49, 0.37, 1.38)
(0.52, 0.31, 1.38)
(0.56, 0.22, 1.39)
(0.58, 0.16, 1.40)
(0.60, 0.09, 1.40)
(0.61, 0.01, 1.41)
(0.61, -0.06, 1.41)
(0.61, -0.13, 1.42)
(0.61, -0.22, 1.43)
(0.59, -0.28, 1.44)
(0.57, -0.35, 1.45)
(0.55, -0.41, 1.45)
(0.52, -0.46, 1.45)
(0.49, -0.51, 1.45)
(0.45, -0.55, 1.46)
(0.39, -0.61, 1.46)
(0.33, -0.64, 1.46)
(0.28, -0.67, 1.47)
(0.18, -0.70, 1.48)
(0.05, -0.72, 1.49)
(-0.05, -0.72, 1.51)
(-0.13, -0.71, 1.51)
(-0.20, -0.70, 1.51)
(-0.27, -0.68, 1.51)
(-0.35, -0.65, 1.52)
(-0.41, -0.63, 1.52)
(-0.47, -0.60, 1.52)
(-0.54, -0.54, 1.51)
(-0.68, -0.33, 1.50)
(-0.71, -0.25, 1.50)
(-0.75, 0.05, 1.50)
(-0.72, 0.25, 1.52)
(-0.69, 0.34, 1.52)
(-0.67, 0.40, 1.53)
(-0.63, 0.47, 1.54)
(-0.59, 0.51, 1.55)
(-0.54, 0.54, 1.55)
(-0.48, 0.57, 1.55)
(-0.43, 0.59, 1.56)
(-0.36, 0.61, 1.56)
(-0.30, 0.62, 1.55)
(-0.22, 0.63, 1.55)
(-0.16, 0.64, 1.55)
(-0.09, 0.64, 1.55)
(-0.00, 0.63, 1.56)
(0.05, 0.62, 1.56)
(0.12, 0.61, 1.56)
(0.18, 0.59, 1.56)
(0.23, 0.58, 1.56)
(0.29, 0.56, 1.56)
(0.34, 0.54, 1.57)
(0.39, 0.51, 1.57)
(0.45, 0.48, 1.57)
(0.49, 0.44, 1.57)
(0.54, 0.39, 1.57)
(0.58, 0.33, 1.58)
(0.61, 0.28, 1.58)
(0.63, 0.20, 1.59)
(0.65, 0.14, 1.59)
(0.65, 0.07, 1.59)
(0.65, -0.01, 1.58)
(0.65, -0.09, 1.58)
(0.65, -0.18, 1.58)
(0.64, -0.25, 1.58)
(0.62, -0.35, 1.57)
(0.60, -0.42, 1.57)
(0.56, -0.47, 1.57)
(0.53, -0.52, 1.58)
(0.48, -0.55, 1.58)
(0.43, -0.58, 1.59)
(0.37, -0.60, 1.59)
(0.30, -0.61, 1.60)
(0.22, -0.61, 1.61)
(0.15, -0.62, 1.61)
(0.05, -0.65, 1.61)
(-0.03, -0.67, 1.62)
(-0.10, -0.68, 1.62)
(-0.19, -0.69, 1.61)
(-0.26, -0.68, 1.61)
(-0.33, -0.67, 1.61)
(-0.40, -0.65, 1.61)
(-0.45, -0.63, 1.61)
(-0.50, -0.59, 1.61)
(-0.54, -0.55, 1.61)
(-0.58, -0.50, 1.62)
(-0.61, -0.45, 1.61)
(-0.64, -0.40, 1.61)
(-0.68, -0.32, 1.61)
(-0.71, -0.24, 1.60)
(-0.74, -0.17, 1.61)
(-0.75, -0.09, 1.60)
(-0.76, -0.00, 1.60)
(-0.76, 0.09, 1.60)
(-0.74, 0.20, 1.60)
(-0.73, 0.28, 1.59)
(-0.70, 0.35, 1.59)
(-0.67, 0.41, 1.59)
(-0.63, 0.47, 1.59)
(-0.59, 0.51, 1.59)
(-0.53, 0.54, 1.60)
(-0.47, 0.57, 1.60)
(-0.41, 0.59, 1.60)
(-0.35, 0.61, 1.61)
(-0.29, 0.62, 1.61)
(-0.23, 0.63, 1.61)
(-0.17, 0.64, 1.61)
(-0.09, 0.64, 1.60)
(-0.00, 0.64, 1.60)
(0.06, 0.64, 1.60)
(0.14, 0.64, 1.59)
(0.22, 0.62, 1.59)
(0.28, 0.60, 1.60)
(0.34, 0.57, 1.60)
(0.40, 0.53, 1.60)
(0.45, 0.49, 1.59)
(0.50, 0.44, 1.59)
(0.55, 0.39, 1.60)
(0.58, 0.33, 1.60)
(0.61, 0.28, 1.60)
(0.63, 0.22, 1.60)
(0.65, 0.16, 1.60)
(0.66, 0.11, 1.60)
(0.66, 0.05, 1.59)
(0.67, -0.01, 1.58)
(0.66, -0.07, 1.58)
(0.64, -0.20, 1.59)
(0.61, -0.29, 1.60)
(0.58, -0.36, 1.60)
(0.54, -0.42, 1.60)
(0.49, -0.48, 1.61)
(0.33, -0.64, 1.61)
(0.25, -0.69, 1.61)
(0.16, -0.72, 1.61)
(-0.07, -0.73, 1.61)
(-0.26, -0.67, 1.61)
(-0.37, -0.63, 1.62)
(-0.45, -0.59, 1.62)
(-0.51, -0.56, 1.62)
(-0.56, -0.52, 1.62)
(-0.60, -0.48, 1.62)
(-0.63, -0.43, 1.62)
(-0.67, -0.37, 1.62)
(-0.70, -0.32, 1.61)
(-0.73, -0.25, 1.61)
(-0.75, -0.19, 1.61)
(-0.76, -0.11, 1.61)
(-0.77, -0.05, 1.61)
(-0.78, 0.04, 1.61)
(-0.77, 0.10, 1.61)
(-0.74, 0.17, 1.57)
(-0.69, 0.22, 1.41)
(-0.58, 0.24, 1.15)
(-0.47, 0.25, 0.92)
(-0.34, 0.23, 0.65)
(-0.23, 0.21, 0.45)
(-0.15, 0.18, 0.30)
(-0.08, 0.16, 0.21)
(-0.04, 0.12, 0.16)
(-0.01, 0.09, 0.14)
(-0.01, 0.05, 0.13)
(-0.01, 0.01, 0.13)
(-0.02, -0.01, 0.13)
(-0.04, -0.04, 0.12)
(-0.06, -0.06, 0.11)
(-0.06, -0.07, 0.11)
(-0.06, -0.08, 0.10)
(-0.06, -0.08, 0.09)
(-0.05, -0.07, 0.09)
(-0.04, -0.05, 0.09)
(-0.04, -0.04, 0.08)
(-0.04, -0.02, 0.08)
    };
%

==> plots/kaist_traj_coords/circle_jetson_slam.tex <==
%
\addplot3[
    fill=none,draw = clr2,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(-0.08, 0.01, 0.00)
(-0.07, 0.01, 0.00)
(-0.08, 0.01, 0.00)
(-0.08, 0.01, 0.00)
(-0.08, 0.01, 0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.07, 0.01, 0.00)
(-0.07, 0.01, 0.00)
(-0.08, 0.01, 0.00)
(-0.07, 0.01, 0.00)
(-0.07, 0.01, 0.00)
(-0.08, 0.01, 0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.00, -0.00)
(-0.07, 0.01, -0.00)
(-0.08, 0.00, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.00, -0.00)
(-0.07, 0.01, -0.00)
(-0.08, 0.00, -0.00)
(-0.08, 0.00, -0.01)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.00, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.00, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.00, -0.00)
(-0.08, 0.01, -0.01)
(-0.07, 0.00, -0.00)
(-0.08, 0.01, -0.00)
(-0.07, 0.00, -0.00)
(-0.07, -0.00, -0.01)
(-0.07, 0.01, -0.00)
(-0.08, 0.00, -0.01)
(-0.07, -0.00, -0.01)
(-0.07, 0.00, -0.00)
(-0.08, 0.00, -0.00)
(-0.08, 0.00, -0.00)
(-0.08, 0.00, -0.01)
(-0.07, 0.00, -0.01)
(-0.07, 0.00, -0.00)
(-0.08, 0.00, -0.00)
(-0.08, 0.01, -0.00)
(-0.08, 0.00, -0.01)
(-0.07, -0.00, -0.01)
(-0.07, 0.01, -0.00)
(-0.08, 0.00, -0.00)
(-0.08, 0.01, 0.00)
(-0.08, 0.01, -0.00)
(-0.07, -0.00, -0.01)
(-0.08, 0.01, -0.00)
(-0.08, 0.01, -0.00)
(-0.07, 0.00, -0.00)
(-0.08, 0.00, 0.00)
(-0.08, 0.00, 0.01)
(-0.08, -0.00, 0.01)
(-0.08, -0.03, 0.00)
(-0.08, -0.02, 0.01)
(-0.08, -0.03, 0.01)
(-0.08, -0.04, 0.01)
(-0.07, -0.03, 0.01)
(-0.07, -0.02, 0.01)
(-0.08, -0.01, 0.02)
(-0.07, 0.00, 0.01)
(-0.08, 0.01, 0.01)
(-0.08, 0.01, 0.02)
(-0.08, 0.03, 0.01)
(-0.08, 0.03, 0.01)
(-0.07, 0.02, 0.01)
(-0.07, 0.02, 0.01)
(-0.08, 0.02, 0.01)
(-0.08, 0.02, 0.01)
(-0.07, 0.02, 0.01)
(-0.07, 0.01, 0.00)
(-0.07, 0.01, 0.00)
(-0.07, 0.01, 0.01)
(-0.06, 0.01, 0.03)
(-0.07, 0.00, 0.06)
(-0.07, 0.02, 0.11)
(-0.07, 0.03, 0.10)
(-0.07, 0.02, 0.08)
(-0.07, 0.02, 0.06)
(-0.06, 0.02, 0.05)
(-0.06, 0.02, 0.09)
(-0.06, 0.02, 0.11)
(-0.07, 0.03, 0.10)
(-0.06, 0.02, 0.06)
(-0.06, 0.02, 0.03)
(-0.05, 0.01, 0.01)
(-0.05, 0.01, 0.01)
(-0.05, 0.02, 0.00)
(-0.06, 0.02, 0.01)
(-0.06, 0.02, 0.01)
(-0.05, 0.02, 0.01)
(-0.06, 0.02, 0.01)
(-0.06, 0.02, 0.00)
(-0.06, 0.02, 0.00)
(-0.06, 0.02, 0.01)
(-0.06, 0.02, 0.00)
(-0.06, 0.02, 0.01)
(-0.05, 0.01, 0.00)
(-0.06, 0.02, 0.00)
(-0.06, 0.02, 0.01)
(-0.06, 0.02, 0.00)
(-0.05, 0.02, 0.00)
(-0.05, 0.01, 0.00)
(-0.06, 0.02, 0.01)
(-0.05, 0.01, 0.00)
(-0.05, 0.02, 0.00)
(-0.05, 0.02, 0.00)
(-0.05, 0.01, 0.01)
(-0.05, 0.02, 0.00)
(-0.05, 0.02, 0.00)
(-0.05, 0.02, 0.00)
(-0.06, 0.02, 0.01)
(-0.05, 0.02, 0.00)
(-0.05, 0.01, 0.01)
(-0.06, 0.02, 0.01)
(-0.05, 0.02, 0.00)
(-0.05, 0.01, 0.01)
(-0.06, 0.02, 0.00)
(-0.06, 0.02, 0.01)
(-0.06, 0.02, 0.01)
(-0.06, 0.02, 0.01)
(-0.06, 0.01, 0.01)
(-0.06, 0.02, 0.00)
(-0.05, 0.02, 0.00)
(-0.05, 0.01, 0.00)
(-0.06, 0.02, 0.01)
(-0.05, 0.02, 0.01)
(-0.05, 0.02, 0.01)
(-0.06, 0.02, 0.01)
(-0.05, 0.02, 0.01)
(-0.05, 0.01, 0.01)
(-0.06, 0.02, 0.01)
(-0.05, 0.01, 0.01)
(-0.05, 0.01, 0.01)
(-0.05, 0.02, 0.00)
(-0.06, 0.01, 0.01)
(-0.05, 0.01, 0.00)
(-0.06, 0.02, 0.00)
(-0.05, 0.01, 0.01)
(-0.06, 0.01, 0.01)
(-0.05, 0.01, 0.01)
(-0.06, 0.01, 0.00)
(-0.06, 0.02, 0.00)
(-0.05, 0.01, 0.00)
(-0.05, 0.02, 0.01)
(-0.05, 0.01, 0.01)
(-0.05, 0.01, 0.00)
(-0.06, 0.01, 0.01)
(-0.05, 0.01, 0.00)
(-0.05, 0.01, 0.00)
(-0.05, 0.01, 0.00)
(-0.06, 0.01, 0.01)
(-0.06, 0.02, 0.01)
(-0.06, 0.02, 0.00)
(-0.05, 0.01, 0.00)
(-0.05, 0.01, 0.00)
(-0.05, 0.01, 0.00)
(-0.05, 0.01, 0.01)
(-0.05, 0.01, 0.01)
(-0.05, 0.01, 0.00)
(-0.05, 0.01, 0.00)
(-0.05, 0.01, 0.00)
(-0.05, 0.01, 0.01)
(-0.05, 0.01, 0.01)
(-0.05, 0.01, 0.00)
(-0.05, 0.01, 0.00)
(-0.06, 0.01, 0.01)
(-0.05, 0.01, 0.01)
(-0.05, 0.02, 0.01)
(-0.05, 0.01, 0.00)
(-0.06, 0.02, 0.01)
(-0.05, 0.01, 0.01)
(-0.05, 0.01, 0.01)
(-0.06, 0.02, 0.01)
(-0.05, 0.02, 0.00)
(-0.05, 0.01, 0.01)
(-0.06, 0.01, 0.01)
(-0.06, 0.02, 0.01)
(-0.06, 0.01, 0.01)
(-0.06, 0.02, 0.01)
(-0.05, 0.01, 0.00)
(-0.05, 0.02, 0.01)
(-0.05, 0.02, 0.00)
(-0.05, 0.02, 0.01)
(-0.08, 0.03, 0.04)
(-0.12, 0.03, 0.16)
(-0.16, 0.03, 0.33)
(-0.19, 0.03, 0.44)
(-0.22, 0.04, 0.51)
(-0.23, 0.04, 0.56)
(-0.23, 0.05, 0.60)
(-0.22, 0.04, 0.63)
(-0.20, 0.04, 0.66)
(-0.18, 0.05, 0.69)
(-0.17, 0.07, 0.71)
(-0.15, 0.05, 0.72)
(-0.15, 0.06, 0.73)
(-0.14, 0.06, 0.75)
(-0.14, 0.06, 0.74)
(-0.13, 0.06, 0.75)
(-0.12, 0.06, 0.76)
(-0.11, 0.13, 0.79)
(-0.10, 0.26, 0.79)
(-0.06, 0.39, 0.79)
(-0.02, 0.52, 0.80)
(0.04, 0.62, 0.82)
(0.12, 0.66, 0.82)
(0.21, 0.68, 0.82)
(0.30, 0.67, 0.82)
(0.39, 0.64, 0.83)
(0.46, 0.57, 0.82)
(0.53, 0.50, 0.81)
(0.58, 0.41, 0.82)
(0.62, 0.31, 0.83)
(0.65, 0.20, 0.84)
(0.67, 0.09, 0.84)
(0.68, -0.03, 0.86)
(0.68, -0.16, 0.87)
(0.66, -0.26, 0.87)
(0.62, -0.36, 0.87)
(0.57, -0.43, 0.88)
(0.51, -0.50, 0.89)
(0.44, -0.55, 0.89)
(0.37, -0.58, 0.89)
(0.29, -0.61, 0.90)
(0.21, -0.63, 0.90)
(0.13, -0.65, 0.91)
(0.04, -0.67, 0.92)
(-0.03, -0.70, 0.92)
(-0.11, -0.70, 0.92)
(-0.18, -0.69, 0.92)
(-0.26, -0.65, 0.92)
(-0.33, -0.62, 0.92)
(-0.41, -0.59, 0.93)
(-0.48, -0.55, 0.93)
(-0.54, -0.51, 0.94)
(-0.59, -0.46, 0.95)
(-0.63, -0.38, 0.96)
(-0.68, -0.30, 0.96)
(-0.72, -0.23, 0.96)
(-0.74, -0.14, 0.97)
(-0.76, -0.07, 0.96)
(-0.76, 0.03, 0.98)
(-0.75, 0.12, 0.98)
(-0.74, 0.20, 0.99)
(-0.72, 0.30, 1.00)
(-0.70, 0.37, 1.00)
(-0.64, 0.44, 1.00)
(-0.58, 0.51, 1.01)
(-0.51, 0.55, 1.01)
(-0.44, 0.60, 1.01)
(-0.36, 0.64, 1.02)
(-0.27, 0.68, 1.03)
(-0.19, 0.71, 1.03)
(-0.11, 0.73, 1.03)
(-0.03, 0.72, 1.02)
(0.04, 0.71, 1.02)
(0.12, 0.70, 1.02)
(0.19, 0.67, 1.01)
(0.27, 0.63, 1.02)
(0.33, 0.60, 1.02)
(0.39, 0.56, 1.01)
(0.44, 0.50, 1.01)
(0.49, 0.44, 1.01)
(0.54, 0.35, 1.02)
(0.58, 0.26, 1.03)
(0.62, 0.17, 1.04)
(0.63, 0.08, 1.04)
(0.65, -0.03, 1.05)
(0.65, -0.14, 1.06)
(0.65, -0.24, 1.07)
(0.64, -0.34, 1.08)
(0.61, -0.42, 1.09)
(0.57, -0.50, 1.10)
(0.52, -0.55, 1.11)
(0.46, -0.59, 1.11)
(0.38, -0.62, 1.10)
(0.31, -0.63, 1.10)
(0.21, -0.64, 1.10)
(0.12, -0.64, 1.10)
(0.03, -0.65, 1.09)
(-0.06, -0.65, 1.10)
(-0.15, -0.65, 1.10)
(-0.24, -0.65, 1.10)
(-0.32, -0.64, 1.10)
(-0.39, -0.62, 1.11)
(-0.46, -0.59, 1.13)
(-0.51, -0.54, 1.13)
(-0.56, -0.49, 1.13)
(-0.60, -0.44, 1.14)
(-0.64, -0.36, 1.14)
(-0.68, -0.29, 1.14)
(-0.70, -0.22, 1.15)
(-0.73, -0.13, 1.14)
(-0.74, -0.05, 1.14)
(-0.74, 0.03, 1.16)
(-0.72, 0.13, 1.16)
(-0.70, 0.23, 1.15)
(-0.66, 0.31, 1.16)
(-0.61, 0.39, 1.17)
(-0.56, 0.47, 1.17)
(-0.51, 0.54, 1.18)
(-0.44, 0.58, 1.18)
(-0.37, 0.63, 1.19)
(-0.29, 0.66, 1.20)
(-0.21, 0.68, 1.19)
(-0.13, 0.71, 1.21)
(-0.05, 0.71, 1.21)
(0.03, 0.70, 1.20)
(0.10, 0.68, 1.21)
(0.17, 0.66, 1.21)
(0.24, 0.63, 1.23)
(0.29, 0.61, 1.24)
(0.35, 0.57, 1.25)
(0.41, 0.51, 1.26)
(0.46, 0.45, 1.25)
(0.52, 0.37, 1.24)
(0.56, 0.30, 1.24)
(0.60, 0.21, 1.24)
(0.62, 0.11, 1.24)
(0.63, 0.02, 1.24)
(0.63, -0.09, 1.25)
(0.63, -0.20, 1.25)
(0.61, -0.28, 1.26)
(0.57, -0.37, 1.27)
(0.53, -0.45, 1.28)
(0.49, -0.51, 1.28)
(0.44, -0.57, 1.27)
(0.38, -0.61, 1.28)
(0.32, -0.65, 1.28)
(0.26, -0.68, 1.28)
(0.18, -0.71, 1.27)
(0.10, -0.73, 1.27)
(0.01, -0.72, 1.27)
(-0.09, -0.72, 1.28)
(-0.19, -0.71, 1.29)
(-0.30, -0.69, 1.30)
(-0.40, -0.66, 1.30)
(-0.47, -0.62, 1.30)
(-0.57, -0.55, 1.30)
(-0.63, -0.49, 1.32)
(-0.69, -0.41, 1.33)
(-0.72, -0.32, 1.32)
(-0.73, -0.24, 1.33)
(-0.74, -0.16, 1.33)
(-0.74, -0.07, 1.33)
(-0.73, 0.01, 1.33)
(-0.72, 0.11, 1.33)
(-0.71, 0.19, 1.33)
(-0.68, 0.25, 1.33)
(-0.64, 0.32, 1.34)
(-0.60, 0.38, 1.35)
(-0.55, 0.46, 1.35)
(-0.49, 0.51, 1.36)
(-0.43, 0.57, 1.38)
(-0.36, 0.61, 1.39)
(-0.28, 0.64, 1.41)
(-0.19, 0.66, 1.42)
(-0.09, 0.68, 1.41)
(-0.01, 0.68, 1.41)
(0.07, 0.68, 1.40)
(0.15, 0.66, 1.38)
(0.21, 0.64, 1.38)
(0.28, 0.60, 1.39)
(0.33, 0.54, 1.38)
(0.39, 0.52, 1.38)
(0.44, 0.45, 1.38)
(0.48, 0.40, 1.39)
(0.52, 0.33, 1.39)
(0.55, 0.26, 1.38)
(0.58, 0.19, 1.39)
(0.60, 0.10, 1.40)
(0.60, 0.01, 1.40)
(0.61, -0.09, 1.41)
(0.61, -0.18, 1.42)
(0.59, -0.27, 1.44)
(0.57, -0.36, 1.44)
(0.54, -0.44, 1.44)
(0.49, -0.49, 1.45)
(0.45, -0.55, 1.45)
(0.38, -0.60, 1.46)
(0.32, -0.65, 1.46)
(0.25, -0.69, 1.46)
(0.17, -0.71, 1.47)
(0.08, -0.72, 1.48)
(-0.02, -0.72, 1.49)
(-0.13, -0.71, 1.50)
(-0.23, -0.69, 1.51)
(-0.31, -0.66, 1.50)
(-0.39, -0.64, 1.51)
(-0.46, -0.61, 1.51)
(-0.53, -0.55, 1.49)
(-0.59, -0.50, 1.50)
(-0.63, -0.43, 1.50)
(-0.67, -0.35, 1.50)
(-0.71, -0.26, 1.50)
(-0.73, -0.17, 1.50)
(-0.75, -0.08, 1.50)
(-0.75, 0.01, 1.51)
(-0.74, 0.10, 1.49)
(-0.73, 0.21, 1.51)
(-0.70, 0.28, 1.52)
(-0.67, 0.37, 1.53)
(-0.64, 0.45, 1.55)
(-0.58, 0.52, 1.55)
(-0.52, 0.56, 1.56)
(-0.45, 0.58, 1.56)
(-0.37, 0.60, 1.57)
(-0.30, 0.63, 1.57)
(-0.22, 0.64, 1.56)
(-0.15, 0.65, 1.57)
(-0.06, 0.64, 1.57)
(0.02, 0.63, 1.56)
(0.10, 0.61, 1.57)
(0.17, 0.60, 1.58)
(0.25, 0.59, 1.57)
(0.31, 0.56, 1.57)
(0.38, 0.53, 1.57)
(0.45, 0.49, 1.57)
(0.51, 0.44, 1.57)
(0.56, 0.38, 1.58)
(0.60, 0.30, 1.58)
(0.62, 0.23, 1.58)
(0.64, 0.16, 1.58)
(0.65, 0.08, 1.58)
(0.65, -0.03, 1.57)
(0.65, -0.15, 1.56)
(0.63, -0.25, 1.58)
(0.61, -0.36, 1.57)
(0.58, -0.43, 1.57)
(0.53, -0.50, 1.57)
(0.48, -0.55, 1.58)
(0.41, -0.58, 1.58)
(0.34, -0.60, 1.59)
(0.25, -0.62, 1.59)
(0.16, -0.62, 1.60)
(0.06, -0.64, 1.60)
(-0.03, -0.66, 1.60)
(-0.13, -0.68, 1.61)
(-0.21, -0.68, 1.61)
(-0.30, -0.68, 1.59)
(-0.38, -0.66, 1.60)
(-0.44, -0.64, 1.60)
(-0.50, -0.59, 1.61)
(-0.55, -0.54, 1.61)
(-0.61, -0.47, 1.63)
(-0.65, -0.41, 1.62)
(-0.69, -0.33, 1.61)
(-0.72, -0.22, 1.62)
(-0.75, -0.14, 1.61)
(-0.76, -0.06, 1.61)
(-0.76, 0.04, 1.61)
(-0.76, 0.15, 1.60)
(-0.74, 0.25, 1.60)
(-0.71, 0.33, 1.60)
(-0.68, 0.41, 1.59)
(-0.63, 0.47, 1.60)
(-0.56, 0.54, 1.60)
(-0.49, 0.57, 1.61)
(-0.41, 0.61, 1.62)
(-0.32, 0.61, 1.62)
(-0.25, 0.64, 1.62)
(-0.18, 0.63, 1.61)
(-0.10, 0.64, 1.61)
(-0.02, 0.66, 1.61)
(0.05, 0.64, 1.61)
(0.13, 0.64, 1.60)
(0.21, 0.64, 1.61)
(0.29, 0.61, 1.60)
(0.36, 0.56, 1.60)
(0.44, 0.50, 1.60)
(0.49, 0.45, 1.60)
(0.54, 0.39, 1.60)
(0.59, 0.32, 1.59)
(0.62, 0.25, 1.59)
(0.64, 0.17, 1.59)
(0.66, 0.09, 1.58)
(0.67, 0.02, 1.58)
(0.67, -0.06, 1.57)
(0.65, -0.14, 1.58)
(0.63, -0.23, 1.59)
(0.60, -0.29, 1.59)
(0.56, -0.38, 1.60)
(0.50, -0.46, 1.60)
(0.44, -0.53, 1.60)
(0.37, -0.58, 1.60)
(0.30, -0.65, 1.60)
(0.21, -0.70, 1.60)
(0.11, -0.73, 1.60)
(0.02, -0.74, 1.60)
(-0.07, -0.73, 1.61)
(-0.17, -0.70, 1.61)
(-0.26, -0.67, 1.61)
(-0.35, -0.64, 1.61)
(-0.43, -0.61, 1.61)
(-0.50, -0.57, 1.62)
(-0.56, -0.53, 1.63)
(-0.62, -0.47, 1.62)
(-0.67, -0.39, 1.62)
(-0.69, -0.33, 1.62)
(-0.73, -0.25, 1.61)
(-0.75, -0.18, 1.62)
(-0.77, -0.09, 1.62)
(-0.78, 0.01, 1.61)
(-0.77, 0.11, 1.61)
(-0.75, 0.19, 1.55)
(-0.66, 0.25, 1.29)
(-0.50, 0.26, 0.99)
(-0.35, 0.25, 0.69)
(-0.22, 0.22, 0.44)
(-0.12, 0.18, 0.26)
(-0.05, 0.15, 0.17)
(-0.01, 0.09, 0.14)
(-0.01, 0.04, 0.14)
(-0.02, 0.02, 0.13)
(-0.03, -0.03, 0.12)
(-0.06, -0.05, 0.11)
(-0.07, -0.08, 0.11)
(-0.06, -0.07, 0.09)
(-0.05, -0.07, 0.08)
(-0.05, -0.05, 0.09)
(-0.04, -0.03, 0.07)
(-0.04, -0.01, 0.04)
};

==> plots/kaist_traj_coords/infinite_gt.tex <==
\addplot3[
    fill=none,draw = clr1,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.01, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.01, -0.01, 0.00)
(-0.01, -0.01, 0.00)
(-0.01, -0.01, 0.00)
(-0.01, -0.01, 0.00)
(-0.01, -0.01, 0.01)
(-0.01, -0.01, 0.01)
(-0.01, -0.00, 0.01)
(-0.01, -0.00, 0.01)
(-0.01, -0.01, 0.01)
(-0.01, -0.01, 0.01)
(-0.01, -0.01, 0.01)
(-0.01, -0.01, 0.01)
(-0.01, -0.02, 0.01)
(-0.01, -0.02, 0.01)
(-0.01, -0.02, 0.02)
(-0.00, -0.01, 0.02)
(-0.01, -0.01, 0.05)
(-0.01, -0.01, 0.05)
(-0.01, -0.01, 0.02)
(-0.00, -0.00, 0.06)
(-0.00, -0.00, 0.04)
(0.00, 0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, -0.00)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.00, -0.00, 0.00)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, 0.00)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, 0.00)
(-0.01, -0.00, 0.00)
(-0.02, -0.01, 0.04)
(-0.05, -0.01, 0.13)
(-0.08, -0.02, 0.28)
(-0.11, -0.02, 0.38)
(-0.13, -0.02, 0.45)
(-0.15, -0.01, 0.50)
(-0.15, -0.00, 0.54)
(-0.16, 0.01, 0.59)
(-0.16, 0.02, 0.62)
(-0.15, 0.03, 0.65)
(-0.14, 0.04, 0.68)
(-0.11, 0.04, 0.72)
(-0.10, 0.04, 0.74)
(-0.08, 0.04, 0.76)
(-0.07, 0.03, 0.77)
(-0.05, 0.03, 0.78)
(0.12, 0.03, 0.80)
(0.25, 0.04, 0.80)
(0.40, 0.06, 0.81)
(0.55, 0.09, 0.81)
(0.72, 0.15, 0.82)
(0.79, 0.19, 0.83)
(0.83, 0.23, 0.83)
(0.83, 0.26, 0.84)
(0.81, 0.29, 0.84)
(0.76, 0.32, 0.85)
(0.70, 0.34, 0.85)
(0.62, 0.34, 0.85)
(0.54, 0.33, 0.86)
(0.47, 0.32, 0.85)
(0.39, 0.30, 0.85)
(0.30, 0.27, 0.85)
(0.23, 0.24, 0.84)
(0.16, 0.20, 0.84)
(0.10, 0.17, 0.85)
(0.05, 0.13, 0.86)
(0.02, 0.10, 0.87)
(-0.01, 0.07, 0.88)
(-0.04, 0.04, 0.88)
(-0.06, 0.01, 0.89)
(-0.08, -0.03, 0.89)
(-0.11, -0.07, 0.90)
(-0.14, -0.10, 0.90)
(-0.18, -0.14, 0.91)
(-0.21, -0.17, 0.91)
(-0.26, -0.21, 0.91)
(-0.30, -0.25, 0.91)
(-0.35, -0.28, 0.90)
(-0.39, -0.32, 0.90)
(-0.45, -0.35, 0.91)
(-0.50, -0.37, 0.91)
(-0.55, -0.39, 0.91)
(-0.63, -0.40, 0.92)
(-0.69, -0.39, 0.92)
(-0.76, -0.36, 0.92)
(-0.86, -0.29, 0.93)
(-0.93, -0.20, 0.94)
(-0.97, -0.13, 0.95)
(-1.00, -0.06, 0.96)
(-1.01, 0.02, 0.96)
(-1.01, 0.08, 0.95)
(-0.99, 0.14, 0.95)
(-0.96, 0.20, 0.94)
(-0.92, 0.25, 0.94)
(-0.87, 0.30, 0.94)
(-0.81, 0.34, 0.93)
(-0.74, 0.37, 0.93)
(-0.64, 0.40, 0.93)
(-0.57, 0.41, 0.94)
(-0.50, 0.40, 0.94)
(-0.40, 0.38, 0.94)
(-0.33, 0.34, 0.95)
(-0.28, 0.31, 0.95)
(-0.24, 0.28, 0.95)
(-0.20, 0.24, 0.97)
(-0.15, 0.19, 0.98)
(-0.12, 0.13, 0.98)
(-0.09, 0.07, 0.99)
(-0.06, 0.01, 0.98)
(-0.03, -0.05, 0.98)
(0.00, -0.09, 0.98)
(0.03, -0.13, 0.98)
(0.05, -0.16, 0.99)
(0.09, -0.19, 1.00)
(0.12, -0.21, 1.01)
(0.15, -0.23, 1.01)
(0.19, -0.24, 1.01)
(0.28, -0.28, 1.01)
(0.34, -0.30, 1.01)
(0.40, -0.33, 1.01)
(0.47, -0.35, 1.01)
(0.54, -0.37, 1.01)
(0.62, -0.39, 1.01)
(0.70, -0.40, 1.01)
(0.76, -0.39, 1.01)
(0.84, -0.36, 1.01)
(0.92, -0.28, 1.00)
(0.95, -0.20, 1.01)
(0.97, -0.13, 1.01)
(0.97, -0.04, 1.01)
(0.96, 0.03, 1.01)
(0.93, 0.10, 1.01)
(0.89, 0.16, 1.01)
(0.84, 0.22, 1.02)
(0.77, 0.27, 1.02)
(0.71, 0.31, 1.03)
(0.62, 0.34, 1.04)
(0.53, 0.36, 1.05)
(0.46, 0.36, 1.06)
(0.39, 0.34, 1.06)
(0.35, 0.32, 1.07)
(0.28, 0.26, 1.07)
(0.22, 0.19, 1.07)
(0.17, 0.09, 1.07)
(0.06, -0.05, 1.07)
(-0.12, -0.18, 1.07)
(-0.24, -0.23, 1.07)
(-0.32, -0.26, 1.07)
(-0.53, -0.32, 1.08)
(-0.60, -0.34, 1.08)
(-0.68, -0.34, 1.09)
(-0.75, -0.34, 1.09)
(-0.80, -0.33, 1.09)
(-0.86, -0.31, 1.09)
(-0.91, -0.29, 1.09)
(-0.95, -0.25, 1.09)
(-0.99, -0.18, 1.09)
(-1.00, -0.12, 1.10)
(-1.00, -0.04, 1.10)
(-0.99, 0.03, 1.10)
(-0.97, 0.10, 1.10)
(-0.93, 0.17, 1.10)
(-0.87, 0.25, 1.10)
(-0.79, 0.33, 1.10)
(-0.73, 0.37, 1.10)
(-0.66, 0.39, 1.10)
(-0.59, 0.41, 1.10)
(-0.51, 0.40, 1.10)
(-0.44, 0.38, 1.11)
(-0.37, 0.35, 1.11)
(-0.31, 0.30, 1.11)
(-0.26, 0.25, 1.11)
(-0.20, 0.17, 1.11)
(-0.17, 0.12, 1.12)
(-0.14, 0.08, 1.12)
(-0.11, 0.04, 1.12)
(-0.07, -0.01, 1.13)
(-0.03, -0.07, 1.14)
(-0.00, -0.12, 1.15)
(0.03, -0.16, 1.15)
(0.06, -0.20, 1.15)
(0.10, -0.24, 1.15)
(0.15, -0.27, 1.14)
(0.19, -0.29, 1.14)
(0.23, -0.31, 1.14)
(0.27, -0.31, 1.14)
(0.31, -0.32, 1.14)
(0.36, -0.33, 1.14)
(0.41, -0.33, 1.15)
(0.46, -0.33, 1.15)
(0.52, -0.33, 1.15)
(0.58, -0.32, 1.15)
(0.66, -0.32, 1.16)
(0.72, -0.31, 1.16)
(0.79, -0.30, 1.17)
(0.85, -0.27, 1.17)
(0.90, -0.24, 1.17)
(0.95, -0.19, 1.18)
(0.98, -0.13, 1.18)
(0.99, -0.08, 1.18)
(1.00, -0.01, 1.18)
(0.99, 0.06, 1.18)
(0.97, 0.11, 1.18)
(0.93, 0.19, 1.18)
(0.88, 0.25, 1.17)
(0.81, 0.31, 1.17)
(0.75, 0.33, 1.17)
(0.69, 0.34, 1.17)
(0.63, 0.34, 1.17)
(0.56, 0.34, 1.17)
(0.51, 0.33, 1.17)
(0.46, 0.32, 1.17)
(0.41, 0.30, 1.17)
(0.35, 0.27, 1.17)
(0.30, 0.24, 1.18)
(0.26, 0.20, 1.19)
(0.21, 0.16, 1.20)
(0.17, 0.11, 1.21)
(0.13, 0.06, 1.21)
(0.08, -0.01, 1.22)
(0.05, -0.05, 1.22)
(0.01, -0.10, 1.23)
(-0.02, -0.13, 1.24)
(-0.05, -0.16, 1.24)
(-0.09, -0.19, 1.24)
(-0.13, -0.21, 1.24)
(-0.17, -0.22, 1.24)
(-0.20, -0.22, 1.24)
(-0.24, -0.23, 1.24)
(-0.27, -0.23, 1.23)
(-0.56, -0.34, 1.23)
(-0.62, -0.36, 1.24)
(-0.72, -0.37, 1.25)
(-0.79, -0.36, 1.25)
(-0.85, -0.35, 1.25)
(-0.91, -0.32, 1.25)
(-0.96, -0.28, 1.24)
(-1.00, -0.22, 1.24)
(-1.02, -0.15, 1.24)
(-1.03, -0.06, 1.24)
(-1.02, 0.03, 1.24)
(-0.97, 0.18, 1.25)
(-0.92, 0.27, 1.26)
(-0.85, 0.33, 1.26)
(-0.76, 0.40, 1.26)
(-0.68, 0.43, 1.26)
(-0.61, 0.44, 1.26)
(-0.53, 0.43, 1.26)
(-0.46, 0.40, 1.26)
(-0.40, 0.36, 1.26)
(-0.33, 0.31, 1.26)
(-0.29, 0.26, 1.26)
(-0.23, 0.19, 1.27)
(-0.20, 0.14, 1.27)
(-0.17, 0.11, 1.27)
(-0.15, 0.07, 1.26)
(-0.12, 0.04, 1.26)
(-0.10, 0.00, 1.26)
(-0.07, -0.03, 1.27)
(-0.03, -0.07, 1.28)
(-0.01, -0.10, 1.28)
(0.06, -0.16, 1.29)
(0.11, -0.19, 1.29)
(0.16, -0.23, 1.29)
(0.23, -0.27, 1.29)
(0.29, -0.29, 1.29)
(0.34, -0.32, 1.28)
(0.40, -0.35, 1.28)
(0.44, -0.36, 1.29)
(0.52, -0.38, 1.29)
(0.58, -0.39, 1.30)
(0.65, -0.39, 1.30)
(0.72, -0.38, 1.30)
(0.79, -0.36, 1.30)
(0.85, -0.32, 1.29)
(0.90, -0.29, 1.29)
(0.94, -0.23, 1.29)
(0.97, -0.18, 1.29)
(0.99, -0.11, 1.30)
(1.00, -0.03, 1.31)
(0.97, 0.07, 1.31)
(0.94, 0.13, 1.31)
(0.90, 0.18, 1.31)
(0.82, 0.24, 1.31)
(0.75, 0.28, 1.31)
(0.67, 0.32, 1.31)
(0.61, 0.34, 1.32)
(0.53, 0.35, 1.32)
(0.46, 0.35, 1.33)
(0.38, 0.33, 1.33)
(0.33, 0.30, 1.33)
(0.28, 0.28, 1.34)
(0.22, 0.22, 1.34)
(0.19, 0.18, 1.35)
(0.16, 0.14, 1.35)
(0.14, 0.11, 1.35)
(0.11, 0.08, 1.35)
(0.08, 0.04, 1.36)
(0.06, -0.01, 1.37)
(0.03, -0.06, 1.36)
(0.00, -0.10, 1.36)
(-0.03, -0.14, 1.37)
(-0.06, -0.17, 1.37)
(-0.10, -0.20, 1.37)
(-0.15, -0.23, 1.36)
(-0.20, -0.26, 1.37)
(-0.26, -0.28, 1.37)
(-0.31, -0.30, 1.38)
(-0.38, -0.33, 1.38)
(-0.44, -0.34, 1.39)
(-0.53, -0.35, 1.39)
(-0.63, -0.36, 1.39)
(-0.70, -0.36, 1.39)
(-0.77, -0.36, 1.39)
(-0.83, -0.34, 1.39)
(-0.89, -0.31, 1.39)
(-0.94, -0.27, 1.40)
(-0.99, -0.22, 1.40)
(-1.01, -0.17, 1.40)
(-1.02, -0.10, 1.41)
(-1.00, 0.05, 1.42)
(-0.95, 0.18, 1.42)
(-0.90, 0.26, 1.43)
(-0.68, 0.44, 1.44)
(-0.48, 0.46, 1.45)
(-0.32, 0.40, 1.45)
(-0.25, 0.34, 1.46)
(-0.19, 0.28, 1.46)
(-0.15, 0.22, 1.46)
(-0.12, 0.16, 1.46)
(-0.08, 0.08, 1.45)
(-0.06, 0.03, 1.45)
(-0.05, -0.03, 1.45)
(-0.04, -0.08, 1.44)
(-0.02, -0.12, 1.44)
(-0.01, -0.16, 1.44)
(0.02, -0.18, 1.44)
(0.04, -0.20, 1.44)
(0.08, -0.22, 1.44)
(0.12, -0.23, 1.44)
(0.16, -0.25, 1.44)
(0.21, -0.26, 1.45)
(0.28, -0.27, 1.45)
(0.34, -0.28, 1.45)
(0.41, -0.30, 1.45)
(0.48, -0.32, 1.46)
(0.56, -0.34, 1.46)
(0.66, -0.36, 1.47)
(0.74, -0.36, 1.47)
(0.80, -0.34, 1.48)
(0.86, -0.32, 1.49)
(0.94, -0.26, 1.49)
(0.97, -0.22, 1.48)
(1.01, -0.15, 1.48)
(1.02, -0.08, 1.47)
(1.02, -0.02, 1.47)
(1.00, 0.06, 1.47)
(0.97, 0.13, 1.47)
(0.91, 0.20, 1.47)
(0.85, 0.26, 1.46)
(0.79, 0.30, 1.46)
(0.73, 0.33, 1.46)
(0.61, 0.34, 1.47)
(0.55, 0.34, 1.48)
(0.48, 0.33, 1.49)
(0.41, 0.31, 1.50)
(0.34, 0.29, 1.50)
(0.27, 0.25, 1.51)
(0.23, 0.22, 1.50)
(0.19, 0.18, 1.50)
(0.15, 0.14, 1.50)
(0.12, 0.10, 1.51)
(0.09, 0.06, 1.52)
(0.06, 0.03, 1.53)
(0.03, -0.00, 1.53)
(-0.00, -0.06, 1.54)
(-0.03, -0.09, 1.55)
(-0.07, -0.15, 1.55)
(-0.11, -0.18, 1.56)
(-0.15, -0.22, 1.56)
(-0.20, -0.24, 1.56)
(-0.25, -0.27, 1.56)
(-0.31, -0.30, 1.55)
(-0.36, -0.31, 1.55)
(-0.42, -0.33, 1.56)
(-0.48, -0.34, 1.56)
(-0.54, -0.35, 1.57)
(-0.59, -0.35, 1.57)
(-0.65, -0.34, 1.57)
(-0.71, -0.33, 1.57)
(-0.76, -0.31, 1.57)
(-0.83, -0.28, 1.57)
(-0.88, -0.25, 1.57)
(-0.93, -0.19, 1.57)
(-0.96, -0.12, 1.57)
(-0.98, -0.05, 1.57)
(-0.98, 0.03, 1.57)
(-0.97, 0.10, 1.57)
(-0.95, 0.18, 1.58)
(-0.91, 0.24, 1.58)
(-0.86, 0.29, 1.58)
(-0.80, 0.34, 1.57)
(-0.73, 0.38, 1.57)
(-0.66, 0.40, 1.56)
(-0.60, 0.41, 1.56)
(-0.54, 0.41, 1.57)
(-0.48, 0.40, 1.58)
(-0.41, 0.37, 1.59)
(-0.31, 0.30, 1.60)
(-0.25, 0.26, 1.61)
(-0.21, 0.22, 1.62)
(-0.16, 0.18, 1.49)
(-0.11, 0.15, 1.28)
(-0.07, 0.11, 1.03)
(-0.04, 0.08, 0.78)
(-0.02, 0.05, 0.57)
(-0.01, 0.03, 0.41)
(-0.01, 0.01, 0.28)
(-0.01, -0.00, 0.14)
(-0.04, -0.02, 0.01)
};
%

==> plots/kaist_traj_coords/infinite_head_gt.tex <==
\addplot3[
    fill=none,draw = clr1,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, 0.00)
(-0.03, 0.00, 0.00)
(-0.03, 0.00, 0.00)
(-0.03, 0.00, 0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.03, 0.00, -0.00)
(-0.02, 0.00, -0.00)
(-0.02, 0.00, 0.00)
(-0.02, 0.00, 0.01)
(-0.02, 0.00, 0.02)
(-0.03, 0.00, 0.02)
(-0.03, 0.00, 0.02)
(-0.03, 0.00, 0.02)
(-0.03, 0.00, 0.03)
(-0.04, -0.00, 0.03)
(-0.03, -0.00, 0.03)
(-0.03, -0.00, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.00, 0.03)
(-0.03, -0.00, 0.03)
(-0.03, -0.00, 0.03)
(-0.03, -0.00, 0.03)
(-0.03, -0.01, 0.03)
(-0.04, -0.01, 0.03)
(-0.04, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.05)
(-0.03, -0.01, 0.07)
(-0.03, -0.01, 0.09)
(-0.03, -0.01, 0.08)
(-0.03, -0.01, 0.07)
(-0.03, -0.01, 0.06)
(-0.03, -0.01, 0.05)
(-0.03, -0.01, 0.05)
(-0.03, -0.01, 0.06)
(-0.03, -0.00, 0.08)
(-0.03, -0.01, 0.09)
(-0.03, -0.00, 0.10)
(-0.02, -0.00, 0.06)
(-0.01, -0.00, 0.00)
(-0.01, 0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.02, 0.00, 0.00)
(-0.05, 0.02, 0.04)
(-0.09, 0.04, 0.14)
(-0.14, 0.07, 0.22)
(-0.17, 0.10, 0.25)
(-0.20, 0.12, 0.28)
(-0.21, 0.13, 0.30)
(-0.21, 0.13, 0.32)
(-0.21, 0.12, 0.33)
(-0.20, 0.12, 0.35)
(-0.18, 0.10, 0.36)
(-0.17, 0.09, 0.38)
(-0.15, 0.07, 0.39)
(-0.14, 0.06, 0.41)
(-0.13, 0.05, 0.42)
(-0.12, 0.04, 0.43)
(-0.11, 0.04, 0.43)
(-0.10, 0.04, 0.43)
(-0.09, 0.04, 0.43)
(-0.08, 0.04, 0.43)
(-0.08, 0.04, 0.43)
(-0.07, 0.05, 0.43)
(-0.07, 0.05, 0.44)
(-0.07, 0.06, 0.44)
(-0.07, 0.06, 0.45)
(-0.06, 0.06, 0.46)
(-0.05, 0.05, 0.47)
(-0.02, 0.05, 0.47)
(0.06, 0.03, 0.47)
(0.13, 0.02, 0.48)
(0.26, 0.01, 0.48)
(0.36, 0.01, 0.48)
(0.46, 0.01, 0.48)
(0.59, 0.01, 0.49)
(0.75, 0.01, 0.49)
(0.94, 0.01, 0.49)
(1.09, 0.02, 0.50)
(1.23, 0.02, 0.50)
(1.33, 0.03, 0.51)
(1.40, 0.02, 0.51)
(1.44, 0.02, 0.50)
(1.45, 0.03, 0.50)
(1.45, 0.06, 0.49)
(1.43, 0.11, 0.49)
(1.41, 0.19, 0.49)
(1.39, 0.29, 0.49)
(1.37, 0.41, 0.50)
(1.35, 0.54, 0.50)
(1.34, 0.68, 0.51)
(1.34, 0.83, 0.51)
(1.34, 1.00, 0.52)
(1.34, 1.15, 0.53)
(1.35, 1.29, 0.53)
(1.36, 1.40, 0.54)
(1.37, 1.46, 0.53)
(1.37, 1.51, 0.53)
(1.35, 1.53, 0.53)
(1.32, 1.53, 0.53)
(1.25, 1.52, 0.53)
(1.17, 1.49, 0.52)
(1.07, 1.46, 0.52)
(0.95, 1.41, 0.52)
(0.79, 1.35, 0.52)
(0.63, 1.31, 0.52)
(0.50, 1.28, 0.53)
(0.19, 1.29, 0.54)
(0.07, 1.32, 0.55)
(-0.01, 1.35, 0.55)
(-0.07, 1.38, 0.55)
(-0.10, 1.40, 0.55)
(-0.10, 1.39, 0.55)
(-0.08, 1.36, 0.54)
(-0.05, 1.30, 0.52)
(-0.02, 1.22, 0.51)
(0.01, 1.11, 0.50)
(0.04, 0.96, 0.50)
(0.05, 0.79, 0.50)
(0.06, 0.56, 0.51)
(0.02, 0.02, 0.49)
(-0.05, -0.19, 0.49)
(-0.04, -0.23, 0.49)
(0.00, -0.23, 0.50)
(0.07, -0.22, 0.50)
(0.15, -0.19, 0.50)
(0.26, -0.15, 0.50)
(0.41, -0.11, 0.51)
(0.55, -0.08, 0.53)
(0.74, -0.05, 0.54)
(0.95, -0.02, 0.54)
(1.11, 0.00, 0.54)
(1.25, 0.03, 0.53)
(1.36, 0.04, 0.53)
(1.45, 0.04, 0.53)
(1.50, 0.04, 0.52)
(1.53, 0.04, 0.51)
(1.53, 0.05, 0.51)
(1.52, 0.08, 0.51)
(1.50, 0.14, 0.51)
(1.42, 0.35, 0.52)
(1.36, 0.56, 0.52)
(1.31, 0.88, 0.53)
(1.29, 1.17, 0.52)
(1.34, 1.56, 0.51)
(1.34, 1.61, 0.51)
(1.30, 1.60, 0.51)
(1.24, 1.57, 0.51)
(1.15, 1.54, 0.51)
(1.05, 1.49, 0.51)
(0.94, 1.43, 0.51)
(0.81, 1.37, 0.52)
(0.66, 1.32, 0.52)
(0.51, 1.29, 0.52)
(0.35, 1.28, 0.53)
(0.22, 1.27, 0.53)
(0.10, 1.28, 0.52)
(0.00, 1.30, 0.52)
(-0.06, 1.32, 0.53)
(-0.09, 1.33, 0.53)
(-0.10, 1.33, 0.53)
(-0.09, 1.31, 0.53)
(-0.06, 1.26, 0.53)
(-0.03, 1.18, 0.53)
(0.00, 1.08, 0.52)
(0.03, 0.98, 0.52)
(0.05, 0.84, 0.51)
(0.05, 0.69, 0.51)
(0.05, 0.49, 0.51)
(0.04, 0.33, 0.51)
(0.03, 0.18, 0.51)
(0.01, 0.04, 0.50)
(-0.02, -0.06, 0.50)
(-0.04, -0.13, 0.50)
(-0.07, -0.16, 0.51)
(-0.08, -0.17, 0.52)
(-0.09, -0.17, 0.53)
(-0.09, -0.15, 0.55)
(-0.09, -0.13, 0.57)
(-0.08, -0.11, 0.59)
(-0.06, -0.08, 0.62)
(-0.04, -0.05, 0.65)
(-0.02, -0.03, 0.70)
(-0.01, -0.02, 0.75)
(0.00, -0.02, 0.81)
(0.01, -0.03, 0.87)
(0.02, -0.04, 0.95)
(0.02, -0.05, 1.00)
(0.02, -0.06, 1.02)
(0.04, -0.06, 1.03)
(0.08, -0.06, 1.04)
(0.13, -0.06, 1.04)
(0.19, -0.05, 1.03)
(0.29, -0.04, 1.03)
(0.38, -0.03, 1.02)
(0.49, -0.02, 1.02)
(0.63, -0.02, 1.03)
(0.79, -0.02, 1.03)
(0.98, -0.02, 1.03)
(1.12, -0.03, 1.04)
(1.25, -0.04, 1.04)
(1.36, -0.05, 1.04)
(1.43, -0.06, 1.04)
(1.48, -0.06, 1.04)
(1.50, -0.04, 1.05)
(1.50, 0.00, 1.04)
(1.49, 0.05, 1.03)
(1.46, 0.15, 1.02)
(1.43, 0.26, 1.01)
(1.40, 0.40, 1.01)
(1.38, 0.54, 1.01)
(1.36, 0.71, 1.00)
(1.34, 0.85, 1.00)
(1.33, 1.03, 1.00)
(1.33, 1.18, 1.01)
(1.35, 1.31, 1.01)
(1.36, 1.40, 1.02)
(1.38, 1.46, 1.02)
(1.37, 1.49, 1.03)
(1.34, 1.49, 1.03)
(1.27, 1.48, 1.03)
(1.17, 1.45, 1.03)
(1.05, 1.42, 1.04)
(0.91, 1.38, 1.04)
(0.78, 1.36, 1.04)
(0.65, 1.33, 1.03)
(0.49, 1.31, 1.02)
(0.34, 1.29, 1.01)
(0.22, 1.29, 1.01)
(0.03, 1.33, 1.00)
(-0.05, 1.36, 1.02)
(-0.05, 1.31, 1.02)
(-0.01, 1.09, 1.03)
(0.03, 0.81, 1.02)
(0.03, 0.55, 1.01)
(0.01, -0.05, 1.01)
(-0.01, -0.22, 1.00)
(0.01, -0.28, 1.00)
(0.04, -0.28, 1.00)
(0.09, -0.26, 1.00)
(0.17, -0.21, 1.00)
(0.26, -0.16, 1.01)
(0.39, -0.10, 1.02)
(0.51, -0.05, 1.02)
(0.65, -0.02, 1.03)
(0.82, -0.00, 1.03)
(1.01, 0.01, 1.03)
(1.21, 0.01, 1.03)
(1.36, -0.01, 1.02)
(1.48, -0.03, 1.01)
(1.53, -0.04, 1.01)
(1.55, -0.03, 1.01)
(1.54, 0.00, 1.01)
(1.52, 0.07, 1.01)
(1.49, 0.16, 1.01)
(1.45, 0.26, 1.01)
(1.41, 0.40, 1.02)
(1.38, 0.54, 1.02)
(1.36, 0.69, 1.02)
(1.34, 0.93, 1.02)
(1.33, 1.09, 1.01)
(1.33, 1.26, 1.01)
(1.34, 1.40, 1.00)
(1.34, 1.48, 1.00)
(1.34, 1.52, 1.00)
(1.32, 1.54, 1.00)
(1.29, 1.54, 1.00)
(1.23, 1.52, 1.00)
(1.14, 1.48, 1.00)
(1.05, 1.44, 1.00)
(0.93, 1.39, 1.00)
(0.81, 1.35, 1.01)
(0.69, 1.31, 1.01)
(0.53, 1.28, 1.01)
(0.38, 1.27, 1.01)
(0.24, 1.28, 1.01)
(0.12, 1.29, 1.02)
(0.03, 1.31, 1.02)
(-0.04, 1.32, 1.02)
(-0.09, 1.33, 1.03)
(-0.11, 1.33, 1.04)
(-0.12, 1.31, 1.06)
(-0.10, 1.27, 1.06)
(-0.07, 1.19, 1.06)
(-0.03, 1.10, 1.05)
(-0.00, 0.99, 1.04)
(0.03, 0.87, 1.03)
(0.05, 0.72, 1.02)
(0.06, 0.56, 1.01)
(0.05, 0.39, 1.00)
(0.04, 0.23, 0.99)
(0.03, 0.10, 0.98)
(0.00, -0.01, 0.98)
(-0.03, -0.09, 0.97)
(-0.05, -0.13, 0.98)
(-0.07, -0.15, 0.99)
(-0.07, -0.15, 0.99)
(-0.08, -0.14, 1.00)
(-0.07, -0.10, 1.02)
(-0.06, -0.07, 1.05)
(-0.05, -0.04, 1.08)
(-0.03, -0.00, 1.14)
(-0.01, 0.01, 1.19)
(-0.00, 0.01, 1.24)
(0.02, 0.01, 1.30)
(0.03, -0.00, 1.36)
(0.04, -0.01, 1.43)
(0.05, -0.03, 1.50)
(0.06, -0.05, 1.51)
(0.08, -0.07, 1.51)
(0.12, -0.09, 1.50)
(0.17, -0.10, 1.50)
(0.23, -0.11, 1.50)
(0.31, -0.11, 1.50)
(0.39, -0.10, 1.51)
(0.48, -0.09, 1.51)
(0.59, -0.08, 1.52)
(0.74, -0.06, 1.52)
(0.89, -0.04, 1.52)
(1.06, -0.02, 1.52)
(1.19, -0.01, 1.51)
(1.31, -0.02, 1.51)
(1.40, -0.03, 1.52)
(1.48, -0.04, 1.52)
(1.51, -0.02, 1.52)
(1.52, 0.02, 1.52)
(1.51, 0.09, 1.53)
(1.49, 0.19, 1.53)
(1.46, 0.30, 1.53)
(1.41, 0.46, 1.53)
(1.38, 0.63, 1.52)
(1.36, 0.79, 1.52)
(1.34, 0.95, 1.51)
(1.33, 1.11, 1.51)
(1.33, 1.24, 1.50)
(1.34, 1.36, 1.50)
(1.35, 1.43, 1.50)
(1.35, 1.46, 1.50)
(1.35, 1.47, 1.50)
(1.32, 1.47, 1.50)
(1.27, 1.45, 1.50)
(1.19, 1.42, 1.50)
(1.10, 1.39, 1.51)
(0.93, 1.34, 1.51)
(0.82, 1.31, 1.51)
(0.58, 1.28, 1.50)
(0.39, 1.27, 1.50)
(0.21, 1.28, 1.50)
(0.04, 1.30, 1.51)
(-0.06, 1.33, 1.51)
(-0.12, 1.36, 1.51)
(-0.14, 1.36, 1.52)
(-0.14, 1.35, 1.52)
(-0.03, 1.16, 1.52)
(0.09, 0.64, 1.50)
(0.05, -0.21, 1.50)
(0.02, -0.41, 1.50)
(0.05, -0.40, 1.50)
(0.11, -0.35, 1.49)
(0.19, -0.29, 1.48)
(0.28, -0.21, 1.47)
(0.39, -0.13, 1.46)
(0.50, -0.05, 1.47)
(0.65, 0.01, 1.49)
(0.83, 0.06, 1.51)
(1.00, 0.08, 1.51)
(1.16, 0.10, 1.52)
(1.28, 0.10, 1.52)
(1.39, 0.08, 1.52)
(1.47, 0.05, 1.52)
(1.52, 0.01, 1.52)
(1.54, -0.00, 1.52)
(1.54, 0.01, 1.51)
(1.52, 0.05, 1.51)
(1.49, 0.11, 1.51)
(1.46, 0.19, 1.52)
(1.41, 0.34, 1.52)
(1.36, 0.56, 1.52)
(1.33, 0.75, 1.52)
(1.32, 0.91, 1.51)
(1.32, 1.16, 1.50)
(1.33, 1.33, 1.49)
(1.36, 1.45, 1.48)
(1.38, 1.52, 1.47)
(1.38, 1.54, 1.47)
(1.36, 1.53, 1.47)
(1.31, 1.51, 1.47)
(1.23, 1.49, 1.48)
(1.13, 1.46, 1.48)
(1.01, 1.43, 1.49)
(0.84, 1.39, 1.50)
(0.69, 1.36, 1.50)
(0.40, 1.33, 1.51)
(0.24, 1.32, 1.51)
(0.13, 1.32, 1.51)
(0.03, 1.33, 1.51)
(-0.06, 1.34, 1.50)
(-0.10, 1.35, 1.50)
(-0.12, 1.35, 1.49)
(-0.11, 1.32, 1.49)
(-0.08, 1.27, 1.50)
(-0.05, 1.18, 1.50)
(0.01, 0.99, 1.50)
(0.06, 0.75, 1.50)
(0.07, 0.59, 1.49)
(0.07, 0.41, 1.49)
(0.06, 0.23, 1.49)
(0.04, 0.05, 1.49)
(0.02, -0.07, 1.47)
(0.01, -0.15, 1.24)
(-0.01, -0.20, 0.81)
(-0.03, -0.19, 0.53)
(-0.04, -0.15, 0.33)
(-0.05, -0.11, 0.20)
(-0.05, -0.07, 0.15)
(-0.06, -0.02, 0.13)
(-0.05, 0.01, 0.13)
(-0.04, 0.03, 0.12)
(-0.03, 0.03, 0.12)
(-0.04, 0.02, -0.00)
};
%

==> plots/kaist_traj_coords/infinite_head_jetson_slam.tex <==
%
\addplot3[
    fill=none,draw = clr2,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(-0.03, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.03, -0.00, -0.01)
(-0.03, 0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.03, -0.01, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.03, -0.00, -0.00)
(-0.02, -0.01, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.02, -0.01, -0.00)
(-0.02, -0.01, -0.01)
(-0.02, -0.00, -0.00)
(-0.03, -0.01, 0.01)
(-0.03, -0.01, 0.01)
(-0.03, -0.01, 0.01)
(-0.03, -0.01, 0.01)
(-0.04, 0.00, 0.02)
(-0.03, -0.01, 0.02)
(-0.03, -0.01, 0.01)
(-0.03, 0.01, 0.03)
(-0.03, 0.02, 0.02)
(-0.03, 0.00, 0.03)
(-0.03, 0.00, 0.03)
(-0.04, 0.00, 0.02)
(-0.04, 0.01, 0.03)
(-0.03, -0.02, 0.03)
(-0.03, -0.02, 0.02)
(-0.03, -0.02, 0.02)
(-0.03, -0.03, 0.03)
(-0.04, -0.02, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.03)
(-0.03, 0.00, 0.05)
(-0.04, 0.02, 0.04)
(-0.03, -0.00, 0.03)
(-0.03, -0.00, 0.03)
(-0.02, -0.01, 0.03)
(-0.03, -0.00, 0.03)
(-0.04, -0.02, 0.04)
(-0.03, 0.00, 0.04)
(-0.03, -0.01, 0.03)
(-0.03, -0.01, 0.05)
(-0.03, -0.01, 0.06)
(-0.02, -0.01, 0.07)
(-0.02, -0.02, 0.07)
(-0.02, -0.01, 0.06)
(-0.03, 0.01, 0.05)
(-0.03, -0.01, 0.05)
(-0.03, -0.01, 0.05)
(-0.02, -0.01, 0.07)
(-0.02, -0.01, 0.08)
(-0.02, -0.00, 0.10)
(-0.02, 0.00, 0.11)
(-0.02, -0.00, 0.07)
(-0.01, -0.00, 0.04)
(-0.00, -0.01, 0.02)
(-0.01, -0.00, 0.01)
(-0.01, -0.00, 0.01)
(-0.01, -0.00, 0.00)
(-0.01, -0.01, -0.00)
(-0.01, -0.01, 0.00)
(-0.01, -0.00, 0.00)
(-0.01, -0.00, 0.00)
(-0.01, -0.00, 0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.01, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, 0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.01, -0.00)
(-0.01, -0.00, 0.00)
(-0.01, -0.00, 0.00)
(-0.02, -0.00, 0.00)
(-0.01, -0.00, -0.00)
(-0.02, 0.00, -0.00)
(-0.02, 0.00, 0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, -0.00)
(-0.02, -0.00, -0.00)
(-0.01, 0.00, 0.00)
(-0.02, 0.00, 0.00)
(-0.02, 0.00, 0.00)
(-0.02, 0.00, 0.00)
(-0.01, -0.00, 0.01)
(-0.02, -0.00, -0.00)
(-0.01, 0.00, 0.00)
(-0.02, 0.00, 0.00)
(-0.02, 0.00, 0.00)
(-0.01, -0.01, 0.00)
(-0.02, 0.00, 0.01)
(-0.01, 0.00, -0.00)
(-0.01, 0.00, -0.00)
(-0.01, -0.01, 0.01)
(-0.01, 0.00, 0.01)
(-0.02, 0.00, 0.00)
(-0.01, 0.00, 0.00)
(-0.01, 0.00, 0.00)
(-0.01, 0.00, 0.00)
(-0.01, 0.00, 0.00)
(-0.01, -0.00, 0.01)
(-0.02, -0.00, 0.00)
(-0.02, 0.00, -0.00)
(-0.01, 0.00, -0.00)
(-0.02, 0.01, 0.00)
(-0.01, 0.00, -0.00)
(-0.02, 0.00, 0.00)
(-0.01, -0.00, -0.00)
(-0.01, -0.00, 0.00)
(-0.02, 0.00, 0.00)
(-0.01, 0.00, -0.00)
(-0.01, -0.00, 0.00)
(-0.01, -0.00, 0.00)
(-0.01, -0.00, 0.00)
(-0.01, -0.00, -0.00)
(-0.02, -0.00, 0.00)
(-0.02, 0.01, -0.00)
(-0.01, 0.00, 0.00)
(-0.01, -0.00, 0.00)
(-0.02, 0.00, 0.00)
(-0.02, 0.00, 0.00)
(-0.01, -0.01, 0.00)
(-0.02, 0.00, 0.00)
(-0.02, 0.00, 0.00)
(-0.01, -0.01, 0.00)
(-0.02, -0.00, 0.01)
(-0.04, -0.00, 0.03)
(-0.08, 0.04, 0.14)
(-0.13, 0.07, 0.20)
(-0.18, 0.11, 0.25)
(-0.20, 0.12, 0.28)
(-0.21, 0.13, 0.30)
(-0.21, 0.13, 0.32)
(-0.21, 0.12, 0.33)
(-0.20, 0.12, 0.35)
(-0.18, 0.09, 0.36)
(-0.16, 0.08, 0.38)
(-0.15, 0.04, 0.41)
(-0.13, 0.04, 0.42)
(-0.12, 0.04, 0.43)
(-0.11, 0.03, 0.43)
(-0.10, 0.03, 0.43)
(-0.10, 0.04, 0.43)
(-0.08, 0.03, 0.43)
(-0.08, 0.04, 0.44)
(-0.07, 0.05, 0.44)
(-0.07, 0.05, 0.44)
(-0.07, 0.05, 0.45)
(-0.07, 0.05, 0.46)
(-0.06, 0.05, 0.47)
(-0.02, 0.05, 0.47)
(0.03, 0.03, 0.47)
(0.10, 0.03, 0.46)
(0.19, 0.03, 0.47)
(0.30, 0.02, 0.47)
(0.41, 0.01, 0.48)
(0.53, 0.01, 0.48)
(0.68, 0.02, 0.49)
(0.87, 0.01, 0.49)
(1.05, 0.03, 0.49)
(1.21, 0.03, 0.51)
(1.32, 0.04, 0.51)
(1.40, 0.04, 0.51)
(1.43, 0.04, 0.51)
(1.45, 0.04, 0.50)
(1.45, 0.08, 0.50)
(1.43, 0.14, 0.49)
(1.40, 0.24, 0.49)
(1.37, 0.37, 0.49)
(1.36, 0.51, 0.49)
(1.34, 0.66, 0.50)
(1.34, 0.84, 0.51)
(1.34, 1.01, 0.51)
(1.34, 1.19, 0.52)
(1.36, 1.32, 0.53)
(1.37, 1.42, 0.53)
(1.37, 1.50, 0.54)
(1.36, 1.52, 0.53)
(1.33, 1.54, 0.53)
(1.26, 1.52, 0.53)
(1.17, 1.50, 0.53)
(1.05, 1.45, 0.53)
(0.91, 1.40, 0.52)
(0.78, 1.34, 0.53)
(0.62, 1.31, 0.53)
(0.46, 1.26, 0.53)
(0.28, 1.26, 0.53)
(0.14, 1.28, 0.54)
(0.03, 1.31, 0.54)
(-0.06, 1.34, 0.55)
(-0.10, 1.37, 0.55)
(-0.11, 1.36, 0.56)
(-0.08, 1.34, 0.55)
(-0.05, 1.30, 0.53)
(-0.02, 1.21, 0.52)
(0.02, 1.11, 0.50)
(0.04, 0.95, 0.50)
(0.06, 0.76, 0.50)
(0.08, 0.55, 0.50)
(0.06, 0.35, 0.50)
(0.05, 0.16, 0.50)
(0.01, 0.02, 0.49)
(-0.02, -0.09, 0.49)
(-0.05, -0.17, 0.49)
(-0.06, -0.21, 0.50)
(-0.03, -0.23, 0.49)
(0.01, -0.22, 0.50)
(0.10, -0.21, 0.50)
(0.20, -0.17, 0.49)
(0.32, -0.13, 0.51)
(0.46, -0.10, 0.51)
(0.64, -0.06, 0.53)
(0.86, -0.03, 0.54)
(1.07, 0.00, 0.54)
(1.24, 0.04, 0.54)
(1.37, 0.06, 0.53)
(1.45, 0.06, 0.53)
(1.51, 0.05, 0.52)
(1.53, 0.05, 0.51)
(1.53, 0.07, 0.51)
(1.52, 0.12, 0.51)
(1.48, 0.20, 0.52)
(1.44, 0.31, 0.52)
(1.39, 0.44, 0.52)
(1.35, 0.60, 0.52)
(1.32, 0.78, 0.52)
(1.29, 0.99, 0.52)
(1.28, 1.18, 0.52)
(1.29, 1.35, 0.51)
(1.31, 1.48, 0.51)
(1.35, 1.56, 0.51)
(1.35, 1.61, 0.51)
(1.34, 1.62, 0.51)
(1.30, 1.60, 0.51)
(1.23, 1.57, 0.50)
(1.12, 1.53, 0.51)
(1.00, 1.47, 0.52)
(0.86, 1.39, 0.51)
(0.70, 1.33, 0.53)
(0.52, 1.29, 0.53)
(0.35, 1.26, 0.52)
(0.19, 1.26, 0.53)
(0.06, 1.27, 0.52)
(-0.03, 1.28, 0.53)
(-0.08, 1.31, 0.53)
(-0.10, 1.32, 0.53)
(-0.10, 1.29, 0.53)
(-0.08, 1.27, 0.54)
(-0.04, 1.19, 0.53)
(0.01, 1.08, 0.52)
(0.04, 0.94, 0.51)
(0.05, 0.81, 0.51)
(0.05, 0.67, 0.51)
(0.06, 0.48, 0.51)
(0.05, 0.31, 0.50)
(0.02, 0.11, 0.51)
(-0.00, -0.02, 0.50)
(-0.03, -0.11, 0.50)
(-0.06, -0.16, 0.50)
(-0.08, -0.17, 0.52)
(-0.09, -0.17, 0.53)
(-0.09, -0.16, 0.56)
(-0.08, -0.14, 0.57)
(-0.07, -0.11, 0.59)
(-0.05, -0.08, 0.63)
(-0.03, -0.05, 0.67)
(-0.01, -0.03, 0.73)
(0.00, -0.03, 0.79)
(0.01, -0.03, 0.87)
(0.02, -0.04, 0.94)
(0.02, -0.06, 1.00)
(0.03, -0.06, 1.02)
(0.05, -0.07, 1.03)
(0.10, -0.06, 1.03)
(0.16, -0.06, 1.03)
(0.24, -0.04, 1.03)
(0.34, -0.03, 1.03)
(0.46, -0.02, 1.02)
(0.58, -0.01, 1.02)
(0.75, -0.02, 1.03)
(0.95, -0.01, 1.03)
(1.11, -0.02, 1.04)
(1.27, -0.03, 1.03)
(1.37, -0.04, 1.03)
(1.46, -0.06, 1.04)
(1.50, -0.05, 1.04)
(1.51, -0.03, 1.04)
(1.50, 0.02, 1.03)
(1.48, 0.11, 1.02)
(1.45, 0.22, 1.01)
(1.42, 0.35, 1.00)
(1.39, 0.52, 1.01)
(1.36, 0.69, 1.01)
(1.34, 0.87, 1.00)
(1.33, 1.05, 1.00)
(1.33, 1.22, 1.01)
(1.35, 1.35, 1.01)
(1.37, 1.43, 1.01)
(1.38, 1.48, 1.02)
(1.38, 1.50, 1.03)
(1.33, 1.50, 1.03)
(1.25, 1.47, 1.03)
(1.14, 1.44, 1.04)
(1.02, 1.41, 1.04)
(0.87, 1.38, 1.04)
(0.72, 1.34, 1.04)
(0.55, 1.31, 1.04)
(0.38, 1.30, 1.02)
(0.24, 1.28, 1.01)
(0.11, 1.29, 1.02)
(0.03, 1.31, 1.01)
(-0.02, 1.34, 1.02)
(-0.04, 1.35, 1.03)
(-0.05, 1.35, 1.03)
(-0.05, 1.31, 1.03)
(-0.03, 1.21, 1.04)
(-0.01, 1.12, 1.04)
(0.02, 0.98, 1.03)
(0.02, 0.84, 1.02)
(0.03, 0.65, 1.01)
(0.03, 0.46, 1.02)
(0.04, 0.24, 1.01)
(0.02, 0.05, 1.03)
(-0.00, -0.09, 1.03)
(-0.00, -0.19, 1.02)
(-0.01, -0.25, 1.01)
(0.02, -0.28, 1.00)
(0.06, -0.28, 1.00)
(0.12, -0.25, 1.01)
(0.20, -0.20, 1.00)
(0.31, -0.15, 1.01)
(0.42, -0.07, 1.01)
(0.56, -0.03, 1.01)
(0.74, -0.00, 1.05)
(0.95, 0.02, 1.04)
(1.15, 0.02, 1.03)
(1.30, 0.01, 1.03)
(1.42, -0.01, 1.02)
(1.50, -0.03, 1.00)
(1.54, -0.03, 1.01)
(1.55, -0.02, 1.01)
(1.54, 0.04, 1.01)
(1.50, 0.13, 1.02)
(1.46, 0.24, 1.01)
(1.42, 0.39, 1.01)
(1.38, 0.54, 1.02)
(1.35, 0.72, 1.02)
(1.33, 0.93, 1.01)
(1.33, 1.11, 1.01)
(1.33, 1.28, 1.01)
(1.33, 1.41, 1.00)
(1.34, 1.49, 1.00)
(1.34, 1.53, 1.01)
(1.32, 1.55, 1.01)
(1.27, 1.55, 1.01)
(1.20, 1.51, 1.02)
(1.10, 1.46, 1.00)
(0.98, 1.41, 1.01)
(0.84, 1.35, 1.01)
(0.69, 1.31, 1.02)
(0.53, 1.26, 1.02)
(0.35, 1.26, 1.01)
(0.21, 1.27, 1.01)
(0.08, 1.30, 1.02)
(-0.01, 1.31, 1.02)
(-0.08, 1.32, 1.03)
(-0.11, 1.33, 1.04)
(-0.12, 1.32, 1.05)
(-0.11, 1.29, 1.06)
(-0.08, 1.21, 1.06)
(-0.04, 1.10, 1.06)
(0.01, 0.98, 1.04)
(0.04, 0.84, 1.03)
(0.05, 0.68, 1.02)
(0.06, 0.49, 1.02)
(0.06, 0.29, 1.00)
(0.02, 0.13, 1.00)
(0.01, 0.01, 0.98)
(-0.02, -0.08, 0.99)
(-0.03, -0.14, 0.98)
(-0.07, -0.16, 1.00)
(-0.07, -0.17, 1.00)
(-0.07, -0.14, 1.02)
(-0.06, -0.10, 1.04)
(-0.06, -0.06, 1.08)
(-0.05, -0.01, 1.10)
(-0.03, 0.01, 1.16)
(-0.01, 0.01, 1.19)
(0.01, 0.01, 1.25)
(0.03, 0.01, 1.32)
(0.04, -0.01, 1.40)
(0.04, -0.03, 1.46)
(0.06, -0.05, 1.48)
(0.07, -0.06, 1.47)
(0.11, -0.07, 1.47)
(0.17, -0.10, 1.46)
(0.24, -0.09, 1.46)
(0.33, -0.09, 1.49)
(0.43, -0.09, 1.50)
(0.54, -0.08, 1.50)
(0.68, -0.05, 1.50)
(0.87, -0.03, 1.52)
(1.04, -0.01, 1.51)
(1.20, 0.00, 1.50)
(1.31, 0.00, 1.51)
(1.42, -0.02, 1.52)
(1.47, -0.02, 1.53)
(1.51, -0.00, 1.51)
(1.53, 0.04, 1.53)
(1.52, 0.11, 1.53)
(1.49, 0.21, 1.54)
(1.44, 0.34, 1.52)
(1.41, 0.49, 1.50)
(1.38, 0.64, 1.52)
(1.35, 0.81, 1.51)
(1.33, 1.01, 1.50)
(1.33, 1.18, 1.49)
(1.33, 1.32, 1.49)
(1.34, 1.42, 1.50)
(1.35, 1.47, 1.51)
(1.35, 1.49, 1.52)
(1.33, 1.47, 1.50)
(1.27, 1.47, 1.50)
(1.19, 1.44, 1.51)
(1.08, 1.40, 1.51)
(0.96, 1.35, 1.51)
(0.79, 1.31, 1.52)
(0.62, 1.26, 1.50)
(0.42, 1.27, 1.50)
(0.23, 1.26, 1.50)
(0.07, 1.28, 1.52)
(-0.05, 1.31, 1.53)
(-0.11, 1.36, 1.51)
(-0.15, 1.36, 1.52)
(-0.14, 1.34, 1.53)
(-0.11, 1.30, 1.52)
(-0.07, 1.24, 1.52)
(-0.01, 1.12, 1.51)
(0.03, 0.99, 1.52)
(0.07, 0.86, 1.51)
(0.10, 0.65, 1.49)
(0.10, 0.43, 1.50)
(0.10, 0.20, 1.49)
(0.10, 0.01, 1.50)
(0.08, -0.14, 1.49)
(0.05, -0.26, 1.49)
(0.02, -0.32, 1.48)
(0.02, -0.40, 1.50)
(0.03, -0.40, 1.49)
(0.08, -0.38, 1.49)
(0.16, -0.32, 1.47)
(0.25, -0.23, 1.47)
(0.36, -0.14, 1.45)
(0.49, -0.05, 1.46)
(0.66, 0.02, 1.49)
(0.86, 0.07, 1.50)
(1.05, 0.11, 1.51)
(1.22, 0.12, 1.52)
(1.35, 0.11, 1.51)
(1.44, 0.09, 1.52)
(1.50, 0.04, 1.52)
(1.54, 0.01, 1.53)
(1.53, 0.02, 1.52)
(1.52, 0.06, 1.51)
(1.48, 0.13, 1.51)
(1.45, 0.23, 1.52)
(1.41, 0.35, 1.52)
(1.37, 0.50, 1.52)
(1.34, 0.67, 1.52)
(1.32, 0.87, 1.51)
(1.31, 1.07, 1.49)
(1.32, 1.25, 1.50)
(1.34, 1.39, 1.48)
(1.36, 1.50, 1.47)
(1.38, 1.55, 1.48)
(1.37, 1.55, 1.47)
(1.33, 1.53, 1.47)
(1.26, 1.51, 1.47)
(1.16, 1.49, 1.48)
(1.03, 1.45, 1.49)
(0.88, 1.41, 1.49)
(0.71, 1.37, 1.51)
(0.52, 1.33, 1.51)
(0.34, 1.31, 1.50)
(0.18, 1.31, 1.52)
(0.06, 1.31, 1.51)
(-0.03, 1.33, 1.51)
(-0.09, 1.35, 1.50)
(-0.12, 1.34, 1.49)
(-0.12, 1.33, 1.49)
(-0.10, 1.27, 1.49)
(-0.05, 1.19, 1.50)
(-0.01, 1.08, 1.51)
(0.03, 0.91, 1.50)
(0.06, 0.76, 1.49)
(0.07, 0.57, 1.49)
(0.08, 0.35, 1.48)
(0.07, 0.16, 1.49)
(0.04, 0.00, 1.49)
(0.02, -0.10, 1.43)
(0.00, -0.18, 1.18)
(-0.01, -0.21, 0.86)
(-0.02, -0.20, 0.57)
(-0.03, -0.16, 0.35)
(-0.04, -0.12, 0.21)
(-0.05, -0.06, 0.15)
(-0.07, -0.01, 0.13)
(-0.06, 0.01, 0.13)
(-0.03, 0.02, 0.13)
(-0.02, 0.03, 0.12)
};


==> plots/kaist_traj_coords/infinite_jetson_slam.tex <==

%
\addplot3[
    fill=none,draw = clr2,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.01, -0.00, -0.00)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(0.00, -0.00, -0.00)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(0.00, -0.00, -0.01)
(-0.01, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.01, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.01, -0.01, -0.00)
(-0.01, -0.02, -0.00)
(-0.02, -0.02, -0.01)
(-0.02, -0.02, 0.00)
(-0.02, -0.02, 0.00)
(-0.02, -0.03, 0.01)
(-0.01, -0.02, 0.01)
(-0.02, -0.03, 0.00)
(-0.02, -0.01, 0.00)
(-0.02, -0.01, 0.00)
(-0.01, -0.00, 0.00)
(-0.00, 0.00, 0.00)
(-0.01, 0.01, 0.01)
(-0.00, 0.01, 0.01)
(-0.01, 0.01, 0.01)
(-0.00, 0.01, 0.01)
(-0.00, 0.01, 0.01)
(-0.00, 0.00, 0.01)
(-0.00, -0.00, 0.01)
(-0.01, -0.01, 0.01)
(-0.01, -0.01, 0.02)
(-0.01, -0.01, 0.03)
(-0.00, 0.00, 0.04)
(-0.00, -0.01, 0.03)
(-0.01, 0.00, 0.01)
(-0.00, -0.01, 0.00)
(-0.01, -0.01, 0.00)
(-0.01, -0.01, 0.00)
(-0.00, -0.01, 0.02)
(0.00, -0.00, 0.03)
(-0.00, 0.01, 0.03)
(-0.01, -0.00, 0.04)
(-0.00, -0.00, 0.04)
(-0.01, 0.01, 0.01)
(-0.01, -0.00, -0.00)
(0.00, 0.00, -0.00)
(-0.00, 0.00, -0.01)
(0.00, 0.00, -0.01)
(0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.00)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.00)
(0.00, -0.00, -0.00)
(0.00, -0.00, -0.00)
(-0.00, -0.00, -0.00)
(-0.00, -0.01, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.00)
(-0.00, -0.00, -0.00)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, -0.00)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, -0.00)
(-0.00, -0.00, -0.00)
(-0.00, -0.01, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.00)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.01, -0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, -0.01)
(0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.00)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, -0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.00)
(-0.00, -0.01, -0.01)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, -0.01)
(-0.00, -0.00, -0.00)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, -0.00)
(-0.00, -0.00, -0.00)
(-0.00, 0.00, -0.00)
(-0.00, -0.00, -0.00)
(0.00, -0.00, -0.00)
(0.00, -0.01, -0.01)
(-0.00, -0.00, -0.00)
(-0.00, -0.00, -0.00)
(0.00, 0.00, -0.01)
(-0.00, -0.00, -0.00)
(-0.00, -0.01, -0.00)
(-0.01, -0.00, 0.01)
(-0.04, -0.01, 0.10)
(-0.07, -0.02, 0.24)
(-0.11, -0.02, 0.35)
(-0.13, -0.01, 0.42)
(-0.15, -0.00, 0.48)
(-0.16, 0.01, 0.51)
(-0.16, 0.02, 0.56)
(-0.16, 0.01, 0.59)
(-0.15, 0.03, 0.63)
(-0.14, 0.04, 0.66)
(-0.13, 0.04, 0.68)
(-0.12, 0.04, 0.69)
(-0.11, 0.05, 0.71)
(-0.10, 0.05, 0.74)
(-0.08, 0.05, 0.75)
(-0.07, 0.05, 0.76)
(-0.05, 0.03, 0.77)
(0.05, 0.03, 0.77)
(0.21, 0.04, 0.80)
(0.39, 0.06, 0.81)
(0.55, 0.09, 0.82)
(0.69, 0.13, 0.83)
(0.77, 0.18, 0.83)
(0.83, 0.22, 0.84)
(0.83, 0.26, 0.84)
(0.80, 0.30, 0.85)
(0.75, 0.33, 0.85)
(0.67, 0.34, 0.86)
(0.58, 0.34, 0.87)
(0.48, 0.33, 0.86)
(0.39, 0.30, 0.85)
(0.31, 0.28, 0.85)
(0.23, 0.24, 0.84)
(0.17, 0.21, 0.84)
(0.11, 0.17, 0.85)
(0.07, 0.15, 0.85)
(0.03, 0.12, 0.86)
(0.01, 0.09, 0.87)
(-0.02, 0.07, 0.87)
(-0.04, 0.03, 0.88)
(-0.07, -0.02, 0.89)
(-0.10, -0.06, 0.90)
(-0.14, -0.10, 0.90)
(-0.18, -0.14, 0.91)
(-0.23, -0.17, 0.91)
(-0.28, -0.22, 0.91)
(-0.33, -0.26, 0.91)
(-0.37, -0.30, 0.90)
(-0.43, -0.34, 0.91)
(-0.48, -0.36, 0.91)
(-0.55, -0.37, 0.91)
(-0.61, -0.39, 0.92)
(-0.67, -0.39, 0.93)
(-0.75, -0.36, 0.92)
(-0.81, -0.33, 0.93)
(-0.88, -0.25, 0.94)
(-0.94, -0.18, 0.95)
(-0.97, -0.10, 0.95)
(-1.00, -0.03, 0.97)
(-1.00, 0.05, 0.95)
(-0.98, 0.11, 0.95)
(-0.95, 0.16, 0.93)
(-0.91, 0.26, 0.93)
(-0.86, 0.31, 0.93)
(-0.79, 0.36, 0.93)
(-0.71, 0.40, 0.94)
(-0.62, 0.41, 0.94)
(-0.54, 0.41, 0.93)
(-0.47, 0.41, 0.94)
(-0.39, 0.39, 0.95)
(-0.33, 0.35, 0.95)
(-0.27, 0.31, 0.95)
(-0.22, 0.27, 0.96)
(-0.17, 0.23, 0.97)
(-0.13, 0.17, 0.98)
(-0.09, 0.10, 0.98)
(-0.06, 0.03, 0.98)
(-0.02, -0.03, 0.98)
(0.00, -0.09, 0.98)
(0.03, -0.13, 0.98)
(0.06, -0.15, 0.99)
(0.08, -0.18, 1.00)
(0.10, -0.21, 1.01)
(0.14, -0.22, 1.01)
(0.19, -0.25, 1.01)
(0.24, -0.27, 1.01)
(0.31, -0.29, 1.01)
(0.38, -0.32, 1.02)
(0.45, -0.34, 1.01)
(0.53, -0.36, 1.02)
(0.61, -0.39, 1.02)
(0.68, -0.40, 1.02)
(0.75, -0.39, 1.02)
(0.81, -0.37, 1.01)
(0.87, -0.33, 1.01)
(0.91, -0.27, 1.01)
(0.94, -0.21, 1.02)
(0.95, -0.12, 1.02)
(0.95, -0.04, 1.02)
(0.93, 0.05, 1.02)
(0.90, 0.13, 1.02)
(0.85, 0.20, 1.02)
(0.80, 0.25, 1.02)
(0.73, 0.29, 1.02)
(0.66, 0.32, 1.03)
(0.59, 0.35, 1.04)
(0.52, 0.36, 1.05)
(0.45, 0.36, 1.06)
(0.40, 0.35, 1.06)
(0.34, 0.33, 1.06)
(0.29, 0.28, 1.07)
(0.26, 0.23, 1.07)
(0.22, 0.18, 1.07)
(0.19, 0.13, 1.08)
(0.15, 0.06, 1.08)
(0.12, 0.02, 1.07)
(0.07, -0.04, 1.07)
(0.03, -0.07, 1.07)
(-0.01, -0.12, 1.07)
(-0.06, -0.15, 1.08)
(-0.11, -0.17, 1.07)
(-0.15, -0.20, 1.08)
(-0.21, -0.22, 1.07)
(-0.25, -0.24, 1.08)
(-0.31, -0.26, 1.08)
(-0.37, -0.28, 1.08)
(-0.43, -0.29, 1.08)
(-0.50, -0.30, 1.07)
(-0.56, -0.32, 1.08)
(-0.63, -0.34, 1.09)
(-0.70, -0.34, 1.09)
(-0.77, -0.34, 1.09)
(-0.83, -0.32, 1.09)
(-0.89, -0.30, 1.09)
(-0.94, -0.26, 1.08)
(-0.97, -0.20, 1.10)
(-0.99, -0.12, 1.10)
(-0.99, -0.04, 1.10)
(-0.97, 0.03, 1.11)
(-0.94, 0.11, 1.11)
(-0.91, 0.20, 1.10)
(-0.86, 0.26, 1.11)
(-0.79, 0.31, 1.10)
(-0.73, 0.36, 1.10)
(-0.64, 0.40, 1.10)
(-0.56, 0.41, 1.11)
(-0.48, 0.40, 1.11)
(-0.40, 0.37, 1.11)
(-0.33, 0.34, 1.11)
(-0.28, 0.27, 1.11)
(-0.21, 0.21, 1.11)
(-0.19, 0.14, 1.11)
(-0.16, 0.10, 1.12)
(-0.11, 0.06, 1.12)
(-0.08, 0.01, 1.13)
(-0.05, -0.04, 1.14)
(-0.02, -0.10, 1.14)
(0.02, -0.16, 1.15)
(0.06, -0.20, 1.15)
(0.10, -0.25, 1.15)
(0.14, -0.28, 1.15)
(0.18, -0.30, 1.15)
(0.22, -0.30, 1.15)
(0.28, -0.32, 1.15)
(0.33, -0.33, 1.14)
(0.39, -0.33, 1.14)
(0.45, -0.33, 1.15)
(0.51, -0.33, 1.15)
(0.58, -0.32, 1.15)
(0.66, -0.32, 1.16)
(0.73, -0.31, 1.16)
(0.81, -0.29, 1.17)
(0.87, -0.26, 1.18)
(0.93, -0.21, 1.18)
(0.96, -0.15, 1.18)
(0.98, -0.07, 1.19)
(0.99, -0.00, 1.19)
(0.98, 0.07, 1.19)
(0.95, 0.14, 1.19)
(0.91, 0.21, 1.19)
(0.86, 0.27, 1.18)
(0.80, 0.31, 1.18)
(0.73, 0.33, 1.18)
(0.66, 0.34, 1.18)
(0.60, 0.34, 1.18)
(0.53, 0.33, 1.18)
(0.46, 0.32, 1.18)
(0.40, 0.30, 1.18)
(0.35, 0.27, 1.18)
(0.30, 0.24, 1.18)
(0.24, 0.19, 1.19)
(0.20, 0.13, 1.20)
(0.15, 0.08, 1.21)
(0.11, 0.02, 1.21)
(0.06, -0.04, 1.22)
(0.02, -0.08, 1.23)
(-0.01, -0.13, 1.24)
(-0.05, -0.17, 1.24)
(-0.09, -0.19, 1.24)
(-0.14, -0.21, 1.24)
(-0.18, -0.22, 1.24)
(-0.22, -0.23, 1.25)
(-0.25, -0.23, 1.24)
(-0.30, -0.24, 1.25)
(-0.35, -0.25, 1.23)
(-0.41, -0.28, 1.23)
(-0.48, -0.30, 1.24)
(-0.55, -0.34, 1.24)
(-0.62, -0.35, 1.25)
(-0.69, -0.37, 1.25)
(-0.77, -0.37, 1.25)
(-0.85, -0.35, 1.24)
(-0.91, -0.31, 1.25)
(-0.97, -0.27, 1.25)
(-1.00, -0.21, 1.24)
(-1.03, -0.10, 1.23)
(-1.02, 0.01, 1.24)
(-0.99, 0.11, 1.24)
(-0.95, 0.20, 1.26)
(-0.88, 0.27, 1.27)
(-0.81, 0.34, 1.27)
(-0.73, 0.40, 1.27)
(-0.65, 0.42, 1.28)
(-0.56, 0.43, 1.26)
(-0.48, 0.41, 1.26)
(-0.41, 0.37, 1.26)
(-0.34, 0.33, 1.26)
(-0.29, 0.25, 1.27)
(-0.23, 0.18, 1.27)
(-0.20, 0.14, 1.27)
(-0.16, 0.10, 1.27)
(-0.14, 0.06, 1.26)
(-0.12, 0.02, 1.27)
(-0.09, -0.02, 1.26)
(-0.07, -0.05, 1.27)
(-0.04, -0.08, 1.28)
(-0.00, -0.11, 1.29)
(0.04, -0.15, 1.29)
(0.09, -0.19, 1.29)
(0.16, -0.23, 1.29)
(0.22, -0.26, 1.29)
(0.29, -0.30, 1.29)
(0.35, -0.33, 1.29)
(0.40, -0.35, 1.29)
(0.47, -0.37, 1.29)
(0.53, -0.38, 1.29)
(0.60, -0.39, 1.29)
(0.68, -0.38, 1.30)
(0.75, -0.36, 1.30)
(0.82, -0.34, 1.30)
(0.87, -0.30, 1.29)
(0.92, -0.25, 1.29)
(0.96, -0.19, 1.29)
(0.98, -0.11, 1.30)
(0.98, -0.03, 1.31)
(0.97, 0.05, 1.31)
(0.94, 0.11, 1.31)
(0.90, 0.17, 1.31)
(0.84, 0.23, 1.31)
(0.77, 0.27, 1.31)
(0.69, 0.31, 1.32)
(0.60, 0.34, 1.33)
(0.52, 0.35, 1.33)
(0.45, 0.34, 1.33)
(0.38, 0.33, 1.34)
(0.32, 0.31, 1.34)
(0.28, 0.27, 1.34)
(0.24, 0.25, 1.34)
(0.21, 0.21, 1.35)
(0.18, 0.17, 1.36)
(0.15, 0.14, 1.36)
(0.12, 0.10, 1.36)
(0.10, 0.06, 1.36)
(0.07, 0.02, 1.36)
(0.04, -0.03, 1.38)
(0.01, -0.08, 1.37)
(-0.02, -0.13, 1.37)
(-0.06, -0.17, 1.38)
(-0.11, -0.20, 1.38)
(-0.16, -0.24, 1.37)
(-0.22, -0.27, 1.37)
(-0.28, -0.28, 1.38)
(-0.35, -0.31, 1.40)
(-0.42, -0.34, 1.40)
(-0.51, -0.35, 1.40)
(-0.58, -0.35, 1.39)
(-0.65, -0.36, 1.39)
(-0.73, -0.36, 1.40)
(-0.80, -0.35, 1.39)
(-0.87, -0.32, 1.40)
(-0.93, -0.28, 1.39)
(-0.98, -0.22, 1.39)
(-1.00, -0.18, 1.41)
(-1.02, -0.10, 1.40)
(-1.01, -0.02, 1.42)
(-0.99, 0.06, 1.42)
(-0.96, 0.16, 1.42)
(-0.90, 0.23, 1.41)
(-0.83, 0.31, 1.43)
(-0.75, 0.37, 1.44)
(-0.67, 0.43, 1.43)
(-0.59, 0.46, 1.46)
(-0.51, 0.47, 1.46)
(-0.42, 0.45, 1.46)
(-0.34, 0.42, 1.46)
(-0.28, 0.37, 1.47)
(-0.22, 0.31, 1.46)
(-0.16, 0.25, 1.47)
(-0.12, 0.18, 1.46)
(-0.09, 0.11, 1.46)
(-0.07, 0.05, 1.46)
(-0.06, -0.01, 1.45)
(-0.04, -0.07, 1.45)
(-0.04, -0.11, 1.45)
(-0.02, -0.15, 1.44)
(0.01, -0.18, 1.44)
(0.05, -0.21, 1.44)
(0.08, -0.21, 1.43)
(0.13, -0.23, 1.43)
(0.19, -0.25, 1.44)
(0.25, -0.26, 1.45)
(0.32, -0.28, 1.44)
(0.40, -0.30, 1.46)
(0.48, -0.31, 1.46)
(0.56, -0.34, 1.46)
(0.64, -0.36, 1.45)
(0.71, -0.35, 1.46)
(0.79, -0.34, 1.48)
(0.85, -0.31, 1.48)
(0.91, -0.27, 1.48)
(0.96, -0.22, 1.47)
(0.99, -0.16, 1.47)
(1.00, -0.09, 1.47)
(1.01, -0.01, 1.47)
(0.99, 0.07, 1.46)
(0.95, 0.15, 1.47)
(0.90, 0.19, 1.46)
(0.84, 0.26, 1.46)
(0.77, 0.30, 1.45)
(0.70, 0.33, 1.46)
(0.63, 0.34, 1.46)
(0.55, 0.35, 1.48)
(0.48, 0.33, 1.49)
(0.41, 0.31, 1.49)
(0.34, 0.29, 1.50)
(0.29, 0.25, 1.50)
(0.24, 0.23, 1.51)
(0.20, 0.19, 1.51)
(0.16, 0.14, 1.50)
(0.12, 0.10, 1.50)
(0.09, 0.07, 1.51)
(0.06, 0.03, 1.53)
(0.03, -0.02, 1.54)
(-0.00, -0.06, 1.54)
(-0.03, -0.10, 1.56)
(-0.07, -0.14, 1.55)
(-0.11, -0.18, 1.56)
(-0.17, -0.22, 1.56)
(-0.22, -0.26, 1.56)
(-0.29, -0.28, 1.56)
(-0.35, -0.30, 1.55)
(-0.42, -0.32, 1.56)
(-0.48, -0.33, 1.56)
(-0.54, -0.34, 1.58)
(-0.60, -0.34, 1.58)
(-0.65, -0.34, 1.58)
(-0.72, -0.32, 1.58)
(-0.77, -0.32, 1.57)
(-0.83, -0.29, 1.57)
(-0.88, -0.25, 1.58)
(-0.93, -0.19, 1.57)
(-0.96, -0.12, 1.56)
(-0.98, -0.04, 1.57)
(-0.98, 0.02, 1.59)
(-0.96, 0.11, 1.58)
(-0.93, 0.18, 1.59)
(-0.88, 0.25, 1.57)
(-0.82, 0.33, 1.59)
(-0.75, 0.37, 1.57)
(-0.67, 0.40, 1.57)
(-0.60, 0.42, 1.57)
(-0.53, 0.42, 1.57)
(-0.46, 0.40, 1.59)
(-0.39, 0.36, 1.60)
(-0.33, 0.32, 1.61)
(-0.26, 0.26, 1.61)
(-0.21, 0.22, 1.61)
(-0.15, 0.17, 1.49)
(-0.10, 0.14, 1.22)
(-0.06, 0.10, 0.94)
(-0.03, 0.06, 0.67)
(-0.01, 0.03, 0.46)
(-0.01, 0.02, 0.30)
(-0.01, -0.00, 0.15)
};

==> plots/kaist_traj_coords/square_gt.tex <==
\addplot3[
    fill=none,draw = clr1,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, 0.00)
(0.00, -0.01, 0.00)
(0.00, -0.01, 0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, -0.00)
(0.00, -0.01, 0.00)
(0.00, -0.01, 0.00)
(0.00, -0.01, 0.00)
(0.00, -0.01, 0.01)
(0.00, -0.01, 0.01)
(0.00, -0.01, 0.01)
(0.00, -0.01, 0.01)
(0.00, -0.01, 0.01)
(0.00, -0.01, 0.01)
(-0.00, -0.01, 0.01)
(-0.00, -0.01, 0.02)
(-0.00, -0.01, 0.02)
(-0.00, -0.01, 0.02)
(-0.00, -0.01, 0.02)
(-0.00, -0.01, 0.02)
(0.00, -0.01, 0.02)
(-0.00, -0.00, 0.02)
(-0.00, -0.00, 0.02)
(0.00, -0.01, 0.02)
(0.00, -0.01, 0.02)
(0.00, -0.01, 0.02)
(0.00, -0.01, 0.02)
(0.01, -0.01, 0.02)
(0.01, -0.01, 0.02)
(0.01, -0.01, 0.02)
(0.00, -0.01, 0.02)
(0.00, -0.01, 0.02)
(0.00, -0.01, 0.02)
(0.00, -0.01, 0.02)
(0.01, -0.01, 0.02)
(0.01, -0.01, 0.01)
(0.01, -0.01, 0.03)
(0.01, -0.01, 0.05)
(0.01, -0.01, 0.06)
(0.01, -0.00, 0.07)
(0.01, -0.00, 0.05)
(0.01, 0.00, 0.04)
(0.01, 0.00, 0.03)
(0.01, -0.00, 0.02)
(0.01, -0.00, 0.03)
(0.01, 0.00, 0.08)
(0.01, 0.00, 0.09)
(0.01, 0.00, 0.07)
(0.01, 0.01, 0.04)
(0.01, 0.00, 0.02)
(0.01, 0.00, 0.01)
(0.01, 0.00, 0.00)
(0.01, 0.00, 0.00)
(0.01, 0.00, 0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, 0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(0.01, 0.00, -0.00)
(-0.02, 0.01, 0.03)
(-0.14, 0.05, 0.32)
(-0.20, 0.07, 0.45)
(-0.24, 0.09, 0.58)
(-0.20, 0.10, 0.68)
(-0.14, 0.09, 0.72)
(-0.04, 0.07, 0.76)
(0.17, 0.02, 0.81)
(0.65, 0.01, 0.81)
(0.99, 0.08, 0.81)
(1.16, 0.24, 0.79)
(1.02, 0.33, 0.79)
(0.02, 0.05, 0.83)
(-0.27, -0.13, 0.87)
(-0.33, -0.19, 0.88)
(-0.26, -0.20, 0.88)
(-0.21, -0.21, 0.88)
(-0.19, -0.22, 0.88)
(-0.17, -0.23, 0.88)
(-0.19, -0.25, 0.88)
(-0.22, -0.28, 0.89)
(-0.27, -0.31, 0.89)
(-0.35, -0.34, 0.90)
(-0.44, -0.38, 0.90)
(-0.54, -0.40, 0.89)
(-0.67, -0.43, 0.88)
(-0.79, -0.44, 0.88)
(-0.91, -0.44, 0.87)
(-1.05, -0.40, 0.87)
(-1.13, -0.35, 0.87)
(-1.19, -0.28, 0.88)
(-1.24, -0.18, 0.88)
(-1.25, -0.02, 0.88)
(-1.23, 0.09, 0.87)
(-1.18, 0.19, 0.87)
(-1.12, 0.29, 0.87)
(-1.04, 0.37, 0.88)
(-0.96, 0.43, 0.89)
(-0.78, 0.52, 0.90)
(-0.62, 0.55, 0.91)
(-0.49, 0.54, 0.91)
(-0.38, 0.50, 0.91)
(-0.31, 0.47, 0.91)
(-0.24, 0.43, 0.91)
(-0.18, 0.38, 0.91)
(-0.15, 0.33, 0.91)
(-0.12, 0.27, 0.91)
(-0.11, 0.21, 0.91)
(-0.11, 0.16, 0.90)
(-0.11, 0.11, 0.91)
(-0.10, 0.05, 0.91)
(-0.09, 0.01, 0.91)
(-0.06, -0.03, 0.91)
(-0.03, -0.06, 0.92)
(0.02, -0.08, 0.92)
(0.07, -0.10, 0.93)
(0.14, -0.12, 0.94)
(0.20, -0.14, 0.95)
(0.27, -0.17, 0.95)
(0.33, -0.21, 0.95)
(0.39, -0.25, 0.95)
(0.45, -0.29, 0.95)
(0.51, -0.33, 0.95)
(0.61, -0.40, 0.95)
(0.70, -0.44, 0.94)
(0.77, -0.46, 0.94)
(0.85, -0.46, 0.94)
(0.93, -0.43, 0.95)
(0.99, -0.39, 0.95)
(1.04, -0.34, 0.96)
(1.07, -0.27, 0.96)
(1.09, -0.19, 0.97)
(1.09, -0.09, 0.97)
(1.08, 0.02, 0.97)
(1.05, 0.11, 0.97)
(1.01, 0.20, 0.97)
(0.96, 0.27, 0.97)
(0.90, 0.34, 0.97)
(0.79, 0.42, 0.96)
(0.71, 0.44, 0.97)
(0.64, 0.44, 0.98)
(0.57, 0.44, 0.99)
(0.51, 0.42, 0.99)
(0.44, 0.40, 1.00)
(0.39, 0.36, 1.00)
(0.34, 0.32, 1.01)
(0.30, 0.27, 1.01)
(0.26, 0.22, 1.01)
(0.23, 0.16, 1.01)
(0.20, 0.12, 1.01)
(0.17, 0.06, 1.01)
(0.13, 0.00, 1.01)
(0.09, -0.05, 1.01)
(0.04, -0.10, 1.02)
(-0.01, -0.15, 1.02)
(-0.06, -0.21, 1.02)
(-0.13, -0.26, 1.03)
(-0.18, -0.30, 1.03)
(-0.24, -0.34, 1.04)
(-0.31, -0.37, 1.04)
(-0.37, -0.40, 1.04)
(-0.42, -0.41, 1.04)
(-0.49, -0.42, 1.05)
(-0.54, -0.43, 1.05)
(-0.61, -0.42, 1.05)
(-0.67, -0.41, 1.06)
(-0.74, -0.40, 1.06)
(-0.81, -0.37, 1.06)
(-0.88, -0.34, 1.06)
(-0.96, -0.29, 1.06)
(-1.02, -0.22, 1.07)
(-1.06, -0.15, 1.07)
(-1.09, -0.07, 1.07)
(-1.12, 0.03, 1.07)
(-1.12, 0.17, 1.08)
(-0.92, 0.53, 1.09)
(-0.20, 0.75, 1.10)
(-0.01, 0.66, 1.09)
(0.11, 0.41, 1.07)
(-0.05, -0.19, 1.06)
(-0.14, -0.49, 1.06)
(-0.10, -0.54, 1.08)
(-0.03, -0.54, 1.10)
(0.04, -0.52, 1.11)
(0.14, -0.49, 1.12)
(0.25, -0.45, 1.13)
(0.34, -0.40, 1.13)
(0.45, -0.35, 1.12)
(0.53, -0.31, 1.12)
(0.66, -0.26, 1.13)
(0.75, -0.23, 1.12)
(0.84, -0.21, 1.12)
(0.92, -0.20, 1.11)
(0.99, -0.19, 1.11)
(1.06, -0.17, 1.12)
(1.12, -0.14, 1.12)
(1.17, -0.09, 1.12)
(1.16, 0.09, 1.12)
(0.95, 0.26, 1.11)
(0.58, 0.39, 1.12)
(0.32, 0.37, 1.16)
(0.22, 0.31, 1.17)
(0.16, 0.21, 1.18)
(0.14, 0.16, 1.18)
(0.12, 0.12, 1.18)
(0.09, 0.06, 1.18)
(0.06, 0.01, 1.18)
(0.02, -0.04, 1.18)
(-0.02, -0.08, 1.19)
(-0.07, -0.14, 1.20)
(-0.11, -0.19, 1.21)
(-0.17, -0.23, 1.21)
(-0.22, -0.28, 1.21)
(-0.29, -0.33, 1.20)
(-0.35, -0.37, 1.20)
(-0.40, -0.40, 1.19)
(-0.48, -0.44, 1.19)
(-0.56, -0.46, 1.19)
(-0.63, -0.47, 1.19)
(-0.73, -0.46, 1.20)
(-0.81, -0.43, 1.20)
(-0.88, -0.40, 1.21)
(-0.94, -0.35, 1.22)
(-1.03, -0.28, 1.24)
(-1.08, -0.21, 1.24)
(-1.14, -0.11, 1.25)
(-1.16, -0.00, 1.26)
(-1.16, 0.09, 1.26)
(-1.14, 0.17, 1.26)
(-1.11, 0.25, 1.27)
(-1.03, 0.36, 1.27)
(-0.95, 0.43, 1.26)
(-0.87, 0.47, 1.26)
(-0.79, 0.49, 1.26)
(-0.70, 0.51, 1.25)
(-0.61, 0.51, 1.25)
(-0.53, 0.51, 1.25)
(-0.45, 0.49, 1.25)
(-0.37, 0.46, 1.24)
(-0.31, 0.42, 1.24)
(-0.26, 0.37, 1.23)
(-0.19, 0.30, 1.22)
(-0.15, 0.25, 1.22)
(-0.11, 0.19, 1.22)
(-0.06, 0.12, 1.22)
(-0.04, 0.08, 1.23)
(0.00, -0.03, 1.25)
(0.02, -0.09, 1.25)
(0.03, -0.13, 1.26)
(0.05, -0.17, 1.26)
(0.08, -0.20, 1.26)
(0.13, -0.23, 1.27)
(0.18, -0.25, 1.27)
(0.32, -0.31, 1.27)
(0.75, -0.46, 1.26)
(0.84, -0.48, 1.27)
(0.99, -0.49, 1.28)
(1.06, -0.47, 1.29)
(1.11, -0.44, 1.30)
(1.14, -0.38, 1.30)
(1.14, -0.28, 1.30)
(1.12, -0.20, 1.31)
(1.09, -0.11, 1.30)
(1.06, -0.02, 1.30)
(1.01, 0.06, 1.29)
(0.97, 0.15, 1.29)
(0.92, 0.22, 1.29)
(0.87, 0.28, 1.29)
(0.74, 0.40, 1.29)
(0.60, 0.45, 1.31)
(0.51, 0.45, 1.32)
(0.46, 0.44, 1.33)
(0.41, 0.41, 1.34)
(0.37, 0.37, 1.35)
(0.33, 0.33, 1.35)
(0.30, 0.28, 1.36)
(0.26, 0.22, 1.36)
(0.22, 0.17, 1.35)
(0.18, 0.11, 1.36)
(0.14, 0.06, 1.36)
(0.07, -0.01, 1.35)
(0.03, -0.06, 1.35)
(-0.02, -0.11, 1.35)
(-0.06, -0.15, 1.35)
(-0.11, -0.18, 1.35)
(-0.20, -0.24, 1.34)
(-0.25, -0.28, 1.35)
(-0.31, -0.32, 1.35)
(-0.36, -0.36, 1.35)
(-0.41, -0.40, 1.36)
(-0.47, -0.42, 1.36)
(-0.53, -0.44, 1.36)
(-0.58, -0.45, 1.36)
(-0.67, -0.44, 1.37)
(-0.76, -0.42, 1.37)
(-0.83, -0.39, 1.38)
(-0.92, -0.34, 1.39)
(-1.01, -0.26, 1.40)
(-1.07, -0.19, 1.41)
(-1.13, -0.10, 1.41)
(-1.16, -0.01, 1.41)
(-1.18, 0.09, 1.42)
(-1.17, 0.18, 1.41)
(-1.15, 0.28, 1.41)
(-1.11, 0.36, 1.41)
(-1.05, 0.42, 1.41)
(-0.98, 0.46, 1.41)
(-0.91, 0.48, 1.41)
(-0.82, 0.49, 1.41)
(-0.73, 0.49, 1.40)
(-0.62, 0.48, 1.40)
(-0.54, 0.47, 1.39)
(-0.44, 0.43, 1.39)
(-0.36, 0.40, 1.39)
(-0.29, 0.36, 1.39)
(-0.24, 0.32, 1.40)
(-0.18, 0.28, 1.40)
(-0.14, 0.24, 1.41)
(-0.10, 0.19, 1.41)
(-0.07, 0.15, 1.41)
(-0.04, 0.10, 1.42)
(-0.01, 0.06, 1.42)
(0.02, 0.02, 1.42)
(0.05, -0.03, 1.42)
(0.08, -0.09, 1.43)
(0.10, -0.15, 1.43)
(0.13, -0.21, 1.44)
(0.15, -0.25, 1.45)
(0.18, -0.29, 1.45)
(0.22, -0.32, 1.45)
(0.26, -0.34, 1.45)
(0.34, -0.38, 1.45)
(0.42, -0.41, 1.45)
(0.49, -0.44, 1.46)
(0.58, -0.47, 1.46)
(0.65, -0.48, 1.45)
(0.73, -0.49, 1.45)
(0.83, -0.47, 1.45)
(0.89, -0.44, 1.45)
(0.95, -0.40, 1.45)
(1.00, -0.35, 1.45)
(1.04, -0.28, 1.46)
(1.06, -0.21, 1.46)
(1.07, -0.14, 1.47)
(1.06, 0.01, 1.48)
(1.04, 0.10, 1.48)
(1.02, 0.18, 1.48)
(0.98, 0.26, 1.48)
(0.93, 0.33, 1.48)
(0.87, 0.38, 1.47)
(0.80, 0.43, 1.47)
(0.74, 0.46, 1.47)
(0.67, 0.46, 1.48)
(0.61, 0.45, 1.48)
(0.54, 0.43, 1.49)
(0.48, 0.39, 1.49)
(0.41, 0.36, 1.50)
(0.36, 0.32, 1.51)
(0.31, 0.27, 1.51)
(0.27, 0.22, 1.51)
(0.21, 0.15, 1.52)
(0.17, 0.10, 1.52)
(0.14, 0.06, 1.52)
(0.10, 0.01, 1.52)
(0.06, -0.04, 1.52)
(0.02, -0.10, 1.52)
(-0.01, -0.14, 1.51)
(-0.05, -0.19, 1.51)
(-0.09, -0.23, 1.50)
(-0.13, -0.27, 1.50)
(-0.18, -0.31, 1.51)
(-0.22, -0.33, 1.51)
(-0.28, -0.34, 1.52)
(-0.34, -0.35, 1.53)
(-0.41, -0.36, 1.54)
(-0.47, -0.36, 1.55)
(-0.55, -0.36, 1.55)
(-0.63, -0.36, 1.55)
(-0.71, -0.37, 1.55)
(-0.93, -0.36, 1.55)
(-1.05, -0.32, 1.56)
(-1.12, -0.27, 1.56)
(-1.17, -0.20, 1.57)
(-1.20, -0.12, 1.57)
(-1.21, 0.02, 1.58)
(-1.19, 0.13, 1.59)
(-1.13, 0.29, 1.59)
(-1.07, 0.39, 1.58)
(-1.01, 0.47, 1.58)
(-0.91, 0.55, 1.59)
(-0.82, 0.59, 1.59)
(-0.55, 0.59, 1.57)
(-0.47, 0.55, 1.57)
(-0.38, 0.48, 1.56)
(-0.29, 0.38, 1.56)
(-0.18, 0.22, 1.56)
(-0.09, 0.12, 1.57)
(0.05, -0.08, 1.57)
(0.11, -0.14, 1.57)
(0.21, -0.25, 1.58)
(0.28, -0.35, 1.60)
(0.31, -0.39, 1.59)
(0.32, -0.40, 1.41)
(0.29, -0.36, 1.15)
(0.22, -0.29, 0.81)
(0.16, -0.24, 0.60)
(0.08, -0.18, 0.40)
(-0.02, -0.10, 0.21)
(-0.13, -0.04, 0.12)
(-0.21, 0.02, 0.10)
(-0.30, 0.07, 0.10)
(-0.39, 0.11, 0.10)
(-0.49, 0.15, 0.03)
};
%


==> plots/kaist_traj_coords/square_jetson_slam.tex <==
%
\addplot3[
    fill=none,draw = clr2,
    very thick,
    line width= \linew ex,
    ]
    coordinates {
(0.04, -0.01, -0.01)
(0.05, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.05, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.02, -0.01)
(0.04, -0.01, -0.00)
(0.04, -0.01, -0.01)
(0.04, -0.01, -0.00)
(0.04, -0.00, -0.01)
(0.05, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.02, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.03, -0.01)
(0.03, -0.03, -0.00)
(0.03, -0.04, -0.00)
(0.03, -0.04, -0.00)
(0.04, -0.02, -0.01)
(0.03, -0.01, 0.00)
(0.03, -0.01, 0.00)
(0.03, 0.01, 0.01)
(0.04, 0.00, 0.01)
(0.04, 0.02, 0.00)
(0.04, 0.01, 0.01)
(0.04, 0.01, 0.01)
(0.03, -0.00, 0.01)
(0.04, -0.00, 0.00)
(0.04, -0.01, -0.00)
(0.04, -0.02, 0.00)
(0.04, -0.03, 0.00)
(0.03, -0.02, 0.00)
(0.04, -0.02, 0.00)
(0.04, -0.02, 0.00)
(0.04, -0.01, 0.00)
(0.04, -0.01, 0.01)
(0.03, -0.00, 0.01)
(0.05, -0.01, 0.01)
(0.04, 0.00, 0.03)
(0.05, -0.01, 0.04)
(0.05, -0.01, 0.04)
(0.04, -0.02, 0.02)
(0.05, -0.00, 0.01)
(0.04, -0.00, 0.01)
(0.04, -0.00, 0.02)
(0.05, -0.00, 0.03)
(0.05, -0.00, 0.05)
(0.06, -0.01, 0.05)
(0.05, -0.00, 0.04)
(0.05, -0.00, 0.01)
(0.04, -0.01, 0.00)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.01, -0.01)
(0.04, 0.01, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, 0.01, -0.01)
(0.04, 0.01, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.01, -0.01)
(0.05, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.05, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.05, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.05, 0.00, -0.01)
(0.04, 0.00, -0.01)
(0.05, -0.01, -0.01)
(0.05, -0.00, -0.01)
(0.04, 0.01, -0.01)
(0.05, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.05, -0.00, -0.01)
(0.05, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.01, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.01, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, 0.00, -0.00)
(0.04, 0.00, -0.01)
(0.05, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.05, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.05, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, 0.00, -0.01)
(0.05, 0.00, -0.01)
(0.04, -0.01, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, -0.00, -0.01)
(0.04, 0.00, -0.01)
(0.04, -0.00, -0.00)
(0.03, -0.01, 0.02)
(-0.01, 0.03, 0.12)
(-0.07, 0.04, 0.28)
(-0.11, 0.05, 0.37)
(-0.15, 0.08, 0.44)
(-0.18, 0.10, 0.51)
(-0.19, 0.11, 0.56)
(-0.18, 0.12, 0.60)
(-0.16, 0.12, 0.63)
(-0.15, 0.11, 0.66)
(-0.11, 0.12, 0.68)
(-0.08, 0.11, 0.71)
(-0.04, 0.11, 0.73)
(-0.01, 0.11, 0.73)
(0.02, 0.10, 0.73)
(0.03, 0.09, 0.74)
(0.04, 0.08, 0.74)
(0.09, 0.13, 0.78)
(0.16, 0.14, 0.77)
(0.29, 0.09, 0.75)
(0.56, 0.10, 0.77)
(0.75, 0.11, 0.75)
(0.90, 0.13, 0.74)
(1.00, 0.17, 0.72)
(1.03, 0.20, 0.73)
(1.02, 0.23, 0.73)
(0.96, 0.25, 0.71)
(0.86, 0.26, 0.71)
(0.74, 0.24, 0.73)
(0.59, 0.25, 0.72)
(0.41, 0.25, 0.75)
(0.29, 0.17, 0.76)
(0.16, 0.11, 0.78)
(0.05, 0.03, 0.80)
(-0.07, -0.04, 0.82)
(-0.19, -0.10, 0.84)
(-0.29, -0.17, 0.86)
(-0.38, -0.23, 0.88)
(-0.43, -0.28, 0.89)
(-0.46, -0.30, 0.89)
(-0.45, -0.29, 0.89)
(-0.41, -0.28, 0.89)
(-0.37, -0.27, 0.89)
(-0.33, -0.27, 0.89)
(-0.32, -0.27, 0.88)
(-0.34, -0.27, 0.89)
(-0.39, -0.29, 0.90)
(-0.48, -0.30, 0.91)
(-0.58, -0.32, 0.93)
(-0.71, -0.35, 0.91)
(-0.84, -0.35, 0.91)
(-0.97, -0.34, 0.91)
(-1.06, -0.32, 0.91)
(-1.17, -0.24, 0.92)
(-1.20, -0.18, 0.93)
(-1.22, -0.04, 0.92)
(-1.21, 0.07, 0.92)
(-1.16, 0.17, 0.92)
(-1.09, 0.28, 0.92)
(-0.98, 0.38, 0.92)
(-0.86, 0.46, 0.93)
(-0.74, 0.51, 0.94)
(-0.62, 0.51, 0.94)
(-0.49, 0.50, 0.93)
(-0.37, 0.47, 0.93)
(-0.27, 0.40, 0.93)
(-0.18, 0.35, 0.93)
(-0.12, 0.29, 0.93)
(-0.09, 0.21, 0.92)
(-0.07, 0.14, 0.92)
(-0.07, 0.08, 0.92)
(-0.07, 0.01, 0.92)
(-0.05, -0.04, 0.92)
(-0.02, -0.08, 0.92)
(0.03, -0.12, 0.92)
(0.08, -0.15, 0.94)
(0.17, -0.16, 0.93)
(0.26, -0.17, 0.93)
(0.35, -0.18, 0.93)
(0.43, -0.22, 0.94)
(0.51, -0.25, 0.93)
(0.59, -0.27, 0.92)
(0.61, -0.26, 0.92)
(0.72, -0.33, 0.91)
(0.75, -0.33, 0.91)
(0.84, -0.34, 0.90)
(0.89, -0.33, 0.90)
(0.92, -0.30, 0.90)
(0.98, -0.25, 0.89)
(1.01, -0.16, 0.91)
(1.00, -0.09, 0.92)
(0.98, 0.00, 0.91)
(0.95, 0.09, 0.91)
(0.89, 0.18, 0.90)
(0.83, 0.27, 0.90)
(0.75, 0.34, 0.90)
(0.68, 0.37, 0.90)
(0.61, 0.38, 0.91)
(0.52, 0.40, 0.93)
(0.43, 0.39, 0.94)
(0.35, 0.35, 0.96)
(0.28, 0.30, 0.97)
(0.21, 0.25, 0.98)
(0.16, 0.17, 0.99)
(0.13, 0.10, 0.99)
(0.09, 0.03, 0.99)
(0.04, -0.03, 0.99)
(-0.01, -0.11, 1.00)
(-0.06, -0.17, 1.01)
(-0.13, -0.23, 1.01)
(-0.19, -0.27, 1.02)
(-0.24, -0.33, 1.03)
(-0.31, -0.36, 1.03)
(-0.38, -0.39, 1.04)
(-0.45, -0.42, 1.05)
(-0.52, -0.42, 1.06)
(-0.59, -0.40, 1.06)
(-0.65, -0.38, 1.06)
(-0.72, -0.36, 1.08)
(-0.82, -0.33, 1.08)
(-0.88, -0.29, 1.09)
(-0.93, -0.23, 1.07)
(-0.98, -0.17, 1.10)
(-1.02, -0.10, 1.10)
(-1.05, -0.01, 1.11)
(-1.07, 0.07, 1.12)
(-1.07, 0.18, 1.12)
(-1.05, 0.27, 1.12)
(-1.01, 0.37, 1.13)
(-0.95, 0.45, 1.13)
(-0.85, 0.54, 1.13)
(-0.74, 0.60, 1.13)
(-0.62, 0.66, 1.13)
(-0.47, 0.71, 1.12)
(-0.33, 0.70, 1.12)
(-0.17, 0.71, 1.11)
(-0.02, 0.65, 1.09)
(0.08, 0.55, 1.08)
(0.15, 0.41, 1.08)
(0.16, 0.26, 1.08)
(0.14, 0.09, 1.09)
(0.09, -0.06, 1.07)
(0.03, -0.22, 1.07)
(-0.03, -0.37, 1.07)
(-0.07, -0.49, 1.08)
(-0.08, -0.56, 1.09)
(-0.05, -0.59, 1.11)
(0.01, -0.59, 1.12)
(0.09, -0.56, 1.12)
(0.19, -0.52, 1.12)
(0.33, -0.45, 1.12)
(0.44, -0.35, 1.11)
(0.54, -0.27, 1.10)
(0.65, -0.20, 1.10)
(0.74, -0.13, 1.10)
(0.83, -0.09, 1.08)
(0.91, -0.07, 1.07)
(0.98, -0.05, 1.07)
(1.04, -0.05, 1.07)
(1.08, -0.03, 1.07)
(1.10, 0.01, 1.06)
(1.10, 0.04, 1.06)
(1.06, 0.10, 1.06)
(1.01, 0.16, 1.06)
(0.93, 0.20, 1.06)
(0.83, 0.24, 1.06)
(0.73, 0.29, 1.06)
(0.62, 0.31, 1.09)
(0.50, 0.33, 1.08)
(0.39, 0.34, 1.10)
(0.30, 0.33, 1.12)
(0.21, 0.31, 1.13)
(0.16, 0.27, 1.14)
(0.10, 0.22, 1.15)
(0.06, 0.16, 1.16)
(0.04, 0.09, 1.17)
(0.01, 0.03, 1.18)
(-0.02, -0.04, 1.17)
(-0.07, -0.09, 1.18)
(-0.12, -0.15, 1.19)
(-0.18, -0.20, 1.20)
(-0.24, -0.26, 1.21)
(-0.31, -0.31, 1.23)
(-0.39, -0.34, 1.23)
(-0.47, -0.36, 1.22)
(-0.54, -0.39, 1.23)
(-0.61, -0.41, 1.22)
(-0.70, -0.41, 1.21)
(-0.79, -0.40, 1.22)
(-0.87, -0.36, 1.23)
(-0.94, -0.30, 1.25)
(-0.99, -0.23, 1.26)
(-1.05, -0.15, 1.28)
(-1.09, -0.07, 1.29)
(-1.12, 0.03, 1.31)
(-1.11, 0.13, 1.31)
(-1.08, 0.23, 1.31)
(-1.03, 0.31, 1.32)
(-0.95, 0.38, 1.31)
(-0.87, 0.43, 1.31)
(-0.77, 0.46, 1.30)
(-0.66, 0.48, 1.29)
(-0.55, 0.48, 1.29)
(-0.44, 0.46, 1.28)
(-0.35, 0.42, 1.27)
(-0.27, 0.37, 1.25)
(-0.20, 0.30, 1.24)
(-0.14, 0.23, 1.23)
(-0.09, 0.17, 1.23)
(-0.04, 0.10, 1.24)
(0.00, 0.04, 1.24)
(0.05, -0.03, 1.25)
(0.06, -0.10, 1.27)
(0.09, -0.16, 1.28)
(0.12, -0.22, 1.27)
(0.15, -0.25, 1.27)
(0.20, -0.27, 1.27)
(0.27, -0.27, 1.27)
(0.34, -0.28, 1.27)
(0.43, -0.30, 1.26)
(0.52, -0.31, 1.26)
(0.62, -0.33, 1.25)
(0.72, -0.34, 1.23)
(0.82, -0.35, 1.24)
(0.92, -0.36, 1.23)
(1.02, -0.36, 1.24)
(1.08, -0.34, 1.23)
(1.11, -0.29, 1.25)
(1.11, -0.23, 1.25)
(1.07, -0.16, 1.25)
(1.02, -0.07, 1.25)
(0.96, 0.03, 1.26)
(0.89, 0.12, 1.25)
(0.83, 0.21, 1.23)
(0.76, 0.28, 1.25)
(0.69, 0.34, 1.24)
(0.62, 0.37, 1.26)
(0.54, 0.40, 1.27)
(0.46, 0.41, 1.29)
(0.40, 0.39, 1.30)
(0.34, 0.36, 1.31)
(0.28, 0.32, 1.32)
(0.25, 0.24, 1.34)
(0.18, 0.19, 1.35)
(0.14, 0.11, 1.33)
(0.08, 0.03, 1.36)
(0.03, -0.04, 1.37)
(-0.03, -0.09, 1.37)
(-0.09, -0.15, 1.36)
(-0.16, -0.19, 1.36)
(-0.22, -0.24, 1.37)
(-0.29, -0.28, 1.37)
(-0.36, -0.31, 1.37)
(-0.43, -0.35, 1.37)
(-0.50, -0.37, 1.37)
(-0.57, -0.40, 1.39)
(-0.63, -0.41, 1.39)
(-0.71, -0.40, 1.40)
(-0.77, -0.36, 1.41)
(-0.85, -0.33, 1.42)
(-0.91, -0.26, 1.43)
(-0.97, -0.20, 1.43)
(-1.03, -0.13, 1.46)
(-1.09, -0.01, 1.47)
(-1.09, 0.01, 1.46)
(-1.09, 0.03, 1.46)
(-1.10, 0.07, 1.46)
(-1.05, 0.39, 1.45)
(-0.97, 0.44, 1.45)
(-0.88, 0.47, 1.46)
(-0.78, 0.48, 1.46)
(-0.67, 0.46, 1.44)
(-0.55, 0.45, 1.45)
(-0.45, 0.42, 1.43)
(-0.35, 0.38, 1.43)
(-0.26, 0.32, 1.42)
(-0.18, 0.27, 1.42)
(-0.12, 0.20, 1.42)
(-0.07, 0.15, 1.43)
(-0.02, 0.10, 1.43)
(0.02, 0.04, 1.44)
(0.06, -0.01, 1.44)
(0.11, -0.06, 1.44)
(0.14, -0.12, 1.45)
(0.18, -0.18, 1.45)
(0.21, -0.24, 1.45)
(0.25, -0.28, 1.46)
(0.29, -0.31, 1.46)
(0.34, -0.32, 1.46)
(0.40, -0.33, 1.45)
(0.49, -0.35, 1.45)
(0.57, -0.36, 1.44)
(0.67, -0.37, 1.43)
(0.76, -0.37, 1.44)
(0.82, -0.36, 1.44)
(0.88, -0.34, 1.42)
(0.94, -0.30, 1.41)
(0.96, -0.24, 1.40)
(1.00, -0.17, 1.40)
(1.00, -0.10, 1.42)
(0.99, -0.01, 1.43)
(0.97, 0.08, 1.44)
(0.94, 0.18, 1.43)
(0.88, 0.26, 1.42)
(0.82, 0.34, 1.41)
(0.74, 0.39, 1.43)
(0.66, 0.42, 1.44)
(0.57, 0.43, 1.44)
(0.48, 0.41, 1.46)
(0.41, 0.35, 1.47)
(0.34, 0.30, 1.48)
(0.27, 0.26, 1.50)
(0.21, 0.19, 1.50)
(0.17, 0.11, 1.50)
(0.12, 0.05, 1.52)
(0.06, -0.01, 1.52)
(0.00, -0.07, 1.53)
(-0.05, -0.13, 1.54)
(-0.09, -0.20, 1.53)
(-0.14, -0.25, 1.52)
(-0.21, -0.29, 1.53)
(-0.26, -0.34, 1.52)
(-0.33, -0.36, 1.53)
(-0.40, -0.36, 1.54)
(-0.48, -0.35, 1.57)
(-0.56, -0.34, 1.57)
(-0.65, -0.31, 1.59)
(-0.72, -0.30, 1.60)
(-0.80, -0.29, 1.60)
(-0.88, -0.28, 1.60)
(-0.96, -0.25, 1.60)
(-1.05, -0.22, 1.63)
(-1.11, -0.17, 1.61)
(-1.14, -0.07, 1.62)
(-1.15, 0.04, 1.64)
(-1.13, 0.15, 1.64)
(-1.09, 0.26, 1.65)
(-1.03, 0.38, 1.64)
(-0.94, 0.49, 1.64)
(-0.83, 0.56, 1.64)
(-0.72, 0.59, 1.63)
(-0.60, 0.57, 1.62)
(-0.49, 0.54, 1.60)
(-0.39, 0.50, 1.60)
(-0.30, 0.42, 1.60)
(-0.23, 0.33, 1.60)
(-0.16, 0.24, 1.59)
(-0.11, 0.16, 1.60)
(-0.07, 0.10, 1.60)
(-0.02, 0.05, 1.59)
(0.03, 0.01, 1.60)
(0.06, -0.03, 1.60)
(0.10, -0.09, 1.60)
(0.15, -0.13, 1.60)
(0.20, -0.17, 1.60)
(0.25, -0.21, 1.59)
(0.30, -0.25, 1.60)
(0.35, -0.29, 1.60)
(0.40, -0.34, 1.62)
(0.45, -0.39, 1.58)
(0.42, -0.38, 1.31)
(0.35, -0.31, 0.98)
(0.26, -0.25, 0.66)
(0.16, -0.19, 0.43)
(0.06, -0.12, 0.24)
(-0.07, -0.04, 0.11)
(-0.19, 0.01, 0.06)
(-0.30, 0.08, 0.11)
(-0.44, 0.14, 0.08)
};


==> plots/traj_coords_kitti_00.tex <==
%
\addplot[
    fill=none,draw = gtclr,
    very thick,
    line width= 0.5pt,%dashed,dash pattern=on 19pt off 1pt,
   % mark = square*,
   % mark size = \mrksize ex,
   % mark options = {fill=mtrnclr,draw=mdtrnclr}
    ]
    coordinates {
(-0.374955, 6.86548)
(-0.799251, 14.6003)
(-1.28081, 22.7743)
(-1.72889, 31.3776)
(-2.25611, 40.5386)
(-2.87134, 49.556)
(-3.43899, 58.274)
(-4.04663, 66.4216)
(-4.64434, 73.4807)
(-5.1338, 79.0495)
(-5.10562, 83.4545)
(-3.65638, 86.8121)
(-0.811071, 88.6416)
(2.66275, 89.3721)
(7.05038, 89.6547)
(12.7819, 89.7273)
(19.7682, 90.0334)
(27.1001, 90.4578)
(34.3242, 90.5624)
(41.1457, 90.0029)
(47.144, 89.2445)
(51.9638, 89.3356)
(55.8359, 91.2711)
(57.8124, 94.9816)
(58.814, 99.4609)
(60.1342, 104.754)
(61.6963, 110.929)
(63.3346, 118.012)
(65.0663, 125.571)
(66.9321, 133.06)
(68.6553, 140.266)
(70.1315, 147.439)
(71.1483, 154.665)
(71.665, 162.055)
(71.9307, 169.517)
(71.8005, 177.11)
(71.4196, 184.763)
(70.9642, 192.373)
(70.5038, 199.316)
(70.1277, 205.673)
(70.0195, 211.65)
(69.9828, 217.579)
(69.9843, 223.672)
(69.9243, 229.793)
(69.7828, 235.366)
(69.0222, 239.832)
(66.6729, 243.07)
(63.3085, 244.683)
(58.8856, 244.928)
(53.3377, 244.676)
(46.3819, 244.141)
(38.579, 243.742)
(30.7198, 243.393)
(23.0473, 243.115)
(15.7015, 242.743)
(8.78779, 242.07)
(2.90781, 241.566)
(-1.71713, 241.331)
(-4.94315, 241.365)
(-6.29222, 241.448)
(-6.44116, 241.459)
(-6.52834, 241.506)
(-7.43398, 241.575)
(-9.58823, 242.097)
(-12.0792, 243.81)
(-13.7224, 247.382)
(-14.2404, 252.724)
(-14.4473, 259.441)
(-14.7087, 267.323)
(-15.0353, 276.156)
(-15.3859, 285.556)
(-15.8349, 295.036)
(-16.3343, 304.294)
(-16.7963, 313.525)
(-17.2237, 323.046)
(-17.719, 332.731)
(-18.2397, 342.181)
(-18.7551, 350.925)
(-19.1908, 358.545)
(-19.4354, 364.405)
(-19.8922, 368.628)
(-21.4873, 372.119)
(-24.8287, 374.589)
(-29.7222, 374.987)
(-35.494, 374.385)
(-42.2942, 373.768)
(-50.2374, 373.372)
(-58.4895, 372.995)
(-66.6152, 372.471)
(-74.6131, 371.928)
(-82.4487, 371.697)
(-89.6954, 371.748)
(-95.3669, 371.646)
(-100.61, 371.211)
(-106.301, 370.553)
(-113.039, 369.849)
(-120.918, 369.337)
(-129.739, 369.206)
(-138.668, 369.063)
(-147.377, 368.71)
(-155.902, 368.175)
(-164.145, 367.671)
(-171.495, 367.269)
(-177.288, 366.876)
(-182.023, 365.894)
(-185.6, 363.065)
(-187.125, 358.297)
(-187.125, 352.422)
(-186.533, 345.585)
(-185.65, 337.789)
(-184.9, 329.439)
(-184.28, 321.001)
(-183.812, 312.407)
(-183.379, 303.927)
(-183.123, 295.602)
(-182.673, 287.222)
(-182.2, 278.529)
(-181.699, 269.743)
(-181.084, 260.859)
(-180.435, 251.891)
(-179.932, 243.222)
(-179.522, 235.418)
(-179.377, 228.83)
(-179.212, 223.965)
(-178.021, 220.278)
(-175.108, 217.34)
(-169.939, 215.825)
(-163.501, 215.552)
(-156.333, 215.475)
(-148.465, 215.609)
(-140.354, 216.015)
(-132.361, 216.726)
(-125.076, 217.289)
(-119.254, 217.487)
(-113.898, 217.53)
(-108.833, 218.146)
(-104.504, 220.454)
(-101.724, 224.346)
(-100.635, 229.003)
(-99.5996, 233.386)
(-97.4914, 236.281)
(-94.5647, 237.578)
(-90.6005, 238.207)
(-85.1395, 238.615)
(-78.3389, 238.957)
(-70.8622, 239.412)
(-62.8848, 239.754)
(-55.0029, 240.209)
(-47.4783, 240.662)
(-40.3748, 241.236)
(-34.1275, 241.882)
(-28.6817, 242.373)
(-24.6845, 242.456)
(-22.0347, 242.112)
(-20.5642, 241.693)
(-18.8531, 240.845)
(-16.5856, 238.456)
(-15.2371, 233.988)
(-14.8518, 227.596)
(-14.744, 219.601)
(-14.4053, 210.299)
(-13.8127, 200.191)
(-13.1261, 189.69)
(-12.5669, 178.745)
(-12.0715, 167.326)
(-11.5281, 155.602)
(-10.8965, 143.749)
(-10.197, 132.061)
(-9.55793, 121.055)
(-9.06123, 111.449)
(-8.71459, 103.667)
(-7.82224, 97.7879)
(-5.15833, 93.6208)
(-0.953586, 91.377)
(3.85871, 90.8059)
(9.39952, 90.5012)
(16.0856, 90.2961)
(23.7796, 90.8267)
(31.4479, 91.1112)
(39.0312, 90.5801)
(47.0427, 89.9711)
(54.9685, 88.7868)
(62.4892, 86.3067)
(70.1352, 83.4001)
(77.9348, 79.6788)
(85.8404, 75.5388)
(93.1043, 70.8557)
(99.4513, 65.5908)
(104.867, 61.221)
(109.621, 57.4005)
(114.495, 53.3017)
(120.173, 49.1005)
(126.576, 44.3781)
(133.518, 39.194)
(140.514, 34.0216)
(147.378, 28.9828)
(153.871, 24.1031)
(159.12, 19.8817)
(163.58, 16.8912)
(168.667, 15.9221)
(174.444, 15.959)
(180.751, 15.6593)
(187.511, 15.1305)
(194.461, 14.578)
(201.755, 13.8698)
(209.306, 13.1735)
(216.945, 12.5879)
(224.809, 11.945)
(232.863, 11.2324)
(240.886, 10.4674)
(248.656, 9.85093)
(255.834, 9.34923)
(261.61, 8.66233)
(266.653, 7.72685)
(270.378, 6.91568)
(272.708, 6.86317)
(274.935, 7.80851)
(276.761, 11.2513)
(278.292, 14.9831)
(279.006, 21.2127)
(279.43, 28.9818)
(280.048, 37.5955)
(280.691, 46.6382)
(281.324, 55.8221)
(282.089, 65.0302)
(282.681, 74.2451)
(283.357, 83.339)
(284.13, 92.3613)
(285.237, 101.285)
(286.642, 109.957)
(287.921, 118.338)
(289.135, 125.865)
(290.524, 132.039)
(291.856, 136.892)
(292.128, 141.677)
(288.832, 145.871)
(285.218, 149.616)
(279.142, 152.489)
(272.241, 156.075)
(264.684, 160.222)
(257.35, 164.953)
(250.164, 170.018)
(242.549, 174.722)
(234.693, 178.932)
(227.043, 183.025)
(219.815, 186.944)
(213.404, 190.278)
(208.298, 192.868)
(204.974, 194.748)
(203.21, 196.106)
(201.474, 197.759)
(198.199, 200.447)
(193.288, 203.734)
(187.275, 207.187)
(180.93, 210.774)
(174.025, 214.609)
(167.327, 218.336)
(161.653, 221.36)
(156.742, 223.119)
(151.588, 223.291)
(145.559, 222.768)
(138.238, 222.213)
(129.721, 221.858)
(120.566, 221.374)
(111.526, 220.772)
(102.797, 220.264)
(94.3437, 219.762)
(86.8534, 219.208)
(80.9726, 219.076)
(75.9606, 220.194)
(72.1689, 223.54)
(70.1277, 228.841)
(69.625, 235.277)
(69.4802, 242.355)
(69.1411, 250.229)
(68.7036, 258.908)
(68.1639, 268.396)
(67.5929, 277.989)
(66.9737, 287.456)
(66.3468, 296.851)
(65.6613, 306.017)
(64.6747, 315.008)
(63.4201, 323.896)
(62.5949, 332.932)
(62.1644, 342.041)
(61.7899, 350.918)
(61.5524, 358.953)
(61.6259, 365.65)
(61.5583, 371.676)
(60.7451, 378.022)
(59.9372, 385.516)
(59.7644, 394.097)
(59.6159, 403.624)
(59.1451, 413.206)
(58.6278, 422.585)
(58.1791, 431.377)
(57.4706, 438.948)
(56.4196, 445.076)
(57.0964, 449.28)
(59.1, 452.419)
(62.1176, 454.031)
(66.9187, 454.289)
(73.0249, 454.594)
(80.359, 455.052)
(88.577, 455.537)
(97.2737, 456.002)
(106.027, 456.486)
(114.663, 456.917)
(122.966, 457.386)
(130.997, 458.22)
(138.748, 459.708)
(146.139, 461.755)
(153.185, 464.427)
(159.891, 467.475)
(166.113, 470.938)
(171.406, 474.442)
(175.306, 477.078)
(178.419, 478.406)
(181.665, 478.385)
(185.324, 476.652)
(189.455, 472.316)
(194.408, 466.101)
(199.985, 458.921)
(205.685, 451.785)
(211.359, 444.786)
(216.925, 437.908)
(222.79, 430.84)
(228.853, 423.583)
(234.911, 416.347)
(239.552, 410.296)
(243.023, 404.864)
(243.761, 399.752)
(241.061, 395.6)
(236.419, 392.301)
(229.928, 389.983)
(221.793, 388.499)
(212.374, 387.365)
(202.413, 386.399)
(192.318, 385.628)
(182.429, 385.082)
(172.834, 384.647)
(163.624, 384.322)
(155.559, 384.244)
(149.059, 383.873)
(144.683, 382.019)
(142.611, 378.231)
(142.15, 373.19)
(142.117, 367.008)
(142.373, 359.412)
(142.836, 350.477)
(143.356, 340.955)
(143.935, 331.394)
(144.534, 321.695)
(145.082, 311.522)
(145.708, 300.964)
(146.39, 290.39)
(147.033, 279.994)
(147.583, 269.77)
(148.136, 259.853)
(148.646, 250.505)
(149.121, 242.376)
(149.628, 235.85)
(149.887, 231.066)
(148.906, 227.392)
(146.332, 224.463)
(141.904, 222.69)
(135.968, 222.086)
(128.45, 221.891)
(119.665, 221.79)
(110.649, 221.433)
(101.893, 220.868)
(93.3962, 220.386)
(85.998, 219.986)
(80.8514, 219.692)
(76.7946, 220.24)
(73.269, 222.355)
(70.7648, 226.272)
(69.6618, 230.754)
(69.3788, 235.602)
(68.5751, 240.383)
(66.0863, 243.807)
(62.0837, 245.413)
(57.1764, 245.424)
(50.8866, 245.111)
(43.0693, 244.864)
(33.9241, 244.386)
(24.2086, 243.837)
(14.6927, 243.168)
(6.01131, 242.398)
(-0.898772, 241.821)
(-5.38651, 241.63)
(-7.77466, 241.793)
(-9.7801, 242.354)
(-12.3443, 244.28)
(-14.1523, 248.337)
(-14.5752, 254.544)
(-14.8075, 262.576)
(-15.1431, 272.307)
(-15.5418, 283.129)
(-16.0525, 294.302)
(-16.5346, 305.63)
(-17.0143, 317.094)
(-17.458, 328.526)
(-17.9072, 339.719)
(-18.4374, 349.999)
(-18.8445, 358.967)
(-19.0282, 366.123)
(-19.4694, 371.274)
(-21.7485, 375.114)
(-25.9991, 376.64)
(-31.3241, 376.002)
(-37.9134, 374.928)
(-46.0267, 374.108)
(-55.3281, 373.487)
(-65.1295, 372.964)
(-74.8798, 372.403)
(-84.3221, 372.038)
(-92.6853, 371.98)
(-100.461, 371.507)
(-108.707, 370.584)
(-118.16, 369.889)
(-128.656, 369.662)
(-139.237, 369.568)
(-149.596, 369.032)
(-159.755, 368.368)
(-169.584, 367.574)
(-179.172, 366.794)
(-188.934, 366.404)
(-198.982, 366.179)
(-209.221, 366.266)
(-219.137, 366.588)
(-227.921, 367.27)
(-235.114, 368.132)
(-240.419, 369.488)
(-244.445, 370.305)
(-248.075, 370.349)
(-251.934, 370.328)
(-255.594, 370.683)
(-258.51, 371.064)
(-261.591, 370.649)
(-265.073, 368.376)
(-267.747, 363.423)
(-269.143, 356.261)
(-269.898, 347.268)
(-270.68, 337.052)
(-271.176, 326.314)
(-271.249, 315.743)
(-270.853, 305.405)
(-270.034, 295.14)
(-268.845, 284.7)
(-267.26, 274.057)
(-265.198, 263.244)
(-262.579, 252.269)
(-259.463, 241.442)
(-255.948, 230.73)
(-252.024, 220.231)
(-247.875, 209.945)
(-243.384, 199.871)
(-238.542, 190.099)
(-233.429, 180.624)
(-227.826, 171.098)
(-221.725, 161.612)
(-215.317, 152.527)
(-208.738, 143.823)
(-201.784, 135.401)
(-194.37, 127.108)
(-186.413, 118.972)
(-177.941, 111.012)
(-169.07, 103.08)
(-160.138, 95.1341)
(-151.375, 87.1795)
(-142.661, 79.2116)
(-133.841, 71.3081)
(-125.063, 63.4304)
(-116.347, 55.6177)
(-107.627, 47.7627)
(-98.7983, 39.8416)
(-89.9029, 31.8743)
(-80.937, 23.913)
(-72.0573, 16.0914)
(-63.479, 8.33949)
(-55.2218, 0.803962)
(-47.6438, -5.97309)
(-41.0314, -11.6624)
(-35.0974, -15.7607)
(-28.8658, -17.5816)
(-22.8954, -16.5017)
(-17.9524, -13.4394)
(-13.3933, -10.5221)
(-9.55004, -8.37838)
(-6.96563, -7.11644)
(-5.11593, -5.95142)
(-3.25196, -4.06313)
(-1.44429, -0.709844)
(-0.490261, 4.69745)
(-0.624242, 11.8178)
(-0.950867, 20.107)
(-1.55834, 29.342)
(-2.31714, 39.1346)
(-2.98182, 49.2229)
(-3.50209, 59.6613)
(-4.09956, 70.3664)
(-4.72637, 80.9688)
(-5.32954, 91.2949)
    };
%
%
\addplot[
    fill=none,draw = orbclr,
    very thick,
    line width= 0.5pt,
   % mark = square*,
   % mark size = \mrksize ex,
   % mark options = {fill=mtrnclr,draw=mdtrnclr}
    ]
    coordinates {
    (-0.162895, 5.84004)
(-0.589263, 13.3235)
(-1.11735, 21.4374)
(-1.63194, 29.9744)
(-2.19616, 38.8158)
(-2.84627, 47.6751)
(-3.46146, 56.2963)
(-4.17327, 64.3966)
(-4.86622, 71.3926)
(-5.43116, 76.9644)
(-5.42764, 81.3865)
(-4.02807, 84.7555)
(-1.22806, 86.6066)
(2.19065, 87.3643)
(6.54758, 87.6933)
(12.2874, 87.8522)
(19.2362, 88.2602)
(26.604, 88.7938)
(33.8243, 89.0046)
(40.6408, 88.5575)
(46.6523, 87.8975)
(51.4133, 88.0613)
(55.275, 90.0397)
(57.1848, 93.6888)
(58.1048, 98.1058)
(59.3521, 103.357)
(60.8031, 109.532)
(62.3103, 116.602)
(63.9136, 124.042)
(65.6136, 131.458)
(67.1236, 138.683)
(68.4585, 145.825)
(69.356, 152.991)
(69.7839, 160.338)
(69.973, 167.74)
(69.7671, 175.24)
(69.2968, 182.869)
(68.7247, 190.449)
(68.1453, 197.674)
(67.6986, 203.835)
(67.6171, 209.68)
(67.5574, 215.622)
(67.4039, 221.879)
(67.1951, 228.068)
(66.9391, 233.693)
(66.0908, 238.054)
(63.7901, 241.143)
(60.4219, 242.667)
(56.0438, 242.768)
(50.4628, 242.39)
(43.261, 241.981)
(35.2936, 241.555)
(27.4689, 240.927)
(19.8971, 240.434)
(12.619, 239.87)
(5.74155, 239.089)
(-0.132441, 238.483)
(-4.761, 238.189)
(-7.96789, 238.158)
(-9.30275, 238.191)
(-9.4408, 238.193)
(-9.53162, 238.202)
(-10.4401, 238.254)
(-12.5392, 238.749)
(-15.0154, 240.462)
(-16.7042, 244.071)
(-17.2934, 249.423)
(-17.5718, 256.081)
(-17.944, 263.874)
(-18.3794, 272.601)
(-18.8957, 281.978)
(-19.5558, 291.343)
(-20.2245, 300.53)
(-20.8519, 309.662)
(-21.4516, 319.141)
(-22.0419, 328.752)
(-22.6117, 338.087)
(-23.2219, 346.772)
(-23.7427, 354.376)
(-24.0778, 360.264)
(-24.5928, 364.48)
(-26.1401, 367.742)
(-29.4472, 370.145)
(-34.3876, 370.427)
(-40.1109, 369.73)
(-46.8981, 369.015)
(-54.8591, 368.452)
(-63.1036, 367.906)
(-71.2332, 367.182)
(-79.2309, 366.442)
(-87.1296, 366.057)
(-94.3731, 365.973)
(-100.043, 365.737)
(-105.283, 365.166)
(-110.982, 364.381)
(-117.684, 363.563)
(-125.533, 362.906)
(-134.302, 362.676)
(-143.208, 362.339)
(-151.916, 361.789)
(-160.415, 361.069)
(-168.626, 360.389)
(-175.954, 359.879)
(-181.74, 359.378)
(-186.428, 358.308)
(-189.859, 355.5)
(-191.269, 350.695)
(-191.159, 344.858)
(-190.456, 337.993)
(-189.471, 330.165)
(-188.563, 321.819)
(-187.807, 313.426)
(-187.195, 304.875)
(-186.592, 296.454)
(-186.106, 288.135)
(-185.435, 279.704)
(-184.774, 271.032)
(-184.108, 262.185)
(-183.306, 253.244)
(-182.468, 244.291)
(-181.771, 235.647)
(-181.199, 227.8)
(-180.9, 221.164)
(-180.622, 216.276)
(-179.352, 212.704)
(-176.364, 209.778)
(-171.299, 208.322)
(-165.049, 208.288)
(-157.997, 208.49)
(-150.174, 208.88)
(-142.101, 209.566)
(-134.142, 210.515)
(-126.854, 211.277)
(-120.996, 211.587)
(-115.603, 211.72)
(-110.544, 212.327)
(-106.253, 214.634)
(-103.664, 218.48)
(-102.653, 222.946)
(-101.61, 227.301)
(-99.4917, 230.178)
(-96.4249, 231.541)
(-92.308, 232.188)
(-86.8504, 232.695)
(-80.1628, 233.239)
(-72.7205, 233.684)
(-64.8365, 234.186)
(-57.0836, 234.838)
(-49.6021, 235.495)
(-42.5397, 236.204)
(-36.2744, 236.898)
(-30.8066, 237.381)
(-26.7991, 237.477)
(-24.1904, 237.223)
(-22.7227, 236.815)
(-21.0612, 236.042)
(-18.7353, 233.689)
(-17.3745, 229.211)
(-16.9273, 222.827)
(-16.6814, 214.857)
(-16.2004, 205.644)
(-15.4515, 195.591)
(-14.6252, 185.153)
(-13.9282, 174.231)
(-13.2818, 162.816)
(-12.6149, 151.135)
(-11.853, 139.512)
(-11.0369, 128.048)
(-10.2161, 117.179)
(-9.59426, 107.693)
(-9.17105, 100.043)
(-8.21333, 94.3464)
(-5.57804, 90.3838)
(-1.50474, 88.3779)
(3.1609, 88.0243)
(8.6841, 87.949)
(15.3682, 87.9379)
(23.0592, 88.6243)
(30.7671, 89.0133)
(38.3738, 88.6497)
(46.4035, 88.2398)
(54.3332, 87.2684)
(61.8355, 84.9656)
(69.4229, 82.2396)
(77.2343, 78.6879)
(85.1206, 74.7352)
(92.4261, 70.2305)
(98.8389, 65.1256)
(104.311, 60.9079)
(109.089, 57.21)
(113.99, 53.251)
(119.67, 49.1911)
(126.122, 44.5952)
(133.12, 39.5475)
(140.176, 34.5008)
(147.11, 29.5577)
(153.661, 24.8138)
(158.992, 20.712)
(163.423, 17.8936)
(168.465, 17.005)
(174.205, 17.047)
(180.504, 16.7883)
(187.22, 16.3217)
(194.207, 15.89)
(201.504, 15.308)
(209.054, 14.7329)
(216.687, 14.2583)
(224.548, 13.7074)
(232.635, 13.1187)
(240.673, 12.4824)
(248.548, 11.9386)
(255.737, 11.5347)
(261.883, 11.0739)
(266.898, 10.1654)
(270.264, 9.39171)
(272.549, 9.38624)
(274.696, 10.3646)
(276.581, 13.0672)
(277.789, 17.6273)
(278.357, 23.9852)
(278.685, 31.8324)
(279.259, 40.4569)
(279.836, 49.4977)
(280.387, 58.5794)
(281.079, 67.6744)
(281.627, 76.7827)
(282.191, 85.8203)
(282.887, 94.868)
(283.933, 103.816)
(285.246, 112.485)
(286.426, 120.847)
(287.505, 128.432)
(288.799, 134.643)
(290.053, 139.53)
(290.255, 144.282)
(288.218, 148.716)
(283.722, 151.921)
(277.665, 154.76)
(270.75, 158.241)
(263.153, 162.272)
(255.799, 166.878)
(248.556, 171.805)
(240.856, 176.36)
(232.95, 180.4)
(225.244, 184.347)
(217.943, 188.139)
(211.487, 191.352)
(206.325, 193.851)
(202.944, 195.651)
(201.114, 196.905)
(199.28, 198.347)
(195.945, 200.942)
(191.168, 204.119)
(185.229, 207.419)
(178.569, 210.967)
(171.596, 214.71)
(164.842, 218.325)
(159.103, 221.23)
(154.18, 222.893)
(149.061, 222.957)
(142.994, 222.365)
(135.654, 221.714)
(127.113, 221.245)
(117.918, 220.652)
(108.835, 219.942)
(100.081, 219.327)
(91.6456, 218.726)
(84.0902, 218)
(78.1649, 217.756)
(73.1079, 218.771)
(69.2087, 221.987)
(67.1202, 227.19)
(66.5808, 233.63)
(66.2947, 240.773)
(65.8158, 248.596)
(65.269, 257.2)
(64.6721, 266.576)
(63.9985, 276.086)
(63.2841, 285.472)
(62.6219, 294.674)
(61.8891, 303.733)
(60.8717, 312.578)
(59.5477, 321.349)
(58.6434, 330.268)
(58.0191, 339.339)
(57.5072, 348.24)
(57.1268, 356.214)
(57.1137, 362.922)
(56.9422, 368.89)
(56.0075, 375.136)
(55.0741, 382.54)
(54.7347, 391.144)
(54.387, 400.639)
(53.7469, 410.195)
(53.1087, 419.534)
(52.5313, 428.346)
(51.7299, 435.867)
(50.5984, 442.016)
(50.5454, 446.604)
(52.7547, 449.739)
(56.2676, 450.989)
(61.0466, 451.284)
(67.113, 451.696)
(74.3893, 452.329)
(82.5568, 452.999)
(91.156, 453.652)
(99.8652, 454.268)
(108.427, 454.863)
(116.722, 455.493)
(124.713, 456.474)
(132.406, 458.113)
(139.763, 460.27)
(146.756, 463.029)
(153.379, 466.215)
(159.521, 469.808)
(164.708, 473.451)
(168.604, 476.135)
(171.74, 477.488)
(175.037, 477.563)
(178.767, 475.824)
(182.977, 471.537)
(188.009, 465.454)
(193.665, 458.408)
(199.452, 451.439)
(205.221, 444.59)
(210.86, 437.902)
(216.873, 431.011)
(223.054, 423.821)
(229.179, 416.906)
(234.598, 410.681)
(237.977, 405.581)
(238.41, 400.57)
(235.783, 396.321)
(231.166, 392.872)
(224.645, 390.46)
(216.482, 388.813)
(207.055, 387.549)
(197.107, 386.443)
(187.008, 385.568)
(177.121, 384.862)
(167.534, 384.23)
(158.402, 383.71)
(150.358, 383.446)
(143.934, 382.921)
(139.718, 381.033)
(137.728, 377.183)
(137.353, 372.203)
(137.41, 366.071)
(137.799, 358.501)
(138.459, 349.606)
(139.165, 340.154)
(139.895, 330.644)
(140.576, 321.008)
(141.237, 310.976)
(141.912, 300.521)
(142.67, 289.994)
(143.466, 279.639)
(144.16, 269.489)
(144.856, 259.622)
(145.462, 250.283)
(146.049, 242.193)
(146.664, 235.65)
(147.004, 230.854)
(146.103, 227.128)
(143.585, 224.074)
(139.239, 222.139)
(133.461, 221.364)
(125.935, 220.95)
(117.133, 220.509)
(108.13, 219.863)
(99.3665, 219.195)
(90.8928, 218.548)
(83.4975, 217.958)
(78.3027, 217.734)
(74.2437, 218.188)
(70.7042, 220.117)
(68.148, 223.76)
(67.0412, 228.225)
(66.7201, 233.025)
(65.8478, 237.644)
(63.2674, 241.124)
(59.2505, 242.672)
(54.3951, 242.595)
(48.1323, 242.267)
(40.3189, 241.858)
(31.1278, 241.196)
(21.3848, 240.489)
(11.8728, 239.666)
(3.25404, 238.778)
(-3.62275, 238.124)
(-8.05474, 237.884)
(-10.4242, 238.032)
(-12.3895, 238.577)
(-14.9703, 240.42)
(-16.8504, 244.486)
(-17.3026, 250.746)
(-17.652, 258.761)
(-18.1846, 268.456)
(-18.8481, 279.179)
(-19.6046, 290.259)
(-20.2997, 301.522)
(-21.0059, 312.9)
(-21.761, 324.292)
(-22.4332, 335.442)
(-23.1248, 345.683)
(-23.6632, 354.648)
(-23.9746, 361.747)
(-24.5253, 366.755)
(-26.7227, 370.281)
(-30.948, 371.75)
(-36.2087, 370.924)
(-42.7118, 369.753)
(-50.8197, 368.834)
(-60.1008, 368.087)
(-69.8712, 367.386)
(-79.5872, 366.612)
(-89.0327, 366.035)
(-97.3969, 365.784)
(-105.148, 365.127)
(-113.37, 364.017)
(-122.759, 363.137)
(-133.172, 362.692)
(-143.687, 362.381)
(-154.016, 361.65)
(-164.129, 360.784)
(-173.936, 359.814)
(-183.522, 358.873)
(-193.242, 358.29)
(-203.267, 357.858)
(-213.466, 357.734)
(-223.352, 357.839)
(-232.138, 358.34)
(-239.329, 359.062)
(-244.651, 360.312)
(-248.674, 361.047)
(-252.273, 361.017)
(-256.124, 360.947)
(-259.784, 361.229)
(-262.696, 361.569)
(-265.728, 361.122)
(-269.177, 358.83)
(-271.686, 353.889)
(-272.92, 346.78)
(-273.486, 337.793)
(-273.991, 327.563)
(-274.204, 316.868)
(-273.984, 306.275)
(-273.272, 295.992)
(-272.178, 285.828)
(-270.729, 275.498)
(-268.895, 264.999)
(-266.61, 254.342)
(-263.743, 243.591)
(-260.398, 232.965)
(-256.696, 222.544)
(-252.575, 212.258)
(-248.255, 202.171)
(-243.61, 192.263)
(-238.625, 182.742)
(-233.351, 173.456)
(-227.661, 164.285)
(-221.459, 155.144)
(-214.95, 146.291)
(-208.251, 137.802)
(-201.242, 129.604)
(-193.767, 121.535)
(-185.801, 113.616)
(-177.32, 105.826)
(-168.447, 98.1556)
(-159.466, 90.4384)
(-150.67, 82.7207)
(-141.932, 75.0041)
(-133.138, 67.322)
(-124.342, 59.6575)
(-115.591, 51.9996)
(-106.853, 44.3656)
(-97.9964, 36.6912)
(-89.0905, 28.9632)
(-80.1258, 21.2423)
(-71.249, 13.6345)
(-62.6433, 6.07782)
(-54.3496, -1.28632)
(-46.7344, -7.94222)
(-40.0701, -13.5403)
(-34.105, -17.554)
(-27.9079, -19.2994)
(-22.0815, -18.1494)
(-17.185, -15.0255)
(-12.6448, -11.9962)
(-8.79817, -9.73643)
(-6.22128, -8.35036)
(-4.37337, -7.18218)
(-2.55828, -5.27849)
(-0.823766, -1.97881)
(0.118785, 3.26273)
(-0.12186, 10.1971)
(-0.57241, 18.458)
(-1.27093, 27.6753)
(-2.15294, 37.3778)
(-2.96907, 47.4001)
(-3.67638, 57.7424)
(-4.44211, 68.3684)
(-5.17551, 78.9634)
(-5.91687, 89.1972)
};
 %    
 %
\addplot[
    fill=none,draw = predclr,
    very thick,
    line width= 0.5pt,%dashed,dash pattern=on 19pt off 1pt,
   % mark = square*,
   % mark size = \mrksize ex,
   % mark options = {fill=mtrnclr,draw=mdtrnclr}
    ]
    coordinates {
    (-0.0497278, 5.81235)
(-0.442371, 13.3256)
(-1.01605, 21.5104)
(-1.56638, 30.1126)
(-2.18918, 39.0168)
(-2.90153, 47.8711)
(-3.57163, 56.5111)
(-4.32114, 64.6196)
(-5.0465, 71.6365)
(-5.68091, 77.2287)
(-5.68061, 81.6996)
(-4.29766, 85.1063)
(-1.49114, 86.9965)
(1.92277, 87.7526)
(6.27992, 88.1059)
(11.999, 88.3005)
(18.9576, 88.7233)
(26.2609, 89.2822)
(33.4894, 89.5225)
(40.3055, 89.0896)
(46.2529, 88.4535)
(51.0713, 88.6537)
(54.8555, 90.631)
(56.7485, 94.2935)
(57.6348, 98.7505)
(58.8175, 104.088)
(60.2126, 110.313)
(61.6666, 117.409)
(63.222, 124.943)
(64.8683, 132.458)
(66.3338, 139.706)
(67.6155, 146.904)
(68.4739, 154.119)
(68.8565, 161.512)
(69.0043, 168.919)
(68.7496, 176.44)
(68.2311, 184.113)
(67.6279, 191.705)
(67.0105, 198.928)
(66.5556, 205.087)
(66.4455, 210.917)
(66.3622, 216.838)
(66.1743, 223.061)
(65.9264, 229.282)
(65.6428, 234.996)
(64.806, 239.417)
(62.4651, 242.58)
(59.036, 244.057)
(54.5748, 244.182)
(48.9632, 243.774)
(41.7148, 243.353)
(33.7467, 242.892)
(25.9348, 242.232)
(18.3503, 241.712)
(10.9988, 241.135)
(4.06392, 240.319)
(-1.84189, 239.696)
(-6.55778, 239.373)
(-9.81381, 239.326)
(-11.1508, 239.351)
(-11.2873, 239.371)
(-11.3809, 239.367)
(-12.2875, 239.422)
(-14.4466, 239.905)
(-16.9241, 241.62)
(-18.707, 245.303)
(-19.286, 250.702)
(-19.6115, 257.389)
(-19.9685, 265.221)
(-20.4346, 273.998)
(-20.9718, 283.386)
(-21.6337, 292.802)
(-22.3056, 302.019)
(-22.935, 311.202)
(-23.5253, 320.669)
(-24.106, 330.285)
(-24.6713, 339.638)
(-25.2754, 348.317)
(-25.8161, 355.914)
(-26.149, 361.824)
(-26.6509, 366.086)
(-28.2162, 369.36)
(-31.5229, 371.822)
(-36.6253, 372.169)
(-42.422, 371.461)
(-49.2435, 370.733)
(-57.1802, 370.147)
(-65.4571, 369.57)
(-73.6003, 368.807)
(-81.6227, 368.047)
(-89.5129, 367.622)
(-96.85, 367.506)
(-102.524, 367.234)
(-107.798, 366.638)
(-113.521, 365.82)
(-120.256, 364.956)
(-128.155, 364.24)
(-137.05, 363.961)
(-146.006, 363.574)
(-154.723, 362.941)
(-163.243, 362.168)
(-171.487, 361.451)
(-178.841, 360.884)
(-184.653, 360.342)
(-189.38, 359.222)
(-192.829, 356.38)
(-194.233, 351.522)
(-194.08, 345.64)
(-193.318, 338.713)
(-192.251, 330.849)
(-191.287, 322.47)
(-190.456, 314.037)
(-189.799, 305.4)
(-189.132, 296.948)
(-188.586, 288.554)
(-187.812, 280.05)
(-187.09, 271.38)
(-186.374, 262.548)
(-185.474, 253.627)
(-184.512, 244.62)
(-183.713, 235.977)
(-183.038, 228.109)
(-182.67, 221.426)
(-182.354, 216.503)
(-181.031, 212.856)
(-177.939, 209.933)
(-172.926, 208.541)
(-166.664, 208.545)
(-159.576, 208.803)
(-151.741, 209.243)
(-143.707, 209.955)
(-135.765, 210.974)
(-128.459, 211.77)
(-122.567, 212.147)
(-117.166, 212.291)
(-112.093, 212.931)
(-107.823, 215.233)
(-105.305, 219.103)
(-104.301, 223.561)
(-103.299, 227.91)
(-101.191, 230.809)
(-98.112, 232.204)
(-93.9851, 232.877)
(-88.5283, 233.438)
(-81.8387, 234.01)
(-74.4227, 234.509)
(-66.5732, 235.054)
(-58.8073, 235.754)
(-51.3199, 236.458)
(-44.2433, 237.207)
(-37.961, 237.958)
(-32.4715, 238.485)
(-28.3886, 238.626)
(-25.733, 238.399)
(-24.2452, 237.994)
(-22.5217, 237.203)
(-20.1462, 234.843)
(-18.7333, 230.355)
(-18.2439, 223.898)
(-17.9317, 215.902)
(-17.3709, 206.651)
(-16.521, 196.518)
(-15.5872, 186.059)
(-14.781, 175.124)
(-14.0436, 163.619)
(-13.3024, 151.875)
(-12.4616, 140.232)
(-11.5623, 128.727)
(-10.6782, 117.825)
(-9.98808, 108.262)
(-9.49862, 100.604)
(-8.49602, 94.7727)
(-5.79583, 90.703)
(-1.74228, 88.7443)
(2.91806, 88.4008)
(8.41226, 88.3708)
(15.0931, 88.3942)
(22.7299, 89.0958)
(30.4329, 89.5229)
(38.0387, 89.1928)
(45.9914, 88.8007)
(54.1155, 87.9834)
(61.6739, 85.7054)
(69.2752, 82.9827)
(77.1347, 79.4325)
(85.0427, 75.4953)
(92.3649, 70.989)
(98.8186, 65.8943)
(104.35, 61.6835)
(109.163, 58.013)
(114.096, 54.059)
(119.812, 50.0147)
(126.348, 45.434)
(133.385, 40.404)
(140.459, 35.4045)
(147.38, 30.5294)
(153.928, 25.8208)
(159.249, 21.7673)
(163.695, 18.9472)
(168.733, 18.0961)
(174.453, 18.1518)
(180.711, 17.9242)
(187.401, 17.4665)
(194.397, 17.047)
(201.714, 16.4845)
(209.233, 15.9229)
(216.854, 15.4688)
(224.732, 14.9325)
(232.813, 14.3469)
(240.888, 13.7165)
(248.755, 13.1814)
(255.94, 12.799)
(262.157, 12.3601)
(267.195, 11.4495)
(270.601, 10.6788)
(272.943, 10.6748)
(275.116, 11.6648)
(276.97, 14.3771)
(278.196, 18.9748)
(278.762, 25.3509)
(279.087, 33.1568)
(279.662, 41.7956)
(280.242, 50.8075)
(280.813, 59.8582)
(281.5, 68.9266)
(282.053, 78.0414)
(282.626, 87.1026)
(283.307, 96.1561)
(284.352, 105.164)
(285.637, 113.85)
(286.816, 122.238)
(287.881, 129.881)
(289.183, 136.133)
(290.467, 141.07)
(290.648, 145.845)
(288.567, 150.349)
(283.986, 153.59)
(277.889, 156.43)
(270.913, 159.922)
(263.26, 163.957)
(255.827, 168.581)
(248.49, 173.5)
(240.722, 178.046)
(232.728, 182.085)
(224.962, 186.024)
(217.604, 189.805)
(211.168, 192.972)
(205.973, 195.485)
(202.56, 197.31)
(200.701, 198.553)
(198.847, 200.023)
(195.457, 202.632)
(190.689, 205.778)
(184.738, 209.054)
(178.063, 212.581)
(171.094, 216.296)
(164.321, 219.863)
(158.573, 222.718)
(153.645, 224.325)
(148.47, 224.367)
(142.411, 223.75)
(135.096, 223.063)
(126.468, 222.56)
(117.18, 221.933)
(108.027, 221.17)
(99.2191, 220.524)
(90.6793, 219.895)
(83.0582, 219.172)
(77.065, 218.882)
(71.956, 219.877)
(68.028, 223.106)
(65.8893, 228.374)
(65.2949, 234.964)
(64.994, 242.139)
(64.3837, 250.098)
(63.8336, 258.903)
(63.2114, 268.319)
(62.5236, 277.843)
(61.7854, 287.244)
(61.1237, 296.467)
(60.3712, 305.513)
(59.3453, 314.388)
(58.0018, 323.189)
(57.1444, 332.033)
(56.4846, 341.191)
(55.9359, 350.118)
(55.5391, 358.161)
(55.4804, 364.909)
(55.2577, 370.914)
(54.269, 377.197)
(53.3404, 384.605)
(52.9693, 393.233)
(52.5818, 402.724)
(51.9318, 412.237)
(51.2517, 421.588)
(50.6449, 430.406)
(49.7949, 438.012)
(48.6388, 444.12)
(48.5862, 448.735)
(50.8136, 451.871)
(54.3612, 453.193)
(59.1374, 453.525)
(65.1615, 453.974)
(72.425, 454.672)
(80.5413, 455.382)
(89.1724, 456.108)
(97.8983, 456.817)
(106.489, 457.501)
(114.757, 458.228)
(122.747, 459.28)
(130.417, 460.948)
(137.754, 463.203)
(144.742, 466.029)
(151.374, 469.297)
(157.505, 472.991)
(162.707, 476.7)
(166.63, 479.411)
(169.785, 480.812)
(173.111, 480.922)
(176.93, 479.208)
(181.15, 474.897)
(186.188, 468.818)
(191.916, 461.77)
(197.767, 454.797)
(203.603, 447.899)
(209.335, 441.176)
(215.406, 434.273)
(221.681, 427.075)
(227.89, 420.143)
(233.311, 413.944)
(236.778, 408.783)
(237.254, 403.658)
(234.646, 399.316)
(229.994, 395.883)
(223.45, 393.44)
(215.247, 391.721)
(205.734, 390.375)
(195.781, 389.195)
(185.726, 388.237)
(175.771, 387.453)
(166.153, 386.747)
(157.046, 386.113)
(148.941, 385.785)
(142.449, 385.196)
(138.217, 383.243)
(136.291, 379.378)
(135.918, 374.32)
(136.022, 368.187)
(136.489, 360.562)
(137.215, 351.645)
(137.996, 342.119)
(138.815, 332.533)
(139.588, 322.894)
(140.343, 312.817)
(141.149, 302.337)
(142.017, 291.839)
(142.98, 281.66)
(143.701, 271.316)
(144.464, 261.336)
(145.122, 251.911)
(145.722, 243.765)
(146.38, 237.185)
(146.745, 232.371)
(145.859, 228.601)
(143.353, 225.483)
(138.969, 223.507)
(133.331, 222.795)
(125.266, 222.283)
(116.387, 221.784)
(107.315, 221.081)
(98.4912, 220.388)
(89.9335, 219.724)
(82.4585, 219.124)
(77.1911, 218.856)
(73.099, 219.282)
(69.5337, 221.251)
(66.9364, 224.919)
(65.8006, 229.428)
(65.4243, 234.344)
(64.5676, 238.999)
(61.9473, 242.523)
(57.8243, 244.078)
(52.9192, 244.005)
(46.6337, 243.648)
(38.7665, 243.217)
(29.5994, 242.51)
(19.8338, 241.781)
(10.2417, 240.918)
(1.55274, 240.007)
(-5.39531, 239.312)
(-9.89819, 239.047)
(-12.2958, 239.203)
(-14.2907, 239.735)
(-16.8941, 241.582)
(-18.8501, 245.714)
(-19.3011, 252.03)
(-19.6688, 260.087)
(-20.2398, 269.827)
(-20.9195, 280.589)
(-21.6744, 291.704)
(-22.3794, 303.009)
(-23.0824, 314.451)
(-23.8307, 325.855)
(-24.5067, 336.997)
(-25.1963, 347.22)
(-25.729, 356.19)
(-26.0431, 363.325)
(-26.6003, 368.362)
(-28.8148, 371.957)
(-33.0618, 373.488)
(-38.5162, 372.68)
(-45.0446, 371.481)
(-53.1621, 370.527)
(-62.4491, 369.762)
(-72.2364, 369.017)
(-81.9818, 368.214)
(-91.4433, 367.591)
(-99.8614, 367.287)
(-107.659, 366.597)
(-115.923, 365.448)
(-125.358, 364.493)
(-135.913, 363.98)
(-146.508, 363.61)
(-156.819, 362.784)
(-166.95, 361.866)
(-176.814, 360.828)
(-186.449, 359.833)
(-196.191, 359.204)
(-206.297, 358.695)
(-216.554, 358.502)
(-226.482, 358.539)
(-235.345, 358.984)
(-242.583, 359.629)
(-247.963, 360.861)
(-252.029, 361.569)
(-255.681, 361.512)
(-259.552, 361.41)
(-263.233, 361.667)
(-266.161, 362.044)
(-269.252, 361.593)
(-272.663, 359.21)
(-275.181, 354.137)
(-276.276, 346.971)
(-276.626, 338.03)
(-276.878, 327.867)
(-276.847, 317.148)
(-276.409, 306.552)
(-275.511, 296.332)
(-274.23, 286.235)
(-272.667, 275.948)
(-270.716, 265.428)
(-268.297, 254.718)
(-265.278, 243.888)
(-261.842, 233.34)
(-258.058, 223.013)
(-253.892, 212.759)
(-249.531, 202.671)
(-244.825, 192.759)
(-239.77, 183.105)
(-234.457, 173.871)
(-228.72, 164.668)
(-222.476, 155.568)
(-215.939, 146.622)
(-209.277, 138.115)
(-202.279, 129.897)
(-194.774, 121.783)
(-186.77, 113.809)
(-178.258, 106.002)
(-169.369, 98.311)
(-160.364, 90.5712)
(-151.454, 82.7428)
(-142.667, 75.0054)
(-133.814, 67.2643)
(-124.971, 59.5874)
(-116.24, 52.0234)
(-107.473, 44.3926)
(-98.5903, 36.7343)
(-89.6681, 28.999)
(-80.6273, 21.2353)
(-71.6661, 13.6066)
(-63.0961, 6.08554)
(-54.8568, -1.23598)
(-47.2458, -7.89181)
(-40.5281, -13.5079)
(-34.5294, -17.5492)
(-28.274, -19.3287)
(-22.3398, -18.1697)
(-17.2944, -14.9731)
(-12.6929, -11.8917)
(-8.77745, -9.63963)
(-6.16981, -8.27615)
(-4.29061, -7.11252)
(-2.41083, -5.19385)
(-0.685867, -1.8848)
(0.231492, 3.31689)
(0.0342367, 10.1694)
(-0.442984, 18.536)
(-1.19159, 27.7877)
(-2.10077, 37.5172)
(-3.02543, 47.5949)
(-3.79245, 57.9396)
(-4.5969, 68.5996)
(-5.39895, 79.2598)
(-6.222, 89.5629)
    };

==> plots/traj_coords_kitti_01.tex <==
%
\addplot[
    fill=none,draw = gtclr,
    very thick,
    line width= 0.5pt,%dashed,dash pattern=on 19pt off 1pt,
   % mark = square*,
   % mark size = \mrksize ex,
   % mark options = {fill=mtrnclr,draw=mdtrnclr}
    ]
    coordinates {
(1.65133, 7.74395)
(6.60264, 14.9122)
(13.9228, 19.3353)
(22.7908, 21.1612)
(32.7868, 20.837)
(43.9328, 19.3479)
(56.7869, 17.2895)
(71.2635, 15.0605)
(87.0054, 12.7071)
(103.87, 9.96613)
(121.486, 6.35122)
(139.68, 1.6993)
(158.373, -3.85146)
(177.517, -10.3183)
(197.093, -17.6074)
(216.872, -25.7452)
(236.64, -34.5071)
(256.142, -43.8903)
(275.487, -54.0621)
(295.195, -65.2062)
(315.385, -77.3073)
(335.613, -90.6143)
(355.5, -104.817)
(374.932, -119.705)
(393.78, -135.083)
(412.1, -150.939)
(430.111, -167.032)
(448.053, -183.045)
(466.314, -198.621)
(484.707, -213.983)
(503.187, -229.221)
(521.657, -244.464)
(540.154, -259.675)
(558.659, -274.914)
(577.201, -290.168)
(595.737, -305.28)
(614.332, -320.304)
(632.959, -335.331)
(651.591, -350.282)
(670.271, -365.123)
(688.966, -379.99)
(707.661, -394.866)
(726.406, -409.585)
(745.235, -424.169)
(764.125, -438.722)
(783.155, -453.121)
(802.108, -467.454)
(821.002, -481.757)
(840.12, -495.913)
(859.408, -510.061)
(878.737, -524.161)
(898.035, -537.873)
(917.262, -551.258)
(936.493, -564.466)
(955.815, -577.619)
(975.288, -590.649)
(994.799, -603.656)
(1014.3, -616.538)
(1033.66, -629.253)
(1052.94, -641.685)
(1072.26, -653.885)
(1091.57, -666.014)
(1110.99, -677.958)
(1130.56, -689.743)
(1150.38, -701.445)
(1170.34, -713.151)
(1190.52, -724.974)
(1210.99, -736.846)
(1231.74, -748.631)
(1252.84, -760.312)
(1274.26, -771.987)
(1295.92, -783.615)
(1317.62, -795.117)
(1339.38, -806.469)
(1361.16, -817.723)
(1382.83, -828.785)
(1404.53, -839.66)
(1426.14, -850.304)
(1447.72, -860.771)
(1469.18, -871.014)
(1490.38, -880.993)
(1511.22, -890.723)
(1531.8, -900.202)
(1552.13, -909.42)
(1572.13, -918.423)
(1591.82, -927.467)
(1611.08, -936.747)
(1629.74, -946.249)
(1647.93, -955.672)
(1665.83, -964.686)
(1683.7, -973.196)
(1701.38, -981.52)
(1718.81, -989.593)
(1736.04, -997.293)
(1752.59, -1004.59)
(1768.42, -1011.69)
(1783.1, -1018.6)
(1796.31, -1025.47)
(1807.66, -1033.44)
(1817.03, -1043.27)
(1823.74, -1054.9)
(1827.25, -1067.74)
(1827.6, -1081.14)
(1824.76, -1094.41)
(1818.45, -1106.54)
(1809.25, -1116.63)
(1797.58, -1124.06)
(1784.07, -1128.79)
(1769.48, -1131.52)
(1754.26, -1133.21)
(1738.93, -1134.53)
(1723.74, -1135.68)
(1709.18, -1136.31)
(1695.67, -1135.1)
(1683.2, -1130.94)
(1672.83, -1123.35)
(1665.41, -1112.88)
(1661.32, -1100.69)
(1661, -1087.65)
(1664.44, -1074.72)
(1670.82, -1062.23)
(1678.47, -1049.6)
    };
%
%
\addplot[
    fill=none,draw = orbclr,
    very thick,
    line width= 0.5pt,
   % mark = square*,
   % mark size = \mrksize ex,
   % mark options = {fill=mtrnclr,draw=mdtrnclr}
    ]
    coordinates {
    (-0.162895, 5.84004)
(1.66223, 8.03859)
(6.85354, 15.5899)
(14.6034, 20.3634)
(23.9049, 22.3566)
(34.5617, 22.1171)
(46.3807, 20.7339)
(59.6841, 18.7811)
(74.5, 16.6989)
(90.4204, 14.5213)
(107.319, 11.9612)
(124.944, 8.56559)
(142.965, 4.17678)
(161.327, -0.997574)
(180.05, -7.05808)
(199.266, -13.9117)
(218.727, -21.6632)
(238.162, -30.031)
(257.323, -39.1211)
(276.393, -49.0516)
(295.804, -59.9309)
(315.617, -71.6973)
(335.493, -84.7169)
(355.055, -98.5711)
(374.349, -113.181)
(393.116, -128.367)
(411.275, -144.073)
(429.093, -159.95)
(446.921, -175.783)
(465.019, -191.168)
(483.157, -206.301)
(501.431, -221.398)
(519.534, -236.373)
(537.725, -251.35)
(555.955, -266.5)
(574.21, -281.719)
(592.482, -296.754)
(610.76, -311.71)
(629.145, -326.779)
(647.51, -341.709)
(666.01, -356.553)
(684.402, -371.322)
(702.682, -386.086)
(721.131, -400.906)
(739.642, -415.616)
(758.082, -430.353)
(776.769, -445.021)
(795.245, -459.551)
(813.667, -474.159)
(832.262, -488.675)
(851.067, -503.154)
(870.019, -517.716)
(888.999, -532.017)
(907.75, -545.88)
(926.483, -559.597)
(945.31, -573.204)
(964.105, -586.622)
(983.106, -600.122)
(1001.8, -613.367)
(1020.52, -626.46)
(1039.1, -639.261)
(1057.59, -651.75)
(1076.3, -664.282)
(1094.99, -676.549)
(1113.96, -688.763)
(1133.04, -700.78)
(1152.48, -713.005)
(1171.99, -725.323)
(1191.9, -737.731)
(1211.97, -749.974)
(1232.26, -762.142)
(1252.96, -774.291)
(1273.94, -786.476)
(1295.02, -798.566)
(1316.25, -810.587)
(1337.34, -822.44)
(1358.5, -834.197)
(1379.63, -845.692)
(1400.47, -856.843)
(1421.28, -867.778)
(1442.05, -878.596)
(1462.59, -889.219)
(1482.73, -899.617)
(1502.66, -909.863)
(1522.29, -919.83)
(1541.69, -929.65)
(1560.75, -939.534)
(1579.14, -949.571)
(1597.09, -959.995)
(1614.63, -970.346)
(1631.91, -980.157)
(1649.2, -989.426)
(1666.37, -998.58)
(1683.24, -1007.33)
(1699.99, -1015.74)
(1715.78, -1023.67)
(1731.26, -1031.48)
(1745.52, -1038.95)
(1758.44, -1046.37)
(1769.54, -1054.83)
(1778.55, -1065.03)
(1784.78, -1076.91)
(1787.78, -1089.92)
(1787.58, -1103.4)
(1784.16, -1116.63)
(1777.41, -1128.62)
(1767.67, -1138.48)
(1755.49, -1145.52)
(1741.49, -1149.86)
(1726.46, -1152.06)
(1710.93, -1153.2)
(1695.37, -1153.96)
(1680.06, -1154.53)
(1665.41, -1154.58)
(1651.75, -1152.85)
(1639.42, -1148.09)
(1629.22, -1139.95)
(1622.18, -1129.06)
(1618.43, -1116.4)
(1618.6, -1102.91)
(1622.76, -1089.72)
(1629.81, -1077.09)
(1638.19, -1064.39)
};
 %    
 %
\addplot[
    fill=none,draw = predclr,
    very thick,
    line width= 0.5pt,%dashed,dash pattern=on 19pt off 1pt,
   % mark = square*,
   % mark size = \mrksize ex,
   % mark options = {fill=mtrnclr,draw=mdtrnclr}
    ]
    coordinates {
  (1.64208, 7.97786)
(6.75188, 15.511)
(14.3384, 20.189)
(23.5901, 22.1402)
(34.0504, 21.8822)
(45.7274, 20.543)
(59.0834, 18.6427)
(73.7683, 16.6544)
(89.6125, 14.492)
(106.509, 11.9725)
(124.08, 8.56056)
(141.659, 4.2337)
(160.108, -0.977692)
(178.903, -7.12141)
(198.185, -14.0423)
(217.697, -21.833)
(237.124, -30.212)
(256.147, -39.1694)
(275.424, -49.1065)
(295.02, -59.9499)
(314.727, -71.5445)
(334.487, -84.3607)
(353.92, -97.8207)
(373.395, -112.152)
(392.279, -127.042)
(410.731, -142.275)
(428.904, -157.631)
(447.028, -173.145)
(465.53, -188.135)
(483.941, -202.71)
(502.606, -217.246)
(520.904, -231.831)
(538.394, -246.172)
(553.281, -259.299)
(571.663, -273.753)
(590.047, -288.242)
(608.71, -302.557)
(627.233, -316.973)
(645.867, -331.316)
(664.645, -345.618)
(683.25, -359.904)
(701.875, -374.188)
(720.705, -388.45)
(739.527, -402.624)
(758.611, -416.828)
(777.674, -430.724)
(796.652, -444.692)
(815.516, -458.574)
(834.578, -472.236)
(853.83, -485.975)
(872.923, -499.575)
(892.455, -513.166)
(911.602, -526.212)
(930.716, -539.064)
(949.987, -552.014)
(969.379, -564.827)
(988.594, -577.499)
(1007.46, -589.946)
(1026.78, -602.537)
(1044.76, -614.512)
(1062.91, -626.236)
(1081.99, -638.228)
(1100.53, -649.697)
(1119.81, -661.27)
(1139.39, -672.889)
(1159.12, -684.547)
(1179.14, -696.384)
(1199.41, -708.184)
(1219.98, -719.887)
(1240.81, -731.438)
(1262.1, -743.003)
(1283.71, -754.453)
(1305.41, -765.857)
(1327.16, -777.098)
(1348.57, -788.099)
(1370.11, -799.08)
(1391.74, -809.873)
(1412.97, -820.177)
(1434.34, -830.26)
(1455.63, -840.213)
(1476.69, -850.117)
(1497.14, -859.771)
(1517.35, -869.416)
(1537.35, -878.912)
(1557.03, -888.231)
(1576.27, -897.516)
(1595.07, -907.087)
(1613.31, -917)
(1631.11, -926.801)
(1648.07, -935.973)
(1665.49, -944.82)
(1682.61, -953.4)
(1699.36, -961.669)
(1716.35, -969.753)
(1732.37, -977.348)
(1748.09, -984.974)
(1762.2, -992.128)
(1775.11, -999.388)
(1786.31, -1007.74)
(1795.39, -1017.86)
(1801.68, -1029.65)
(1804.85, -1042.72)
(1804.75, -1056.23)
(1801.45, -1069.52)
(1794.77, -1081.7)
(1785.09, -1091.64)
(1772.96, -1098.82)
(1759.04, -1103.29)
(1743.99, -1105.64)
(1728.47, -1106.99)
(1712.98, -1107.98)
(1697.67, -1108.81)
(1683.01, -1109.09)
(1669.3, -1107.59)
(1656.94, -1103.02)
(1646.59, -1095.05)
(1639.3, -1084.21)
(1635.29, -1071.55)
(1635.34, -1058.05)
(1638.45, -1047.45)
(1642.31, -1039.59)
(1646.76, -1032.45)
    };


==> plots/traj_coords_kitti_02.tex <==
%
\addplot[
    fill=none,draw = gtclr,
    very thick,
    line width= 0.5pt,%dashed,dash pattern=on 19pt off 1pt,
   % mark = square*,
   % mark size = \mrksize ex,
   % mark options = {fill=mtrnclr,draw=mdtrnclr}
    ]
    coordinates {
(-0.107508, 12.038)
(-0.361713, 25.2719)
(-0.640096, 37.9025)
(-0.745188, 49.2518)
(-0.192585, 59.6228)
(2.03751, 68.7499)
(6.2425, 76.312)
(12.3375, 81.8935)
(20.1195, 85.3339)
(28.9149, 86.1149)
(37.9377, 85.5071)
(47.1691, 84.6725)
(56.6121, 83.62)
(66.3446, 82.4824)
(76.4739, 81.3278)
(87.0266, 80.1434)
(97.9802, 79.0508)
(109.267, 77.9127)
(120.303, 76.1184)
(130.752, 72.9934)
(140.644, 68.4077)
(149.929, 62.1136)
(158.172, 54.0492)
(164.524, 44.2871)
(169.238, 33.5452)
(173.181, 22.6515)
(177.075, 11.8961)
(181.733, 1.5804)
(187.591, -7.65333)
(194.911, -15.2662)
(203.829, -20.724)
(213.983, -23.2975)
(224.418, -22.6558)
(234.323, -19.1063)
(243.258, -12.8625)
(250.935, -4.77851)
(257.501, 4.73342)
(263.578, 15.0528)
(269.365, 25.6117)
(275.199, 36.3054)
(281.082, 47.2218)
(286.806, 58.0362)
(292.001, 68.4345)
(297.196, 78.213)
(303.576, 87.0307)
(311.59, 93.752)
(320.915, 97.5534)
(330.786, 98.2575)
(340.256, 95.7719)
(348.506, 90.25)
(354.51, 82.0496)
(357.591, 72.5923)
(359.319, 62.8594)
(360.447, 53.4421)
(362.035, 45.3845)
(365.53, 39.5881)
(371.522, 36.6045)
(379.412, 36.678)
(387.659, 39.3315)
(394.859, 44.4016)
(400.257, 51.4178)
(404.179, 59.2246)
(406.317, 67.738)
(406.425, 77.0596)
(405.861, 87.1875)
(405.002, 97.9669)
(403.92, 109.298)
(402.437, 120.565)
(400.72, 131.636)
(399.004, 142.657)
(397.456, 153.635)
(395.986, 164.703)
(394.544, 175.902)
(393.193, 187.151)
(392.358, 198.504)
(392.068, 209.955)
(392.329, 221.538)
(393.232, 233.222)
(394.76, 244.904)
(396.998, 256.698)
(400.125, 268.417)
(403.806, 279.649)
(407.886, 290.552)
(412.022, 301.113)
(416.035, 311.141)
(420.111, 321.222)
(424.847, 331.489)
(430.532, 341.856)
(436.703, 351.938)
(443.009, 362.065)
(449.29, 372.224)
(455.44, 382.333)
(461.743, 392.335)
(468.163, 402.022)
(474.293, 410.822)
(480.242, 419.102)
(485.819, 426.731)
(490.885, 433.186)
(495.136, 438.6)
(498.421, 443.033)
(500.699, 447.405)
(500.987, 452.515)
(498.923, 457.981)
(495.615, 463.65)
(491.86, 469.993)
(487.766, 477.082)
(483.443, 484.497)
(478.986, 492.054)
(474.474, 499.698)
(470.199, 506.818)
(466.496, 513.005)
(463.432, 518.243)
(460.821, 522.729)
(458.316, 526.288)
(454.696, 528.488)
(449.674, 528.526)
(444.074, 525.962)
(438.177, 521.971)
(432.717, 517.376)
(427.872, 512.235)
(423.775, 506.747)
(420.275, 500.788)
(417.09, 494.257)
(414.127, 487.373)
(411.407, 480.379)
(408.983, 473.408)
(406.837, 466.989)
(404.923, 461.533)
(402.978, 456.176)
(400.894, 450.429)
(398.351, 444.146)
(395.597, 437.489)
(392.55, 430.418)
(389.091, 423.044)
(385.223, 415.38)
(381.171, 407.624)
(376.78, 399.794)
(372.053, 391.94)
(366.986, 383.995)
(361.938, 376.407)
(356.942, 369.425)
(352.219, 362.902)
(348.159, 357.373)
(344.303, 353.204)
(340.118, 350.682)
(335.123, 350.547)
(330.389, 353.038)
(325.436, 356.969)
(319.426, 360.804)
(312.475, 363.278)
(304.735, 364.209)
(296.548, 363.778)
(288.112, 362.825)
(279.818, 361.863)
(271.627, 361.432)
(263.475, 362.055)
(255.43, 363.82)
(247.564, 366.995)
(240.282, 371.701)
(233.981, 377.606)
(228.717, 384.571)
(224.788, 392.55)
(222.34, 401.614)
(221.475, 411.585)
(222.098, 421.88)
(223.453, 432.198)
(225.061, 442.776)
(226.787, 453.669)
(228.638, 464.768)
(230.663, 475.867)
(232.652, 486.91)
(234.659, 497.905)
(236.759, 508.757)
(238.809, 519.44)
(240.673, 529.933)
(242.392, 540.219)
(244.248, 550.275)
(246.274, 559.976)
(248.676, 569.315)
(251.591, 578.275)
(254.712, 587.056)
(257.592, 595.916)
(260.419, 604.72)
(263.996, 613.099)
(268.923, 620.888)
(275.076, 627.888)
(282.311, 633.693)
(290.632, 638.442)
(299.967, 642.642)
(309.755, 646.644)
(319.539, 650.539)
(328.956, 654.88)
(337.521, 659.416)
(344.943, 663.549)
(351.256, 667.054)
(355.953, 669.509)
(358.866, 670.913)
(360.931, 672.271)
(362.722, 675)
(362.909, 679.666)
(360.899, 685.387)
(357.169, 691.802)
(352.562, 699.206)
(347.294, 707.54)
(341.564, 716.557)
(335.5, 726.188)
(329.204, 736.234)
(322.683, 746.563)
(316.33, 756.777)
(310.03, 766.877)
(303.631, 776.939)
(296.518, 786.892)
(288.362, 796.16)
(279.491, 804.899)
(269.911, 813)
(259.868, 819.966)
(249.8, 825.85)
(240.135, 830.954)
(231.252, 835.253)
(223.662, 838.873)
(217.617, 841.763)
(212.379, 843.097)
(207.281, 842.05)
(203.224, 838.174)
(200.566, 832.313)
(198.679, 824.983)
(196.88, 816.651)
(194.926, 807.54)
(192.847, 797.763)
(190.673, 787.568)
(188.364, 777.124)
(185.571, 766.373)
(182.502, 755.421)
(179.928, 744.138)
(177.814, 732.58)
(176.016, 720.855)
(174.388, 709.061)
(172.979, 697.018)
(171.776, 685.2)
(170.669, 673.869)
(169.619, 662.779)
(168.498, 651.782)
(167.412, 640.671)
(166.337, 629.402)
(165.15, 617.965)
(163.89, 606.386)
(162.675, 594.689)
(161.435, 582.879)
(160.204, 570.857)
(158.99, 558.79)
(157.75, 546.799)
(156.483, 534.783)
(155.251, 522.735)
(154.124, 510.743)
(152.912, 498.691)
(151.643, 486.731)
(150.324, 474.718)
(149.106, 462.686)
(147.959, 450.74)
(146.883, 439.251)
(145.967, 427.523)
(145.328, 415.963)
(145.085, 404.35)
(145.27, 392.876)
(145.709, 381.912)
(146.368, 371.508)
(147.236, 361.709)
(148.59, 352.704)
(150.99, 344.393)
(154.172, 336.468)
(158.031, 329.293)
(163.153, 322.881)
(169.807, 317.444)
(177.735, 313.742)
(186.761, 311.764)
(196.659, 310.56)
(207.279, 309.44)
(218.008, 307.909)
(228.651, 305.619)
(238.491, 302.378)
(247.239, 297.97)
(254.738, 292.777)
(260.503, 287.519)
(264.115, 282.701)
(265.692, 277.982)
(264.88, 272.841)
(260.954, 267.994)
(254.878, 263.067)
(248.055, 256.929)
(241.176, 249.725)
(234.583, 241.834)
(228.968, 234.331)
(224.398, 227.963)
(219.727, 223.881)
(213.939, 222.34)
(207.903, 224.003)
(201.683, 227.636)
(194.123, 231.384)
(185.318, 234.309)
(175.763, 236.426)
(165.903, 238.126)
(155.982, 239.546)
(146.27, 240.935)
(136.823, 242.685)
(127.787, 245.185)
(119.225, 249.058)
(111.411, 254.485)
(104.423, 261.296)
(98.4032, 269.514)
(93.4905, 278.797)
(89.7485, 288.9)
(87.1921, 299.474)
(85.8737, 310.321)
(85.3098, 321.292)
(85.145, 332.176)
(84.9554, 343.021)
(84.601, 353.791)
(83.9074, 364.523)
(82.6707, 375.14)
(80.935, 385.699)
(78.6498, 396.218)
(76.159, 406.653)
(73.7164, 417.099)
(71.5186, 427.747)
(69.9692, 438.514)
(69.0608, 449.26)
(68.3994, 460.014)
(68.0927, 470.754)
(68.0213, 481.581)
(67.8537, 492.542)
(68.0569, 503.848)
(68.5336, 515.18)
(68.8372, 526.519)
(68.9014, 537.723)
(68.9378, 548.817)
(69.2306, 559.811)
(69.449, 570.788)
(69.5588, 581.728)
(69.6182, 592.553)
(69.7349, 603.215)
(70.1849, 613.785)
(71.006, 624.164)
(71.9988, 634.232)
(72.7219, 644.169)
(73.187, 653.939)
(73.6607, 663.683)
(74.5997, 673.531)
(75.8158, 683.667)
(77.1847, 694.245)
(78.5281, 705.247)
(80.0603, 716.489)
(81.9708, 727.738)
(84.1943, 738.812)
(86.5631, 749.785)
(89.2187, 760.634)
(92.1011, 771.385)
(95.1358, 781.873)
(98.3893, 792.206)
(101.824, 802.355)
(105.347, 812.401)
(108.841, 821.904)
(112.723, 830.923)
(117.532, 839.558)
(122.951, 847.426)
(128.326, 854.281)
(133.334, 860.23)
(137.662, 865.413)
(141.058, 868.832)
(144.04, 870.691)
(147.723, 871.475)
(152.483, 870.654)
(157.976, 868.197)
(164.446, 865.046)
(171.817, 861.53)
(179.649, 857.761)
(187.017, 853.993)
(193.537, 850.785)
(199.268, 849.048)
(204.697, 849.877)
(209.272, 853.755)
(212.837, 859.995)
(215.753, 867.762)
(218.806, 876.35)
(221.585, 885.151)
(224.384, 893.704)
(227.869, 901.479)
(232.695, 907.916)
(238.827, 912.711)
(246.353, 915.616)
(255.098, 916.562)
(264.675, 916.319)
(274.815, 915.419)
(285.477, 913.857)
(296.025, 911.585)
(306.202, 908.713)
(316.535, 905.63)
(327.05, 902.356)
(338.193, 898.752)
(349.089, 895.052)
(359.491, 891.373)
(368.667, 888.078)
(375.885, 885.498)
(382.044, 883.354)
(388.36, 881.155)
(395.664, 878.574)
(403.995, 875.751)
(413.208, 872.564)
(423.172, 868.793)
(433.272, 864.412)
(442.62, 859.901)
(451.302, 855.903)
(458.828, 852.752)
(465.9, 849.9)
(473.461, 846.863)
(481.611, 843.496)
(490.115, 840.01)
(498.913, 836.417)
(507.99, 832.784)
(517.214, 829.17)
(525.653, 825.926)
(533.12, 823.154)
(540.049, 819.919)
(546.035, 815.313)
(550.358, 808.642)
(552.812, 800.244)
(554.974, 790.794)
(557.417, 780.676)
(560.172, 769.854)
(563.008, 758.732)
(565.897, 747.583)
(568.807, 736.265)
(571.61, 725.192)
(574.339, 713.93)
(576.557, 702.488)
(578.547, 690.863)
(580.243, 679.013)
(581.541, 667.267)
(582.407, 655.765)
(583.007, 644.106)
(583.603, 632.274)
(584.317, 620.519)
(585.096, 608.67)
(585.881, 596.974)
(586.869, 585.41)
(588.795, 574.196)
(591.381, 563.118)
(594.086, 552.263)
(596.478, 541.654)
(598.345, 531.936)
(600.143, 523.869)
(601.473, 517.226)
(601.127, 511.227)
(598.568, 505.727)
(593.367, 501.284)
(586.212, 497.914)
(578.041, 494.086)
(569.469, 489.588)
(560.764, 484.817)
(551.85, 479.87)
(542.756, 474.759)
(533.87, 469.704)
(525.726, 464.936)
(518.873, 460.607)
(513.112, 457.159)
(507.512, 455.742)
(501.887, 456.951)
(496.938, 461.187)
(492.843, 468.068)
(488.132, 476.394)
(482.658, 485.938)
(476.8, 495.777)
(470.786, 505.674)
(464.625, 515.845)
(458.495, 526.228)
(452.35, 536.511)
(446.195, 547)
(440.01, 557.551)
(433.641, 568.165)
(427.175, 578.853)
(420.657, 589.64)
(414.189, 600.38)
(407.586, 611.193)
(400.941, 622.035)
(394.594, 632.366)
(388.361, 642.539)
(382.211, 652.654)
(376.054, 662.497)
(369.804, 672.467)
(363.376, 682.701)
(356.823, 693.11)
(350.32, 703.426)
(343.902, 713.551)
(337.486, 723.558)
(331.105, 733.721)
(324.576, 744.111)
(317.818, 754.995)
(311.154, 765.556)
(304.316, 775.953)
(297.108, 785.873)
(289.198, 795.34)
(280.339, 804.313)
(270.868, 812.379)
(260.941, 819.414)
(250.547, 825.561)
(239.991, 830.968)
(229.58, 836.009)
(219.147, 841.027)
(208.799, 845.837)
(198.373, 850.542)
(187.739, 855.307)
(177.16, 860.241)
(166.572, 865.351)
(156.146, 870.705)
(146.086, 877.057)
(136.695, 884.52)
(127.569, 892.491)
(118.28, 900.33)
    };
%
%
\addplot[
    fill=none,draw = orbclr,
    very thick,
    line width= 0.5pt,
   % mark = square*,
   % mark size = \mrksize ex,
   % mark options = {fill=mtrnclr,draw=mdtrnclr}
    ]
    coordinates {
  (-0.118445, 12.0587)
(-0.374161, 25.327)
(-0.62876, 37.9569)
(-0.73228, 49.3886)
(-0.168395, 59.7299)
(2.06382, 68.8332)
(6.27855, 76.3452)
(12.3658, 81.8935)
(20.1294, 85.2851)
(28.9887, 86.0394)
(38.004, 85.3757)
(47.1917, 84.4723)
(56.6745, 83.3571)
(66.4978, 82.1367)
(76.6563, 80.9188)
(87.1869, 79.6925)
(98.1161, 78.5418)
(109.372, 77.3811)
(120.35, 75.565)
(130.733, 72.4271)
(140.506, 67.8566)
(149.719, 61.5617)
(157.876, 53.5439)
(164.133, 43.8361)
(168.771, 33.1891)
(172.675, 22.2914)
(176.546, 11.5159)
(181.185, 1.16248)
(187.064, -8.18343)
(194.467, -15.8594)
(203.459, -21.353)
(213.647, -23.9331)
(224.037, -23.214)
(233.945, -19.5998)
(242.732, -13.3611)
(250.305, -5.27531)
(256.749, 4.27644)
(262.686, 14.6838)
(268.302, 25.2966)
(273.916, 35.9684)
(279.631, 46.8845)
(285.201, 57.7348)
(290.238, 68.1265)
(295.27, 77.9165)
(301.484, 86.7521)
(309.343, 93.5463)
(318.525, 97.4117)
(328.271, 98.2304)
(337.588, 95.8654)
(345.82, 90.4656)
(351.959, 82.3376)
(355.138, 72.9601)
(356.949, 63.3331)
(358.156, 53.9622)
(359.839, 45.9413)
(363.361, 40.2508)
(369.272, 37.4009)
(377.133, 37.5318)
(385.368, 40.2072)
(392.467, 45.2979)
(397.792, 52.3125)
(401.596, 60.0483)
(403.621, 68.5102)
(403.688, 77.8039)
(403.037, 87.757)
(402.068, 98.4703)
(400.843, 109.745)
(399.271, 120.904)
(397.429, 131.902)
(395.604, 142.901)
(393.95, 153.819)
(392.358, 164.844)
(390.787, 175.987)
(389.288, 187.171)
(388.3, 198.51)
(387.891, 209.915)
(388.006, 221.406)
(388.763, 232.979)
(390.135, 244.644)
(392.211, 256.398)
(395.195, 268.128)
(398.763, 279.413)
(402.746, 290.312)
(406.739, 300.807)
(410.641, 310.841)
(414.599, 320.878)
(419.247, 331.172)
(424.897, 341.59)
(430.96, 351.763)
(437.131, 361.831)
(443.289, 371.958)
(449.324, 382.017)
(455.527, 392.049)
(461.826, 401.7)
(467.87, 410.463)
(473.727, 418.754)
(479.21, 426.361)
(484.202, 432.838)
(488.406, 438.257)
(491.652, 442.673)
(493.831, 447.058)
(494.068, 452.124)
(491.991, 457.543)
(488.693, 463.234)
(484.96, 469.59)
(480.805, 476.653)
(476.471, 484.035)
(472.013, 491.612)
(467.489, 499.2)
(463.223, 506.303)
(459.534, 512.451)
(456.478, 517.629)
(453.895, 522.065)
(451.389, 525.593)
(447.843, 527.775)
(442.827, 527.831)
(437.261, 525.277)
(431.391, 521.28)
(425.997, 516.705)
(421.23, 511.603)
(417.174, 506.146)
(413.66, 500.183)
(410.502, 493.682)
(407.536, 486.856)
(404.843, 479.882)
(402.452, 472.93)
(400.305, 466.507)
(398.427, 461.057)
(396.486, 455.706)
(394.429, 450)
(391.923, 443.755)
(389.173, 437.118)
(386.171, 430.07)
(382.696, 422.673)
(378.915, 415.087)
(374.882, 407.371)
(370.527, 399.572)
(365.804, 391.743)
(360.816, 383.882)
(355.731, 376.284)
(350.77, 369.354)
(346.055, 362.855)
(342.035, 357.362)
(338.227, 353.199)
(334.001, 350.671)
(329.019, 350.521)
(324.292, 353.037)
(319.331, 356.955)
(313.322, 360.781)
(306.403, 363.243)
(298.732, 364.145)
(290.581, 363.731)
(282.172, 362.791)
(273.923, 361.823)
(265.756, 361.395)
(257.652, 361.997)
(249.646, 363.73)
(241.792, 366.902)
(234.518, 371.592)
(228.205, 377.495)
(223.001, 384.405)
(219.097, 392.321)
(216.654, 401.326)
(215.801, 411.276)
(216.44, 421.509)
(217.805, 431.84)
(219.4, 442.375)
(221.089, 453.258)
(222.935, 464.28)
(224.939, 475.331)
(226.907, 486.298)
(228.926, 497.221)
(231.006, 508.089)
(233.055, 518.736)
(234.923, 529.229)
(236.648, 539.466)
(238.487, 549.495)
(240.514, 559.216)
(242.885, 568.554)
(245.759, 577.473)
(248.852, 586.223)
(251.709, 595.029)
(254.511, 603.817)
(258.052, 612.174)
(262.94, 619.914)
(269.071, 626.883)
(276.252, 632.682)
(284.534, 637.414)
(293.795, 641.617)
(303.501, 645.62)
(313.279, 649.55)
(322.681, 653.938)
(331.21, 658.443)
(338.578, 662.621)
(344.855, 666.109)
(349.543, 668.557)
(352.448, 670.003)
(354.497, 671.32)
(356.226, 674.089)
(356.34, 678.773)
(354.316, 684.542)
(350.639, 690.999)
(346.043, 698.492)
(340.855, 706.859)
(335.185, 715.913)
(329.229, 725.544)
(322.966, 735.717)
(316.581, 746.188)
(310.356, 756.338)
(304.078, 766.471)
(297.735, 776.52)
(290.676, 786.433)
(282.592, 795.699)
(273.807, 804.417)
(264.317, 812.491)
(254.329, 819.486)
(244.321, 825.446)
(234.73, 830.577)
(225.899, 834.904)
(218.325, 838.583)
(212.327, 841.466)
(207.153, 842.795)
(202.125, 841.752)
(198.034, 837.931)
(195.374, 832.133)
(193.463, 824.864)
(191.606, 816.55)
(189.598, 807.466)
(187.439, 797.718)
(185.194, 787.585)
(182.822, 777.176)
(179.996, 766.554)
(176.843, 755.628)
(174.113, 744.269)
(171.918, 732.673)
(170.035, 720.974)
(168.321, 709.155)
(166.794, 697.104)
(165.527, 685.363)
(164.36, 674.072)
(163.214, 663.001)
(162.018, 651.965)
(160.84, 640.827)
(159.718, 629.596)
(158.479, 618.172)
(157.186, 606.577)
(155.931, 594.894)
(154.645, 583.08)
(153.379, 571.125)
(152.133, 559.131)
(150.857, 547.107)
(149.538, 535.109)
(148.261, 523.088)
(147.093, 511.071)
(145.867, 499.088)
(144.581, 487.138)
(143.198, 475.148)
(141.934, 463.167)
(140.73, 451.318)
(139.611, 439.781)
(138.688, 428.288)
(138.03, 416.737)
(137.763, 405.161)
(137.914, 393.75)
(138.345, 382.805)
(138.98, 372.457)
(139.832, 362.753)
(141.19, 353.8)
(143.597, 345.467)
(146.764, 337.58)
(150.598, 330.482)
(155.75, 324.092)
(162.415, 318.674)
(170.359, 314.955)
(179.465, 313.034)
(189.432, 311.836)
(200.035, 310.707)
(210.737, 309.185)
(221.357, 306.91)
(231.155, 303.673)
(239.921, 299.267)
(247.421, 294.113)
(253.191, 288.905)
(256.836, 284.065)
(258.401, 279.331)
(257.596, 274.212)
(253.668, 269.333)
(247.587, 264.41)
(240.818, 258.318)
(233.959, 251.121)
(227.345, 243.199)
(221.775, 235.756)
(217.256, 229.462)
(212.667, 225.414)
(206.923, 223.898)
(200.901, 225.549)
(194.705, 229.172)
(187.22, 232.837)
(178.44, 235.766)
(168.886, 237.9)
(159.055, 239.607)
(149.171, 241.018)
(139.475, 242.402)
(130.079, 244.127)
(121.088, 246.59)
(112.517, 250.469)
(104.695, 255.868)
(97.7021, 262.639)
(91.6848, 270.789)
(86.7574, 280.075)
(83.0064, 290.19)
(80.4492, 300.764)
(79.1136, 311.622)
(78.5387, 322.538)
(78.3613, 333.405)
(78.1759, 344.193)
(77.8313, 354.872)
(77.1323, 365.534)
(75.8954, 376.126)
(74.1656, 386.616)
(71.8761, 397.096)
(69.3893, 407.539)
(66.9414, 417.96)
(64.7603, 428.564)
(63.203, 439.303)
(62.2887, 450.04)
(61.6603, 460.733)
(61.3625, 471.431)
(61.3, 482.242)
(61.1755, 493.145)
(61.3975, 504.39)
(61.8826, 515.621)
(62.1763, 526.873)
(62.2481, 538.031)
(62.3154, 549.114)
(62.63, 560.02)
(62.895, 570.885)
(62.9983, 581.771)
(63.0318, 592.602)
(63.1707, 603.22)
(63.6509, 613.692)
(64.4876, 623.988)
(65.4747, 634.065)
(66.2527, 643.897)
(66.7142, 653.601)
(67.1918, 663.351)
(68.1462, 673.141)
(69.3883, 683.217)
(70.7749, 693.775)
(72.1419, 704.757)
(73.7024, 715.932)
(75.6153, 727.108)
(77.8386, 738.147)
(80.2399, 749.125)
(82.9149, 760.031)
(85.806, 770.757)
(88.8689, 781.299)
(92.1382, 791.661)
(95.5553, 801.845)
(99.0789, 811.832)
(102.554, 821.28)
(106.443, 830.233)
(111.23, 838.771)
(116.603, 846.537)
(121.982, 853.371)
(126.994, 859.279)
(131.296, 864.424)
(134.703, 867.845)
(137.661, 869.682)
(141.335, 870.44)
(146.061, 869.617)
(151.547, 867.139)
(157.983, 863.966)
(165.354, 860.417)
(173.139, 856.636)
(180.463, 852.841)
(186.934, 849.635)
(192.698, 847.884)
(198.06, 848.67)
(202.63, 852.531)
(206.25, 858.746)
(209.216, 866.51)
(212.286, 875.083)
(215.108, 883.899)
(217.929, 892.447)
(221.436, 900.21)
(226.272, 906.561)
(232.417, 911.329)
(239.883, 914.18)
(248.645, 915.117)
(258.31, 914.826)
(268.433, 913.894)
(279.005, 912.259)
(289.471, 909.938)
(299.6, 907.032)
(309.845, 903.904)
(320.316, 900.607)
(331.407, 896.965)
(342.271, 893.222)
(352.609, 889.493)
(361.728, 886.155)
(368.896, 883.557)
(375.003, 881.377)
(381.268, 879.141)
(388.507, 876.52)
(396.787, 873.637)
(405.948, 870.414)
(415.878, 866.601)
(425.822, 862.209)
(435.134, 857.694)
(443.725, 853.685)
(451.196, 850.529)
(458.21, 847.682)
(465.71, 844.626)
(473.756, 841.315)
(482.209, 837.856)
(490.962, 834.283)
(499.967, 830.664)
(509.116, 827.06)
(517.593, 823.799)
(525.068, 821.078)
(531.958, 817.869)
(537.92, 813.31)
(542.204, 806.711)
(544.668, 798.31)
(546.825, 788.93)
(549.272, 778.859)
(552.003, 768.12)
(554.828, 757.049)
(557.719, 745.962)
(560.625, 734.774)
(563.465, 723.659)
(566.202, 712.507)
(568.44, 701.158)
(570.422, 689.577)
(572.12, 677.808)
(573.448, 666.129)
(574.359, 654.546)
(574.982, 642.883)
(575.612, 631.042)
(576.376, 619.222)
(577.213, 607.391)
(578.037, 595.735)
(579.058, 584.264)
(581.003, 573.112)
(583.632, 562.102)
(586.373, 551.3)
(588.801, 540.728)
(590.708, 531.085)
(592.538, 523.055)
(593.921, 516.437)
(593.663, 510.465)
(591.168, 504.976)
(585.993, 500.547)
(578.852, 497.208)
(570.743, 493.422)
(562.222, 488.967)
(553.498, 484.247)
(544.587, 479.326)
(535.532, 474.26)
(526.686, 469.279)
(518.613, 464.556)
(511.79, 460.269)
(506.033, 456.854)
(500.467, 455.463)
(494.877, 456.604)
(489.97, 460.787)
(485.872, 467.683)
(481.17, 476.057)
(475.696, 485.459)
(469.843, 495.237)
(463.803, 505.205)
(457.665, 515.254)
(451.58, 525.514)
(445.42, 535.816)
(439.297, 546.257)
(433.126, 556.861)
(426.768, 567.493)
(420.294, 578.163)
(413.795, 588.898)
(407.299, 599.711)
(400.724, 610.544)
(394.107, 621.418)
(387.783, 631.827)
(381.562, 642.026)
(375.456, 652.038)
(369.349, 661.82)
(363.126, 671.765)
(356.723, 681.99)
(350.237, 692.43)
(343.855, 702.739)
(337.481, 712.938)
(331.125, 723.036)
(324.847, 733.185)
(318.42, 743.767)
(311.854, 754.556)
(305.183, 765.131)
(298.407, 775.526)
(291.27, 785.415)
(283.409, 794.884)
(274.645, 803.811)
(265.251, 811.903)
(255.389, 818.958)
(245.064, 825.135)
(234.588, 830.593)
(224.183, 835.722)
(213.782, 840.79)
(203.535, 845.599)
(193.202, 850.318)
(182.596, 855.131)
(171.951, 860.183)
(161.384, 865.327)
(150.94, 870.762)
(140.909, 877.085)
(131.595, 884.5)
(122.517, 892.441)
(113.265, 900.258)
};
 %    
 %
\addplot[
    fill=none,draw = predclr,
    very thick,
    line width= 0.5pt,%dashed,dash pattern=on 19pt off 1pt,
   % mark = square*,
   % mark size = \mrksize ex,
   % mark options = {fill=mtrnclr,draw=mdtrnclr}
    ]
    coordinates {
   (-0.107508, 12.038)
(-0.361713, 25.2719)
(-0.640096, 37.9025)
(-0.745188, 49.2518)
(-0.192585, 59.6228)
(2.03751, 68.7499)
(6.2425, 76.312)
(12.3375, 81.8935)
(20.1195, 85.3339)
(28.9149, 86.1149)
(37.9377, 85.5071)
(47.1691, 84.6725)
(56.6121, 83.62)
(66.3446, 82.4824)
(76.4739, 81.3278)
(87.0266, 80.1434)
(97.9802, 79.0508)
(109.267, 77.9127)
(120.303, 76.1184)
(130.752, 72.9934)
(140.644, 68.4077)
(149.929, 62.1136)
(158.172, 54.0492)
(164.524, 44.2871)
(169.238, 33.5452)
(173.181, 22.6515)
(177.075, 11.8961)
(181.733, 1.5804)
(187.591, -7.65333)
(194.911, -15.2662)
(203.829, -20.724)
(213.983, -23.2975)
(224.418, -22.6558)
(234.323, -19.1063)
(243.258, -12.8625)
(250.935, -4.77851)
(257.501, 4.73342)
(263.578, 15.0528)
(269.365, 25.6117)
(275.199, 36.3054)
(281.082, 47.2218)
(286.806, 58.0362)
(292.001, 68.4345)
(297.196, 78.213)
(303.576, 87.0307)
(311.59, 93.752)
(320.915, 97.5534)
(330.786, 98.2575)
(340.256, 95.7719)
(348.506, 90.25)
(354.51, 82.0496)
(357.591, 72.5923)
(359.319, 62.8594)
(360.447, 53.4421)
(362.035, 45.3845)
(365.53, 39.5881)
(371.522, 36.6045)
(379.412, 36.678)
(387.659, 39.3315)
(394.859, 44.4016)
(400.257, 51.4178)
(404.179, 59.2246)
(406.317, 67.738)
(406.425, 77.0596)
(405.861, 87.1875)
(405.002, 97.9669)
(403.92, 109.298)
(402.437, 120.565)
(400.72, 131.636)
(399.004, 142.657)
(397.456, 153.635)
(395.986, 164.703)
(394.544, 175.902)
(393.193, 187.151)
(392.358, 198.504)
(392.068, 209.955)
(392.329, 221.538)
(393.232, 233.222)
(394.76, 244.904)
(396.998, 256.698)
(400.125, 268.417)
(403.806, 279.649)
(407.886, 290.552)
(412.022, 301.113)
(416.035, 311.141)
(420.111, 321.222)
(424.847, 331.489)
(430.532, 341.856)
(436.703, 351.938)
(443.009, 362.065)
(449.29, 372.224)
(455.44, 382.333)
(461.743, 392.335)
(468.163, 402.022)
(474.293, 410.822)
(480.242, 419.102)
(485.819, 426.731)
(490.885, 433.186)
(495.136, 438.6)
(498.421, 443.033)
(500.699, 447.405)
(500.987, 452.515)
(498.923, 457.981)
(495.615, 463.65)
(491.86, 469.993)
(487.766, 477.082)
(483.443, 484.497)
(478.986, 492.054)
(474.474, 499.698)
(470.199, 506.818)
(466.496, 513.005)
(463.432, 518.243)
(460.821, 522.729)
(458.316, 526.288)
(454.696, 528.488)
(449.674, 528.526)
(444.074, 525.962)
(438.177, 521.971)
(432.717, 517.376)
(427.872, 512.235)
(423.775, 506.747)
(420.275, 500.788)
(417.09, 494.257)
(414.127, 487.373)
(411.407, 480.379)
(408.983, 473.408)
(406.837, 466.989)
(404.923, 461.533)
(402.978, 456.176)
(400.894, 450.429)
(398.351, 444.146)
(395.597, 437.489)
(392.55, 430.418)
(389.091, 423.044)
(385.223, 415.38)
(381.171, 407.624)
(376.78, 399.794)
(372.053, 391.94)
(366.986, 383.995)
(361.938, 376.407)
(356.942, 369.425)
(352.219, 362.902)
(348.159, 357.373)
(344.303, 353.204)
(340.118, 350.682)
(335.123, 350.547)
(330.389, 353.038)
(325.436, 356.969)
(319.426, 360.804)
(312.475, 363.278)
(304.735, 364.209)
(296.548, 363.778)
(288.112, 362.825)
(279.818, 361.863)
(271.627, 361.432)
(263.475, 362.055)
(255.43, 363.82)
(247.564, 366.995)
(240.282, 371.701)
(233.981, 377.606)
(228.717, 384.571)
(224.788, 392.55)
(222.34, 401.614)
(221.475, 411.585)
(222.098, 421.88)
(223.453, 432.198)
(225.061, 442.776)
(226.787, 453.669)
(228.638, 464.768)
(230.663, 475.867)
(232.652, 486.91)
(234.659, 497.905)
(236.759, 508.757)
(238.809, 519.44)
(240.673, 529.933)
(242.392, 540.219)
(244.248, 550.275)
(246.274, 559.976)
(248.676, 569.315)
(251.591, 578.275)
(254.712, 587.056)
(257.592, 595.916)
(260.419, 604.72)
(263.996, 613.099)
(268.923, 620.888)
(275.076, 627.888)
(282.311, 633.693)
(290.632, 638.442)
(299.967, 642.642)
(309.755, 646.644)
(319.539, 650.539)
(328.956, 654.88)
(337.521, 659.416)
(344.943, 663.549)
(351.256, 667.054)
(355.953, 669.509)
(358.866, 670.913)
(360.931, 672.271)
(362.722, 675)
(362.909, 679.666)
(360.899, 685.387)
(357.169, 691.802)
(352.562, 699.206)
(347.294, 707.54)
(341.564, 716.557)
(335.5, 726.188)
(329.204, 736.234)
(322.683, 746.563)
(316.33, 756.777)
(310.03, 766.877)
(303.631, 776.939)
(296.518, 786.892)
(288.362, 796.16)
(279.491, 804.899)
(269.911, 813)
(259.868, 819.966)
(249.8, 825.85)
(240.135, 830.954)
(231.252, 835.253)
(223.662, 838.873)
(217.617, 841.763)
(212.379, 843.097)
(207.281, 842.05)
(203.224, 838.174)
(200.566, 832.313)
(198.679, 824.983)
(196.88, 816.651)
(194.926, 807.54)
(192.847, 797.763)
(190.673, 787.568)
(188.364, 777.124)
(185.571, 766.373)
(182.502, 755.421)
(179.928, 744.138)
(177.814, 732.58)
(176.016, 720.855)
(174.388, 709.061)
(172.979, 697.018)
(171.776, 685.2)
(170.669, 673.869)
(169.619, 662.779)
(168.498, 651.782)
(167.412, 640.671)
(166.337, 629.402)
(165.15, 617.965)
(163.89, 606.386)
(162.675, 594.689)
(161.435, 582.879)
(160.204, 570.857)
(158.99, 558.79)
(157.75, 546.799)
(156.483, 534.783)
(155.251, 522.735)
(154.124, 510.743)
(152.912, 498.691)
(151.643, 486.731)
(150.324, 474.718)
(149.106, 462.686)
(147.959, 450.74)
(146.883, 439.251)
(145.967, 427.523)
(145.328, 415.963)
(145.085, 404.35)
(145.27, 392.876)
(145.709, 381.912)
(146.368, 371.508)
(147.236, 361.709)
(148.59, 352.704)
(150.99, 344.393)
(154.172, 336.468)
(158.031, 329.293)
(163.153, 322.881)
(169.807, 317.444)
(177.735, 313.742)
(186.761, 311.764)
(196.659, 310.56)
(207.279, 309.44)
(218.008, 307.909)
(228.651, 305.619)
(238.491, 302.378)
(247.239, 297.97)
(254.738, 292.777)
(260.503, 287.519)
(264.115, 282.701)
(265.692, 277.982)
(264.88, 272.841)
(260.954, 267.994)
(254.878, 263.067)
(248.055, 256.929)
(241.176, 249.725)
(234.583, 241.834)
(228.968, 234.331)
(224.398, 227.963)
(219.727, 223.881)
(213.939, 222.34)
(207.903, 224.003)
(201.683, 227.636)
(194.123, 231.384)
(185.318, 234.309)
(175.763, 236.426)
(165.903, 238.126)
(155.982, 239.546)
(146.27, 240.935)
(136.823, 242.685)
(127.787, 245.185)
(119.225, 249.058)
(111.411, 254.485)
(104.423, 261.296)
(98.4032, 269.514)
(93.4905, 278.797)
(89.7485, 288.9)
(87.1921, 299.474)
(85.8737, 310.321)
(85.3098, 321.292)
(85.145, 332.176)
(84.9554, 343.021)
(84.601, 353.791)
(83.9074, 364.523)
(82.6707, 375.14)
(80.935, 385.699)
(78.6498, 396.218)
(76.159, 406.653)
(73.7164, 417.099)
(71.5186, 427.747)
(69.9692, 438.514)
(69.0608, 449.26)
(68.3994, 460.014)
(68.0927, 470.754)
(68.0213, 481.581)
(67.8537, 492.542)
(68.0569, 503.848)
(68.5336, 515.18)
(68.8372, 526.519)
(68.9014, 537.723)
(68.9378, 548.817)
(69.2306, 559.811)
(69.449, 570.788)
(69.5588, 581.728)
(69.6182, 592.553)
(69.7349, 603.215)
(70.1849, 613.785)
(71.006, 624.164)
(71.9988, 634.232)
(72.7219, 644.169)
(73.187, 653.939)
(73.6607, 663.683)
(74.5997, 673.531)
(75.8158, 683.667)
(77.1847, 694.245)
(78.5281, 705.247)
(80.0603, 716.489)
(81.9708, 727.738)
(84.1943, 738.812)
(86.5631, 749.785)
(89.2187, 760.634)
(92.1011, 771.385)
(95.1358, 781.873)
(98.3893, 792.206)
(101.824, 802.355)
(105.347, 812.401)
(108.841, 821.904)
(112.723, 830.923)
(117.532, 839.558)
(122.951, 847.426)
(128.326, 854.281)
(133.334, 860.23)
(137.662, 865.413)
(141.058, 868.832)
(144.04, 870.691)
(147.723, 871.475)
(152.483, 870.654)
(157.976, 868.197)
(164.446, 865.046)
(171.817, 861.53)
(179.649, 857.761)
(187.017, 853.993)
(193.537, 850.785)
(199.268, 849.048)
(204.697, 849.877)
(209.272, 853.755)
(212.837, 859.995)
(215.753, 867.762)
(218.806, 876.35)
(221.585, 885.151)
(224.384, 893.704)
(227.869, 901.479)
(232.695, 907.916)
(238.827, 912.711)
(246.353, 915.616)
(255.098, 916.562)
(264.675, 916.319)
(274.815, 915.419)
(285.477, 913.857)
(296.025, 911.585)
(306.202, 908.713)
(316.535, 905.63)
(327.05, 902.356)
(338.193, 898.752)
(349.089, 895.052)
(359.491, 891.373)
(368.667, 888.078)
(375.885, 885.498)
(382.044, 883.354)
(388.36, 881.155)
(395.664, 878.574)
(403.995, 875.751)
(413.208, 872.564)
(423.172, 868.793)
(433.272, 864.412)
(442.62, 859.901)
(451.302, 855.903)
(458.828, 852.752)
(465.9, 849.9)
(473.461, 846.863)
(481.611, 843.496)
(490.115, 840.01)
(498.913, 836.417)
(507.99, 832.784)
(517.214, 829.17)
(525.653, 825.926)
(533.12, 823.154)
(540.049, 819.919)
(546.035, 815.313)
(550.358, 808.642)
(552.812, 800.244)
(554.974, 790.794)
(557.417, 780.676)
(560.172, 769.854)
(563.008, 758.732)
(565.897, 747.583)
(568.807, 736.265)
(571.61, 725.192)
(574.339, 713.93)
(576.557, 702.488)
(578.547, 690.863)
(580.243, 679.013)
(581.541, 667.267)
(582.407, 655.765)
(583.007, 644.106)
(583.603, 632.274)
(584.317, 620.519)
(585.096, 608.67)
(585.881, 596.974)
(586.869, 585.41)
(588.795, 574.196)
(591.381, 563.118)
(594.086, 552.263)
(596.478, 541.654)
(598.345, 531.936)
(600.143, 523.869)
(601.473, 517.226)
(601.127, 511.227)
(598.568, 505.727)
(593.367, 501.284)
(586.212, 497.914)
(578.041, 494.086)
(569.469, 489.588)
(560.764, 484.817)
(551.85, 479.87)
(542.756, 474.759)
(533.87, 469.704)
(525.726, 464.936)
(518.873, 460.607)
(513.112, 457.159)
(507.512, 455.742)
(501.887, 456.951)
(496.938, 461.187)
(492.843, 468.068)
(488.132, 476.394)
(482.658, 485.938)
(476.8, 495.777)
(470.786, 505.674)
(464.625, 515.845)
(458.495, 526.228)
(452.35, 536.511)
(446.195, 547)
(440.01, 557.551)
(433.641, 568.165)
(427.175, 578.853)
(420.657, 589.64)
(414.189, 600.38)
(407.586, 611.193)
(400.941, 622.035)
(394.594, 632.366)
(388.361, 642.539)
(382.211, 652.654)
(376.054, 662.497)
(369.804, 672.467)
(363.376, 682.701)
(356.823, 693.11)
(350.32, 703.426)
(343.902, 713.551)
(337.486, 723.558)
(331.105, 733.721)
(324.576, 744.111)
(317.818, 754.995)
(311.154, 765.556)
(304.316, 775.953)
(297.108, 785.873)
(289.198, 795.34)
(280.339, 804.313)
(270.868, 812.379)
(260.941, 819.414)
(250.547, 825.561)
(239.991, 830.968)
(229.58, 836.009)
(219.147, 841.027)
(208.799, 845.837)
(198.373, 850.542)
(187.739, 855.307)
(177.16, 860.241)
(166.572, 865.351)
(156.146, 870.705)
(146.086, 877.057)
(136.695, 884.52)
(127.569, 892.491)
(118.28, 900.33)
    };


==> related_work.tex <==
%%
%\paragraph{FAST Corners} 
%%
%are preferred in VO or SLAM systems due to its speed efficiency. While there exists its many implementations \cite{opencv, arrayfire}, none of them handles many non-corners being misclassified as corners.
%%
%\paragraph{Restricted Feature Count}
%% 
%is used commonly to improve VO runtime by dividing image into grids and picking one feature per-grid. \cite{fastergpu} presents such an approach for GPU, however its design is limited only to monocular VO, which prevent its use in visual-SLAM. For example, its unconfigurable scale-factor of two in multi-scale setting aggressively drops the resolution, resulting in a fewer features which are further reduced to only one feature per-grid in the image, irrespective of the number of scales. It leads to inadequate map-points in SLAM (Fig.~\ref{fig:slam_kitti}), causing tracking failures. In addition, this approach is inefficient for small grids-sizes when deployed onto embedded computing devices.
%%
%%\vspace{-1.75ex}
%%
%%\subsection{Visual Odometery, Visual-SLAM \& Robotic Autonomy}
%\paragraph{VO, SLAM \& Robotic Autonomy}
%%
%Representative VO systems include \cite{forster2016svo, dmvio, rebecq2021simultaneous}. Recent \cite{vobenchmark} shows the significance to run VO systems onto Jetson devices, however it merely benchmarks the existing implementations. 
%\par
%\cite{orb2, iceba} are pioneering SLAM systems reknowned for their high accuracy. These approaches however due to their CPU-only workload and high complexity, run quite slower on mini-computers while exhaust them quickly. For this reason, recent UAV-based autonomy \cite{towards} which used SLAM to execute brick pick-transport-place task, performed SLAM computations on remote computer due to limited onboard computing power. Similarly \cite{edgeslam} explores network computing for SLAM but is not suitable for isolated robotic systems. \cite{hamandi2020direct} focuses on control system but relies on external system VICON, indicating the need of fast, accurate and resource efficient SLAM pipeline. SLAMCore \cite{slamcore} demonstrates efficient CPU SLAM but is not open-source, and do not harness GPU.
%\par
%Deep learning based VO \cite{undeepvo} and visual-SLAM \cite{droidslam} systems have also emerged, however their generalization gap and huge computational demands put them out of reach of the embedded computing devices. For example, \cite{droidslam} uses two desktop grade GPUs yet performs below real-time.

%%
%\paragraph{FAST Corners} 
%%
%are preferred over \cite{harris, shitomasi} in VO or SLAM systems due to its speed efficiency. While there exists its many implementations \cite{kfast, arrayfire, xiong2019improved}, none of them handles many non-corners being misclassified as corners. \cite{xiong2019improved} adapts FAST for satellite images however its complex sine-cosine calculations are not favorable over the baseline FAST due to the performance issues in a GPU kernel.
%%VO and SLAM systems widely use \cite{harris, shitomasi, fast, orb} but FAST \cite{fast} is preferred due to its speed efficiency. While there exists other FAST implementations \cite{kfast, arrayfire}, none of them addresses the issue of shot-noise being classified as corner. The work \cite{xiong2019improved} slightly modifies FAST detection however its complex sine-cosine calculations makes it less favorable over the original one due to the performance issues in GPU kernel.
%%
%\paragraph{Restricted Feature Count}
%% 
%is used commonly to improve VO runtime \cite{vo, realvo} by dividing image into grids and picking one feature per-grid. \cite{fastergpu} presents such an approach for GPU, however it is limited only to monocular VO, and its design limitations prevent its use in visual-SLAM. For example, its fixed scale-factor of $2$ in multi-scale setting aggressively drops the resolution, resulting in a fewer keypoints per-scale which are further limited to only one keypoint per-grid at the native scale (image resolution) irrespective of the number of scales. This results in inadequate map-points in SLAM (Figure~\ref{fig:slam_kitti}), leading to tracking failures. In addition, this approach is inefficient for small grids-sizes when deployed onto embedded computing devices.
%%
%%\vspace{-1.75ex}
%%
%%\subsection{Visual Odometery, Visual-SLAM \& Robotic Autonomy}
%\paragraph{VO, SLAM \& Robotic Autonomy}
%%
%To name a few, the representative VO systems include \cite{bloesch2015robust, forster2016svo}, delayed marginalized \cite{dmvio} and event-camera VO \cite{rebecq2021simultaneous}. Recent \cite{vobenchmark} shows the significance to run VO systems onto Jetson devices, however it merely benchmarks the existing implementations. 
%\par
%While \cite{orb2, orb3, iceba} are the most pioneering SLAM approaches reknowned for their high accuracy. These approaches however due to their CPU-only workload and high complexity, run quite slower on mini-computers while exhaust them quickly. For this reason, recent UAV-based aerial autonomy \cite{towards} which used SLAM to execute brick pick-transport-place task, performed SLAM computations on remote computer due to limited onboard computing power. Similarly \cite{edgeslam} explores network computing for SLAM but is not suitable for isolated robotic systems. \cite{hamandi2020direct} focuses on control system but relies on external positioning system VICON, indicating the need of fast, accurate and resource efficient SLAM pipeline. SLAMCore \cite{slamcore} demonstrates efficient CPU SLAM but is not open-source, and still do not take advantage of GPU.
%\par
%Deep learning based VO \cite{undeepvo} and visual-SLAM \cite{droidslam} systems have also emerged, however their generalization gap and huge computational demands put them out of reach of the embedded computing devices. For example, \cite{droidslam} uses two desktop grade GPUs yet performs below real-time.

